Online Federation For Mixtures of Proprietary Agents with Black-Box Encoders

Most industry-standard generative AIs and feature encoders are proprietary, offering only black-box access: their outputs are observable, but their internal parameters and architectures remain hidden from the end-user. This black-box access is especially limiting when constructing mixture-of-expert type ensemble models since the user cannot optimize each proprietary AI's internal parameters. Our problem naturally lends itself to a non-competitive game-theoretic lens where each proprietary AI (agent) is inherently competing against the other AI agents, with this competition arising naturally due to their obliviousness of the AI's to their internal structure. In contrast, the user acts as a central planner trying to synchronize the ensemble of competing AIs. We show the existence of the unique Nash equilibrium in the online setting, which we even compute in closed-form by eliciting a feedback mechanism between any given time series and the sequence generated by each (proprietary) AI agent. Our solution is implemented as a decentralized, federated-learning algorithm in which each agent optimizes their structure locally on their machine without ever releasing any internal structure to the others. We obtain refined expressions for pre-trained models such as transformers, random feature models, and echo-state networks. Our ``proprietary federated learning'' algorithm is implemented on a range of real-world and synthetic time-series benchmarks. It achieves orders-of-magnitude improvements in predictive accuracy over natural benchmarks, of which there are surprisingly few due to this natural problem still being largely unexplored.

==> Historical_Versions/2024_03_08.tex <==
% % david.emerson@vectorinstitute.ai
% % fatemeh.tavakoli@vectorinstitute.ai


% \documentclass[8pt]{article}

% \usepackage[top=0.9in,bottom=1.1in,left=1.05in,right=1.05in]{geometry}



% %


% %\usepackage{amsthm} 
% %\theoremstyle{remark}
% %\newtheorem{remark}{Remark}


% \title{Optimal Federated Learning For Distributed Transformers}
% \date{}

% \input{packages}
% \input{mathcommands}
% \input{Commenting}


% \begin{document}

% \maketitle

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract} 
% In this paper, we consider the problem of optimally training a set of sequential generative models distributed across a network using a fixed number of communication rounds.
% We derive closed-form expressions for the optimal online updates for the local models and the optimal mixture implemented by the server when predicting from the distributed ensemble.  Our algorithm requires the system to periodically synchronize, and we derive a closed-form expression for the optimal synchronization as the solution to a Nash equilibrium in which each local model strives to maximally contribute to the predictive accuracy of the ensemble.  

% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%% Section 1: Instruction %%%%%%
% %\section{Introduction}
% %\label{chp:intro}

% %Input data $x=(x_1, ..., x_d)\in \mathbb{R}^d$. 
% % \begin{comment}

% \section{The Ensemble Model}
% \label{s:EnsembleModel}
% Let $\varepsilon_{\cdot}\eqdef (\varepsilon_t)_{t\in \mathbb{Z}}$ be a $\mathbb{R}^{d_y}$-valued stochastic process (noise) defined on a probability space $(\Omega,\mathcal{A},\mathbb{P})$ with $\varepsilon_t \in L^2_{\mathbb{P}}(\mathbb{R}^{d_Y})$ for all $t\in \mathbb{Z}$, and suppose that for each $t \in \mathbb{Z}$ there exists a Borel function $f:(\mathbb{R}^{d_x})^{\mathbb{Z}_-}\to \mathbb{R}^{d_y}$.  
% For each \textit{realized path} $x_{\cdot}\eqdef (x_t)_{t\in \mathbb{Z}} \in (\mathbb{R}^{d_x})^{\mathbb{Z}}$ we define the $\mathbb{R}^{d_y}$-valued stochastic process
% \[
% Y_t = f\circ \tau_t\big(x_{(-\infty,t]}\big) + \varepsilon_t
% ,
% \]
% where the time-shift operator $\tau_t:\prod_{s\le t}\, \mathbb{R}^{d_X}\ni x_{(-\infty,t]}\to (u_s)_{s\in \mathbb{Z}_-}\in (\mathbb{R}^{d_X})^{\mathbb{Z}_-}$ simply relabels the index of $x_{\cdot}$ so that the index of it most recent point is $0$ and not $t$; that is, for each $s\in \mathbb{Z}_-$ we have $u_s\eqdef x_{s+t}$.


% % Suppose that we observe a pair of processes process $Y_{\cdot} \eqdef (Y_{t})_{t\in \mathbb{Z}}$ and $X_{\cdot} \eqdef  (X_t)_{t\in \mathbb{Z}}$ respectively evolving on $\mathbb{R}^{d_{y}}$ and on $\mathbb{R}^{d_{x}}$, for some $d_y,d_x\in \mathbb{N}_+$.  

% Our objective is to solve the sequential regression task to learn $f$ using a set of $N$ pre-trained \textit{generative models} $\{\hat{f}^i\}_{i=1}^N$, designed to predict the residual changes in sequential data.  
% For each $i=1,\dots,N$, the $i^{th}$ \textit{generative models} $\hat{f}^i:(\mathbb{R}^{d_{x}})^{\mathbb{Z}}\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{Z}}$ where, for each $t\in \mathbb{Z}$ and each realized path $x_{\cdot}\in (\mathbb{R}^{d_x})^{\mathbb{Z}}$ the $t^{th}$ component of $\hat{f}^i$ is given by predicting the residual from the previous prediction at time $t-1$
% \begin{equation}
% \label{eq:residualModel}
% \begin{aligned}
%     \hat{f}^i\big(x_{\cdot}\big)_t 
%     & \eqdef  
%         \hat{Y}_{t-1}^i + \hat{Y}_t^i 
%     \\
%         \hat{Y}_t^i
%     & \eqdef 
%     % \underbrace{
%         (\beta_t^i)^{\top}
%     % }_{\mbox{}}
% % \\
%     % Z_t^i & \eqdef 
%     \underbrace{
%         \operatorname{ReLU}\bullet\big(
%             \phi^i\circ \tau_t\big(x_{(-\infty,t]}\big)
%             +\sigma_t^i\,W_t^i
%         \big)
%     }_{\mbox{Deep Features}}
% \end{aligned}
% \end{equation}
% where $\bullet$ denotes componentwise composition of the $\operatorname{ReLU}\eqdef \max\{0,\cdot\}$ activation function, encoders given by Borel functions $\phi^i:(\mathbb{R}^{d_x})^{\mathbb{Z}_-}\to \mathbb{R}^{d_z}$, $\sigma^i:\mathbb{Z}\to 
% \mathbb{R}
% % \mathbb{R}^{d_{z}\times d_z}
% $, $W^i_{\cdot}\eqdef (W^i_t)_{t\in \mathbb{Z}}$ is a $\mathbb{R}^{d_z}$-dimensional noise process independent of $X_{\cdot}$ and of $Y_{\cdot}$ is a family of i.i.d.\ standard normal random variables, $\beta_{\cdot}^i\eqdef (\beta_t^i)_{t\in \mathbb{Z}}$ is predictable with respect to the $\sigma$-algebra generated by $Y_{\cdot}$ and $\{\hat{Y}_{\cdot}^i\}_{i=1}^N$.  
% Each $\beta_{\cdot}^i$ is optimized online, thus fine-tuning the final layer of the model and allowing it to adapt to the newly observed information present in $Y_{\cdot}$.


% Our objective is to optimally adaptively \textit{synchronize} these $N$ generative models, into a single generative ensemble model $\hat{F}:(\mathbb{R}^{d_{x}})^{\mathbb{Z}}\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{Z}}$ to maximize their performance.  The resulting ensemble is represented by
% \[
%     \hat{F}(x_{\cdot})_t \eqdef \sum_{i=1}^N\, w_t^i\, \hat{f}^i(x_{\cdot})_t
% \]
% for mixture coefficients $w_{\cdot}\eqdef (w_t)_{t\in \mathbb{Z}}$ with each $w_t$ belonging to the $N$-simplex $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{i=1}^N\,w_i=1\}$.
% We consider the online \textit{one-shot} case, namely where the user actively optimizes the $w_{\cdot}$ and $\beta_{\cdot}$ parameters drawing from the one single trajectory progressively observed from $y_{\cdot}$; from which we gather information on the infinite-memory dynamical system $f$.


% \paragraph{Federated Computing Model}
% Each generative model $\hat{f}^i$ is stored locally on different machine $M^i$, in the network.  The $i^{th}$ machine communicates with the server at two different frequencies short term communication rounds between the local machines (nodes) and the central server.  Periodically, with period $T\in \mathbb{N}$, the server coordinates a randomly chosen subset of $0<\bar{N}\ll N$ local machines (nodes) in the distributed ensemble.

% \textit{Short communication rounds} occur at each instance time $t$ at which point each local machine individually optimizes its prediction $\hat{Y}_t^i$ by optimizing the control $\beta_t^i$ using the currently available time-series data 
% % by solving the ridge regression problem 
% \begin{equation}
% \label{eq:ridge_local}
%     \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=0}^t\,
%         e^{-\alpha^i(t-s)}
%         \,\|y_s-\beta_t^i\,Z_s^i\|^2
%         +
%         \gamma^i\|\beta_t^i\|^2
%     %%
%     \qquad \qquad 
%     \mbox{ for }t=0,\dots,T-1
% \end{equation}
% where the hyperparameter $\alpha^i\ge 0$ controls the exponentially decaying of importance on past time-series data and $\gamma^i> 0$ (see Proposition~\ref{prop:localgreedyupdates} for the ridge regression-like closed-form).
% Each local machine then sends its predictions $\hat{Y}_t^1,\dots,\hat{Y}_t^N$ to the server that generates a prediction from the ensemble.  This means that the rule by which the server identifies the time $t$ proportions $w_t$ with which it combines the $N$ distributed models to generate an only depends on the prediction of each model and not its internal parameters
% \[
%     w_t = w\big(
%         \hat{Y}_t^1,\dots,\hat{Y}_t^N
%     \big)
% \]
% for some function $w:\mathbb{R}^{d_y\times N}\to \Delta_N$.  
% The optimal function $w$, is the function minimizing the \textit{regret functional}
% \begin{align} 
%     J_0(w) 
%  = 
%      \sum_{t=1}^T 
%          \mathbb{E}  \, 
%          \Big[ 
%          \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%           + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] 
% ,  
% \notag 
% %\label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  Its expression is given in Theorem~\ref{thm:OptimalWeights}.



% \AK{I think, with no change in the analysis, we may instead only update a small random set of the models during the long communication rounds.  Perhaps the optimal communication frequency can be obtained by optimizing the total computational cost and the random sample of competing models.}

% \textit{Synchronization rounds} occur periodically at pre-specified period $T\in \mathbb{N}_+$.  
% In each such round
% % During short communication rounds, 
% the $N$ machines communicate their past $T$ predictions with one another; however, they do not communicate their entire model with one another since that would take an infeasible bandwidth due to the size of each local model.  
% Instead, the local machines are only aware of the predictions generated by one another with the objective of maximizing their predictive power.  

% Consequentially, each local machine can be interpreted as an agent competing with the optimal behaviour, i.e.\ value of $\beta_t^i$, as a solution to a Nash \textit{equilibrium} between these machines.  Thus, given the weight $w_1,\dots,w_T$, each local machine $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize its local objective function
% % \allowdisplaybreaks
% \begin{align} 
% \label{DTJi}  
%  % & 
%  J_i(\beta^i, \beta^{-i}) = 
%  \sum_{t=0}^{T} 
%  \add{ 
%     e^{-\alpha^i(T-t)} 
% }
%  \,
%  \mathbb{E} \Big\{  
%  \Big[ 
%  \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big] 
%   % + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 
%   \Big\}   
%   , \quad i = 1, ..., N ,  
% \end{align} 
% where $\beta^{-i}=(\beta^1, ..., \beta^{i-1}, \beta^{i+1}, ..., \beta^N)$ and $\alpha^i\ge 0$ is a pre-specified hyperparameter controlling the impact of distant past observations on the current game the local machines are playing with one another.  
% The optimal value for the $i^{th}$ machine, which we denote by $(\beta^i_{t:\text{sync}})_{t=0}^T$, is given in closed-form in Proposition~\ref{prop:NashEqmExistence}.  The following synchronization, we set
% \[
%     \beta_T^i\eqdef \beta_{T:sync}^i
% \]
% for each $i=1,\dots,N$.


% \AK{I think we should only sample the best $N$ performing models at any round.}

% \begin{algorithm}[ht!]%[H]%
% \caption{Proposed Federated Learning Algorithm}
% \label{alg:localnodes}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Current time $t\in \mathbb{N}$, Target time-series $(y_s)_{s\le t}$, pre-trained models $\{(\varphi^i,\sigma_{\cdot}^i,\hat{\mathbf{Y}}_{t-1}^i)\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$.
% \DontPrintSemicolon
%         \State \eIf{$t \bmod T\neq 0$}{
%             \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
%                 \ForParallel{
%                     $\beta_t^i \leftarrow 
%                     \big(
%                         {X^i}^{\top} X_t + \gamma^i I_{d_z}
%                     \big)^{-1}\, X_t^{\top} \, \bar{y}_t$
%                     \tcp*{Local Weighted Regression}
%                     \State 
%                       $(\hat{\mathbf{Y}}_t)_i
%                       \leftarrow
%                       \hat{\mathbf{Y}}_{t-1}^i
%                       + 
%                       (\beta_t^i)^{\top}\,
%                       \operatorname{ReLU}\bullet\big(
%                         \phi^i\circ \tau_t\big(x_{(-\infty,t]}\big)
%                         +\sigma_t^i\,W_t^i
%                     \big)
%                       $
%                       \tcp*{Generate Local Prediction}
%                         }
%                    }{
%                \For{$s=T-t,\dots,T$}{
%                    $
%                    \boldsymbol{\beta}^{\text{sync}}_s = [\beta^{\text{sync},1\top}_s, ..., \beta^{\text{sync}N,\top}_s ]^\top = - ( \Gamma + \mathbf{A}(s) )^{-1} \big( \mathbf{B}(s) \hat{Y}_t + \mathbf{C}(s) \big) 
%                    $
%                    \;
%                    $
%                    \beta_t^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_T)_i
%                    $
%                    \;
%                    $
%                    \hat{\mathbf{Y}}_t
%                       \leftarrow
%                       \hat{\mathbf{Y}}_{t-1}
%                       + 
%                       \Big(
%                             (\beta_t^i)^{\top}\,
%                           \operatorname{ReLU}\bullet\big(
%                             \phi^i\circ \tau_t\big(x_{(-\infty,t]}\big)
%                             +\sigma_t^i\,W_t^i
%                         \big)
%                     \Big)_{i=1}^N
%                    $
%                    \tcp*{Synchronize Local Models}
%                }
%               }
%     $
%         w_t \leftarrow
%   \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%     \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t -  \mathbf{c} \Big]
%     $
%      \;
%      $w_t \leftarrow 
%     \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t - w_t$
%     \tcp*{Update Mixture Weights}
%     %%
%     \State \Return $w_t^{\top} \hat{\mathbf{Y}}_t$.
%     \tcp*{Generate Prediction}
% \end{algorithmic}
% \textbf{Note:} The helper functions $\mathbf{A},\mathbf{B},\mathbf{C},\Gamma$ are defined in circa Proposition~\ref{prop:NashEqmExistence} and the matrices $K$, $G$, and $\mathbf{c}$ are defined in~\eqref{eq:Gc_Def}.
% \end{algorithm}

% \begin{comment}

% \subsection{The Optimization Problem}
% \label{s:EnsembleModel__ss:OprimizationProblem}

% We place ourselves at a given time $t-T\in \mathbb{Z}$, which we relabel without loss of generality to be $t-T=0$.  This means that we have observed a realization $(y_t)_{t\in \mathbb{Z};\,s\le T}$ of the process $Y_{\cdot}$ up to time $T$, and we also have observed the realized path $(y_t)_{t\in \mathbb{Z};\,s\le T}$, on which it depends, up to time $T$ as well.  In the interest of computational efficiency, suppose that we only want to use the newly observed time-series data, from time $0$ to time $T$, to update the mixture parameters $w_{\cdot}$.  In this case, the optimality of any candidate updates to $w_{\cdot}$ may be quantified by the following \textit{regret functional}
% \begin{align} 
%     J_0(w) 
%  = 
%      \sum_{t=1}^T \,\sum_{i=1}^N 
%          \mathbb{E}  \, 
%          \Big[ 
%          \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%           + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] 
% ,  
% \notag 
% \label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  


% Given: $M$ paths $(y_{[0:T]}^m,x_{[0:T]}^m)_{m=1}^M$.  Fix a reservoir system $\varphi:\mathbb{R}^L\times \mathbb{R}^d\rightarrow \mathbb{R}^p$, for a ``latent dimension'  $L$ and a reservoir dimension ``$p$'', where $L,p\in \mathbb{N}$.  \textit{In practice, $\varphi$ will be a pre-trained DL model like AlexNet or something.}  Consider a ``good'' linear approximation to $\varphi$, $Bz + Cx \approx \varphi$ \textit{to be made precise}.
% \begin{enumerate}
%     \item \textbf{Proposal Stage:}  Each player proposes (calibrates) a model 
%     $X^i_t = X^i_0 + \int_0^t A_i X^i_s ds + \int_0^t \sigma_i d W^i_s$ by minimizing
%     \[
%     \min_{A,\sigma}\, \frac1{J}\sum_{m=j}^J \mathbb{E}\big[\| X_t^i - x_t^{m_{i,j}}  \|^2 \big]
%     \]
%     where $(m_{i,1},\dots,m_{i,J})$ is a different (random) subset of the training paths.  \textit{Link to N-fold cross-validation in current formulation.  Link to ``masking'' as a type of noising.  Our objective is then to recover true "full information" ie ``unmasking/denoising''.}
%     \item \textbf{Competition State:} Each player competes to justify their proposed model 
%     \[
%     \begin{aligned}
%         & Z^i_t = Z^i_0 + 
% \int_0^t \varphi(Z^i_s, X^i_s) ds  \approx 
% Z^i_0 + 
% \int_0^t B Z^i_s + C X^i_s ds \\ 
% & \hat{Y}^i_t = \beta^i Z_0^i + \int_0^t \beta^i_s Z^i_s 
%  ds  , \quad i = 1, ..., N . 
%     \end{aligned}
%     \]
%     as being the correct one.  They do so by minimizing~\eqref{Ji}.  
%     \item \textbf{Selection State:} Fix a ``memory parameter'' $M\in \mathbb{N}_+$ and consider a compact set of continuous functions $\mathcal{H}$, in the uniform convergence on compacts topology, mapping $w:\mathbb{R}^{(1+d)M}\rightarrow \Delta_N$.  We learn closed-loop dynamics by optimizing
%     \[
%         \min_{w\in \mathcal{H}}\, \frac1{M}\,\sum_{m=1}^M\,
%         \mathbb{E}\Big[
%             \sum_{t=0}^T\,e^{-t}\,\|y_t - \sum_{i=1}^N\, w(y_{[t-M:t-1]},x_{[t-M:t-1]})_i \hat{Y}^i\|^2
%         \Big]
%     \]
%     \textit{we will implement $\mathcal{H}$ as a class of NNs, or randomized NNs.  We benchmark against the greed_{y} algorithm~\eqref{Nashw}}
% \end{enumerate}

% \end{comment}




% \section{Main Results}
% \label{s:Analysis}

% % Z is input signal
% % X is input noise/randomness (no randomness is an option!)

% We consider a model with $N$ agents $\{\mathcal{A}_i\}_{i=1}^N$. 
% Let each agent $\mathcal{A}_i$ has input signal sequence $\{Z^i_t\}_{t\geq 0}$ and a readout map.  
% \AK{This needs to be updated, but only at the end.}[.]
% \begin{equation}
% \begin{aligned} 
% & X^i_{t+1} =  A_i X^i_t + \sigma W^i_t , \quad X^i_\cdot \in \mathbb{R}^{dx \times 1} , \\  
% & Z^i_{t+1} =  \varphi(Z^i_t, X^i_{t+1}) ,  \quad Z^i_\cdot \in \mathbb{R}^{d_{z} \times 1} ,  \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t Z^i_t , \quad \hat{Y}^i_\cdot \in \mathbb{R}^{d_{y} \times 1} , \ i = 1, ..., N ,   
% \end{aligned} 
% \label{DTRCsystem}
% \end{equation} 
% where $W^i_t$, $i=1$, ..., $N$, $t=0$, ..., $T$ are identically independently distributed standard normal random variables. 
% Consider a major agent who also acts as a central planner and chooses weight vector sequence on the $N$-simplex   
% \begin{align} 
% w_t= (w^1_t, ..., w^N_t)^\top \in \Delta_N , \quad t = 0, 1, ..., T \notag  
% \end{align} 
% for the minor players' output $\hat{Y}^i$ in order to minimize the total loss  
% \begin{align} 
%  J_0(w) = \mathbb{E}  \sum_{t=1}^T \Big[ 
%  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] ,  
%   \notag 
%   \label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  

% Given the weight $w_t = (w^1_t, ..., w^N_t)$, $t=0$, $1$, ..., $T$, each minor agent $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize the individual cost 
% \allowdisplaybreaks
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 \Big\}   , \quad i = 1, ..., N ,  \label{DTJi}  
%   \end{align} 
%  where $\beta^{-i}=(\beta^1, ..., \beta^{i-1}, \beta{i+1}, ..., \beta^N)$. 




% \subsection{The Nash Equilibrium between the Minor Players}
% Denote 
% \begin{align} 
%  & \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top, \quad \hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top, \quad   
% \mathbf{e}^N_i = e^N_i \otimes I_{d_{z}} = [0, ..., I_{d_{z}} , ..., 0]^\top,  \notag \\ 
%  & \Gamma = \diag[\gamma_1, ..., \gamma_N] \notag 
% \end{align} 
% then the costs \eqref{DTJi} for the $N$ agents can be written as  
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \mathbf{w}^\top_t \hat{Y}_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y_T - \mathbf{w}_T^\top \hat{Y}_T \Big\|^2 \Big\}   , \quad i = 1, ..., N. 
%   \label{DTJicompact}
%  \end{align} 

%  We aim to find a set of Nash equilibrium strategies $(\beta^1, ..., \beta^N)$ for the $N$ agent such that 
%  \begin{align} 
%  J_i(\beta^i, \beta^{-i}) 
%  \leq J_i(u, \beta^{-i}), 
%  \quad \forall u \in \mathbb{R}^{d_{z} \times d_{y}} , 
%  \quad  \forall i = 1, ..., N. \label{NEbeta}
%  \end{align} 



% We introduce the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% $t=0$, $1$ ..., $T$. 
% \begin{equation} 
% \begin{cases}  
%   P_i(t) = 
%  [ \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]^\top P_i(t+1) [  \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]  \\ 
%   \hspace{2cm} + [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ]^\top 
%  [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ] 
%  + \mathbf{w}_t \mathbf{w}_t^\top  \\ 
%   \Gamma + \mathbf{A}(t) \, \text{is invertible}  \\ 
%   P_i(T) =  \mathbf{w}_T \mathbf{w}_T^\top  , \quad i = 1, 2, ..., N , 
%  \end{cases}
%  \label{eqn:Pi}
%  \end{equation} 

% \allowdisplaybreaks 
% \begin{equation}  
%  \begin{cases} 
%   S_i(t) =   \mathbf{B}(t)^\top (I + \mathbf{A})^{-1} 
%  [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t) ] (I+\mathbf{A})^{-1} \mathbf{C}   \\ 
%   \hspace{1cm} - P_i(t+1) \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{C} 
%  - \mathbf{B}^\top (I + \mathbf{A})^{-1}\mathbf{D} S_i(t+1) 
%  - \mathbf{w}_t y_t 
%  + S_i(t+1) , 
%   \\ 
%  S_i(T) = - \mathbf{w}_T y_T   . 
% \end{cases}   
% \label{eqn:Si}
% \end{equation} 
% %The matrices $\mathbf{A}(\cdot) = (A_{ij}(\cdot))_{1\leq i , j \leq N}$,  
% %$\mathbf{B}(\cdot) = \big[ B_1(\cdot)^\top, ..., B_N(\cdot)^\top \big]^\top$, 
% %and $\mathbf{C}(\cdot) = \big[ C_1(\cdot)^\top, ..., C_N(\cdot)^\top \big]$ are defined by  
% %\begin{align} 
% %& A_{ij}(t) = \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i( t+1 ) e_j Z^{j\top}_t \Big\} ,   \label{Aij} \\ 
% %& B_i(t) = \mathbb{E}(Z^i_t) e_i^\top  P_i(t+1)  , \notag \\ 
% %& C_i(t) = \mathbb{E}(Z^i_t) e_i^\top  S_i(t+1) , 
% %\quad 1 \leq i , j \leq N . \notag 
% %\end{align} 
% In \eqref{eqn:Pi} and \eqref{eqn:Si}, the matrices $\mathbf{A}(\cdot)$,  
% $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, and $\mathbf{D}(\cdot)$ are defined by  
% \allowdisplaybreaks 
% \begin{align} 
% &\mathbf{A}(t) = \begin{bmatrix} 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_1 Z^{1\top}_t ] & 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_N Z^{N\top}_t ] \\ 
%  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_1 Z^{1\top}_t ] & 
%  \mathbb{E} [(e_2 Z^{1\top}_t)^\top P_2(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_N Z^{N\top}_t ] \\ 
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \mathbb{E}[ (e_N Z^{N\top}_t)^\top P_N(t+1) e_1 Z^{1\top}_t ]& 
%  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_N Z^{N\top}_t ]
% \end{bmatrix} \notag \\ 
% & \mathbf{B}(t) = 
%  \begin{bmatrix} 
%  \mathbb{E} (e_1 Z^{1\top}_t )^\top P_1(t+1) \\ 
%  \mathbb{E}(e_2 Z^{2\top}_t )^\top P_2(t+1) \\ 
%  \vdots \\  
%  \mathbb{E} (e_N Z^{N\top}_t) P_N(t+1) 
%  \end{bmatrix} ,  
%  \qquad 
%  \mathbf{C}(t) = 
%  \begin{bmatrix} 
%  \mathbb{E}(e_1 Z^{1\top}_t )^\top S_1(t+1) \\ 
%  \mathbb{E}(e_2 Z^{2\top}_t )^\top S_2(t+1) \\ 
%  \vdots \\ 
%  \mathbb{E}(e_N Z^{N\top}_t) S_N(t+1) 
%  \end{bmatrix} , 
%  \notag \\ 
% & \mathbf{D}(t) 
%  = 
%  \begin{bmatrix} 
%  \mathbb{E}( e_1 Z^{1\top}_t ) , \, 
% \mathbb{E} ( e_2 Z^{2\top}_t ) ,  \,
%  \cdots , \, 
% \mathbb{E} ( e_N Z^{N\top}_t )
%  \end{bmatrix} . 
%  \notag 
% \end{align} 

% %\begin{align} 
% % \mathbf{e}_i = e_i \otimes I_{N} 
% % = [0, ..., 0, I_{d_{z}}, 0, ..., 0] \notag 
% %\end{align} 






% The following proposition links the existence of a Nash equilibrium of \eqref{DTRCsystem} and \eqref{DTJi} to the solvability of the system \eqref{eqn:Pi}. 
% \begin{proposition}[Nash Equilibrium of Minor Players]
% \label{prop:NashEqmExistence}
% Suppose the system \eqref{eqn:Pi} for $(P_i)_{i=1}^N$ admits a solution for $t=0$, $1$, ..., $T$.  
% Then the $N$-player Nash game \eqref{DTJi} admits a unique feedback Nash equilibrium 
% \begin{align} 
% \boldsymbol{\beta}_t = [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% \big( \mathbf{B}(t) \hat{Y}_t + \mathbf{C}(t) \big) , \quad t = 0, 1, ..., T. 
% \label{eqmvecbeta} 
% \end{align} 
% \end{proposition}

% \AK{Let us write the special case as a corollary.}

% For each $i=1,\dots,N$, let $(a_t^i)_{t\in \mathbb{N}}$ and $(\sigma_t^i)_{t\in \mathbb{N}}$ respectively be sequences in $\mathbb{R}^{d_z\times 1}$ and in $(0,\infty)$.  
% Suppose that the system in~\eqref{DTRCsystem} is 
% \begin{equation}
% \begin{aligned} 
% & Z^i_{t+1} =  
% \operatorname{ReLU}\bullet\big(
%     a_t + \sqrt{\sigma_t^i}\, W_t^i
% \big) ,  
% % \quad Z^i_\cdot \in \mathbb{R}^{d_{z} \times 1} ,  
% \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t Z^i_t 
% .
% % , \quad \hat{Y}^i_\cdot \in \mathbb{R}^{d_{y} \times 1} , \ i = 1, ..., N ,   
% \end{aligned} 
% \label{DTRCsystemReLU}
% \end{equation} 


% \begin{corollary} 
% If $\varphi(\cdot)$ in \eqref{DTRCsystem} takes the form in \eqref{DTRCsystemReLU},  
% \end{corollary} 

% \begin{proof} 

% \begin{align} 
%  & \mathbb{E} \big[ Z^i_t e_i^\top P_i(t+1) e_j Z^{j\top}_t \big]  
%  =  \mathbb{E} \big[ Z^i_t  ( P_i(t+1) )_{ij}  Z^{j\top}_t \big] \notag 
% \end{align} 
% The diagonal submatrices of $\mathbf{A}(t)$ take the form  
% \begin{align} 
%  &  \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_i Z^{i\top}_t ]  \notag \\ 
%   = &  \mathbb{E} [  Z^i_t e_i^\top P_i(t+1) e_i Z^{i\top}_t ] \notag \\ 
% = &   \mathbb{E} [  Z^i_t  ( P_i(t+1) )_{ii} Z^{i\top}_t ]  \notag \\ 
%  = & \Big( \mathbb{E}\big[  (Z_{t+1}^i)_j ( P_i(t+1) )_{ii}  (Z_{t+1}^i)_k \big]  \Big)_{1\leq j, k \leq dz} . \notag 
% \end{align} 
% By Lemma~\ref{lem:Mean_Cov_ResModel}, the entries in the diagonal submatrices of $\mathbf{A}(t)$ are given by  
% \begin{align} 
%  & \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii}\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = \big[ \mathbb{E}( Z_{t+1}^i )
%     \mathbb{E}( Z_{t+1}^{i\top} ) \big]_{jk} 
%     & \mbox{ if }   j \neq k
%     \end{cases} 
%     \notag 
% \end{align} 
% where 
% \begin{align} 
%  & \big[ \mathbb{E}( Z_{t+1}^i )
%     \mathbb{E}( Z_{t+1}^{i\top} ) \big] \notag \\ 
%     =& 
%     \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big) \Big\} 
%     \Big\{ 
%      a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big)
%     \Big\}^\top . \notag 
% \end{align} 


% Since the white noises $\{W^i_t\}_{i, t}$, are independent, \eqref{DTRCsystemReLU} implies that 
% $Z^i_t$ and $Z^j_t$ are independent for $i\neq j$. 
% The off-diagonal submatrices of $\mathbf{A}(t)$ can be written as   
% \begin{align} 
%  & \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_j Z^{j\top}_t ] \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  e_i^\top P_i(t+1) e_j  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  ( P_i(t+1) )_{ij}  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big) \Big\} (P_i(t+1))_{ij} 
%         \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^j}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^j}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^j}
%             % \,
%             a_t^2
%         \Big) \Big\}^\top    \notag 
% \end{align} 
% where $\mathbb{E} [  Z^i_t ]$ and $\mathbb{E} [  Z^j_t ]$ are given explicitly by Lemma~\ref{lem:Mean_Cov_ResModel}. 


% \end{proof} 



% Under these dynamics, the following lemma gives enough information to compute the relevant matrices in Proposition~\ref{prop:NashEqmExistence}.
% \begin{lemma}[{Mean and Covariance of $Z_{\cdot}^i$ in the System~\eqref{DTRCsystem}}]
% \label{lem:Mean_Cov_ResModel}
% Consider the setting of~\eqref{DTRCsystem}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[Z_{t+1}^i] 
%     = &
%         a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big)
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of~\eqref{DTRCsystem}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion.
% \end{proof}

% \subsection{The Short Communication Rounds}
% \label{s:ShortComm}
% We first give an expression for the optimal control of the local model, when optimizing their predicting performance before the synchronization time $T$.
% \begin{proposition}[Intermittent Optimal Controls for Local Machines]
% \label{prop:localgreedyupdates}
% Let $\alpha^i\ge 0$ and $\gamma^i>0$.  Then unique solution to~\eqref{eq:ridge_local} is given by
% \[
%         \beta_t^i 
%     =
%         \big(
%             {X^i}^{\top} X_t + \gamma^i I_{d_z}
%         \big)^{-1}\, X_t^{\top} \, \bar{y}_t
% \]
% where $X_t \eqdef (e^{-\alpha^i (t-0)} Z_0,\dots,e^{-\alpha^i(t-s)}Z_s,\dots, Z_t) \in \mathbb{R}^{(1+t)\times d_z}$ and $\bar{y}_t \eqdef (e^{\alpha^i(t-s)}y_s)_{s=0}^t \in \mathbb{R}^{(1+t)\times d_y}$.
% \end{proposition}
% \begin{proof}[{Proof of Proposition~\ref{prop:localgreedyupdates}}]
% Observe that the loss function in~\eqref{eq:ridge_local} can be re-written as
% \allowdisplaybreaks
% \begin{align}
% \label{eq:redux_ridge}
%         \sum_{s=0}^t\,
%             e^{-\alpha^i(t-s)}
%             \,\|y_s-\beta_t^i\,Z_s^i\|^2
%             +
%             \gamma^i\|\beta_t^i\|^2
%     =
%         \sum_{s=0}^t\,
%             \,\|\big(e^{-\alpha^i(t-s)}y_s\big)-\beta_t^i\,(e^{-\alpha(t-s)} Z_s^i)\|^2
%             +
%             \gamma^i\|\beta_t^i\|^2
% \end{align}
% and the right-hand side of~\eqref{eq:redux_ridge} is simply a standard ridge-regression problem.  Since this is a strictly convex problem, there is a unique $\beta_t^i\in \mathbb{R}^{d_y\times d_x}$ minimizing the right-hand side of~\eqref{eq:redux_ridge}.  The desired closed-form expression is given in \citep[Equation (3.44)]{HastieTibshiraniFriedman_2001ESLBook}.
% \end{proof}

% \subsubsection{The Major Player's Selection of Optimal Weights} 

% Consider the objective of the major player/central planner is to optimize 
% \begin{align} 
%     \min_{w_{\cdot}}\,
%  J_0(w) = \mathbb{E}  \sum_{t=1}^T \Big[  
%  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] .  
%   \label{DTJ0}
% \end{align} 
% where the minimization is taken over all decision rules $w_{\cdot} \eqdef \{w_t\}_{t=1}^T = \{(w^1_t, ..., w^N_t)\}_{t=1}^T$ whose paths lie in the $N$-simplex $\Delta_N \eqdef  \{w\in [0,1]^N:\, \sum_{n=1}^N\, w_n=1\}$.  
% Our first main result shows that there exists a unique solution to the optimization problem~\eqref{DTJ0}.
% \begin{theorem}[Optimal Coordination]
% \label{thm:OptimalWeights}
% The quadratic programming problem \eqref{MajorPlayer:QP} admits a unique solution $w^\star = (w^{1, \star}, ..., w^{N, \star})$ given by 
% \begin{align} 
% \notag
%   w^\star   =   \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
% % \\    
%   % &
%   -  & \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%   \\
%   &\times 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t  -  \mathbf{c} \Big] . 
%   \label{eqn:OptimalWeights}  
% \end{align} 
% where we denote 
% \begin{align} 
%  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N}, 
%  \quad 
%  G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  \mbox{ and }
%  \quad 
%   \mathbf{c} =  \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%   \label{eq:Gc_Def}
% \end{align} 

% \end{theorem} 



% \section{Proofs}
% \label{s:Proofs}

% This section contains the proofs of our main results.

% \subsection{{Proof of Proposition~\ref{prop:NashEqmExistence}}}
% \label{s:Proofs__ss:prop:NashEqmExistence}
% \begin{proof}
% Let $V_i(t,\hat{\mathbf{y}})$, $i=1$,...,$N$ be the value functions of the $N$ players associated with \eqref{DTRCsystem} and \eqref{DTJi}. 
% %\begin{align}  
% % & V_i(t, \hat{\mathbf{y}}) 
% %=  \sup_{\beta^i} \mathbb{E} \Big\{  
% % \Big\| y^i_t - \sum_{i=1}^N w^i 
% % \hat{y}^i \Big\|^2 
% %  + \| \beta^i \|^2    
% %+ V_i(t+1, \hat{\mathbf{y}} + 
% % \sum_{j=1}^N  e_j Z^{j\top}_t\beta^j) 
% %  \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
% %   & V_i(T, \hat{\mathbf{y}}) 
% %   = \notag 
% %\end{align} 
% From \eqref{DTJicompact}, the value functions at time $T$ with $\hat{Y}_T=\hat{\mathbf{y}}$ satisfy 
% \begin{align} 
%  V_i(T, \hat{\mathbf{y}}) 
%  =  \Big\| y_T -  \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%  = \hat{\mathbf{y}}^\top \mathbf{w}_T \mathbf{w}_T^\top \hat{\mathbf{y}} 
%  - 2 y_T \mathbf{w}_T^\top \hat{\mathbf{y}} + |y_T|^2 .  
%  \label{Vi(T)}
% \end{align} 
% By the dynamic programming principle, the value functions at $T-1$ with $\hat{Y}_{T-1}= \hat{\mathbf{y}}=(\hat{y}^{1\top}, ..., \hat{y}^{N\top})^\top$ satisfies  
% \begin{align} 
% V_i(T-1, \hat{\mathbf{y}}) 
% = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    + V_i(T, \hat{\mathbf{y}} + \sum_{j=1}^N  e_j Z^{j\top}_{T-1} \beta^j ) 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
%    = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%   + \gamma_i \| \beta^i \|^2     + \Big\| y_T - \sum_{j=1}^N w^j_T \Big( \hat{y}^j +  Z^{j\top}_{T-1}  \beta^j \Big)  \Big\|^2 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
% = & \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%  + \Big\| y_T - \mathbf{w}^\top \hat{\mathbf{y}} \Big\|^2   \notag \\  
%  &    + \mathbb{E} \Big\{  \gamma_i \| \beta^i \|^2 + \Big\| \sum_{j=1}^N w^j_T Z^{j\top}_{T-1} \beta^j \Big\|^2 
%   - 2 \Big( y_T - \sum_{j=1}^N w^j_T \hat{y}^j \Big)^\top \sum_{j=1}^N w^j_T Z^{j\top}_{T-1} \beta^j 
%     \Big\} .
%    \label{DPeqnVi(T-1)}
% \end{align} 
% By the first order condition for the right side of \eqref{DPeqnVi(T-1)}, we have 
% \begin{align} 
%  \gamma_i \beta^i +  \sum_{j=1}^N \mathbb{E} \big[  Z^i_{T-1} w^i_T w^j_T Z^{j\top}_{T-1} \big]  \beta^j  
%    + \mathbb{E} \big[ Z^i_{T-1} \big] w^i_T \sum_{j=1}^N w^j_T \hat{y}^j   - Z^i_{T-1} w^i_T y_T 
%  = 0 , \quad i = 1, ..., N \notag 
% \end{align} 
% which can be written in the compact form 
% \begin{align} 
%  \Gamma [\beta^{1\top}, ..., \beta^{N \top}]^\top = - \mathbf{A}(T-1) [\beta^{1\top}, ..., \beta^{N \top}]^\top 
%  - \mathbf{B} (T-1) \hat{\mathbf{y}} - \mathbf{C}(T-1) .  
% \end{align} 
% Since \eqref{eqn:Pi} admits a solution by the hypothesis of the proposition, we have that $\Gamma + \mathbf{A}(T-1)$ is invertible, and hence 
% \begin{align} 
%   \boldsymbol{\beta}_{T-1} = [\beta^{1\top}_{T-1}, ..., \beta^{N \top}_{T-1} ]^\top = - ( \Gamma  + \mathbf{A}(T-1) )^{-1} 
% \big( \mathbf{B}(T-1) \hat{Y}_{T-1} + \mathbf{C}(T-1) \big) . 
% \label{eqmbetaT-1}
% \end{align} 

% Substituting \eqref{eqmbetaT-1} into \eqref{DPeqnVi(T-1)}, 
% we obtain that $V_i(T-1, \hat{\mathbf{y}})$ take the form 
% \begin{align} 
%   V_i(T-1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(T-1) \hat{\mathbf{y}}  
%   + 2 S_i(T-1)^\top \hat{\mathbf{y}} + r_i(T-1) , \quad i = 1, ..., N. \notag  
%  \end{align} 
%  where $P_i(T-1)$ and $S_i(T-1)$ are determined by \eqref{eqn:Pi} and \eqref{eqn:Si}. 

% Assume by induction that at $t$ the value functions $\{V_i(t+1, \hat{\mathbf{y}})\}_{i=1}^N$ take the affine-quadratic form 
% \begin{align} 
%   V_i(t+1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t+1) \hat{\mathbf{y}}  
%   + 2 S_i(t+1)^\top \hat{\mathbf{y}} + r_i(t+1) , \quad i = 1, ..., N , \notag  
%  \end{align} 
% with $P_i$ and $S_i$ determined from \eqref{eqn:Pi} and \eqref{eqn:Si}, respectively. 
% We show that at $t$ with state $\hat{Y}_t=\hat{\mathbf{y}}$ the value functions $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ also take the form 
% \begin{align} 
%   V_i(t, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) , \quad i = 1, ..., N . \notag  
%  \end{align} 
% %and the equilibrium strategy $\boldsymbol{\beta}=[\beta^{1\top}, ..., \beta^{N\top} ]$ is indeed given by \eqref{eqmvecbeta}. 

 
% By the dynamic programming principle, $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ satisfy the system of dynamic programming equations:  
% \begin{align} 
% V_i(t, \hat{\mathbf{y}}) 
% = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_t - \sum_{i=1}^N w_t^i \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    + V_i(t+1, \hat{\mathbf{y}} + \sum_{j=1}^N  e_j Z^{j\top}_t \beta^j ) 
%    \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
%   =& \sup_{\beta^i} \mathbb{E} 
%   \Big\{  \Big\| y_t - \sum_{i=1}^N w^i_t \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2 
%    + \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{j\top}_t  \beta^j  \Big]^\top P_i(t+1) 
%   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{j\top}_t  \beta^j  \Big] \notag \\ 
%  &   \hspace{5cm}  + 2 S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{i\top}_t  \beta^j  \Big] 
%   + r_i(t+1)   \Big| \hat{Y}_t = \mathbf{\hat{y}}    \Big\} \notag \\ 
% %%%%% 
%   = &  \sup_{\beta^i} \Big\{ \Big\| y_t - \sum_{i=1}^N w^i_t \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2 + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}}  
%   + 2 \hat{\mathbf{y}}^\top P_i(t+1) \sum_{j=1}^N e_j \mathbb{E}(Z^{j\top}_t) \beta^j \notag \\ 
%    & + \sum_{j, k=1}^N \beta^{j\top} \mathbb{E} \Big\{ (e_j Z^{j\top}_t )^\top P_i(t+1) e_k Z^{k\top}_t \Big\}  \beta^k 
%    + 2 S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j \mathbb{E}(Z^{j \top}_t )  \beta^j  \Big] 
%    + r_i(t+1) \Big\} \notag \\ 
%    & i = 1, ..., N . 
%   \label{DPeqnV(y)}
% \end{align} 
% By the first order condition for the right side of \eqref{DPeqnV(y)}, we have 
% \begin{align} 
%  - \gamma_i \beta^i = &  \mathbb{E}(Z^i_t) e_i^\top P_i(t+1) \hat{\mathbf{y}}  
%   + \sum_{j=1}^N  \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i(t+1) e_j Z^{j\top}_t \Big\}  \beta^j  
%   + \mathbb{E}(Z^i_t) e_i^\top  S_i(t+1) \notag \\ 
%   = &  \sum_{j=1}^N  \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i(t+1) e_j Z^{j\top}_t \Big\}  \beta^j  
%   + \mathbb{E}(Z^i_t) e_i^\top [ P_i(t+1) \hat{\mathbf{y}}  +  S_i(t+1) ] ,   
%  \label{betaifirstorderV(y)} \\ 
%  & i = 1, 2, ..., N. \notag 
% \end{align} 


% Then \eqref{betaifirstorderV(y)} can be written in the compact form  
% \begin{align} 
% - \Gamma [\beta^{1\top}, ..., \beta^{N \top}]^\top = \mathbf{A}(t) [\beta^{1\top}, ..., \beta^{N \top}]^\top 
%  + \mathbf{B} (t) \hat{\mathbf{y}} + \mathbf{C}(t) , \notag 
% \end{align} 
% and therefore the equilibrium strategy at time $t$ is determined by 
% \begin{align} 
% [\beta^{1\top}, ..., \beta^{N \top}]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% \big( \mathbf{B}(t) \hat{\mathbf{y}} + \mathbf{C}(t) \big) .  \notag   
% \end{align} 
% %With the defined $\mathbf{A}$ and $\mathbf{B}$, we can write the system \eqref{DPeqnV(y)} as 

% %By induction, we have shown that 
% \end{proof} 


% \begin{comment} 
% From \eqref{Aij}, we have 
% \allowdisplaybreaks
% \begin{align} 
%    A_{ij}(t) = & \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i( t+1 ) e_j Z^{j\top}_t \Big\} \notag \\  
% = & \mathbb{E} \mathrm{Tr} \Big\{  P_i( t+1 ) e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big\} \notag \\ 
% = &  \mathrm{Tr} \Big\{  P_i( t+1 )  \mathbb{E} \Big[  e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big] \Big\} 
% \notag 
% \end{align}
%  For $\mathbb{E} \Big[  e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big]$, we can find a matrices $M^i_t$ and $M^j_t$ such that 
%  \begin{align} 
%  \mathbb{E} \Big[  e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big] = M^i_t M_t^{j\top} . 
%  \end{align} 
%  It then follows that 
%  \allowdisplaybreaks
% \begin{align} 
%    A_{ij}(t) = & \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i( t+1 ) e_j Z^{j\top}_t \Big\} \notag \\  
% = & \mathbb{E} \mathrm{Tr} \Big\{  P_i( t+1 ) e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big\} \notag \\ 
% = &  \mathrm{Tr} \Big\{  P_i( t+1 )  \mathbb{E} \Big[  e_j Z^{j\top}_t (e_i Z^{i\top}_t )^\top \Big] \Big\} 
% \notag \\ 
% = & \mathrm{Tr} \Big\{  P_i( t+1 )  M^i_t M^{j\top}_t \Big\} \notag \\ 
% = & M_t^{j \top} P_i(t+1) M_t^i \notag 
% \end{align} 

% Assuming $Z^i_t$ and $Z^j_t$ are independent for all $i\neq j$, we have 
% \allowdisplaybreaks
% \begin{align} 
%    A_{ij}(t) = & \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i( t+1 ) e_j Z^{j\top}_t \Big\} \notag \\  
% = & 
% [e_i \mathbb{E}(Z^{i\top}_t) ]^\top P_i( t+1 ) e_j \mathbb{E}(Z^{j\top}_t)  
% \notag 
% \end{align}

% We substitute \eqref{eqmvecbeta} into \eqref{DPeqnV(y)}: 
% \begin{align} 
%  V_i(t, \hat{\mathbf{y}}) = & 
%   \boldsymbol{\beta}^\top \big[ \mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}^\top P_i(t+1) \mathbf{D}  \big] \boldsymbol{\beta} 
%   + 2 \big[ \hat{\mathbf{y}}^\top P_i(t+1) + S_i(t+1)^\top \big] \mathbf{D} \boldsymbol{\beta}  \notag \\  
%  &  +  \Big\| y^i_t - \sum_{i=1}^N w^i \hat{y}^i \Big\|^2  + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}} + 2 S_i(t+1)^\top \hat{\mathbf{y}} , 
% \end{align} 

% \begin{align} 
%  \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) 
%   = & 
%   (\hat{\mathbf{y}}^\top \mathbf{B}^\top + \mathbf{C}^\top) (I + \mathbf{A}^\top)^{-1} 
%   [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}^\top P_i(t+1) \mathbf{D}] (I + \mathbf{A})^{-1} (\mathbf{B} \hat{\mathbf{y}} + \mathbf{C} ) \notag \\ 
%   & - 2 [ \hat{\mathbf{y}}^\top P_i(t+1) + S_i^\top(t+1) ] \mathbf{D} (I+\mathbf{A})^{-1} (\mathbf{B} \hat{\mathbf{y}} + \mathbf{C} ) \notag \\ 
%   & + |y^i_t|^2 + \hat{\mathbf{y}}^\top \mathbf{w} \mathbf{w}^\top \hat{\mathbf{y}} 
%    - 2 y^i_t \mathbf{w}^\top \hat{\mathbf{y}} 
%     + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}} + 2 S_i(t+1)^\top \hat{\mathbf{y}}   \notag 
% \end{align} 
% Then we obtain the equation for $P_i(\cdot)$: 
% \allowdisplaybreaks 
% \begin{align} 
%  P_i(t) = & \mathbf{B}^\top (I + \mathbf{A}^\top)^{-1}
% [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}^\top P_i(t+1) \mathbf{D} ] (I+\mathbf{A})^{-1} 
% \mathbf{B}  \notag \\ 
% & - P_i(t+1) \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{B} 
%  - \mathbf{B}^\top (I + \mathbf{A}^\top)^{-1} 
%  \mathbf{D}^\top P_i(t+1) 
%  + \mathbf{w} \mathbf{w}^\top + P_i(t+1) 
%  \notag 
%  \end{align}  

%  \begin{align} 
%  & P_i(t) = 
%  [ \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{B} - I ]^\top P_i(t+1) [  \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{B} - I ] \notag \\ 
%  & \hspace{2cm} + [ \mathbf{e}_i^\top \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{B} ]^\top 
%  [ \mathbf{e}_i^\top \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{B} ] 
%  + \mathbf{w} \mathbf{w}^\top \notag \\ 
%  & (I + \mathbf{A})^{-1} \quad \text{exists} \notag \\ 
%  & P_i(T) =  \mathbf{w} \mathbf{w}^\top \notag 
%  \end{align} 



% \allowdisplaybreaks
% \begin{align} 
%  r_i(t) 
%  = & \mathbf{C}^\top (I + \mathbf{A}^\top)^{-1}
% [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}^\top P_i(t+1) \mathbf{D} ] (I+\mathbf{A})^{-1} 
% \mathbf{C} \notag \\ 
% & - S_i(t+1)^\top \mathbf{D} 
% (I + \mathbf{A})^{-1} \mathbf{C} 
% - \mathbf{C}^\top  
% (I + \mathbf{A})^{-1} 
% \mathbf{D}^\top S_i(t+1) 
%  + |y^i_t|^2 \notag \\ 
%  r_i(T) = & |y^i_t|^2 \notag 
% \end{align} 
% \end{comment}

% \subsection{{Proof of Theorem~\ref{thm:OptimalWeights}}}
% \label{s:Proofs__ss:OptimalWeights}
% We minimize \eqref{DTJ0} over all $\Delta_N$-valued decision rules $w_{\cdot}$.  
% At each time $t$, the major player needs to solve the nonlinear programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N) }  \big\| y_t - \sum_{j=1}^N w^j \hat{y}^j_t \big\|^2 
%  + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 \\ 
% & \text{subject to} \ \mathbf{g}(w)=(w^1-1, ..., w^N-1, -w^1, ..., -w^N) \leq 0 , \quad 
%  h(w) = w^1 + ... + w^N - 1 = 0 . 
% \end{aligned} 
% \label{MajorPlayer:NLoptim}
% \end{equation} 

% Denote 
% \begin{align} 
% % \hat{\mathbf{Y}}_t = \big[ \hat{y}^1_t, \cdots , \hat{y}^N_t \big] , \quad 
%   \mathbf{1}_{1\times N} = \big[ 1, ..., 1 \big] \in \mathbb{R}^{1\times N} , \quad 
%  % \hat{\boldsymbol{\lambda}} = \big[ \hat{\lambda}_1, ..., \hat{\lambda}_N \big]^\top , \quad 
%  % \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N} . \notag 
% \end{align} 



% Since the objective function of the nonlinear programming problem \eqref{MajorPlayer:NLoptim} can be written as 
% \begin{align} 
%   \Big\| y_t - \sum_{j=1}^N w^j \hat{y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 
%  = &  \Big( y^\top_t - \sum_{j=1}^N w^j \hat{y}^{j\top}_t \Big) 
%  \Big( y_t - \sum_{j=1}^N w^j \hat{y}^j_t \Big) + \sum_{j=1}^N \kappa_j w^{j 2}   \notag \\ 
%  = & N \sum_{i,j=1}^N w^i \hat{y}^{i\top}_t \hat{y}^j_t w^j 
%   - 2  y^\top_t   \sum_{j=1}^N w^j \hat{y}^j_t 
%    + y^\top_t y_t + \sum_{j=1}^N \kappa_j w^{j 2} \notag \\ 
%  = &  w^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) w 
%   - 2  y^\top_t  \hat{\mathbf{Y}}_t w 
%    + y^\top_t y_t . \notag 
% \end{align} 
% Therefore the nonlinear programming problem \eqref{MajorPlayer:NLoptim} is equivalent to the following quadratic programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N)^\top } \frac{1}{2}  w^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t     + \mathrm{K} \big) w 
%   -  y^\top_t  \hat{\mathbf{Y}}_t w , \\ 
% & \text{subject to} \ G w \leq \mathbf{c} ,
% \end{aligned} 
% \label{MajorPlayer:QP}
% \end{equation} 
% where $G$ and $\boldsymbol{c}$ are defined in~\eqref{eq:Gc_Def}.



% To prove Theorem~\ref{thm:OptimalWeights}, we need to use the results of the following Theorems~\ref{thm:NSQP} and \ref{thm:QPdual} from \cite{Berkovitz2001}. 
% According to \cite[Theorem V.6.1]{Berkovitz2001}, the following theorem gives a necessary and sufficient condition for solutions of \eqref{MajorPlayer:QP}. 
% \begin{theorem} 
% \label{thm:NSQP}
% A necessary and sufficient condition for a point $w^\star=(w^{1, \star}, ..., w^{N, \star})^\top$ to be a solution of the quadratic programming problem \eqref{MajorPlayer:QP} is that 
% \begin{align} 
% G w^\star \leq \mathbf{c} \label{NSQP:Gw<=c} 
% \end{align} 
% and there exists a vector $\boldsymbol{\lambda} \geq 0$ in $\mathbb{R}^{2N+2}$ such that 
% \begin{align} 
%  & \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  w^\star - \hat{\mathbf{Y}}_t^\top y_t 
%   + G^\top \boldsymbol{\lambda} = 0 , \label{NSQP:w+lambda} \\ 
%  & \boldsymbol{\lambda}^\top (G w^\star - \mathbf{c}) = 0 . \label{NSQP:wlambda}  
% \end{align} 
% \end{theorem}

% Introduce the dual quadratic programming problem: 
% \begin{equation} 
% \begin{aligned}  
% & \max \big\{ \theta (\boldsymbol{\lambda}) : \ \boldsymbol{\lambda} \geq 0 , \ \theta(\boldsymbol{\lambda}) > -\infty \big\} , 
%  \\ 
% & \theta(\boldsymbol{\lambda}) = \inf \{ L( \mathbf{x}, \boldsymbol{\lambda}) : \ \mathbf{x} \in \mathbb{R}^N \} ,  \\ 
% & L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}  
%   -  y^\top_t  \hat{\mathbf{Y}}_t \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) .   
% \end{aligned} 
% \label{MajorPlayer:DQP} 
% \end{equation} 

% By \cite[Theorem V.6.2]{Berkovitz2001}, we have the following relation between the quadratic programming problem \eqref{MajorPlayer:QP} and the dual problem \eqref{MajorPlayer:DQP}. 
% \begin{theorem} 
% \label{thm:QPdual}
% Let the quadratic programming problem \eqref{MajorPlayer:QP} has a solution $w^\star=(w^{1, \star}, ..., w^{N, \star})$. Then the dual problem \eqref{MajorPlayer:DQP} has a solution $\boldsymbol{\lambda}_\star$, and the solution $\boldsymbol{\lambda}_\star$ is exactly the multiplier $\boldsymbol{\lambda}$ in Theorem~\ref{thm:NSQP} corresponding to $w^\star$. 
% \end{theorem} 

% With Theorems~\ref{thm:NSQP} and \ref{thm:QPdual}, we are ready to prove Theorem~\ref{thm:OptimalWeights}. 

% \begin{proof}[Proof of Theorem~\ref{thm:OptimalWeights}]  

% By Theorem~\ref{thm:NSQP}, we can determine the optimal weights $w^\star=(w^{1,\star}, ..., w^{N,\star})$ from 
% \eqref{NSQP:w+lambda}. The multiplier $\boldsymbol{\lambda}$ in \eqref{NSQP:w+lambda} is the solution of the dual problem \ref{MajorPlayer:DQP}. 

% We first solve the dual problem \eqref{MajorPlayer:DQP} for the optimal $\boldsymbol{\lambda}$. 
% The function $L(\mathbf{x}, \boldsymbol{\lambda})$ in \eqref{MajorPlayer:DQP} can be rewritten as  
% \begin{align} 
%  L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = & \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  \mathbf{x}  
%   -  y^\top_t \hat{\mathbf{Y}}_t \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) \notag \\ 
%    = &  \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}  
%   - \Big[ y^\top_t  \hat{\mathbf{Y}}_t - \boldsymbol{\lambda}^\top G \Big] \mathbf{x} 
%    - \boldsymbol{\lambda}^\top \mathbf{c} . 
%    \label{L(x,lambda)2}   
% \end{align} 
% For each $\boldsymbol{\lambda}$ fixed, the function $L(\cdot, \boldsymbol{\lambda})$ given by \eqref{L(x,lambda)2} is a convex function on $\mathbb{R}^N$. Then $\mathbf{x}_{\boldsymbol{\lambda}}$ is a minimizer of $L(\cdot, \boldsymbol{\lambda})$ if and only if $\nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda}) = 0$. 
% It then follows from \eqref{L(x,lambda)2} that 
% \begin{align} 
%  0 = & \nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda})  \notag \\ 
%  = & \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \Big[  \hat{\mathbf{Y}}^\top_t y_t - G^\top \boldsymbol{\lambda}  \Big] , 
%  \notag 
% \end{align} 
% which further gives that 
% \begin{align} 
% 0 = &   \mathbf{x}_{\boldsymbol{\lambda}}^\top \big(   N\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t 
%  + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \mathbf{x}_{\boldsymbol{\lambda}}^\top \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] .  
%   \label{0=<x,gradL>}  
% \end{align} 
% Substituting \eqref{0=<x,gradL>} into \eqref{MajorPlayer:DQP}, we obtain an explicit form of $\theta(\boldsymbol{\lambda})$
% \begin{align} 
%  \theta(\boldsymbol{\lambda}) = & L(\mathbf{x}_{\boldsymbol{\lambda}}, \boldsymbol{\lambda}) \notag \\ 
%  =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%   \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  
%   \mathbf{x}_{\boldsymbol{\lambda}}   
%   - \Big[  y^\top_t \hat{\mathbf{Y}}_t - \boldsymbol{\lambda}^\top G \Big] 
%    \mathbf{x}_{\boldsymbol{\lambda}}  
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top\big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t  + \mathrm{K} \big) 
%     \mathbf{x}_{\boldsymbol{\lambda}}   
%   -  \mathbf{x}_{\boldsymbol{\lambda}}^\top \big( N\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t 
%    + \mathrm{K} \big)    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =&  - \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%    \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} . \notag 
% \end{align}  

% With the above explicit form of $\theta(\boldsymbol{\lambda})$, the dual quadratic programming problem \eqref{MajorPlayer:DQP} is then equivalent to 
% \begin{equation} 
% \begin{aligned} 
% & \max_{\mathbf{x}, \ \boldsymbol{\lambda}} \ 
% - \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} ,   \\ 
% & \text{subject to:} \ 
%  \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x} 
%   - \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] = 0 .  
% \end{aligned} 
% \label{MajorPlayer:DQPequiv} 
% \end{equation} 
% Since $N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K}$ is positive definite, the equality constraint in \eqref{MajorPlayer:DQPequiv} 
% implies that 
% \begin{align} 
%    \mathbf{x} 
% =  \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)^{-1} \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] . 
% \label{xsublambda}
% \end{align} 
% With \eqref{xsublambda} substituted into \eqref{MajorPlayer:DQPequiv}, 
% the dual problem \eqref{MajorPlayer:DQPequiv} is then equivalent to the following unconstrained optimization problem: 
% \begin{align} 
%  \max_{\boldsymbol{\lambda}} \ -\frac{1}{2}  \Big[  \hat{\mathbf{Y}}^\top_t 
%    y_t - G^\top \boldsymbol{\lambda}  \Big]^\top 
%    \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)^{-1} 
%  \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] 
%  - \boldsymbol{\lambda}^\top \mathbf{c} . 
% \label{MajorPlayer:DQPunconstrained} 
% \end{align} 
% We solve the unconstrained optimization problem \eqref{MajorPlayer:DQPunconstrained} for a $\boldsymbol{\lambda}_\star$:  
% \begin{align} 
%  \boldsymbol{\lambda}_\star = \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t 
%  y_t  -  \mathbf{c} \Big] . 
%  \label{lambdasubstar} 
% \end{align} 
% Then we substitute $\boldsymbol{\lambda}_\star$ into \eqref{NSQP:w+lambda} to solve for the optimal weight vector $w^\star=(w^{1,\star}, ..., w^{N,\star})^\top$: 
% \begin{align} 
%    w^\star = &  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K}  \Big)^{-1} \Big[ \hat{\mathbf{Y}}_t^\top  y_t 
%   - G^\top \boldsymbol{\lambda}_\star \Big]  \notag  \\ 
%   = &  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
%   \notag \\    
%   & -  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t 
%   y_t -  \mathbf{c} \Big] , 
%   \notag  
% \end{align} 
% which is \eqref{eqn:OptimalWeights}.  
% \end{proof} 








% \begin{comment}

% \newpage 
% ~
% \newpage
% \noindent Fix $w\in \mathbb{R}^p$, $\phi:\mathbb{R}^p\times \mathbb{R}^d\rightarrow\mathbb{R}^p$, $z\in \mathbb{R}^p$, $x\in \mathbb{R}^d$.  Fix a continuous paths $y_{\cdot} \eqdef (y_s)_{s\in [0,t]}$ and $x_{\cdot} \eqdef (x_s)_{s\in [0,t]}$, and define the paths
% \begin{equation}
% \label{eq:controlled_reservoir_system}
% \begin{aligned}
%     z_t & = z + \int_0^t\, \phi(z_s,x_s)\,ds\\
%     \hat{\beta}_t & = \pi(z_0^0,y_0) + \int_0^t\, \pi(z_s^0,y_s)\, y_s\,ds
%     ,
% \end{aligned}
% \end{equation}
% where $\pi(z,y) \eqdef  (zz^{\top})^{-1}zy$.  Given the paths $x_{\cdot}$, $y_{\cdot}$, and the reservoir $\phi$, the evolution $\hat{\beta}_{\cdot}$ is optimal in the sense that it minimizes the cumulative distance between the (controlled) reservoir system $(z_{\cdot},\beta_{\cdot})$ and the target $y_{\cdot}$; quantified by
% \[
%     \hat{\beta}_{\cdot}\in \operatorname{argmin}_{\beta_{\cdot}}\,\int_{0}^t \Big\| \beta_s^{\top}\,z_t - y_s \Big\|^2 \,ds
% .
% \]
% Unfortunately, we cannot observe the path $y_{\cdot}$ beyond the current moment in time, and therefore, one must extrapolate.  A robust extrapolation tends to take one of two forms, one is a worst-case adversarial form where one considers all possible trajectories of $y_{\cdot}$ as being equally likely and tries to optimize the readout/control $\beta_{\cdot}$ for it, leading to a very conservative readout.  Another, more practical alternatively, which also allows for generation, is to assume a \textit{system} of (stochastic/random) priors paths on $x$, run the optimal (controlled) reservoir system~\eqref{eq:controlled_reservoir_system} for each assumed prior on $x$, allowing us to predict the evolution of $y$ well into the future.


% \noindent  This can be done by calibrating several SDE models to the observed path $x_{\cdot}$.  For $i=0,\dots,N$, $X^i_{\cdot}$ be a strong solution to the SDE
% \begin{equation}
% \label{eq:Prior_X}
%     X_t^i = x + \int_0^t\, \mu^i(X_s^i)ds + \int_0^t\, \sigma^i(X_s^i)\,dW^i_s
%     .
% \end{equation}
% These will function as our system of \textit{encoders}.
% Each of these induces a stochastic reservoir system
% \[
% \begin{aligned}
%         Z_t^i & = z + \int_0^t \,\phi(Z_s^i,X_s^i)\,ds \\
%         Y_t^i & = \beta^{i\top}\, Z_t^i,
% \end{aligned}
% \]
% for $i=1,\dots,N$.
% Each $Y^i_{\cdot}$ represents one possible evolution of the reservoir under the assumption that the inputs path will evolve according to the SDE~\eqref{eq:Prior_X}.  These acts as our system of \textit{decoders}.  

% The main role of these decoders is that, once an input path is generated by~\eqref{eq:Prior_X} one may forecast the most likely evolution of the target into the future, assuming that: 1) the prior on $X_{\cdot}$ is correct and 2) that the reservoir accurately approximates the causal map $x_{\cdot}\mapsto y_{\cdot}$ pathwise.  Since there is ample research on if and when (2) holds \cite{XXX}, we focus on efforts on the implications of (1).

% Our objective is to route the information of each stochastic reservoir system into our \textit{primary} (controlled) stochastic reservoir model $Z^0_{\cdot}$ by controlling the readout map $\beta_{\cdot}^0$ so as to aggregate the average information across all plausible reservoirs.  We do this by optimizing the objective function
% \[
% J^0_t(\beta^0_{\cdot})  \eqdef  
% \mathbb{E}\Big[
%     \int_0^{t+\tau}\, \|\beta^{0}_s - \hat{\beta}_{s\wedge t}\|^2 + 
%     \|
%     \beta_t^0 Z_s^0 -
%     \sum_{i=1}^N\,w_{t}^i\,Y_s^i
%     \|^2
%     \,ds
% \Big],
% \]
% where the weights $(w_t^i)_{\cdot}$ are chosen by \textbf{...TBD...} and satisfy $\sum_{i=1}^N\,w^i_t=1$ and $0\le w^i_t\le 1$ for all $i=1,\dots,N$ and all $t\ge 0$.  The optimal readout (control) is given of rolling-window regression type
% \[
%     \beta^0_t = \pi\Big(Z_0,\sum_{n=1}^N\,w_{t}^n\,Y_s^i\Big) + \int_0^t\, \pi\Big(Z_s,
%     \sum_{i=1}^N\,w_{t}^i\,Y_s^i
%     \Big)
%     \,
%     ds
% \]
% which is found by solving the associated first-order conditions to this control problem.  Unfortunately, however, such a model is not adversarially robust in the sense that it does not arise as an equilibrium solution to a \textit{game} where each ($i^{th}$) player is trying to fool (control) the system to sway $\beta_{\cdot}^0$ towards $Y_{\cdot}^i$.

% \subsection{Robustification}
% Consider instead a set of $N$ \textit{players} $\hat{Y}_{\cdot}^1,\dots,\hat{Y}_{\cdot}^N$ which dynamically control the readout of their stochastic reservoir $Z^{i}_{\cdot}$.
% \[
%     \hat{Y}_t^i = \beta^{i:\top}Z_0^i + \int_0^t\, \beta^{i:\top}_sZ_s^i\,ds
% \]
% Each such agent/player aims to push the mass of all players towards the static reservoir's dynamics $Y_{\cdot}^i$.
% For each $i=1,\dots,N$, consider the objective function
% \[
% J^i_t(\beta^i_{\cdot})  \eqdef  
% \mathbb{E}\Big[
%     \int_0^t\, 
%     \|
%     \sum_{i=1}^N\,w_s^i
%     % \beta^i_s Z_s^i
%     \hat{Y}_s^i
%     -Y_s^i
%     \|^2
%     \,ds
% \Big].
% \]
% Our objective is to play the interactive game by instead optimizing 
% \[
% J^0_t(\beta^0_{\cdot})  \eqdef  
% \mathbb{E}\Big[
%     \int_0^{t+\tau}\, \|\beta^{0}_s - \hat{\beta}_{s\wedge t}\|^2 + 
%     \|
%     \beta_t^0 Z_s^0 -
%     \sum_{i=1}^N\,w_{t}^i\,\hat{Y}_s^i
%     \|^2
%     \,ds
% \Big],
% \]




% \appendix 
% \end{comment}

% \begin{comment} 
% \section{The Major Player's Problem} 

% Consider the major player's objective:  
% \begin{align} 
%  J_0(w) = \mathbb{E} \Big[ \sum_{t=1}^T \sum_{i=1}^N 
%  \Big\| y^i_t  - \sum_{j=1}^N w^j_t \hat{y}^j_t \Big\|^2 \Big] . 
% \notag 
%   % \label{DTJ0}
% \end{align} 
% The major player aims to find $\{w_t\}_{t=1}^T$ to minimize \eqref{DTJ0}. 
% At each time $t$, the major player solves the nonlinear programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N) } \sum_{i=1}^N \big\| y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big\|^2 \\ 
% & \text{subject to} \ \mathbf{g}(w)=(w^1-1, ..., w^N-1, -w^1, ..., -w^N) \leq 0 , \quad 
%  h(w) = w^1 + ... + w^N - 1 = 0 . 
% \end{aligned} 
% \notag 
% %\label{MajorPlayer:NLoptim}
% \end{equation} 
% By the Karush-Kuhn-Tucker theorem, if $w=(w_1, ..., w_N)^\top$ is a solution of the nonlinear programming problem 
% \eqref{MajorPlayer:NLoptim}, then there exist $\lambda_0\geq 0$, $\boldsymbol{\lambda}=(\lambda_1, ..., \lambda_N, \lambda_{N+1}, ..., \lambda_{2N})^\top \geq 0$, and $\mu$ such that 
% \begin{equation} 
% \begin{aligned}  
%  & \text{(i)}. \ (\lambda_0, \boldsymbol{\lambda}, \mu ) \neq 0 .  \\ 
%  & \text{(ii)}. \ \langle \boldsymbol{\lambda} ,  \mathbf{g}(w) \rangle = 0 .  \\ 
%  & \text{(iii)}. \ \lambda_0  \nabla_{w} \Big[ \sum_{i=1}^N \big\| y^i_t - \sum_{i=1}^N w^i \hat{y}^i_t \big\|^2 \Big]  
%   + \boldsymbol{\lambda}^\top \nabla \mathbf{g}(w) + \mu \nabla h(w) = 0 .  
% \end{aligned} 
% \label{KKT(i)-(iii)} 
% \end{equation} 

% Condition \eqref{KKT(i)-(iii)}-(ii) can be written as 
% \begin{align} 
%  (\lambda_1 - \lambda_{N+1} ) w^1 + (\lambda_2 - \lambda_{N+2}) w^2 + \cdots + 
%  (\lambda_N - \lambda_{2N}) w^N - \lambda_1 - \cdots - \lambda_N = 0 . 
%  \label{KKT(ii)MajorPlayer}
% \end{align} 

% Condition \eqref{KKT(i)-(iii)}-(iii) can be written as 
% \begin{equation} 
% \begin{aligned} 
%  & - 2 \lambda_0 \hat{y}^{1\top}_t  \sum_{i=1}^N \big( y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big) + \lambda_1 - \lambda_{N+1} 
%  + \mu = 0  , \\ 
%  & - 2 \lambda_0 \hat{y}^{2\top}_t  \sum_{i=1}^N \big( y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big) + \lambda_2 - \lambda_{N+2} 
%  + \mu = 0 , \\ 
%  & \qquad \vdots  \\ 
%  & - 2 \lambda_0 \hat{y}^{N\top}_t  \sum_{i=1}^N \big( y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big) + \lambda_N - \lambda_{2N} 
%  + \mu = 0  . 
% \end{aligned} 
% \label{KKT(iii)MajorPlayer}
% \end{equation} 

% Let 
% \begin{align} 
%  \hat\lambda_1 = \lambda_1 - \lambda_{N+1}, \quad \hat\lambda_2 = \lambda_2 - \lambda_{N+2}, \cdots, \quad   
%  \hat\lambda_N = \lambda_N - \lambda_{2N} . \notag 
% \end{align} 
% Then conditions \eqref{KKT(ii)MajorPlayer} and \eqref{KKT(iii)MajorPlayer} can be written respectively as 
% \begin{align} 
%  \hat\lambda_1 w^1 + \hat\lambda_2 w^2 + \cdots + \hat\lambda_N w^N 
%   -\lambda_1 - \cdots - \lambda_N = 0  
%  \label{KKT(ii)MajorPlayer:<hatlambda,w>=0}
% \end{align} 
% and 
% \begin{align} 
% \lambda_0 
% \begin{bmatrix} 
%  \hat{y}^{1\top}_t \hat{y}^1_t & \hat{y}^{1\top}_t \hat{y}^2_t & \cdots & \hat{y}^{1\top}_t \hat{y}^N_t \\ 
%  \hat{y}^{2\top}_t \hat{y}^1_t & \hat{y}^{2\top}_t \hat{y}^2_t & \cdots & \hat{y}^{2\top}_t \hat{y}^N_t \\
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \hat{y}^{N\top}_t \hat{y}^1_t & \hat{y}^{N\top}_t \hat{y}^2_t & \cdots & \hat{y}^{N\top}_t \hat{y}^N_t
% \end{bmatrix} 
% \begin{bmatrix} 
% w^1 \\ w^2 \\ \vdots \\ w^N 
% \end{bmatrix} 
% = 
% \frac{1}{2} 
% \begin{bmatrix} 
% 2 \lambda_0 \hat{y}^{1\top}_t \sum_{i=1}^N y^i_t + \hat{\lambda}_1 + \mu \\ 
% 2 \lambda_0 \hat{y}^{2\top}_t \sum_{i=1}^N y^i_t + \hat{\lambda}_2 + \mu \\ 
% \vdots \\ 
% 2 \lambda_0 \hat{y}^{N\top}_t \sum_{i=1}^N y^i_t + \hat{\lambda}_N + \mu 
% \end{bmatrix} .
% \label{KKT(iii)MajorPlayermatrix}
% \end{align} 



% If $\lambda_0=0$, we have from \eqref{KKT(iii)MajorPlayermatrix} that 
% \begin{align} 
%  \hat\lambda_1 = \hat\lambda_2 = \cdots = \hat\lambda_N = -\mu . 
%  \label{hatlambda=-mu} 
% \end{align} 
% If $\lambda_0=0$ and $\mu\neq 0$, we have from \eqref{KKT(ii)MajorPlayer:<hatlambda,w>=0} and 
% \eqref{hatlambda=-mu} that 
% $-\mu = \lambda_1 + \cdots + \lambda_N >0$. 
% If $\lambda_0=0$ and $\mu=0$, we have from \eqref{KKT(i)-(iii)}-(i) and \eqref{hatlambda=-mu} that 
% \begin{align} 
% \boldsymbol\lambda=(\lambda_1, ..., \lambda_N, \lambda_{N+1}, ..., \lambda_{2N}) \neq 0 
% \quad \text{and}  \quad 
% \lambda_1=\lambda_{N+1} - \mu, \ \lambda_2 = \lambda_{N+2} - \mu , \ ..., \ \lambda_{N}=\lambda_{2N} - \mu . 
% \notag 
% \end{align} 
% It then follows from \eqref{KKT(ii)MajorPlayer:<hatlambda,w>=0} that any $(w^1, ..., w^N)\in \Delta_N$ solves the programming problem 
% \eqref{MajorPlayer:NLoptim}. (Xuwei: This scenario needs to be addressed and excluded!)  


% If \eqref{MajorPlayer:NLoptim} admits an interior solution $w=(w^1, ..., w^N)$ with $0<w^i<1$ for all $i=1$, ..., $N$, we have 
% $\mathbf{g}(w)=(w^1 -1, ..., w^N-1, -w^1, ..., -w^N) < 0$. Also note that $\nabla h(w) = [1, 1, ..., 1]\in \mathbb{R}^N$ is an independent vector. 
% If \eqref{MajorPlayer:NLoptim} admits a solution $w=(w^1, ..., w^N)$ such that $w^{i_1}=\cdots=w^{i_k}=0$ for some 
% $\{i_1, \cdots, i_k\} \subset \{1, ..., N\}$. We have that $\nabla g_{i_l}(w) = -(e^{N}_{i_l})^\top$ and therefore the vectors
% $\nabla g_{i_1}(w)$, ... $\nabla g_{i_k}(w)$, and $\nabla h(w)$ are linearly independent. 
% By \cite[Theorem 5.2, Corollary 1]{Berkovitz2001}, we have that $\lambda_0 \neq 0$. 






% For $\lambda_0>0$, up to rescaling the multipliers, we can let $\lambda_0=1$. Then \eqref{KKT(iii)MajorPlayermatrix} can be written as 
% \begin{align} 
% \begin{bmatrix} 
%  \hat{y}^{1\top}_t \hat{y}^1_t & \hat{y}^{1\top}_t \hat{y}^2_t & \cdots & \hat{y}^{1\top}_t \hat{y}^N_t \\ 
%  \hat{y}^{2\top}_t \hat{y}^1_t & \hat{y}^{2\top}_t \hat{y}^2_t & \cdots & \hat{y}^{2\top}_t \hat{y}^N_t \\
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \hat{y}^{N\top}_t \hat{y}^1_t & \hat{y}^{N\top}_t \hat{y}^2_t & \cdots & \hat{y}^{N\top}_t \hat{y}^N_t
% \end{bmatrix} 
% \begin{bmatrix} 
% w^1 \\ w^2 \\ \vdots \\ w^N 
% \end{bmatrix} 
% = 
% \begin{bmatrix} 
%   \hat{y}^{1\top}_t  \\ 
%   \hat{y}^{2\top}_t   \\ 
% \vdots \\ 
%   \hat{y}^{N\top}_t   
% \end{bmatrix} 
% \sum_{i=1}^N y^i_t
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%  \hat{\lambda}_1  \\ 
%  \hat{\lambda}_2  \\ 
% \vdots \\ 
%  \hat{\lambda}_N  
% \end{bmatrix} 
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%   \mu \\ 
%  \mu \\ 
% \vdots \\ 
%  \mu 
% \end{bmatrix} \notag  
% \end{align} 

% \begin{align} 
% \begin{bmatrix} 
% w^1 \\ w^2 \\ \vdots \\ w^N 
% \end{bmatrix} 
% = 
% \begin{bmatrix} 
%  \hat{y}^{1\top}_t \hat{y}^1_t & \hat{y}^{1\top}_t \hat{y}^2_t & \cdots & \hat{y}^{1\top}_t \hat{y}^N_t \\ 
%  \hat{y}^{2\top}_t \hat{y}^1_t & \hat{y}^{2\top}_t \hat{y}^2_t & \cdots & \hat{y}^{2\top}_t \hat{y}^N_t \\
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \hat{y}^{N\top}_t \hat{y}^1_t & \hat{y}^{N\top}_t \hat{y}^2_t & \cdots & \hat{y}^{N\top}_t \hat{y}^N_t
% \end{bmatrix}^{-1} 
% \left\{ 
% \begin{bmatrix} 
%   \hat{y}^{1\top}_t  \\ 
%   \hat{y}^{2\top}_t   \\ 
% \vdots \\ 
%   \hat{y}^{N\top}_t   
% \end{bmatrix} 
% \sum_{i=1}^N y^i_t
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%  \hat{\lambda}_1  \\ 
%  \hat{\lambda}_2  \\ 
% \vdots \\ 
%  \hat{\lambda}_N  
% \end{bmatrix} 
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%   \mu \\ 
%  \mu \\ 
% \vdots \\ 
%  \mu 
% \end{bmatrix} \right\} \geq 0 .  \label{w>=0}  
% \end{align} 
% From \eqref{KKT(ii)MajorPlayer:<hatlambda,w>=0}, we further have that 
% \begin{align} 
%  \sum_{i=1}^N \lambda_i = & \big[ \hat\lambda_1 \ \hat\lambda_2 \ \cdots \ \hat\lambda_N \big]
%  \begin{bmatrix} 
% w^1 \\ w^2 \\ \vdots \\ w^N 
% \end{bmatrix}  \notag \\ 
% = & 
% \big[ \hat\lambda_1 \ \hat\lambda_2 \ \cdots \ \hat\lambda_N \big] 
% \begin{bmatrix} 
%  \hat{y}^{1\top}_t \hat{y}^1_t & \hat{y}^{1\top}_t \hat{y}^2_t & \cdots & \hat{y}^{1\top}_t \hat{y}^N_t \\ 
%  \hat{y}^{2\top}_t \hat{y}^1_t & \hat{y}^{2\top}_t \hat{y}^2_t & \cdots & \hat{y}^{2\top}_t \hat{y}^N_t \\
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \hat{y}^{N\top}_t \hat{y}^1_t & \hat{y}^{N\top}_t \hat{y}^2_t & \cdots & \hat{y}^{N\top}_t \hat{y}^N_t
% \end{bmatrix}^{-1} 
% \left\{ 
% \begin{bmatrix} 
%   \hat{y}^{1\top}_t  \\ 
%   \hat{y}^{2\top}_t   \\ 
% \vdots \\ 
%   \hat{y}^{N\top}_t   
% \end{bmatrix} 
% \sum_{i=1}^N y^i_t
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%  \hat{\lambda}_1  \\ 
%  \hat{\lambda}_2  \\ 
% \vdots \\ 
%  \hat{\lambda}_N  
% \end{bmatrix} 
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%   \mu \\ 
%  \mu \\ 
% \vdots \\ 
%  \mu 
% \end{bmatrix} \right\} .  
% \label{constraint:sumlambda=hatlambdaw} 
% \end{align} 



% Since $\sum_{i=1}^N w^i = 1$, we have 
% \begin{align} 
%  1 = & \big[ 1 \ 1 \ \cdots \ 1 \big]
%  \begin{bmatrix} 
% w^1 \\ w^2 \\ \vdots \\ w^N 
% \end{bmatrix}  \notag \\ 
% = & 
% \big[ 1 \ 1 \ \cdots \ 1 \big] 
% \begin{bmatrix} 
%  \hat{y}^{1\top}_t \hat{y}^1_t & \hat{y}^{1\top}_t \hat{y}^2_t & \cdots & \hat{y}^{1\top}_t \hat{y}^N_t \\ 
%  \hat{y}^{2\top}_t \hat{y}^1_t & \hat{y}^{2\top}_t \hat{y}^2_t & \cdots & \hat{y}^{2\top}_t \hat{y}^N_t \\
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \hat{y}^{N\top}_t \hat{y}^1_t & \hat{y}^{N\top}_t \hat{y}^2_t & \cdots & \hat{y}^{N\top}_t \hat{y}^N_t
% \end{bmatrix}^{-1} 
% \left\{ 
% \begin{bmatrix} 
%   \hat{y}^{1\top}_t  \\ 
%   \hat{y}^{2\top}_t   \\ 
% \vdots \\ 
%   \hat{y}^{N\top}_t   
% \end{bmatrix} 
% \sum_{i=1}^N y^i_t
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%  \hat{\lambda}_1  \\ 
%  \hat{\lambda}_2  \\ 
% \vdots \\ 
%  \hat{\lambda}_N  
% \end{bmatrix} 
% + 
% \frac{1}{2} 
% \begin{bmatrix} 
%   \mu \\ 
%  \mu \\ 
% \vdots \\ 
%  \mu 
% \end{bmatrix} \right\} \label{constraint:1=sumw}
% \end{align} 

% We need to find $w=(w^1, ..., w^N)$ and the multipliers $\{ \lambda_i \}_{i=1}^{2N}$ and $\mu$ that satisfy 
% \eqref{w>=0}, \eqref{constraint:sumlambda=hatlambdaw}, and \eqref{constraint:1=sumw}. 
% Since $w=(w^1, ..., w^N)$ is uniquely determined by \eqref{w>=0}, we focus on finding $\{ \lambda_i \}_{i=1}^{2N}$ and $\mu$ 
% that satisfy 
% \eqref{w>=0}, \eqref{constraint:sumlambda=hatlambdaw}, and \eqref{constraint:1=sumw}. 


% Denote 
% \begin{align} 
%  \hat{\mathbf{Y}}_t = \big[ \hat{y}^1_t, \cdots , \hat{y}^N_t \big] , \quad 
%   \mathbf{1} = \big[ 1, ..., 1 \big] , \quad 
%   \hat{\boldsymbol{\lambda}} = \big[ \hat{\lambda}_1, ..., \hat{\lambda}_N \big]^\top  \notag 
% \end{align} 
% Then \eqref{constraint:1=sumw} can be written as 
% \begin{align} 
%  1 = \mathbf{1} (\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}_t^\top \sum_{i=1}^N y^i_t + \frac{1}{2} \hat{\boldsymbol{\lambda}} 
%   + \frac{1}{2} \mathbf{1}^\top \mu \Big] \notag 
% \end{align} 
% Then we have 
% \begin{align} 
%  \mu = 2 \big[ \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \mathbf{1}^\top \big]^{-1} 
%  \Big\{ 1 - \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}_t^\top \sum_{i=1}^N y^i_t + \frac{1}{2} \hat{\boldsymbol{\lambda}}  \Big] 
%  \Big\} . \label{muhatlambda} 
% \end{align} 
% We substitute \eqref{muhatlambda} into \eqref{constraint:sumlambda=hatlambdaw} to obtain
% \begin{align} 
%  \sum_{i=1}^N \lambda_i = & \hat{\boldsymbol{\lambda}}^\top 
%   ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}^\top_t \sum_{i=1}^N y^i_t + \frac{1}{2}\hat{\boldsymbol{\lambda}} + \frac{1}{2}\mathbf{1}^\top \mu \Big] \notag \\ 
%  = & \hat{\boldsymbol{\lambda}}^\top ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}^\top_t \sum_{i=1}^N y^i_t + \frac{1}{2}\hat{\boldsymbol{\lambda}}  \Big] 
%  \notag \\ 
%   & + \hat{\boldsymbol{\lambda}}^\top ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \mathbf{1}^\top  \big[ \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \mathbf{1}^\top \big]^{-1} \notag \\ 
%  & - \hat{\boldsymbol{\lambda}}^\top ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \mathbf{1}^\top  \big[ \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \mathbf{1}^\top \big]^{-1} 
%    \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}_t^\top \sum_{i=1}^N y^i_t + \frac{1}{2} \hat{\boldsymbol{\lambda}}  \Big]  
% \end{align} 


% We substitute \eqref{muhatlambda} into \eqref{w>=0} to obtain 
% \begin{align} 
%  \mathbf{0} \leq & ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \Big[ \hat{\mathbf{Y}}^\top_t \sum_{i=1}^N y^i_t + \frac{1}{2} 
%  \hat{\boldsymbol{\lambda}} + \frac{1}{2} \mathbf{1}^\top \mu \Big] \notag \\ 
% = & ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \Big[ \hat{\mathbf{Y}}^\top_t \sum_{i=1}^N y^i_t + \frac{1}{2} 
%  \hat{\boldsymbol{\lambda}}  \Big] \notag \\ 
%  & +  (\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1}  \mathbf{1}^\top 
%   \big[ \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} \mathbf{1}^\top \big]^{-1} 
%  \Big\{ 1 - \mathbf{1} ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t)^{-1} 
%  \Big[ \hat{\mathbf{Y}}_t^\top \sum_{i=1}^N y^i_t + \frac{1}{2} \hat{\boldsymbol{\lambda}}  \Big] 
%  \Big\} .  \notag 
% \end{align} 

% Since 
% \begin{align} 
% & \frac{\partial}{\partial w^k} 
%  \sum_{i=1}^N \big\| y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big\|^2 
%  = \hat{y}^{k\top}_t \sum_{i=1}^N \big( y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big) ,  \notag \\ 
%  %%% 
% & \frac{\partial^2}{\partial w^k \partial w^l } 
%  \sum_{i=1}^N \big\| y^i_t - \sum_{j=1}^N w^j \hat{y}^j_t \big\|^2 
%  = \hat{y}^{k\top}_t \hat{y}^l_t , \notag 
% \end{align}  
% the Hessian matrix of the major player's objective function \eqref{MajorPlayer:NLoptim} is given by
% \begin{align} 
% H = \big( \hat{y}^{k\top}_t \hat{y}^l_t \big)_{1\leq k, l \leq N} 
% = \begin{bmatrix} 
%   \hat{y}^{1\top}_t  \\ 
%   \hat{y}^{2\top}_t   \\ 
% \vdots \\ 
%   \hat{y}^{N\top}_t   
% \end{bmatrix} 
% \begin{bmatrix} 
%   \hat{y}^1_t  & 
%   \hat{y}^2_t   & 
% \cdots & 
%   \hat{y}^N_t   
% \end{bmatrix} ,  
% \label{HessianMajorPlayer}
% \end{align} 
% which is semi-positive definite. 
% Therefore the major player's objective is convex.  
% \end{comment} 

% \begin{comment}

% \newpage 
% \appendix 
% \newpage 

% \section{Work to Date} 
% Let 
% \begin{align} 
%  & Z^0_t = \varphi(Z^0_{t-1}, X_t)  \notag \\ 
% & Y^0_t = \beta^{0T}_t Z^0_t   \notag 
% \end{align}

% \begin{align} 
%   & Z^i_t = \psi(Z^i_{t-1}, X_t) \notag \\ 
%  & Y^i_t = \beta^{i\top}_t Z^i_t , \quad i = 1, 2, ..., N. \notag 
% \end{align}

% The objective is to find a 
% \begin{align} 
%  \min_{\beta^0} \mathbb{E} \Big[ \frac{1}{\tau} \sum_{t=\tau+1}^{T+\tau} \Big\| \beta^{0T}_t 
%   Z^0_t - \sum_{i=1}^N \beta^{iT}_t Z^i(X_{[0,t]}) 
%  \Big\|^2 \Big]  + \frac{1}{1+T} \sum_{t=0}^T \Big\| \beta^{0T}_t Z^0_t - y_t \Big\|^2 \notag 
% \end{align}

% First order condition for $t=0, 1, ..., T$: 
% \begin{align} 
%  \frac{2}{1+T}  Z^0_t (\beta^{0\top}_t Z^0_t - y_t) = 0 , \notag 
% \end{align} 
% which gives the optimal $\beta^0_t$ for each $t=0$, $1$, ..., $T$: 
% \begin{align} 
%   \beta^0_t = (Z^0_t Z^{0\top}_t )^{-1} Z^0_t y_t  \notag 
% \end{align} 

% For $t=T+1$, ..., $T+\tau$, the first order condition 
% \begin{align} 
%   \frac{2}{\tau} Z^0_t \Big( \beta^{0\top} Z^0_t - \sum_{i=1}^N \beta^{i\top}_t Z^i_t \Big) = 0 \notag 
% \end{align} 
% which gives the optimal $\beta^0_t$ for each $t=T+1$, $T+2$, ..., $T+\tau$:  
% \begin{align} 
%   \beta^0_t = (Z^0_t Z^{0\top}_t )^{-1} Z^0_t \sum_{i=1}^N \beta^{i\top}_t Z^i_t .   \notag 
% \end{align} 



% \subsection{Game-Theoretic Modeling}
% Consider $N$ reservoirs 
% \begin{equation}
% \begin{aligned} 
% & Z^i_t = Z^i_0 + 
% \int_0^t \varphi(Z^i_s, X^i_s) ds  \\ 
% & Y^i_t = \beta^i_t Z^i_t , \quad i = 1, ..., N . 
% \end{aligned} 
% \label{Ri} 
% \end{equation}



% We employ a game-theoretic approach to model the interaction between reservoirs. Let the reservoirs be players in the game-theoretic framework. 
% The players choose \textit{non-negative} weights $(w^1_\cdot, w^2_\cdot, ..., w^N_\cdot)$ to minimize the distance 
% \begin{align} 
%  J_i(w^i, w^{-i}) = \int_0^T \Big\| y^i_t - \sum_{i=1}^N w^i_t \beta^i_t Z^i_t \Big\|^2 dt , \quad i = 1, ..., N. \label{Ji}  
% \end{align} 
% We aim to find a Nash equilibrium $(w^{1\star}_\cdot, ..., w^{N\star}_\cdot)$ 
% for \eqref{Ri} and \eqref{Ji} such that 
% \begin{align} 
%  J_i(w^{i\star}, w^{-i \star}) \leq 
%  J_i(w^{i}_\cdot, w^{-i\star}_\cdot) , \quad 
%  \forall \, i = 1, 2, ..., N. 
% \notag 
% \end{align} 
% For $(w^{1, \star}, ..., w^{N, \star})$ to be a Nash equilibrium, it should satisfy the first order condition for all $t\in[0, T]$:    
% \begin{align} 
%  \Big\| y^i_t - \sum_{j=1}^N w^{i,\star}_t \beta^j_t Z^j_t \Big\| \beta^i_t Z^i_t = 0 , \quad i = 1, ..., N , \notag 
% \end{align} 
% which is equivalent to 
% \begin{align} 
%  y^i_t \beta^i_t z^i_t - \sum_{i=1}^N w^{i\star} \beta^i_t Z^i_t \beta^j_t Z^j_t = 0 , \quad i = 1, ..., N. \label{NE-firstorder}
% \end{align} 

% Denote 
% \begin{align} 
%  B_t = 
%  [ \beta^1_t Z^1_t, ..., \beta^N_t Z^N_t ]^\top 
%  [ \beta^1_t Z^1_t, ..., 
%  \beta^N_t Z^N_t] \notag 
% \end{align} 
% Then we have the unique Nash equilibrium 
% $[w^{1\star}_\cdot, ..., w^{N\star}_\cdot ]$ 
% \begin{align} 
%  [ w^{1 \star}_t, ..., w^{N \star}_t ]^\top 
%   = B_t^{-1} [y^1_t \beta^1_t Z^1_t, ..., y^N_t \beta^N_t Z^N_t ]^\top ,  \quad  
%   0\leq t \leq T .
%   \label{Nashw}
% \end{align} 

% \subsection{Modified - Real Game}
% Consider 
% \begin{equation}
% \begin{aligned} 
% & X^i_t = X^i_0 + \int_0^t A_i X^i_s ds 
% + \int_0^t \sigma_i d W^i_s\\ 
% & Z^i_t = Z^i_0 + 
% \int_0^t \varphi(Z^i_s, X^i_s) ds  \approx 
% Z^i_0 + 
% \int_0^t B Z^i_s + C X^i_s ds \\ 
% & \hat{Y}^i_t = \beta^i Z_0^i + \int_0^t \beta^i_s Z^i_s 
%  ds  , \quad i = 0, 1, ..., N . 
% \end{aligned} 
% \label{Ri_linear} 
% \end{equation} 
% {\color{blue} X: The functions $a(\cdot)$ and $\varphi$ should be linear}

% Denote 
% \begin{align}
% \hat{Y} \eqdef (\hat{Y}^{1\top},..., \hat{Y}^{N \top})^\top , \quad 
% Z  \eqdef  (Z^{1\top}, ..., Z^{N\top})^\top, \quad 
% X \eqdef  (X^{1\top}, ..., X^{N\top})^\top . \notag 
% \end{align} 

% For each $i=1,\dots,N$, set $\beta^{-i} \eqdef  (\beta^j)_{j=1,\dots,N;\,j\neq i}$.  The objectives of the players are 
% \allowdisplaybreaks
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \int_0^T \Big\| y^i_t - \sum_{i=1}^N w^i_t \hat{Y}^i_t \Big\|^2 
%   + \| \beta^i_t \|^2 dt , \quad i = 1, ..., N. \label{Ji}  \\ 
% %\end{align} 
% %\begin{align} 
% & J_0 (\beta^0, \mathbf{w}, \beta^1, ..., \beta^N) =  \int_0^T \Big\| y^0_t - \sum_{i=1}^N w^i_t \hat{Y}^i_t \Big\|^2 
%   + \| \beta^0_t \|^2 dt \label{J0}
% \end{align} 

% We define the value functions for the followers 
% \begin{align} 
% V_i (t, \hat{\mathbf{y}}, \mathbf{z}, \mathbf{x} ) = \mathbb{E} \Big[ \int_t^T \Big\| y^i_s - \sum_{i=1}^N w^i_s \hat{Y}^i_s \Big\|^2 
%  + \| \beta^i_s \|^2 d s \, \Big| \, 
%  \hat{Y}_t = \hat{\mathbf{y}} , Z_t = \mathbf{z}, X_t = \mathbf{x} \Big] , \quad i = 1, ..., N.  \notag 
% \end{align} 
% By the dynamic programming approach, the value functions satisfy the equations  
% \begin{align} 
% & \frac{\partial}{\partial t} V_i(t, \hat{\mathbf{y}}, \mathbf{z}, \mathbf{x} ) 
%  + \sup_{\beta_i} \Big\{ \sum_{j=1}^N \beta_j^\top z_j^\top 
%  \frac{\partial V_i}{\partial y_j}   
%   + \sum_{j=1}^N \varphi(z_j, x_j) \frac{\partial V_i}{\partial  z_j} 
%    + \sum_{j=1}^N a(x_j) \frac{\partial V_i}{\partial x_j} 
% + \Big\| y^i_s - \sum_{i=1}^N w^i \hat{y}_i \Big\|^2 + \| \beta_i \|^2 \Big\} = 0 \notag \\ 
% & i = 1, ..., N. \notag 
% \end{align} 
% By the first order condition, we have 
% \begin{align} 
%  z_i \frac{\partial V_i}{\partial y_i} + 2 \beta_i = 0 \notag 
% \end{align} 

% \begin{align} 
%   \beta_i = -\frac{1}{2} z_i^\top \frac{\partial V_i(t, \hat{\mathbf{y}, \mathbf{x}, \mathbf{z}} )}{\partial y_i}
% \end{align} 



% \textbf{The Discrete-time model} 

% \begin{align} 
% & X^i_{t+1} =  A_i X^i_t + \sigma W^i_t \notag \\  
% & Z^i_{t+1} =  \varphi(Z^i_t, X^i_{t+1}) = 
%  B_i Z^i_t + C X^i_{t+1} \notag \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \hat{\beta}^{i\top}_t Z^i_t , \qquad i = 1, ..., N. \notag 
% \end{align} 


% \allowdisplaybreaks
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y^i_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \| \beta^i_t \|^2  \Big]  + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2\Big\}   , \quad i = 1, ..., N. 
%   %\label{DTJi}  
%  \end{align} 

% Let $\{e^N_i\}_{i=1}^N$ be the standard basis of $\mathbb{R}^N$, and  
% denote 
% \begin{align}
% & \hat{Y} \eqdef (\hat{Y}^{1\top},..., \hat{Y}^{N \top})^\top , \quad 
% Z  \eqdef  (Z^{1\top}, ..., Z^{N\top})^\top, \quad 
% X \eqdef  (X^{1\top}, ..., X^{N\top})^\top , \notag \\ 
% & \mathbf{e}^N_i = e^N_i \otimes I_{d_{z}} = [0, ..., I_{d_{z}} , ..., 0]^T . 
% \end{align} 
% Then 
% \begin{align} 
%  \hat{Y}_{t+1} = \hat{Y}_t + \sum_{i=1}^N e_i Z^\top_t 
%  \mathbf{e}_i \beta^i_t   
%  \notag 
% \end{align} 

 
% %\begin{align} 
% %& J_0 (\beta^0, \mathbf{w}, \beta^1, ..., \beta^N) =  \sum_{t=0}^T \Big\| y^0_t - \sum_{i=1}^N w^i_t \hat{Y}^i_t \Big\|^2 
% %  + \| \beta^0_t \|^2 dt \label{DTJ0}
% %\end{align} 

% At time $t=T-1$, we have 
% \begin{align} 
% V_i(T-1, \hat{\mathbf{y}}, \mathbf{z}, \mathbf{x})  = \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y^i_t - \sum_{j=1}^N w^j \hat{y}^j \Big\|^2 
%   + \| \beta^i \|^2  + \Big\| y^i_T - \sum_{j=1}^N w^j ( \hat{y}^j + \beta^{j\top} z^j ) \Big\|^2 \Big\} \notag 
% \end{align} 
% The equilibrium strategy at $t=T-1$ satisfies 
% \begin{align} 
%   \beta^i +  z^i \Big[ y^i_T - \sum_{j=1}^N w^j ( \hat{y}^j + \beta^{j\top} z^j ) \Big]    = 0 , \quad i = 1, ..., N ,  
%   \label{FOC:betaT-1}
% \end{align} 

% \begin{align} 
%  w^i \beta^{i\top} z^i + w^i z^{i\top} z^i y^i_T - w^i z^{iT} z^i \sum_{j=1}^N w^j(\hat{y}^j + \beta^{j\top} z^j ) = 0 , 
%   i = 1, ..., N \notag  
% \end{align}  

% \begin{align} 
%  \sum_{i=1}^N w^i \beta^{i\top} z^i + \sum_{i=1}^N w^i z^{i\top} z^i y^i_T 
%   - \sum_{i=1}^N w^i z^{iT} z^i \sum_{j=1}^N w^j(\hat{y}^j + \beta^{j\top} z^j ) = 0 \notag 
% \end{align}  

% \begin{align} 
%  \Big[ 1 - \sum_{j=1}^N w^j z^{j\top} z^j \Big] \sum_{i=1}^N w^i \beta^{i\top} z^i 
%  + \sum_{i=1}^N w^i z^{i\top} z^i \Big[ y^i_T  -  \sum_{j=1}^N w^j \hat{y}^j \Big] = 0 \label{MFcontrol}    
% \end{align} 

% \begin{align} 
%   \sum_{i=1}^N w^i \beta^{i\top} z^i =
%  - \Big[ 1 - \sum_{j=1}^N w^j z^{j\top} z^j \Big]^{-1} \sum_{i=1}^N w^i z^{i\top} z^i \Big[ y^i_T  -  \sum_{j=1}^N w^j \hat{y}^j \Big]  \notag 
% \end{align} 

% From \eqref{FOC:betaT-1} and \eqref{MFcontrol}, we have the equilibrium strategy at $t=T-1$ for $i=1, ..., N$: 
% \begin{align} 
%  \beta^i = & - z^i \Big[ y^i_T - \sum_{j=1}^N w^j \hat{y}^j \Big] + z^i \sum_{j=1}^N w^j \beta^{j\top} z^j  
%  \notag \\ 
%  = & - z^i \Big[ y^i_T - \sum_{j=1}^N w^j \hat{y}^j \Big] 
%    - z^i \Big[ 1 - \sum_{j=1}^N w^j z^{j\top} z^j \Big]^{-1} \sum_{i=1}^N w^i z^{i\top} z^i \Big[ y^i_T  -  \sum_{j=1}^N w^j \hat{y}^j \Big] \notag  
% \end{align} 



% We have that $V_i(t, \hat{\mathbf{y}}, \mathbf{z}, \mathbf{x})$ takes the form  
% \begin{align} 
%   V_i(t, \hat{\mathbf{y}}, \mathbf{z} , \mathbf{x} ) = [ \hat{\mathbf{y}}^\top, \mathbf{z}^\top , \mathbf{x}^\top ] P_i(t) [\hat{\mathbf{y}}^\top, \mathbf{z}^\top , \mathbf{x}^\top ]^\top 
%   + 2 S_i(t)^\top [\hat{\mathbf{y}}^\top, \, \mathbf{z}^\top ]^\top + r_i(t) \notag  
%  \end{align} 
% By the dynamic programming principle, $V_i$ satisfy the dynamic programming equation:  
% \begin{align} 
% V_i(t, \hat{\mathbf{y}}, \mathbf{z}, \mathbf{x})  = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y^i_t - \sum_{i=1}^N w^i \hat{y}^i \Big\|^2 
%   + \| \beta^i \|^2  \notag \\ 
% & \hspace{2.5cm}  + V_i(t+1, \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{z}^\top \mathbf{e}_j \beta^j, Z_{t+1} , X_{t+1} ) 
%    \Big| \hat{Y}_t = \mathbf{\hat{y}}, Z_t = \mathbf{z}, 
%    X_t = \mathbf{x}  \Big\} \notag \\ 
%   =& \sup_{\beta^i} \mathbb{E} 
%   \Big\{  \Big\| y^i_t - \sum_{i=1}^N w^i \hat{y}^i \Big\|^2 
%   + \| \beta^i \|^2 \notag \\ 
%  &  + [ \hat{\mathbf{y}}^\top + \sum_{j=1}^N (\mathbf{z}^\top \mathbf{e}_i \beta^j)^\top , Z_{t+1}^\top , X_{t+1}^\top ] P_i(t+1) 
%   [ \hat{\mathbf{y}}^\top + \sum_{j=1}^N (e_j z^{j\top}\beta^j)^\top ,  Z_{t+1}^\top , X_{t+1}^\top ]^\top \notag \\ 
%  &   \hspace{3cm}  + 2 S_i(t+1)^\top [ \hat{\mathbf{y}}^\top + \sum_{j=1}^N ( e_j z^{j\top}\beta^j )^\top , Z_{t+1}^\top , X_{t+1}^\top ]^\top 
%   + r_i(t+1)   \Big| \hat{Y}_t = \mathbf{\hat{y}}, Z_t = \mathbf{z}, 
%    X_t = \mathbf{x}   \Big\} 
%   \label{DPeqn}
% \end{align} 

% By the first order condition, 
% \begin{align} 
%  -\beta^i =    [ z^i e_i^\top , \, 0, \, 0  ] P_i(t+1) [\hat{\mathbf{y}}^\top + \sum_{j=1}^N ( e_j z^{j\top}\beta^j )^\top , Z_{t+1}^\top, X_{t+1}^\top]^\top  
%  +  [z^i e_i^\top, \, 0, \, 0] S_i(t+1) 
%  \label{betaifirstorder}
% \end{align} 

% \begin{align} 
%  - \sum_{i=1}^N e_i z^{i\top} \beta^i = &   \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) 
%  \big[ \sum_{j=1}^N ( e_j z^{j\top} \beta^j )^\top , 0 , 0 \big]^\top \notag \\ 
%   & + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) \big[ \hat{\mathbf{y}}^\top, Z_{t+1}^\top , X_{t+1}^\top \big]^\top \notag \\ 
%   &  + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] S_i(t+1) \notag 
% \end{align} 

% \begin{align} 
%  - \sum_{i=1}^N e_i z^{i\top} \beta^i = &  + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) 
%  \big[ I_{N \times N} , 0 , 0 \big]^\top \sum_{j=1}^N  e_j z^{j\top} \beta^j  \notag \\ 
%   & + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) \big[ \hat{\mathbf{y}}^\top, Z_{t+1}^\top , X_{t+1}^\top \big]^\top \notag \\ 
%   &  + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] S_i(t+1) \notag 
% \end{align} 


% \allowdisplaybreaks 
% \begin{align}  
%  - \sum_{i=1}^N e_i z^{i\top} \beta^i = & - \Big\{ I_{N\times N} + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) 
%  \big[ I_{N \times N} , 0 , 0 \big]^\top \Big\}^{-1} \cdot  \notag \\ 
%   &  \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] 
%    \Big( P_i(t+1) \big[ \hat{\mathbf{y}}^\top, Z_{t+1}^\top , X_{t+1}^\top \big]^\top + S_i(t+1) \Big) 
%    \label{sumezbeta}
% \end{align} 

% From \eqref{betaifirstorder} we have   
% \begin{align} 
%  -\beta^i = &    [ z^i e_i^\top , \, 0, \, 0  ] P_i(t+1) [ I_{N\times N} , 0, 0 ]^\top \sum_{j=1}^N  e_j z^{j\top}\beta^j  \notag \\ 
%  & + [ z^i e_i^\top , \, 0, \, 0  ] P_i(t+1) [\hat{\mathbf{y}}^\top  , Z_{t+1}^\top, X_{t+1}^\top]^\top     \notag \\ 
%  & +  [z^i e_i^\top, \, 0, \, 0] S_i(t+1) 
%  \label{betai=sumezbeta} 
% \end{align} 

% We substitute \eqref{sumezbeta} into \eqref{betai=sumezbeta} to obtain the equilibrium for $i=1$, ..., $N$:  
% \begin{align} 
%  -\beta^i = &   - [ z^i e_i^\top , \, 0, \, 0  ] P_i(t+1) [ I_{N\times N} , 0, 0 ]^\top 
%  \Big\{ I_{N\times N} + \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] P_i(t+1) 
%  \big[ I_{N \times N} , 0 , 0 \big]^\top \Big\}^{-1} \cdot  \notag \\ 
%   &  \sum_{i=1}^N \big[ e_i z^{i\top} z^i e_i^\top, 0 , 0 \big] 
%    \Big( P_i(t+1) \big[ \hat{\mathbf{y}}^\top, Z_{t+1}^\top , X_{t+1}^\top \big]^\top + S_i(t+1) \Big) \notag \\  
%  & + [ z^i e_i^\top , \, 0, \, 0  ] P_i(t+1) [\hat{\mathbf{y}}^\top  , Z_{t+1}^\top, X_{t+1}^\top]^\top     
%   +  [z^i e_i^\top, \, 0, \, 0] S_i(t+1) 
% \notag  
% \end{align} 

% We further substitute \eqref{betai=sumezbeta} and \eqref{sumezbeta} into \eqref{DPeqn}
% \end{comment} 




% % \bibliographystyle{spmpsci}      % mathematics and physical sciences
% %\bibliographystyle{spphys}       % APS-like style for physics
% \bibliographystyle{plain} %plain
% \bibliography{Refs}   % name your BibTeX data base

% %\bibliographystyle{spmpsci}  
% %\bibliography{HYmfsocRef}









% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\newpage


% \end{document} 

==> Historical_Versions/2024_03_09.tex <==
% % david.emerson@vectorinstitute.ai
% % fatemeh.tavakoli@vectorinstitute.ai


% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2023


% % ready for submission
% % \usepackage{neurips_2024}
% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% \usepackage[preprint]{neurips_2024}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2023}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2023}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors

% \usepackage[top=0.9in,bottom=1.1in,left=1.05in,right=1.05in]{geometry}



% %


% %\usepackage{amsthm} 
% %\theoremstyle{remark}
% \usepackage{amsthm}
% % \newtheorem{remark}{Remark}[section]
% \newtheorem{example}{Example}[section]


% \title{Optimal Federated Learning For Generative Sequential Learners}

% \input{packages}
% \input{mathcommands}
% \input{Commenting}

% \author{%
%   Xuwei Yang\\
%   Department of Mathematics\\
%   McMaster University\\
%   Ontario, Canada \\
%   \texttt{kratsioa@mcmaster.ca} \\
%   % examples of more authors
%   \And
%   Anastasis Kratsios\thanks{Corresponding Author. 
%   Funded by NSERC DG No.\ RGPIN-2023-04482.} \\
%   Department of Mathematics\\
%   McMaster University and the Vector Institute\\
%   Ontario, Canada \\
%   \texttt{kratsioa@mcmaster.ca} \\
% }




% \begin{document}

% \maketitle

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract} 
% In this paper, we consider the problem of optimally training a set of sequential generative models distributed across a network using a fixed number of communication rounds.
% We derive closed-form expressions for the optimal online updates for the local models and the optimal mixture implemented by the server when predicting from the distributed ensemble.  Our algorithm requires the system to periodically synchronize, and we derive a closed-form expression for the optimal synchronization as the solution to a Nash equilibrium in which each local model strives to maximally contribute to the predictive accuracy of the ensemble.  

% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%% Section 1: Instruction %%%%%%
% %\section{Introduction}
% %\label{chp:intro}

% %Input data $x=(x_1, ..., x_d)\in \mathbb{R}^d$. 
% % \begin{comment}

% \section{Problem Setting and Main Results}
% \label{s:Setup}

% \subsection{The Generative Ensemble}
% \label{s:Setup__ss:EnsembleModel}
% Our general results consider ensembles of generative sequential learning models $f^{(i)}$  with at most three inputs at any time $t\in \mathbb{N}$.  For each such $t\in \mathbb{N}_+$, the $i^{th}$ expert model takes the (common) historical input sequence $x_{[0:t]}\in \mathbb{R}^{(1+t)\,d_{x\times 1}}$, an individual source of randomness $\epsilon_r^i$ which is a $d_{\epsilon}\times 1$-valued random variable, and an individual hidden state $Z_t^i\in \mathbb{R}^{d_z\times 1}$. These three inputs are used to generate the latent state $Z_{t+1}$ using an \textit{encoder} $\phi^{(i)}:\mathbb{R}^{d_x\times 1}\times \mathbb{R}^{d_z\times 1}\times \mathbb{R}^{d_{\epsilon}\times 1}\to \mathbb{R}^{d_z\times 1}$ via
% \begin{equation}
% \label{eq:latent_state}
%     Z_{t+1}^i 
% \eqdef 
%     \varphi^{(i)}(x_{[0:t]}^i,Z_t^i,\epsilon_t^i)
% .
% \end{equation}
% Once the latent state is generated, it is used to update the residual of the prediction generated at the previous time $t$ via a \textit{dynamically updating} linear decoding layer
% \begin{equation}
% \label{eq:residual_update}
%     \hat{Y}^i_{t+1} 
% = 
%     \hat{Y}^i_t + \beta^{i\top}_t Z^i_t 
% \end{equation}
% where $\beta_t^i\in \mathbb{R}^{d_y\times 1}$.  Both initial states $\hat{Y}_0^i\in \mathbb{R}^{d_y\times 1}$ and $Z_0^i\in \mathbb{R}^{d_z\times 1}$ are fixed a-priori.  Each generative sequential deep learning model (expert) is defined by
% \[
% \begin{aligned}
%     f^{(i)}: \mathbb{R}^{\mathbb{N}} & \to \mathbb{R}^{\mathbb{N}}\\
%     x_{\cdot} & \mapsto \hat{Y}^i_t
% \end{aligned}
% \]
% for each $t\in \mathbb{N}$, $\hat{Y}^{i}_t$ is computed using the sequential encoder~\eqref{eq:latent_state} (note this depends on $x_{[0:t]}$ and subsequently decoding via~\eqref{eq:residual_update}.

% We will focus on the following three classes of examples.  
% The first is a pre-trained deep learning model that allow for dynamically fine-tunes the final linear decoder layer.
% \begin{example}[Pre-Trained Transformer with Fine-Tunable Linear Decoder]
% \label{ex:finte_tine}
% For $i=1,\dots,N$, let $\phi^{(i)}:\mathbb{R}^{%(1+t)
% d_x
% \times 1}\to \mathbb{R}^{d_z\times 1}$ be all but the final linear decoder layer $\beta_0\in \mathbb{R}^{d_z\times 1}$ of a pre-trained transformer network. \AK{write def of a transformer after}[.]  
% Then
% \[
%     \varphi^{(i)}(x_{[0:t]},\epsilon_t,z_t) \eqdef \phi^{(i)}(%x_{[0:t]})
%         x_t)
%     .
% \]
% \end{example}
% The next example is a particular instance of a \textit{generative} extreme learning machine, a random feature network with continually regenerated random biases.
% \begin{example}[A Generative Model: Random Feature Network]
% \label{ex:Random_NeuralNetwork}
% For each $i=1,\dots,N$, fix a $d_z\times d_z$-dimensional weights random matrix $A^{i}$ and a $d_x$-dimensional random vector $d_z$-dimensional vector $b^{i}$
% \begin{equation}
% \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t 
%             \operatorname{ReLU}\bullet\big(
%                 A^{i} x_t + b^{i} + (\sigma_t^i)^{1/2}\, W_t^i
%             \big)
% \end{equation}
% where $W_t^i\sim N_{d_z}(0,1)$ are independent of $A$ and $b$, and $\sigma_t^i\in [0,\infty)$.
% Here, $\varepsilon_t^i\eqdef (\sigma_t^i)^{1/2}\, W_t^i$, 
% $\phi(x_{[0:t]},\varepsilon_t,z_t)\eqdef 
% \operatorname{ReLU}(Ax_t +b + \varepsilon_t)$, and $Z_t^i\eqdef \operatorname{ReLU}\bullet\big(
%                 A^{i} x_t + b^{i} + (\sigma_t^i)^{1/2}\, W_t^i
%             \big)$.
% \end{example}
% Extending the previous example, our setting also includes \textit{reservoir computers} where one can regenerate a small source of randomness at each time increment; allowing for generative modelling.  
% \begin{example}[A Generative Model: Reservoir Computer]
% \label{ex:ResComp}
% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}.  Let $B$ be a $d_z\times d_z$-dimensional random matrix, independent of the $W_{\cdot}$.  
% If we allow for a hidden state $Z_t$ generated at any time to be remembered, then we obtain an Echo State Network (ESN), which is a special case of a general reservoir computer
% \begin{equation}
% \label{eq:reservoir}
% \begin{aligned}
% Z_{t+1}^i\eqdef & \operatorname{ReLU}\bullet\big(
%     Ax_t + BZ_t^i + b+ (\sigma_t^i)^{1/2}\, W_t^i
% \big)
% \\
% \hat{Y}^i_{t+1} \eqdef & \hat{Y}^i_t + \beta^{i\top}_t Z_t^i
% .
% \end{aligned}
% \end{equation}
% Two subtle differences between~\eqref{eq:reservoir} and standard ESN formulations is that we allow for the final layer of the ESN to be dynamically updated, which is not usually the case in reservoir computing.  Further,~\eqref{eq:reservoir} updates the residuals unlike standard ESNs. 
% \end{example}


% \subsection{The Federated Learning Problem}
% \label{s:Setup__ss:Federated}

% The objective of the server is to optimally adaptively \textit{synchronize} these $N$ generative models, into a single generative ensemble model $\hat{F}:(\mathbb{R}^{d_{x}})^{\mathbb{Z}}\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{Z}}$ to maximize their performance.  The resulting ensemble is represented by
% \[
%     \hat{F}(x_{\cdot})_t \eqdef \sum_{i=1}^N\, w_t^i\, \hat{f}^i(x_{\cdot})_t
% \]
% for mixture coefficients $w_{\cdot}\eqdef (w_t)_{t\in \mathbb{Z}}$ with each $w_t$ belonging to the $N$-simplex $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{i=1}^N\,w_i=1\}$.
% We consider the online \textit{one-shot} case, namely where the server actively optimizes the $w_{\cdot}$ and $\beta_{\cdot}$ parameters drawing from the one single trajectory progressively observed from $y_{\cdot}$; from which we gather information on the infinite-memory dynamical system $f$.


% \paragraph{Federated Computing Model}
% Each generative expert model $\hat{f}^i$ is stored locally on a different machine in the computational network.  The $i^{th}$ machine communicates with the server using two different mechanisms at two different frequencies.  Fix a \textit{synchronization frequency} $T\in \mathbb{N}$.  For each time $t\in \mathbb{N}$ is not divisible by $T$, each expert model greedily optimizes its linear readout layer without communicating with any other expert, by optimizing 
% \begin{equation}
% \label{eq:ridge_local}
%     \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=t-T\vee 0}^t\,
%         e^{-\alpha^i(t-s)}
%         \,\|y_s-\beta_t^i\,Z_s^i\|^2
%         +
%         \gamma^i\|\beta_t^i\|^2
% .
% \end{equation}
% This allows for rapid and fully parallelized online optimization of each model but has the drawback that the ensemble may deviate from its optimum.  
% The following gives the well-known optimal solution of the exponential-weighed ridge-regression problem~\eqref{eq:ridge_local}.
% \begin{proposition}[Experts: Optimal Linear Decoder With No Expert Communication]
% \label{prop:localgreedyupdates}
% Let $\alpha^i\ge 0$ and $\gamma^i>0$.  Then unique solution to~\eqref{eq:ridge_local} is given by
% \[
%         \beta_t^i 
%     =
%         \big(
%             {X^i}^{\top} X_t + \gamma^i I_{d_z}
%         \big)^{-1}\, X_t^{\top} \, \bar{y}_t
% \]
% where $X_t \eqdef (e^{-\alpha^i (t-0)} Z_0,\dots,e^{-\alpha^i(t-s)}Z_s,\dots, Z_t) \in \mathbb{R}^{(1+t)\times d_z}$ and $\bar{y}_t \eqdef (e^{\alpha^i(t-s)}y_s)_{s=0}^t \in \mathbb{R}^{(1+t)\times d_y}$.
% \end{proposition}
% Each expert then immediately communicates their prediction $\hat{Y}_t^i$ to the central server, whose objective is to mix the expert predictions to maximize the predictive power of the ensemble.  The expert does this under the constraint that it cannot over-leverage any one expert prediction; this means that the server must weight the mixture of expert prediction, using a weight $w_t$ belonging to the $N$-simplex is $\Delta_N\eqdef \{w\in [0,1]^N:\,\sum_{n=1}^N\,w_n\}$.
% The optimal weight $w_t$ is chosen such that it optimizes the following penalized \textit{regret functional}
% \begin{align} 
%     J_0(w) 
%  = 
%      \sum_{s=(t-T)\vee 0}^T 
%      e^{-\alpha^0 s}
%          \mathbb{E}  \, 
%        \Big[  \Big\| y_s  - \sum_{j=1}^N w^j_s \hat{Y}^j_s \Big\|^2 
%           + \sum_{j=1}^N \kappa_j \big\| w^j_s \big\|^2 \Big]  
% ,  
% \notag 
% \label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  We compute the optimizer of~\eqref{DTJ0} in the following closed-loop form.
% \begin{theorem}[Server: Optimal Mixture Weights]
% \label{thm:OptimalWeights}
% There exists a unique optimizer 
% $w^{\star} = (w^{i, \star})_{i=1}^N$ 
% of $J_0$ in defined in~\eqref{DTJ0} in $\Delta_N$.   Moreover, $w^{\star}$ given in closed-form by
% \begin{align} 
% \notag
%   w^\star   =   \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
% % \\    
%   % &
%   -  & \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%   \\
%   &\times 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t  -  \mathbf{c} \Big] . 
%   \label{eqn:OptimalWeights}  
% \end{align} 
% where we denote 
% \begin{align} 
%  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N}, 
%  \quad 
%  G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  \mbox{ and }
%  \quad 
%   \mathbf{c} =  \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%   \label{eq:Gc_Def}
% \end{align} 
% \end{theorem} 


% \textit{Synchronization rounds} occur periodically at pre-specified period $T\in \mathbb{N}_+$.  
% In each such round
% % During short communication rounds, 
% the $N$ machines communicate their past $T$ predictions with one another; however, they do not communicate their entire model with one another since that would take an infeasible bandwidth due to the size of each local model.  
% Instead, the local machines are only aware of the predictions generated by one another with the objective of maximizing their predictive power.  

% Consequentially, each local machine can be interpreted as an agent competing with the optimal behaviour, i.e.\ value of $\beta_t^i$, as a solution to a Nash \textit{equilibrium} between these machines.  Thus, given the weight $w_1,\dots,w_T$, each local machine $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize its local objective function
% % \allowdisplaybreaks
% \begin{align} 
% \label{eq:Objective_nth_expert}  
%  % & 
%  J_i(\beta^i, \beta^{-i}) = 
%  \sum_{t=0}^{T} 
%     e^{-\alpha^i t} 
%  \,
%  \mathbb{E} \Big\{  
%  \Big[ 
%  \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big] 
%   % + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 
%   \Big\}   
%   , \quad i = 1, ..., N ,  
% \end{align} 
% where $\beta^{-i}=
% (\beta^j)_{j=1;i\neq i}^N
% % (\beta^1, ..., \beta^{i-1}, \beta^{i+1}, ..., \beta^N)
% $ and $\alpha^i\ge 0$ is a pre-specified hyperparameter controlling the impact of distant past observations on the current game the local machines are playing with one another.  
% The optimal value for the $i^{th}$ machine, which we denote by $(\beta^i_{t:\text{sync}})_{t=0}^T$, is given in closed-form in Proposition~\ref{prop:NashEqmExistence}.  The following synchronization, we set $\beta_T^i\eqdef \beta_{T:sync}^i$ for each $i=1,\dots,N$.

% % The following proposition links the existence of a Nash equilibrium of \eqref{DTRCsystem} and \eqref{eq:Objective_nth_expert} to the solvability of the system \eqref{eqn:Pi}. 
% \begin{proposition}[Experts: Optimal Re-synchronization via The Nash Equilibrium]
% \label{prop:NashEqmExistence}
% Suppose the system \eqref{eqn:Pi} for $(P_i)_{i=1}^N$ admits a solution for $t=0$, $1$, ..., $T$.  
% Then the $N$-player Nash game \eqref{eq:Objective_nth_expert} admits a unique feedback Nash equilibrium 
% \begin{align} 
% \boldsymbol{\beta}_t = [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% \big( \mathbf{B}(t) \hat{Y}_t + \mathbf{C}(t) \big) , \quad t = 0, 1, ..., T. 
% \label{eqmvecbeta} 
% \end{align} 
% where 
% We introduce the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% $t=0$, $1$ ..., $T$. 
% \begin{equation} 
% \begin{cases}  
%   P_i(t) = 
%  [ \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]^\top P_i(t+1) [  \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]  \\ 
%   \hspace{2cm} + [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ]^\top 
%  [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ] 
%  + \mathbf{w}_t \mathbf{w}_t^\top  \\ 
%   \Gamma + \mathbf{A}(t) \, \text{is invertible}  \\ 
%   P_i(T) =  \mathbf{w}_T \mathbf{w}_T^\top  , \quad i = 1, 2, ..., N , 
%  \end{cases}
%  \label{eqn:Pi}
%  \end{equation} 

% \allowdisplaybreaks 
% \begin{equation}  
%  \begin{cases} 
%   S_i(t) =   \mathbf{B}(t)^\top (I + \mathbf{A})^{-1} 
%  [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t) ] (I+\mathbf{A})^{-1} \mathbf{C}   \\ 
%   \hspace{1cm} - P_i(t+1) \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{C} 
%  - \mathbf{B}^\top (I + \mathbf{A})^{-1}\mathbf{D} S_i(t+1) 
%  - \mathbf{w}_t y_t 
%  + S_i(t+1) , 
%   \\ 
%  S_i(T) = - \mathbf{w}_T y_T   . 
% \end{cases}   
% \label{eqn:Si}
% \end{equation} 
% %
% %
% %
% In \eqref{eqn:Pi} and \eqref{eqn:Si}, the matrices $\mathbf{A}(\cdot)$,  
% $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, and $\mathbf{D}(\cdot)$ are defined by  
% \allowdisplaybreaks 
% \begin{align} 
% &\mathbf{A}(t) = \begin{bmatrix} 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_1 Z^{1\top}_t ] & 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_N Z^{N\top}_t ] \\ 
%  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_1 Z^{1\top}_t ] & 
%  \mathbb{E} [(e_2 Z^{1\top}_t)^\top P_2(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_N Z^{N\top}_t ] \\ 
%  \vdots & \vdots & \ddots & \vdots \\ 
%  \mathbb{E}[ (e_N Z^{N\top}_t)^\top P_N(t+1) e_1 Z^{1\top}_t ]& 
%  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_2 Z^{2\top}_t ]
%  & \cdots & 
%  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_N Z^{N\top}_t ]
% \end{bmatrix} \notag \\ 
% & \mathbf{B}(t) = 
%  \begin{bmatrix} 
%  \mathbb{E} (e_1 Z^{1\top}_t )^\top P_1(t+1) \\ 
%  \mathbb{E}(e_2 Z^{2\top}_t )^\top P_2(t+1) \\ 
%  \vdots \\  
%  \mathbb{E} (e_N Z^{N\top}_t) P_N(t+1) 
%  \end{bmatrix} ,  
%  \qquad 
%  \mathbf{C}(t) = 
%  \begin{bmatrix} 
%  \mathbb{E}(e_1 Z^{1\top}_t )^\top S_1(t+1) \\ 
%  \mathbb{E}(e_2 Z^{2\top}_t )^\top S_2(t+1) \\ 
%  \vdots \\ 
%  \mathbb{E}(e_N Z^{N\top}_t) S_N(t+1) 
%  \end{bmatrix} , 
%  \notag \\ 
% & \mathbf{D}(t) 
%  = 
%  \begin{bmatrix} 
%  \mathbb{E}( e_1 Z^{1\top}_t ) , \, 
% \mathbb{E} ( e_2 Z^{2\top}_t ) ,  \,
%  \cdots , \, 
% \mathbb{E} ( e_N Z^{N\top}_t )
%  \end{bmatrix} . 
%  \notag 
% \end{align} 
% \end{proposition}







% wherein only the local machines (nodes) and the central server.  Periodically, with period $T\in \mathbb{N}$, the server coordinates a randomly chosen subset of $0<\bar{N}\ll N$ local machines (nodes) in the distributed ensemble.

% \textit{Short communication rounds} occur at each instance time $t$ at which point each local machine individually optimizes its prediction $\hat{Y}_t^i$ by optimizing the control $\beta_t^i$ using the currently available time-series data 
% % by solving the ridge regression problem 
% \begin{equation}
% \label{eq:ridge_local}
%     \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=0}^t\,
%         e^{-\alpha^i(t-s)}
%         \,\|y_s-\beta_t^i\,Z_s^i\|^2
%         +
%         \gamma^i\|\beta_t^i\|^2
%     %%
%     \qquad \qquad 
%     \mbox{ for }t=0,\dots,T-1
% \end{equation}
% where the hyperparameter $\alpha^i\ge 0$ controls the exponentially decaying of importance on past time-series data and $\gamma^i> 0$ (see Proposition~\ref{prop:localgreedyupdates} for the ridge regression-like closed-form).
% Each local machine then sends its predictions $\hat{Y}_t^1,\dots,\hat{Y}_t^N$ to the server that generates a prediction from the ensemble.  This means that the rule by which the server identifies the time $t$ proportions $w_t$ with which it combines the $N$ distributed models to generate an only depends on the prediction of each model and not its internal parameters
% \[
%     w_t = w\big(
%         \hat{Y}_t^1,\dots,\hat{Y}_t^N
%     \big)
% \]
% for some function $w:\mathbb{R}^{d_y\times N}\to \Delta_N$.  
% The optimal function $w$, is the function minimizing the \textit{regret functional}
% \begin{align} 
%     J_0(w) 
%  = 
%      \sum_{t=1}^T 
%      e^{-\alpha^0 t}
%          \mathbb{E}  \, 
%        \Big[  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%           + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big]  
% ,  
% \notag 
% %\label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  Its expression is given in Theorem~\ref{thm:OptimalWeights}.



% \AK{I think, with no change in the analysis, we may instead only update a small random set of the models during the long communication rounds.  Perhaps the optimal communication frequency can be obtained by optimizing the total computational cost and the random sample of competing models.}[.]

% \textit{Synchronization rounds} occur periodically at pre-specified period $T\in \mathbb{N}_+$.  
% In each such round
% % During short communication rounds, 
% the $N$ machines communicate their past $T$ predictions with one another; however, they do not communicate their entire model with one another since that would take an infeasible bandwidth due to the size of each local model.  
% Instead, the local machines are only aware of the predictions generated by one another with the objective of maximizing their predictive power.  

% Consequentially, each local machine can be interpreted as an agent competing with the optimal behaviour, i.e.\ value of $\beta_t^i$, as a solution to a Nash \textit{equilibrium} between these machines.  Thus, given the weight $w_1,\dots,w_T$, each local machine $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize its local objective function
% % \allowdisplaybreaks
% \begin{align} 
% \label{eq:Objective_nth_expert}  
%  % & 
%  J_i(\beta^i, \beta^{-i}) = 
%  \sum_{t=0}^{T} 
%     e^{-\alpha^i t} 
%  \,
%  \mathbb{E} \Big\{  
%  \Big[ 
%  \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big] 
%   % + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 
%   \Big\}   
%   , \quad i = 1, ..., N ,  
% \end{align} 
% where $\beta^{-i}=
% (\beta^j)_{j=1;i\neq i}^N
% % (\beta^1, ..., \beta^{i-1}, \beta^{i+1}, ..., \beta^N)
% $ and $\alpha^i\ge 0$ is a pre-specified hyperparameter controlling the impact of distant past observations on the current game the local machines are playing with one another.  
% The optimal value for the $i^{th}$ machine, which we denote by $(\beta^i_{t:\text{sync}})_{t=0}^T$, is given in closed-form in Proposition~\ref{prop:NashEqmExistence}.  The following synchronization, we set
% \[
%     \beta_T^i\eqdef \beta_{T:sync}^i
% \]
% for each $i=1,\dots,N$.

% \section{The Algorithm}
% \label{s:AlgoMain}

% \AK{I think we should only sample the best $N$ performing models at any round.}

% \begin{algorithm}[H]%[ht!]%
% \caption{Proposed Federated Learning Algorithm}
% \label{alg:FedMain}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Current time $t\in \mathbb{N}$, Hidden States $\{Z_t^i\}_{i=1}^N$, expert models $\{\varphi^i\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$, Batch size $1\le b\le N$.
% \DontPrintSemicolon
%         \State \eIf{$t \bmod T\neq 0$}{
%             \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
%                 \State \tcc{Update Experts in Parallel}
%                 \State \ForParallel{\State $\beta_t^i \leftarrow 
%                     \big(
%                         {X^i}^{\top} X_t + \gamma^i I_{d_z}
%                     \big)^{-1}\, X_t^{\top} \, \bar{y}_t$
%                     \tcp*{Local Weighted Regression}
%                     \State Generate $\varepsilon_t^i$
%                     \tcp*{Generate Random State}
%                     \State $Z_{t+1}\leftarrow \varphi(x_{[0:t]},\varepsilon_t^i,Z_{t+1}^i)$
%                     \tcp*{Update Hidden State}
%                     \State 
%                       $(\hat{\mathbf{Y}}_t)_i
%                       \leftarrow
%                       \hat{\mathbf{Y}}_{t-1}^i
%                       + 
%                       (\beta_t^i)^{\top}\,
%                       Z_t$
%                       \tcp*{Update Residual Prediction}
%                         }
%                    }{
%             %%%% Synchronization Step
%             \State \tcc{Synchronize Subset of Local Experts via Random Nash Game}
%                 \State $\boldsymbol{\beta}^{\text{sync}}_s \leftarrow $ Run Synchronize Sub-Routine: Algorithm~\ref{alg:sync_subroutine}
%                 \tcp*{Synchronized Weights}
%                 \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
%                     \State \ForParallel{
%                     \State $\beta_t^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_T)_i$\;
%                     \State Generate $\varepsilon_t^i$ \tcp*{Generate Random State}
%                     \State $
%                     \hat{\mathbf{Y}}_t
%                     \leftarrow
%                     \hat{\mathbf{Y}}_{t-1}
%                     + 
%                     (\beta_t^i)^{\top}\,
%                     \varphi(x_{[0:t]},\varepsilon_t^i,Z_t^i)
%                     $\;
%                 }
%               }
%     \State \tcc{Server Syncronizes Local Expert Predictions}
%     \State $
%         w_t \leftarrow
%   \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%     \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t -  \mathbf{c} \Big]
%     $
%      \;
%     \State $w_t \leftarrow 
%     \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t - w_t$
%     \tcp*{Update Mixture Weights}
%     %%
%     \State \Return $w_t^{\top} \hat{\mathbf{Y}}_t$.
%     \tcp*{Ensemble Prediction}
% \end{algorithmic}
% \textbf{Note:} The helper functions $\mathbf{A},\mathbf{B},\mathbf{C},\Gamma$ are defined in circa Proposition~\ref{prop:NashEqmExistence} and the matrices $K$, $G$, and $\mathbf{c}$ are defined in~\eqref{eq:Gc_Def}.
% \end{algorithm}


% Every $T$ round, the server synchronizes a (uniformly) randomly selected batch of $ b \le N$ experts from all the available experts.  
% Since each expert is working on a separate machine, which may not be large enough to load the states of all the experts simultaneously, they must reach a consensus with limited communication.  The optimal consensus can be framed as a \textit{non-cooperative game} amongst the randomly chosen $b$ experts, each of which seeks to excerpt predictive influence on the ensemble, to the proportion allotted by the server according to $w_t$.  The optimal discussion which the ensemble can take can be formulated as a Nash equilibrium, in which no expert can improve their predictive influence on the mixture by further modifying their linear decoder~\eqref{eq:Objective_nth_expert}.
% The subroutine in Algorithm~\ref{alg:sync_subroutine} computes precisely this Nash equilibrium using $T$ iterations.

% \AK{Xuwei: Write Proposition in Algo 2 Format}
% \begin{algorithm}[H]%[ht!]%
% \caption{Synchronization Subroutine}
% \label{alg:sync_subroutine}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Current time $t\in \mathbb{N}$, Target time-series $(y_s)_{s\le t}$, pre-trained models $\{(\varphi^i,\sigma_{\cdot}^i,\hat{\mathbf{Y}}_{t-1}^i)\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$.
% \DontPrintSemicolon
%        \For{$s=T-t,\dots,T$}{
%            $
%            \boldsymbol{\beta}^{\text{sync}}_s = [\beta^{\text{sync},1\top}_s, ..., \beta^{\text{sync}N,\top}_s ]^\top = - ( \Gamma + \mathbf{A}(s) )^{-1} \big( \mathbf{B}(s) \hat{Y}_t + \mathbf{C}(s) \big) 
%            $
%            \;
%            $
%            \beta_t^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_T)_i
%            $
%            \;
%            $
%            \hat{\mathbf{Y}}_t
%               \leftarrow
%               \hat{\mathbf{Y}}_{t-1}
%               + 
%               \Big(
%                     (\beta_t^i)^{\top}\,
%                   \operatorname{ReLU}\bullet\big(
%                     \phi^i\circ \tau_t\big(x_{(-\infty,t]}\big)
%                     +\sigma_t^i\,W_t^i
%                 \big)
%             \Big)_{i=1}^N
%            $
%            \tcp*{Synchronize Local Models}
%        }
%     %%
%     \State \Return $w_t^{\top} \hat{\mathbf{Y}}_t$.
%     \tcp*{Synchronized Weights}
% \end{algorithmic}
% \textbf{Note:} The helper functions $\mathbf{A},\mathbf{B},\mathbf{C},\Gamma$ are defined in circa Proposition~\ref{prop:NashEqmExistence} and the matrices $K$, $G$, and $\mathbf{c}$ are defined in~\eqref{eq:Gc_Def}.
% \end{algorithm}

% Next, we analyze Algorithm~\ref{alg:FedMain} and the subroutine in Algorithm~\ref{alg:sync_subroutine}.
% \section{Theoretical Analysis}
% \label{s:Analysis}

% Our theoretical analysis of Algorithms~\ref{alg:FedMain} and~\ref{alg:sync_subroutine} is broken tinto two steps.  First, we analyze the optimality of the server/(major player), which mixes the prediction generated by the $N$ experts (minor players).  Then, we analyze the optimality of the prediction generated by each agent either in the (slow) synchronization phase, where a random subset of $b$ agents plays a Nash game to synchronize their linear encoders, or in the (fast) intermediate times, where each expert selfishly optimizes their linear readout layer independently of the behaviour of the other experts.

% \subsubsection{The Server's Optimal Mixting Problem}
% \label{s:Optimal_Server__akaMajorPlayer}

% Consider the objective of the major player/central planner is to optimize 
% \begin{align} 
%     \min_{w_{\cdot}}\,
%  J_0(w) = \mathbb{E}  \sum_{t=1}^T e^{-\alpha^0 t } \Big[  
%  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] .  
%   \label{DTJ0}
% \end{align} 
% where the minimization is taken over all decision rules $w_{\cdot} \eqdef \{w_t\}_{t=1}^T = \{(w^1_t, ..., w^N_t)\}_{t=1}^T$ whose paths lie in the $N$-simplex $\Delta_N \eqdef  \{w\in [0,1]^N:\, \sum_{n=1}^N\, w_n=1\}$.  
% Our first main result shows that there exists a unique solution to the optimization problem~\eqref{DTJ0}.
% \begin{theorem}[Optimal Coordination]
% \label{thm:OptimalWeights}
% The quadratic programming problem \eqref{MajorPlayer:QP} admits a unique solution $w^\star = (w^{1, \star}, ..., w^{N, \star})$ given by 
% \begin{align} 
% \notag
%   w^\star   =   \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
% % \\    
%   % &
%   -  & \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%   \\
%   &\times 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t  -  \mathbf{c} \Big] . 
%   \label{eqn:OptimalWeights}  
% \end{align} 
% where we denote 
% \begin{align} 
%  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N}, 
%  \quad 
%  G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  \mbox{ and }
%  \quad 
%   \mathbf{c} =  \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%   \label{eq:Gc_Def}
% \end{align} 

% \end{theorem} 




% \begin{comment}
% We consider a model with $N$ agents $\{\mathcal{A}_i\}_{i=1}^N$. 
% Let each agent $\mathcal{A}_i$ has input signal sequence $\{Z^i_t\}_{t\geq 0}$ and a linear decoder.  
% \AK{This needs to be updated, but only at the end.}[.]
% \begin{equation}
% \begin{aligned} 
% & X^i_{t+1} =  A_i X^i_t + \sigma W^i_t , \quad X^i_\cdot \in \mathbb{R}^{dx \times 1} , \\  
% & Z^i_{t+1} =  \varphi(Z^i_t, X^i_{t+1}) ,  \quad Z^i_\cdot \in \mathbb{R}^{d_{z} \times 1} ,  \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t Z^i_t , \quad \hat{Y}^i_\cdot \in \mathbb{R}^{d_{y} \times 1} , \ i = 1, ..., N ,   
% \end{aligned} 
% \label{DTRCsystem}
% \end{equation} 
% where $W^i_t$, $i=1$, ..., $N$, $t=0$, ..., $T$ are identically independently distributed standard normal random variables. 
% \end{comment}

% \begin{comment}
% Consider a central planner/major player who also acts as a central planner and chooses weight vector sequence on the $N$-simplex   
% \begin{align} 
% w_t= (w^1_t, ..., w^N_t)^\top \in \Delta_N , \quad t = 0, 1, ..., T \notag  
% \end{align} 
% for the minor players' output $\hat{Y}^i$ in order to minimize the total loss  
% \begin{align} 
%  J_0(w) = \mathbb{E}  \sum_{t=1}^T \Big[ 
%  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] ,  
%   \notag 
%   \label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  

% Given the weight $w_t = (w^1_t, ..., w^N_t)$, $t=0$, $1$, ..., $T$, each minor agent $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize the individual cost 
% \allowdisplaybreaks
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 \Big\}   , \quad i = 1, ..., N ,  \label{eq:Objective_nth_expert}  
%   \end{align} 
%  where $\beta^{-i}=(\beta^1, ..., \beta^{i-1}, \beta{i+1}, ..., \beta^N)$. 
% \end{comment}



% \subsection{The Nash Equilibrium between the Minor Players}
% Denote 
% \begin{align} 
%  & \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top, \quad \hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top, \quad   
% \mathbf{e}^N_i = e^N_i \otimes I_{d_{z}} = [0, ..., I_{d_{z}} , ..., 0]^\top,  \notag \\ 
%  & \Gamma = \diag[\gamma_1, ..., \gamma_N] \notag 
% \end{align} 
% then the costs \eqref{eq:Objective_nth_expert} for the $N$ agents can be written as  
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \mathbf{w}^\top_t \hat{Y}_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y_T - \mathbf{w}_T^\top \hat{Y}_T \Big\|^2 \Big\}   , \quad i = 1, ..., N. 
%   \label{eq:Objective_nth_expertcompact}
%  \end{align} 

%  We aim to find a set of Nash equilibrium strategies $(\beta^1, ..., \beta^N)$ for the $N$ agent such that 
%  \begin{align} 
%  J_i(\beta^i, \beta^{-i}) 
%  \leq J_i(u, \beta^{-i}), 
%  \quad \forall u \in \mathbb{R}^{d_{z} \times d_{y}} , 
%  \quad  \forall i = 1, ..., N. \label{NEbeta}
%  \end{align} 



% % We introduce the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% % $t=0$, $1$ ..., $T$. 
% % \begin{equation} 
% % \begin{cases}  
% %   P_i(t) = 
% %  [ \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]^\top P_i(t+1) [  \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]  \\ 
% %   \hspace{2cm} + [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ]^\top 
% %  [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ] 
% %  + \mathbf{w}_t \mathbf{w}_t^\top  \\ 
% %   \Gamma + \mathbf{A}(t) \, \text{is invertible}  \\ 
% %   P_i(T) =  \mathbf{w}_T \mathbf{w}_T^\top  , \quad i = 1, 2, ..., N , 
% %  \end{cases}
% %  \label{eqn:Pi}
% %  \end{equation} 

% % \allowdisplaybreaks 
% % \begin{equation}  
% %  \begin{cases} 
% %   S_i(t) =   \mathbf{B}(t)^\top (I + \mathbf{A})^{-1} 
% %  [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t) ] (I+\mathbf{A})^{-1} \mathbf{C}   \\ 
% %   \hspace{1cm} - P_i(t+1) \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{C} 
% %  - \mathbf{B}^\top (I + \mathbf{A})^{-1}\mathbf{D} S_i(t+1) 
% %  - \mathbf{w}_t y_t 
% %  + S_i(t+1) , 
% %   \\ 
% %  S_i(T) = - \mathbf{w}_T y_T   . 
% % \end{cases}   
% % \label{eqn:Si}
% % \end{equation} 
% % %
% % %
% % %
% % In \eqref{eqn:Pi} and \eqref{eqn:Si}, the matrices $\mathbf{A}(\cdot)$,  
% % $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, and $\mathbf{D}(\cdot)$ are defined by  
% % \allowdisplaybreaks 
% % \begin{align} 
% % &\mathbf{A}(t) = \begin{bmatrix} 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_1 Z^{1\top}_t ] & 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_N Z^{N\top}_t ] \\ 
% %  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_1 Z^{1\top}_t ] & 
% %  \mathbb{E} [(e_2 Z^{1\top}_t)^\top P_2(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_N Z^{N\top}_t ] \\ 
% %  \vdots & \vdots & \ddots & \vdots \\ 
% %  \mathbb{E}[ (e_N Z^{N\top}_t)^\top P_N(t+1) e_1 Z^{1\top}_t ]& 
% %  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_N Z^{N\top}_t ]
% % \end{bmatrix} \notag \\ 
% % & \mathbf{B}(t) = 
% %  \begin{bmatrix} 
% %  \mathbb{E} (e_1 Z^{1\top}_t )^\top P_1(t+1) \\ 
% %  \mathbb{E}(e_2 Z^{2\top}_t )^\top P_2(t+1) \\ 
% %  \vdots \\  
% %  \mathbb{E} (e_N Z^{N\top}_t) P_N(t+1) 
% %  \end{bmatrix} ,  
% %  \qquad 
% %  \mathbf{C}(t) = 
% %  \begin{bmatrix} 
% %  \mathbb{E}(e_1 Z^{1\top}_t )^\top S_1(t+1) \\ 
% %  \mathbb{E}(e_2 Z^{2\top}_t )^\top S_2(t+1) \\ 
% %  \vdots \\ 
% %  \mathbb{E}(e_N Z^{N\top}_t) S_N(t+1) 
% %  \end{bmatrix} , 
% %  \notag \\ 
% % & \mathbf{D}(t) 
% %  = 
% %  \begin{bmatrix} 
% %  \mathbb{E}( e_1 Z^{1\top}_t ) , \, 
% % \mathbb{E} ( e_2 Z^{2\top}_t ) ,  \,
% %  \cdots , \, 
% % \mathbb{E} ( e_N Z^{N\top}_t )
% %  \end{bmatrix} . 
% %  \notag 
% % \end{align} 

% % The following proposition links the existence of a Nash equilibrium of \eqref{DTRCsystem} and \eqref{eq:Objective_nth_expert} to the solvability of the system \eqref{eqn:Pi}. 
% % \begin{proposition}[Nash Equilibrium of Minor Players]
% % \label{prop:NashEqmExistence}
% % Suppose the system \eqref{eqn:Pi} for $(P_i)_{i=1}^N$ admits a solution for $t=0$, $1$, ..., $T$.  
% % Then the $N$-player Nash game \eqref{eq:Objective_nth_expert} admits a unique feedback Nash equilibrium 
% % \begin{align} 
% % \boldsymbol{\beta}_t = [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% % \big( \mathbf{B}(t) \hat{Y}_t + \mathbf{C}(t) \big) , \quad t = 0, 1, ..., T. 
% % \label{eqmvecbeta} 
% % \end{align} 
% % \end{proposition}




% \subsection{Parallelized Selfish Expert Optimization}
% \label{s:ShortComm}
% We first express the optimal control of the local model, when optimizing their predicting performance before the synchronization time $T$.




% \section{Applications}
% \label{s:Examples}

% \subsection{{Pre-Trained Transformer with Fine-Tunable Linear Decoder - Example~\ref{ex:finte_tine}}}
% Consider the setting of Example~\ref{ex:finte_tine}.  Then, the matrices $\mathbf{A}(\cdot)$,  
% $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, and $\mathbf{D}(\cdot)$ in
% \eqref{eqn:Pi} and \eqref{eqn:Si} can be dramatically simplified, and all expectations can be removed.  
% In this setting they reduce to
% \allowdisplaybreaks 
% \begin{align} 
% \mathbf{A}(t) & = 
% \begin{bmatrix} 
% e_i\phi^{(i)}(x_t)^{\top} P_i(t+1) e_j\phi^{(j)}(x_t)^{\top}
% \end{bmatrix}_{i,j=1}^N
% \notag \\ 
% & \mathbf{B}(t) = 
%  \begin{bmatrix} 
%  (e_i \phi(x_t)^{i\top}_t )^\top P_1(t+1) \\ 
%  \end{bmatrix}_{i=1}^N 
%  ,  
%  \notag \\ 
%  & \mathbf{C}(t) = 
%  \begin{bmatrix} 
%  e_i \phi(x_t)^{\top} S_i(t+1) 
%  \end{bmatrix}_{i=1}^N 
%  , 
%  \notag \\ 
% & \mathbf{D}(t) 
%  = 
%  \begin{bmatrix} 
%  e_j \phi^{(j)}(x_t)^{\top}
%  \end{bmatrix}_{j=1}^{N\,\top}
%  . 
%  \notag 
% \end{align} 


% \subsection{{Generative Random Feature Network - Example~\ref{ex:Random_NeuralNetwork}}}
% \label{s:Analysis__ss:ELN}

% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}.

% \AK{$a_t\eqdef A^{(i)}x_t+b^{(i)}$ ... @Xuwei please make the update.}

% For each $i=1,\dots,N$, let $(a_t^i)_{t\in \mathbb{N}}$ and $(\sigma_t^i)_{t\in \mathbb{N}}$ respectively be sequences in $\mathbb{R}^{d_z\times 1}$ and in $(0,\infty)$.  
% Suppose that the system in~\eqref{DTRCsystem} is 
% \begin{equation}
% \begin{aligned} 
% & Z^i_{t+1} =  
% \operatorname{ReLU}\bullet\big(
%     a_t + \sqrt{\sigma_t^i}\, W_t^i
% \big) ,  
% % \quad Z^i_\cdot \in \mathbb{R}^{d_{z} \times 1} ,  
% \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t Z^i_t 
% .
% % , \quad \hat{Y}^i_\cdot \in \mathbb{R}^{d_{y} \times 1} , \ i = 1, ..., N ,   
% \end{aligned} 
% \label{DTRCsystemReLU}
% \end{equation} 


% \begin{corollary} 
% \label{cor:Random_NN}
% If $\varphi(\cdot)$ in \eqref{DTRCsystem} takes the form in \eqref{DTRCsystemReLU},  
% \end{corollary} 

% \begin{proof} [{Proof of Corollary~\ref{cor:Random_NN}}]

% \begin{align} 
%  & \mathbb{E} \big[ Z^i_t e_i^\top P_i(t+1) e_j Z^{j\top}_t \big]  
%  =  \mathbb{E} \big[ Z^i_t  ( P_i(t+1) )_{ij}  Z^{j\top}_t \big] \notag 
% \end{align} 
% The diagonal submatrices of $\mathbf{A}(t)$ take the form  
% \begin{align} 
%  &  \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_i Z^{i\top}_t ]  \notag \\ 
%   = &  \mathbb{E} [  Z^i_t e_i^\top P_i(t+1) e_i Z^{i\top}_t ] \notag \\ 
% = &   \mathbb{E} [  Z^i_t  ( P_i(t+1) )_{ii} Z^{i\top}_t ]  \notag \\ 
%  = & \Big( \mathbb{E}\big[  (Z_{t+1}^i)_j ( P_i(t+1) )_{ii}  (Z_{t+1}^i)_k \big]  \Big)_{1\leq j, k \leq dz} . \notag 
% \end{align} 
% By Lemma~\ref{lem:Mean_Cov_ResModel}, the entries in the diagonal submatrices of $\mathbf{A}(t)$ are given by  
% \begin{align} 
%  & \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii}\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = \big[ \mathbb{E}( Z_{t+1}^i )
%     \mathbb{E}( Z_{t+1}^{i\top} ) \big]_{jk} 
%     & \mbox{ if }   j \neq k
%     \end{cases} 
%     \notag 
% \end{align} 
% where 
% \begin{align} 
%  & \big[ \mathbb{E}( Z_{t+1}^i )
%     \mathbb{E}( Z_{t+1}^{i\top} ) \big] \notag \\ 
%     =& 
%     \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big) \Big\} 
%     \Big\{ 
%      a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big)
%     \Big\}^\top . \notag 
% \end{align} 


% Since the white noises $\{W^i_t\}_{i, t}$, are independent, \eqref{DTRCsystemReLU} implies that 
% $Z^i_t$ and $Z^j_t$ are independent for $i\neq j$. 
% The off-diagonal submatrices of $\mathbf{A}(t)$ can be written as   
% \begin{align} 
%  & \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_j Z^{j\top}_t ] \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  e_i^\top P_i(t+1) e_j  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  ( P_i(t+1) )_{ij}  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big) \Big\} (P_i(t+1))_{ij} 
%         \Big\{  a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^j}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^j}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^j}
%             % \,
%             a_t^2
%         \Big) \Big\}^\top    \notag 
% \end{align} 
% where $\mathbb{E} [  Z^i_t ]$ and $\mathbb{E} [  Z^j_t ]$ are given explicitly by Lemma~\ref{lem:Mean_Cov_ResModel}. 


% \end{proof} 



% Under these dynamics, the following lemma gives enough information to compute the relevant matrices in Proposition~\ref{prop:NashEqmExistence}.
% \begin{lemma}[{Mean and Covariance of $Z_{\cdot}^i$ in the System~\eqref{DTRCsystem}}]
% \label{lem:Mean_Cov_ResModel}
% Consider the setting of~\eqref{DTRCsystem}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[Z_{t+1}^i] 
%     = &
%         a_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             a_t^2
%         \Big)
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of~\eqref{DTRCsystem}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion.
% \end{proof}





% \newpage


% \section{Proofs}
% \label{s:Proofs}

% This section contains the proofs of our main results.

% \subsection{{Proof of Proposition~\ref{prop:localgreedyupdates}}}
% \begin{proof}[{Proof of Proposition~\ref{prop:localgreedyupdates}}]
% Observe that the loss function in~\eqref{eq:ridge_local} can be re-written as
% \allowdisplaybreaks
% \begin{align}
% \label{eq:redux_ridge}
%         \sum_{s=0}^t\,
%             e^{-\alpha^i(t-s)}
%             \,\|y_s-\beta_t^i\,Z_s^i\|^2
%             +
%             \gamma^i\|\beta_t^i\|^2
%     =
%         \sum_{s=0}^t\,
%             \,\|\big(e^{-\alpha^i(t-s)}y_s\big)-\beta_t^i\,(e^{-\alpha(t-s)} Z_s^i)\|^2
%             +
%             \gamma^i\|\beta_t^i\|^2
% \end{align}
% and the right-hand side of~\eqref{eq:redux_ridge} is simply a standard ridge-regression problem.  Since this is a strictly convex problem, there is a unique $\beta_t^i\in \mathbb{R}^{d_y\times d_x}$ minimizing the right-hand side of~\eqref{eq:redux_ridge}.  The desired closed-form expression is given in \citep[Equation (3.44)]{HastieTibshiraniFriedman_2001ESLBook}.
% \end{proof}


% \subsection{{Proof of Proposition~\ref{prop:NashEqmExistence}}}
% \label{s:Proofs__ss:prop:NashEqmExistence}
% \begin{proof}
% Let $V_i(t,\hat{\mathbf{y}})$, $i=1$,...,$N$ be the value functions of the $N$ players associated with \eqref{DTRCsystem} and \eqref{eq:Objective_nth_expert}. 
% %\begin{align}  
% % & V_i(t, \hat{\mathbf{y}}) 
% %=  \sup_{\beta^i} \mathbb{E} \Big\{  
% % \Big\| y^i_t - \sum_{i=1}^N w^i 
% % \hat{y}^i \Big\|^2 
% %  + \| \beta^i \|^2    
% %+ V_i(t+1, \hat{\mathbf{y}} + 
% % \sum_{j=1}^N  e_j Z^{j\top}_t\beta^j) 
% %  \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
% %   & V_i(T, \hat{\mathbf{y}}) 
% %   = \notag 
% %\end{align} 
% From \eqref{eq:Objective_nth_expertcompact}, the value functions at time $T$ with $\hat{Y}_T=\hat{\mathbf{y}}$ satisfy 
% \begin{align} 
%  V_i(T, \hat{\mathbf{y}}) 
%  =  \Big\| y_T -  \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%  = \hat{\mathbf{y}}^\top \mathbf{w}_T \mathbf{w}_T^\top \hat{\mathbf{y}} 
%  - 2 y_T \mathbf{w}_T^\top \hat{\mathbf{y}} + |y_T|^2 .  
%  \label{Vi(T)}
% \end{align} 
% By the dynamic programming principle, the value functions at $T-1$ with $\hat{Y}_{T-1}= \hat{\mathbf{y}}=(\hat{y}^{1\top}, ..., \hat{y}^{N\top})^\top$ satisfies  
% \begin{align} 
% V_i(T-1, \hat{\mathbf{y}}) 
% = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    
%   + e^{-\alpha^i} V_i(T, \hat{\mathbf{y}} + \sum_{j=1}^N  e_j Z^{j\top}_{T-1} \beta^j ) 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
%    = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%   + \gamma_i \| \beta^i \|^2     + e^{-\alpha^i} \Big\| y_T - \sum_{j=1}^N w^j_T \Big( \hat{y}^j +  Z^{j\top}_{T-1}  \beta^j \Big)  \Big\|^2 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
% = & \Big\| y_{T-1} - \mathbf{w}_T^\top \hat{\mathbf{y}} \Big\|^2 
%  + e^{-\alpha^i t} \Big\| y_T - \mathbf{w}^\top \hat{\mathbf{y}} \Big\|^2   \notag \\  
%  &    + \mathbb{E} \Big\{  \gamma_i \| \beta^i \|^2 + e^{-\alpha^i} \Big\| \sum_{j=1}^N w^j_T Z^{j\top}_{T-1} \beta^j \Big\|^2 
%   - 2 e^{-\alpha^i} \Big( y_T - \sum_{j=1}^N w^j_T \hat{y}^j \Big)^\top \sum_{j=1}^N w^j_T Z^{j\top}_{T-1} \beta^j 
%     \Big\} .
%    \label{DPeqnVi(T-1)}
% \end{align} 
% By the first order condition for the right side of \eqref{DPeqnVi(T-1)}, we have 
% \begin{align} 
%  \gamma_i \beta^i +  \sum_{j=1}^N \mathbb{E} \big[  Z^i_{T-1} w^i_T w^j_T Z^{j\top}_{T-1} \big]  \beta^j  
%    + \mathbb{E} \big[ Z^i_{T-1} \big] w^i_T \sum_{j=1}^N w^j_T \hat{y}^j   - Z^i_{T-1} w^i_T y_T 
%  = 0 , \quad i = 1, ..., N \notag 
% \end{align} 
% which can be written in the compact form 
% \begin{align} 
%  \Gamma [\beta^{1\top}, ..., \beta^{N \top}]^\top = - \mathbf{A}(T-1) [\beta^{1\top}, ..., \beta^{N \top}]^\top 
%  - \mathbf{B} (T-1) \hat{\mathbf{y}} - \mathbf{C}(T-1) .  
% \end{align} 
% Since \eqref{eqn:Pi} admits a solution by the hypothesis of the proposition, we have that $\Gamma + \mathbf{A}(T-1)$ is invertible, and hence 
% \begin{align} 
%   \boldsymbol{\beta}_{T-1} = [\beta^{1\top}_{T-1}, ..., \beta^{N \top}_{T-1} ]^\top = - ( \Gamma  + \mathbf{A}(T-1) )^{-1} 
% \big( \mathbf{B}(T-1) \hat{Y}_{T-1} + \mathbf{C}(T-1) \big) . 
% \label{eqmbetaT-1}
% \end{align} 

% Substituting \eqref{eqmbetaT-1} into \eqref{DPeqnVi(T-1)}, 
% we obtain that $V_i(T-1, \hat{\mathbf{y}})$ take the form 
% \begin{align} 
%   V_i(T-1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(T-1) \hat{\mathbf{y}}  
%   + 2 S_i(T-1)^\top \hat{\mathbf{y}} + r_i(T-1) , \quad i = 1, ..., N. \notag  
%  \end{align} 
%  where $P_i(T-1)$ and $S_i(T-1)$ are determined by \eqref{eqn:Pi} and \eqref{eqn:Si}. 

% Assume by induction that at $t$ the value functions $\{V_i(t+1, \hat{\mathbf{y}})\}_{i=1}^N$ take the affine-quadratic form 
% \begin{align} 
%   V_i(t+1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t+1) \hat{\mathbf{y}}  
%   + 2 S_i(t+1)^\top \hat{\mathbf{y}} + r_i(t+1) , \quad i = 1, ..., N , \notag  
%  \end{align} 
% with $P_i$ and $S_i$ determined from \eqref{eqn:Pi} and \eqref{eqn:Si}, respectively. 
% We show that at $t$ with state $\hat{Y}_t=\hat{\mathbf{y}}$ the value functions $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ also take the form 
% \begin{align} 
%   V_i(t, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) , \quad i = 1, ..., N . \notag  
%  \end{align} 
% %and the equilibrium strategy $\boldsymbol{\beta}=[\beta^{1\top}, ..., \beta^{N\top} ]$ is indeed given by \eqref{eqmvecbeta}. 

 
% By the dynamic programming principle, $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ satisfy the system of dynamic programming equations:  
% \begin{align} 
% V_i(t, \hat{\mathbf{y}}) 
% = & \sup_{\beta^i} \mathbb{E} \Big\{  \Big\| y_t - \sum_{i=1}^N w_t^i \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    + V_i(t+1, \hat{\mathbf{y}} + \sum_{j=1}^N  e_j Z^{j\top}_t \beta^j ) 
%    \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
%   =& \sup_{\beta^i} \mathbb{E} 
%   \Big\{  \Big\| y_t - \sum_{i=1}^N w^i_t \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2 
%    + \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{j\top}_t  \beta^j  \Big]^\top P_i(t+1) 
%   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{j\top}_t  \beta^j  \Big] \notag \\ 
%  &   \hspace{5cm}  + 2 S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j Z^{i\top}_t  \beta^j  \Big] 
%   + r_i(t+1)   \Big| \hat{Y}_t = \mathbf{\hat{y}}    \Big\} \notag \\ 
% %%%%% 
%   = &  \sup_{\beta^i} \Big\{ \Big\| y_t - \sum_{i=1}^N w^i_t \hat{y}^i \Big\|^2 
%   + \gamma_i \| \beta^i \|^2 + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}}  
%   + 2 \hat{\mathbf{y}}^\top P_i(t+1) \sum_{j=1}^N e_j \mathbb{E}(Z^{j\top}_t) \beta^j \notag \\ 
%    & + \sum_{j, k=1}^N \beta^{j\top} \mathbb{E} \Big\{ (e_j Z^{j\top}_t )^\top P_i(t+1) e_k Z^{k\top}_t \Big\}  \beta^k 
%    + 2 S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N e_j \mathbb{E}(Z^{j \top}_t )  \beta^j  \Big] 
%    + r_i(t+1) \Big\} \notag \\ 
%    & i = 1, ..., N . 
%   \label{DPeqnV(y)}
% \end{align} 
% By the first order condition for the right side of \eqref{DPeqnV(y)}, we have 
% \begin{align} 
%  - \gamma_i \beta^i = &  \mathbb{E}(Z^i_t) e_i^\top P_i(t+1) \hat{\mathbf{y}}  
%   + \sum_{j=1}^N  \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i(t+1) e_j Z^{j\top}_t \Big\}  \beta^j  
%   + \mathbb{E}(Z^i_t) e_i^\top  S_i(t+1) \notag \\ 
%   = &  \sum_{j=1}^N  \mathbb{E} \Big\{ (e_i Z^{i\top}_t )^\top P_i(t+1) e_j Z^{j\top}_t \Big\}  \beta^j  
%   + \mathbb{E}(Z^i_t) e_i^\top [ P_i(t+1) \hat{\mathbf{y}}  +  S_i(t+1) ] ,   
%  \label{betaifirstorderV(y)} \\ 
%  & i = 1, 2, ..., N. \notag 
% \end{align} 


% Then \eqref{betaifirstorderV(y)} can be written in the compact form  
% \begin{align} 
% - \Gamma [\beta^{1\top}, ..., \beta^{N \top}]^\top = \mathbf{A}(t) [\beta^{1\top}, ..., \beta^{N \top}]^\top 
%  + \mathbf{B} (t) \hat{\mathbf{y}} + \mathbf{C}(t) , \notag 
% \end{align} 
% and therefore the equilibrium strategy at time $t$ is determined by 
% \begin{align} 
% [\beta^{1\top}, ..., \beta^{N \top}]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% \big( \mathbf{B}(t) \hat{\mathbf{y}} + \mathbf{C}(t) \big) .  \notag   
% \end{align} 
% %With the defined $\mathbf{A}$ and $\mathbf{B}$, we can write the system \eqref{DPeqnV(y)} as 

% %By induction, we have shown that 
% \end{proof} 


% \subsection{{Proof of Theorem~\ref{thm:OptimalWeights}}}
% \label{s:Proofs__ss:OptimalWeights}
% We minimize \eqref{DTJ0} over all $\Delta_N$-valued decision rules $w_{\cdot}$.  
% At each time $t$, the major player needs to solve the nonlinear programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N) }  \big\| y_t - \sum_{j=1}^N w^j \hat{y}^j_t \big\|^2 
%  + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 \\ 
% & \text{subject to} \ \mathbf{g}(w)=(w^1-1, ..., w^N-1, -w^1, ..., -w^N) \leq 0 , \quad 
%  h(w) = w^1 + ... + w^N - 1 = 0 . 
% \end{aligned} 
% \label{MajorPlayer:NLoptim}
% \end{equation} 

% Denote 
% \begin{align} 
% % \hat{\mathbf{Y}}_t = \big[ \hat{y}^1_t, \cdots , \hat{y}^N_t \big] , \quad 
%   \mathbf{1}_{1\times N} = \big[ 1, ..., 1 \big] \in \mathbb{R}^{1\times N} , \quad 
%  % \hat{\boldsymbol{\lambda}} = \big[ \hat{\lambda}_1, ..., \hat{\lambda}_N \big]^\top , \quad 
%  % \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N} . \notag 
% \end{align} 



% Since the objective function of the nonlinear programming problem \eqref{MajorPlayer:NLoptim} can be written as 
% \begin{align} 
%   \Big\| y_t - \sum_{j=1}^N w^j \hat{y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 
%  = &  \Big( y^\top_t - \sum_{j=1}^N w^j \hat{y}^{j\top}_t \Big) 
%  \Big( y_t - \sum_{j=1}^N w^j \hat{y}^j_t \Big) + \sum_{j=1}^N \kappa_j w^{j 2}   \notag \\ 
%  = & N \sum_{i,j=1}^N w^i \hat{y}^{i\top}_t \hat{y}^j_t w^j 
%   - 2  y^\top_t   \sum_{j=1}^N w^j \hat{y}^j_t 
%    + y^\top_t y_t + \sum_{j=1}^N \kappa_j w^{j 2} \notag \\ 
%  = &  w^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) w 
%   - 2  y^\top_t  \hat{\mathbf{Y}}_t w 
%    + y^\top_t y_t . \notag 
% \end{align} 
% Therefore the nonlinear programming problem \eqref{MajorPlayer:NLoptim} is equivalent to the following quadratic programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N)^\top } \frac{1}{2}  w^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t     + \mathrm{K} \big) w 
%   -  y^\top_t  \hat{\mathbf{Y}}_t w , \\ 
% & \text{subject to} \ G w \leq \mathbf{c} ,
% \end{aligned} 
% \label{MajorPlayer:QP}
% \end{equation} 
% where $G$ and $\boldsymbol{c}$ are defined in~\eqref{eq:Gc_Def}.



% To prove Theorem~\ref{thm:OptimalWeights}, we need to use the results of the following Theorems~\ref{thm:NSQP} and \ref{thm:QPdual} from \cite{Berkovitz2001}. 
% According to \cite[Theorem V.6.1]{Berkovitz2001}, the following theorem gives a necessary and sufficient condition for solutions of \eqref{MajorPlayer:QP}. 
% \begin{theorem} 
% \label{thm:NSQP}
% A necessary and sufficient condition for a point $w^\star=(w^{1, \star}, ..., w^{N, \star})^\top$ to be a solution of the quadratic programming problem \eqref{MajorPlayer:QP} is that 
% \begin{align} 
% G w^\star \leq \mathbf{c} \label{NSQP:Gw<=c} 
% \end{align} 
% and there exists a vector $\boldsymbol{\lambda} \geq 0$ in $\mathbb{R}^{2N+2}$ such that 
% \begin{align} 
%  & \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  w^\star - \hat{\mathbf{Y}}_t^\top y_t 
%   + G^\top \boldsymbol{\lambda} = 0 , \label{NSQP:w+lambda} \\ 
%  & \boldsymbol{\lambda}^\top (G w^\star - \mathbf{c}) = 0 . \label{NSQP:wlambda}  
% \end{align} 
% \end{theorem}

% Introduce the dual quadratic programming problem: 
% \begin{equation} 
% \begin{aligned}  
% & \max \big\{ \theta (\boldsymbol{\lambda}) : \ \boldsymbol{\lambda} \geq 0 , \ \theta(\boldsymbol{\lambda}) > -\infty \big\} , 
%  \\ 
% & \theta(\boldsymbol{\lambda}) = \inf \{ L( \mathbf{x}, \boldsymbol{\lambda}) : \ \mathbf{x} \in \mathbb{R}^N \} ,  \\ 
% & L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}  
%   -  y^\top_t  \hat{\mathbf{Y}}_t \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) .   
% \end{aligned} 
% \label{MajorPlayer:DQP} 
% \end{equation} 

% By \cite[Theorem V.6.2]{Berkovitz2001}, we have the following relation between the quadratic programming problem \eqref{MajorPlayer:QP} and the dual problem \eqref{MajorPlayer:DQP}. 
% \begin{theorem} 
% \label{thm:QPdual}
% Let the quadratic programming problem \eqref{MajorPlayer:QP} has a solution $w^\star=(w^{1, \star}, ..., w^{N, \star})$. Then the dual problem \eqref{MajorPlayer:DQP} has a solution $\boldsymbol{\lambda}_\star$, and the solution $\boldsymbol{\lambda}_\star$ is exactly the multiplier $\boldsymbol{\lambda}$ in Theorem~\ref{thm:NSQP} corresponding to $w^\star$. 
% \end{theorem} 

% With Theorems~\ref{thm:NSQP} and \ref{thm:QPdual}, we are ready to prove Theorem~\ref{thm:OptimalWeights}. 

% \begin{proof}[Proof of Theorem~\ref{thm:OptimalWeights}]  

% By Theorem~\ref{thm:NSQP}, we can determine the optimal weights $w^\star=(w^{1,\star}, ..., w^{N,\star})$ from 
% \eqref{NSQP:w+lambda}. The multiplier $\boldsymbol{\lambda}$ in \eqref{NSQP:w+lambda} is the solution of the dual problem \ref{MajorPlayer:DQP}. 

% We first solve the dual problem \eqref{MajorPlayer:DQP} for the optimal $\boldsymbol{\lambda}$. 
% The function $L(\mathbf{x}, \boldsymbol{\lambda})$ in \eqref{MajorPlayer:DQP} can be rewritten as  
% \begin{align} 
%  L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = & \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  \mathbf{x}  
%   -  y^\top_t \hat{\mathbf{Y}}_t \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) \notag \\ 
%    = &  \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}  
%   - \Big[ y^\top_t  \hat{\mathbf{Y}}_t - \boldsymbol{\lambda}^\top G \Big] \mathbf{x} 
%    - \boldsymbol{\lambda}^\top \mathbf{c} . 
%    \label{L(x,lambda)2}   
% \end{align} 
% For each $\boldsymbol{\lambda}$ fixed, the function $L(\cdot, \boldsymbol{\lambda})$ given by \eqref{L(x,lambda)2} is a convex function on $\mathbb{R}^N$. Then $\mathbf{x}_{\boldsymbol{\lambda}}$ is a minimizer of $L(\cdot, \boldsymbol{\lambda})$ if and only if $\nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda}) = 0$. 
% It then follows from \eqref{L(x,lambda)2} that 
% \begin{align} 
%  0 = & \nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda})  \notag \\ 
%  = & \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \Big[  \hat{\mathbf{Y}}^\top_t y_t - G^\top \boldsymbol{\lambda}  \Big] , 
%  \notag 
% \end{align} 
% which further gives that 
% \begin{align} 
% 0 = &   \mathbf{x}_{\boldsymbol{\lambda}}^\top \big(   N\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t 
%  + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \mathbf{x}_{\boldsymbol{\lambda}}^\top \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] .  
%   \label{0=<x,gradL>}  
% \end{align} 
% Substituting \eqref{0=<x,gradL>} into \eqref{MajorPlayer:DQP}, we obtain an explicit form of $\theta(\boldsymbol{\lambda})$
% \begin{align} 
%  \theta(\boldsymbol{\lambda}) = & L(\mathbf{x}_{\boldsymbol{\lambda}}, \boldsymbol{\lambda}) \notag \\ 
%  =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%   \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)  
%   \mathbf{x}_{\boldsymbol{\lambda}}   
%   - \Big[  y^\top_t \hat{\mathbf{Y}}_t - \boldsymbol{\lambda}^\top G \Big] 
%    \mathbf{x}_{\boldsymbol{\lambda}}  
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top\big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t  + \mathrm{K} \big) 
%     \mathbf{x}_{\boldsymbol{\lambda}}   
%   -  \mathbf{x}_{\boldsymbol{\lambda}}^\top \big( N\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t 
%    + \mathrm{K} \big)    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =&  - \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%    \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} . \notag 
% \end{align}  

% With the above explicit form of $\theta(\boldsymbol{\lambda})$, the dual quadratic programming problem \eqref{MajorPlayer:DQP} is then equivalent to 
% \begin{equation} 
% \begin{aligned} 
% & \max_{\mathbf{x}, \ \boldsymbol{\lambda}} \ 
% - \frac{1}{2}  \mathbf{x}^\top \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} ,   \\ 
% & \text{subject to:} \ 
%  \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big) \mathbf{x} 
%   - \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] = 0 .  
% \end{aligned} 
% \label{MajorPlayer:DQPequiv} 
% \end{equation} 
% Since $N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K}$ is positive definite, the equality constraint in \eqref{MajorPlayer:DQPequiv} 
% implies that 
% \begin{align} 
%    \mathbf{x} 
% =  \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)^{-1} \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] . 
% \label{xsublambda}
% \end{align} 
% With \eqref{xsublambda} substituted into \eqref{MajorPlayer:DQPequiv}, 
% the dual problem \eqref{MajorPlayer:DQPequiv} is then equivalent to the following unconstrained optimization problem: 
% \begin{align} 
%  \max_{\boldsymbol{\lambda}} \ -\frac{1}{2}  \Big[  \hat{\mathbf{Y}}^\top_t 
%    y_t - G^\top \boldsymbol{\lambda}  \Big]^\top 
%    \big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \big)^{-1} 
%  \Big[  \hat{\mathbf{Y}}^\top_t  y_t  - G^\top \boldsymbol{\lambda}  \Big] 
%  - \boldsymbol{\lambda}^\top \mathbf{c} . 
% \label{MajorPlayer:DQPunconstrained} 
% \end{align} 
% We solve the unconstrained optimization problem \eqref{MajorPlayer:DQPunconstrained} for a $\boldsymbol{\lambda}_\star$:  
% \begin{align} 
%  \boldsymbol{\lambda}_\star = \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t 
%  y_t  -  \mathbf{c} \Big] . 
%  \label{lambdasubstar} 
% \end{align} 
% Then we substitute $\boldsymbol{\lambda}_\star$ into \eqref{NSQP:w+lambda} to solve for the optimal weight vector $w^\star=(w^{1,\star}, ..., w^{N,\star})^\top$: 
% \begin{align} 
%    w^\star = &  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K}  \Big)^{-1} \Big[ \hat{\mathbf{Y}}_t^\top  y_t 
%   - G^\top \boldsymbol{\lambda}_\star \Big]  \notag  \\ 
%   = &  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
%   \notag \\    
%   & -  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}   G^\top 
%   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t 
%   y_t -  \mathbf{c} \Big] , 
%   \notag  
% \end{align} 
% which is \eqref{eqn:OptimalWeights}.  
% \end{proof} 










% % \bibliographystyle{spmpsci}      % mathematics and physical sciences
% %\bibliographystyle{spphys}       % APS-like style for physics
% \bibliographystyle{plain} %plain
% \bibliography{Refs}   % name your BibTeX data base

% %\bibliographystyle{spmpsci}  
% %\bibliography{HYmfsocRef}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \end{document} 

==> Historical_Versions/2025_03_01.tex <==
% % david.emerson@vectorinstitute.ai
% % fatemeh.tavakoli@vectorinstitute.ai


% \documentclass[twoside,11pt]{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2023


% % ready for submission
% % \usepackage{neurips_2024}
% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %\usepackage[preprint]{neurips_2024} 

% \usepackage{jmlr2e}
% \usepackage{blindtext}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2023}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2023}


% %\usepackage[utf8]{inputenc} % allow utf-8 input
% %\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% %\usepackage{hyperref}       % hyperlinks
% %\usepackage{url}            % simple URL typesetting
% %\usepackage{booktabs}       % professional-quality tables
% %\usepackage{amsfonts}       % blackboard math symbols
% %\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% %\usepackage{microtype}      % microtypography
% %\usepackage{xcolor}         % colors

% % \usepackage[top=0.9in,bottom=1.1in,left=1.05in,right=1.05in]{geometry}

% %

% %\theoremstyle{remark}
% %\usepackage{amsmath}
% %\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% %\usepackage{microtype}      % microtypography
% %\usepackage{minted}
% %\usemintedstyle{dracula}
% %\newtheorem{remark}{Remark}[section]
% %\newtheorem{example}{Example}[section]
% %\newtheorem{corollary}{Corollary}[section]


% %\usepackage{booktabs} 
% %\usepackage{multirow} 
% %\usepackage{graphicx}
% %\usepackage{subcaption}
% %\usepackage{comment}

% \input{packages}
% \input{mathcommands}
% \input{Commenting}













% % Heading arguments are {volume}{year}{pages}{date submitted}{date published}{paper id}{author-full-names}

% \usepackage{lastpage}
% \jmlrheading{23}{2022}{1-\pageref{LastPage}}{1/21; Revised 5/22}{9/22}{21-0000}{Xuwei Yang, Fatemeh Tavakoli, Anastasis Kratsios, and David Emerson}

% % Short headings should be running head and authors last names

% \ShortHeadings{Online Federation For Mixtures of Proprietary Agents with Black-Box Access}{Xuwei Yang, Fatemeh Tavakoli, Anastasis Kratsios, and David Emerson}
% \firstpageno{1}

% \begin{document} 

% \title{Online Federation For Mixtures of Proprietary Agents\\ with Black-Box Access}



% \author{\name Xuwei Yang 
%   \email yangx212@mcmaster.ca \\
% \addr Department of Mathematics\\
%   McMaster University\\
%   Ontario, Canada 
%   \AND
%    \name
%    Fatemeh Tavakoli
%    \email 
% fatemeh.tavakoli@vectorinstitute.ai
%    \\
% \addr Vector Institute\\
%     Ontario, Canada 
%   \AND
%   Anastasis Kratsios\thanks{Corresponding Author. 
%   Funded by NSERC DG No.\ RGPIN-2023-04482.} 
%   \email 
%   kratsioa@mcmaster.ca
%   \\
%  \addr  Department of Mathematics\\
%   McMaster University and the Vector Institute\\
%   Ontario, Canada 
%   \AND
%   \name David Emerson 
%   \email 
% david.emerson@vectorinstitute.ai \\ 
% \addr  Vector Institute\\
%     Ontario, Canada 
% }

% \editor{}

% \maketitle

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract} 
% %% Static Problem and setting
% \add{Most industry-standard generative models are \textit{proprietary} (black-box access), meaning that while their predictions are available, their internal structure and parameters remain private.  Since modern AI pipelines typically use mixtures of such deep learning models, the black-box nature makes classical optimization algorithms problematic, as users cannot access internal parameter updates or (partial) gradients.
% %%% What we do
% To address this gap, we propose a federated optimization algorithm for mixtures of \textit{proprietary} sequential generative models, wherein the user can access all input-output pairs of each model generated online, but they do not know the internal structure of the model.
% %%% How We Solve/why goodio
% Viewing this \textit{proprietary federated learning} problem through a game-theoretic lens, we employ optimal control techniques to derive closed-form expressions for the Nash-optimal online updates of each proprietary model, treated as an agent, and for the optimal mixture coordinated by the server, acting as a central planner.   These closed-form updates yield a highly computationally efficient algorithm. We further derive simplified closed-form expressions for mixtures of Echo-State Networks (agents), random feature models, and pre-trained transformers.  
% %%% It works in practice
% Each case is evaluated experimentally on diverse time-series prediction tasks with qualitatively different properties, ranging from economic datasets to concept drift scenarios. Our algorithm achieves predictive accuracy orders of magnitude better than the benchmarks.}
% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%% Section 1: Instruction %%%%%%
% %\section{Introduction}
% %\label{chp:intro}

% %Input data $x=(x_1, ..., x_d)\in \mathbb{R}^d$. 
% % \begin{comment}

% \section{Introduction} 
% \label{s:Intro}

% % What is Propreitary setting and why its important
% \add{%
% The modern era of mainstream deep learning has witnessed the emergence of several proprietary models with public black-box access, meaning users can observe the inputs and predictions produced by these models, but the underlying structure and parameters remain unknown. For example, most proprietary LLMs, such as~\cite{chatgpt} and~\cite{guo2024deepseek}, offer this type of \textit{black-box access}. Similarly, different teams within a single organization, such as separate trading desks in a bank, may release AI-driven predictions while keeping the details of their models confidential for security reasons.
% In each case, the user is confronted with the following question: \textit{How can a single user synchronize an ensemble of agents, each using their own proprietary model, to optimally predict a single task while utilizing all available non-proprietary information?}
% }

% % Why FL, but why not classical FL
% \add{Our problem naturally lends itself to a \textit{federated learning} (FL) approach, where a single computational task is distributed among a large number of agents. Each agent computes locally and shares its prediction with others, while the user (or central server) synchronizes these agents to maximize predictive success.
% Unfortunately, FL with black-box access does not fall into the standard FL toolbox. This is because standard FL \textit{does} seek to construct a single prediction on the central several by aggregating the predictions made by an ensemble of decentralized agents, each deploying their own model. However, how this aggregation is performed is at odds with our proprietary requirement on each agent's model.
% This is because traditional federated learning setups, e.g.~\cite{Even22SampleOptimalityFL,Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}, work by (partially) averaging local model parameters on the central server or their (partial) gradients, meaning that full (white-box) or partial (grey-box) model access is available to the user.}

% % What each person is allowed to do
% \add{
% We focus on the online setting, where all agents are dynamically predicting an evolving time-series while continuously receiving a single (possibly high-dimensional) time-series as input, along with the (non-proprietary) predictions of every other agent and the aggregation weights used by the central server to mix each proprietary agent's predictions.  
% Importantly, the central server dynamically updates the mixture weights to maximize overall performance, promoting \textit{cooperation} among the agents. Simultaneously, since each agent lacks access to the internal structure or mechanism by which other agents optimize their parameters, they naturally compete to maximize the influence of their predictions within the mixture created by the central server.
% }

% %%%
% \add{
% In this way, our federated learning framework with proprietary black-box agents can naturally be approached using a game-theoretic lens. From this perspective, each agent competes to have its prediction dominate the mixture, leading to a Nash equilibrium as the optimal strategy. Simultaneously, the central server’s problem is best understood through a control-theoretic lens, where the goal is to dynamically update the aggregation weights to optimize the ensemble’s online prediction of the evolving time-series that the agents are collectively forecasting.
% }

% \add{
% This paper develops the \textit{kernelized} setting, where after an initial full training phase—during which each agent fully optimizes its model using an initial segment of training data—the agents are then restricted to dynamically updating only their final learned layer. Each agent’s utility function is quantified by its running mean squared error (MSE) based on how well the ensemble predicts the target time-series, penalized by a term that discourages irregular "bang-bang" strategies, which involve rapid switches between states or decisions.
% }
% % The approach involves training local models on the agents and periodically exchanging model parameters, rather than data, to construct a global model shared across all agents. 






% \paragraph{Contributions}

% In this paper, we propose a game-theoretic approach to federated learning that integrates proprietary black-box agents while preserving privacy and optimizing ensemble prediction accuracy. Our framework introduces periodic synchronization, where agents independently make predictions and share them with a central server, which optimally aggregates their outputs. This interaction is modeled as a Nash game, balancing individual privacy with collective accuracy. 
% We will focus on the following three classes of examples.  
% (1) The first is a pre-trained deep learning model that allows for dynamically fine-tuning the final linear decoder layer.  (2) The next example is a particular instance of a \textit{generative} extreme learning machine; a random feature network with continually regenerated random biases. Finally, (3) we consider recurrent models such as \textit{reservoir computers} where one can regenerate a small source of randomness at each time increment, allowing for generative modelling. 
% By leveraging proprietary models, our approach reduces the central server’s computational burden and enhances predictive performance on evolving time-series data. Numerical experiments demonstrate that our method outperforms traditional FL techniques that do not incorporate game-theoretic optimization.


% \begin{comment} 
% In this paper, we introduce a game-theoretic approach to FL that incorporates proprietary black-box agents, each of which periodically synchronizes at fixed time intervals. 
% Between synchronization rounds, each agent independently makes predictions based on its local data and transmits them to a central server. 
% During synchronization, agents utilize these optimized weights to make non-cooperative predictions, while also gaining access to the predictions of other agents. This structured interaction among agents is modelled using a Nash game, providing a mechanism to balance the privacy of individual agents and the accuracy of the ensemble model. %and computational efficiency. 
% By utilizing the proprietary models of individual agents, our game-theoretic synchronization scheme alleviates the computational workload on the central server and improves prediction accuracy of the ensemble.
% Our framework ensures efficient cooperation between proprietary agents while maintaining optimal predictive performance over evolving time series data.
% Through numerical experiments, we demonstrate that our method outperforms conventional FL approaches that do not leverage game-theoretic strategies. To the best of our knowledge, this is the first study to apply the game theory to improve the ensemble prediction accuracy by leveraging the computational power of proprietary agents.
% \end{comment}

% \begin{comment} 
% In this paper, we introduce a game-theoretic approach to FL that incorporates multiple generative experts, each of which periodically synchronizes. Our FL framework operates through synchronization rounds occurring at fixed time intervals. Between synchronization rounds, each agent independently makes predictions based on its local data and transmits them to a central server. The server then computes optimal weights for these individual predictions to minimize the overall ensemble prediction error. During synchronization, agents utilize these optimized weights to make non-cooperative predictions, while also gaining access to the predictions of other agents. This structured interaction among agents is modeled using Nash game theory, providing a mechanism to balance accuracy and computational efficiency. 
% By distributing the learning task across clients, our game-theoretic synchronization scheme alleviates the computational workload on the central server.  
% Through numerical experiments, we demonstrate that our method outperforms conventional FL approaches that do not leverage game-theoretic strategies. To the best of our knowledge, this is the first study to apply the game theory to improve the ensemble prediction accuracy by leveraging the computational power of local agents.
% \end{comment} 
% \AK{I moved this here, please intergrate naturally into contributions \textit{with} links to corollaries}

% We will focus on the following three classes of examples.  
% (1) The first is a pre-trained deep learning model that allows for dynamically fine-tuning the final linear decoder layer.  (2) The next example is a particular instance of a \textit{generative} extreme learning machine; a random feature network with continually regenerated random biases. Finally, (3) we consider recurrent models such as \textit{reservoir computers} where one can regenerate a small source of randomness at each time increment, allowing for generative modelling. 


% \paragraph{Organization of the Paper}
% The paper is organized as follows. 
% In Section~\ref{s:Setup}, we introduce the generative sequential learning models and the federated learning scheme. 
% In Section~\ref{s:Examples}, we examine various FL agents and demonstrate through numerical experiments the advantage of our game-theoretic FL approach.  


% \subsection{Related Work}
% \label{s:Introduction__ss:RelatedWork}

% \AK{Compress to like 2 paragraphs tops}
% %Though this decentralization reduces the computational burden placed on a single machine, 
% %Federated learning (FL) is a decentralized machine learning paradigm that enables multiple clients to collaboratively train models while preserving data privacy. 
% Traditional federated learning methods, such as FedAvg~\cite{mcmahan2017FedAvg}, 
% aggregate locally-optimized parameters or gradient updates on a central server, which periodically synchronizes local models~\cite{Even22SampleOptimalityFL}. 
% %Standard FL schemes rely on idealized assumptions such as homogeneous clients, identically and independently distributed (i.i.d.) datasets, and synchronized updates from clients.  
% %These methods rely on the assumptions that individual agents have i.i.d. datasets, similar system capacities, and uniform data accessibility. 
% These methods reply on idealized assumptions such as homogeneous clients, identically and independently distributed (i.i.d.) datasets, and synchronized updates from clients. 
% However, these stylized assumptions tend not to match real-world use
% cases, wherein agents face heterogeneous data distributions, different system
% capacities, and de-synchronized updates 
% \cite{Kairouz21AdvancesFL, Li20FLfuture}.  
% %\cite{kairouz2021advances, li2020federated}. 
% %The heterogeneity and de-synchronization leads to biased global models and lower accuracy of prediction. 
% %It immediately introduces several challenges due to competing heterogeneities between the individual agents' objectives, resulting in a de-synchronization of the system's overall objective. 
% %To address these challenges, asynchronous FL techniques allow clients to update the global model independently based on their availability~\cite{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}. 
% %This is typically resolved by periodically synchronizing agents~\cite{Even22SampleOptimalityFL}, with the idea being that the agent's optimal policies are in a game-theoretic equilibrium.  
% %Although there are several general FL guarantees, showing that various types of policies are eventually in equilibrium~\cite{EqmOptmCollaborationFL}. 
% %This paper focuses precisely allowing the training of machine learning models across multiple local datasets residing on individual agents without sharing raw data \cite{FL:ConceptApplications}. 


% % One major issue in FL is the weights that aggregating agents’ updates (predictions). 
% Due to heterogeneity between agents, the uniform weights of the clients to update the global model \cite{mcmahan2017FedAvg} leads to biased global models and lower accuracy of prediction~\cite{Zhao22nonIID}. 
% %To address heterogeneity, 
% %change the weights of aggregation.
% FedProx \cite{FedOptimHeteroNet} incorporates regularization to stabilize updates across heterogeneous clients, while Scaffold \cite{Karimireddy20Scaffold} employs variance reduction to mitigate client drift caused by sampling heterogeneity.
% Another challenge in FL is desynchronization of updates from agents due to varying computational speeds and capacity of agents. 
% Asynchronous FL methods address this by allowing each agent to update the global model independently as soon as it completes its local computation~\cite{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}. 
% %The lens through which we will examine asynchronous FL pipelines is that of optimization through a game-theoretic perspective, though several other important lenses are natural when studying different, e.g. statistical or XXX, aspects which we will not consider here. 



% %Traditional federated learning (FL) methods, such as FedAvg~\cite{mcmahan2017FedAvg}, aggregate locally-optimized parameters or gradient updates on a central server, which periodically synchronizes the local models~\cite{SampleOptimalityFL}. These approaches crucially assume that individual agents have i.i.d.\ datasets, similar system capacities, and uniform data accessibility. However, these stylized assumptions tend not to match real-world use cases, wherein agents face heterogeneity via their individual data distributions and system capacities, among other differences. Asynchronous FL methods, e.g.~\cite{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}, address this heterogeneity by allowing each agent to update the global model independently as soon as it completes its local computation.  
% %The lens through which we will examine asynchronous FL pipelines is that of \textit{optimization} through a \textit{game theoretic} perspective, though several other important lenses are natural when studying different, e.g.\ statistical or XXX, aspects which we will not consider here. 
% %Another issue in FL is the weights that aggregating agents' updates (predictions). 
% %Due to heterogeneity between agents, the weights of the clients to update the global model are not uniform as~\cite{mcmahan2017FedAvg} which assume that all clients are homogeneous. \cite{Karimireddy20Scaffold} to reduce the affects of sampling heterogeneity of clients. 
% %For FL with non-i.i.d. data, \cite{Zhao22}



% \paragraph{Game Theoretic Approaches to Machine Learning}

% % \AK{Populate}
% %Federated learning can be naturally cast as a multi-agent system, where participants may act collaboratively or non-cooperatively depending on constraints such as communication costs, computational resources, and privacy considerations. Game theory provides a framework for analyzing these strategic interactions and optimizing model aggregation, synchronization frequency, and client participation incentives. 
% Recent works have begun incorporating game-theoretic perspectives into FL, modelling interactions among clients and the central server as multi-agent strategic games. %These approaches enable incentive-aware optimization, but they often focus on static formulations rather than dynamic adaptation.
% While in some FL settings, agents update their local models collaboratively~\cite{CollaboraionFL:Game}, in other stances, factors such as communication costs and privacy constraints lead agents to update the model in a non-cooperative manner. 
% %In this context, we can leverage a game-theoretic approach to FL.   
% %The game-theoretic approach can be applied to various aspects of FL. Agents collaborate by sharing datasets for collective learning, with the goal of minimizing the total sample size while ensuring that each agent meets the lower bound of individual error. 
% %\cite{Blum21EqmOptmFL} introduces the notions of stable equilibrium and envy-free equilibrium. 
% %In hedonic games agents choose to join different federating groups to achieve better performance~\cite{CollaborationEqmFL},
% %\cite{OptimalityStabilityFL:Game}, \cite{HedonicGamesShareData25}. 
% %\cite{Murhekar:23} finds an optimal trade-off between FL learning payoff and data sharing cost. 
% %\cite{Xie24mixed} game between the central server and adversarial clients, in which the adversary aims to attack the training % while the server aims to achieve low overall training error. 
% %Several works have formalized equilibrium concepts in FL. 
% \cite{Blum21EqmOptmFL} introduce the notions of stable equilibrium and envy-free equilibrium to ensure fairness in FL model aggregation. In hedonic games, agents self-organize into federated coalitions to optimize their predictive performance \cite{CollaborationEqmFL, OptimalityStabilityFL:Game, HedonicGamesShareData25}. Other works investigate the trade-offs between FL learning performance and data-sharing costs \cite{Murhekar:23}, ensuring that clients benefit from collaboration without incurring excessive privacy risks.
% In robust FL against adversarial threats, \cite{Xie24mixed} model FL as a mixed-strategy game between a central server and adversarial clients, where the server aims to optimize model accuracy, while the adversary strategically perturbs updates to degrade performance.


% \subsection{Sequential Deep Learning - Causality/Adaptedness Constraints}
% \AK{I add}
% %In FL schemes, clients focus on individual objectives 


% \subsection{Notation and Conventions}
% \add{
% Throughout this manuscript, we use the following notation, which we collect here for simple accessibility. 
% We denote $\mathbb{N} \eqdef \{0, 2, \cdots \}$ and $\mathbb{N}_+\eqdef \{x\in \mathbb{N}:\, x>0\}$.  For any $N\in \mathbb{N}_+$, the \textit{simplex} $\Delta_N$ is the set of $w\in \mathbb{R}^N$ satisfying the following positivity and normalization constraints
% \begin{align}
% \label{eq:NSimplexDef}
%     \underbrace{
%         % \sum_{n=1}^N\, w_n  
%         w^1_\cdot + \dots + w^N_\cdot 
%         = 1
%     }_{\term{c1:netting}}
% \mbox{ and }
%     \underbrace{
%         w^1_\cdot , w^2_\cdot ,\dots,w^N_\cdot   \ge 0 
%     }_{\term{c2:leveraging}}
% .
% \end{align}
% We henceforth fix a latent complete probability space $(\Omega,\mathcal{F},\mathbb{P})$.  For any $d,D\in \mathbb{N}_+$ and $1\le p<\infty$, use $L^p(\mathbb{R}^d)$ (resp.\ $L^p(\mathbb{R}^{d\times D})$) to denote the space of $\mathbb{R}^d$ (resp.\ $\mathbb{R}^{d\times D})$) valued random variables $X$ whose expected $p^{th}$ power of their Euclidean $\|\cdot\|_2$ (resp.\ Frobenius $\|\cdot\|_F$) norm is finite $\mathbb{E}[\|X\|^p_2]<\infty$ (resp.\ $\mathbb{E}[\|X\|_F^p]<\infty$), where the expectation is taken with respect to $\mathbb{P}$.
% \paragraph{Row and Column Vectors and Matrices}
% We will nearly always specify if a vector is a row or column vector and its dimensions.  However, when clear from the context, we at times identify the space of row vectors $\mathbb{R}^{d\times 1}\cong \mathbb{R}^d$ and the space of column vectors $\mathbb{R}^{1\times d}\cong \mathbb{R}^d$ (for the relevant $d\in \mathbb{N}_+$) to keep notation light.  For each $d\in \mathbb{N}_+$, $I_d$ the $d \times d$-identity matrix.  Moreover, $\mathbf{1}_d\in \mathbb{R}^d$ has all its entries equal to $1$.} 


% \section{The Online Proprietary Federated Setting}
% \label{s:Setup}

% \paragraph{The Agents - Online Sequential Learners}
% % \label{s:Setup__ss:EnsembleModel}
% \add{We consider $N\in \mathbb{N}_+$ generative \textit{proprietary} sequential learners $f^{(1)},\dots,f^{(N)}$} with at most three inputs at any time $t\in \mathbb{N}$.  For each such $t\in \mathbb{N}_+$, the $i^{th}$ expert model takes the (common) historical input sequence $x_{[0:t]}\in \mathbb{R}^{(1+t)\,d_x \times 1}$, an individual source of randomness $\epsilon_t^i$ which is an integrable $d_{\epsilon}\times 1$-valued random variable, and an individual hidden state $Z_t^i\in \mathbb{R}^{d_z\times 1}$\add{; where $d_x,d_z,d_{\epsilon}\in \mathbb{N}_+$}.  
% These three inputs are used to generate the latent state $Z_{t+1}$ using a \textit{static} \textbf{encoder} $\varphi^{(i)}:\mathbb{R}^{d_x\times 1}\times \mathbb{R}^{d_z\times 1}\times \mathbb{R}^{d_{\epsilon}\times 1}\to \mathbb{R}^{d_y 
% \times d_z}$ via
% \begin{equation}
% \label{eq:latent_state}
%     Z_{t}^i 
% \eqdef 
%     \underbrace{
%         \varphi^{(i)}\big(x_{[0:t]}
%         % ^i
%         ,Z_{t-1}^i,\epsilon_t^i\big)
%     }_{\text{(Deep) Feature Encoder}}
% .
% \end{equation}
% The (deep) feature encoder is either pre-trained or trained on an initial segment of time-series data, formally regarded as before the time when prediction begins to roll out online; i.e.\ $t=0$ and any negative times are considered part of an offline pre-training phase not considered here.  Thus, one and after time $t>0$, the feature encoder is no longer updated in this paper, and the (deep) learning model effectively becomes a kernel model.  We require that $Z_t^{(i)}\in L^1(\mathbb{R}^{d_y\times d_z})$ for each $t\in \mathbb{N}$.


% Once the latent state is generated, it is used to update the \textit{residual} of the prediction generated at the previous time $t$ via a \textit{dynamically updating} linear \textbf{decoder}
% %\begin{equation}
% %\label{eq:residual_update}
% % \hat{Y}^i_{t+1} = 
% % \hat{Y}^i_t + \beta^{i\top}_t Z^i_t 
% %\end{equation} 
% \begin{equation} 
% \label{eq:residual_update}
%     \underbrace{
%         \hat{Y}^i_{t+1}
%     }_{\text{Prediction}}
% = 
%         \underbrace{
%             \hat{Y}^i_t 
%         }_{\text{Historical State (Memory)}}
%     +  
%     \underbrace{
%         \overbrace{Z^i_t 
%         }^{\text{feature}}
%         % \overbrace{
%             \colorwblk{\beta^{i}_t}
%         ,
%         % }^{\text{linear}}
%     }_{\text{Residual (Update)}}
% \end{equation} 
% where $\hat{Y}_t^i \in \mathbb{R}^{d_y \times 1}$, $Z_t^i\in \mathbb{R}^{d_y \times d_z}$, and $\beta_t^i \in \mathbb{R}^{d_z \times 1}$; where $d_y\in \mathbb{N}_+$.  Both initial states $\hat{Y}_0^i\in \mathbb{R}^{d_y\times 1}$ and $Z_0^i\in \mathbb{R}^{d_y \times d_z}$ are fixed a priori.  

% Following the theoretical reservoir computing literature, e.g.~\cite{grigoryeva2018echo}, each generative sequential is a \textit{causal} deep learning agent defined by
% \begin{equation}
% \label{eq:agents_predictions}
% \begin{aligned}
%     f^{(i)}: (\mathbb{R}^{d_{x}})^{\mathbb{N}}&\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{N}}\\
%     (x_t)_{t=0}^{\infty} & \mapsto \big(\hat{Y}^i_t\big)_{t=0}^{\infty}
% \end{aligned}
% \end{equation}
% where, for each $t\in \mathbb{N}$ each $\hat{Y}^{i}_t$ is computed recursively using the sequentially by first encoding the input path $x_{[0:t]}$ via~\eqref{eq:latent_state} and then predicting the residual via~\eqref{eq:residual_update}.  By \textit{causality}, we mean that for each time $t\ge 0$, the prediction $\hat{Y}_t^i$ only depends on the input sequence as \textit{observed thus far}, i.e.\ on $x_{[0:t]}$, and not on any of its future realizations, i.e.\ not on $x_s$ for any $s>t$.
  

% For example, in echo-state networks (ESNs)~\cite{jaeger2001echo,maass2002real} or extreme learning machines such as random feature networks (RFNs)~\cite{huang2006universal,rahimi2008weighted}, the deep features in~\eqref{eq:latent_state} are randomly initialized and left untrained and residual updates $(\beta_t)_{t=0}^{\infty}$ in~\eqref{eq:residual_update} are trained before the online-time $t=0$ and then fixed (thus are constant) for all times $t\ge 0$.  In pre-trained models, such as transformers~\cite{vaswani2017attention}, the deep features are pre-trained on an offline dataset, i.e.\ before time $t=0$, and the residual decoding/readout layer~\eqref{eq:residual_update} is also typically left fixed.


% \paragraph{The Server - Adaptive Mixture of Experts/Agents}
% % \label{s:Setup__ss:Federated}
% We assume that $N>1$ with the case that $N=1$ is trivial since $w_1=1$.
% The objective of the server is to adaptively \textit{synchronize} these $N$ generative models, into a single generative ensemble model $\hat{F}:(\mathbb{R}^{d_{x}})^{\mathbb{N}}\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{N}}$ to maximize their performance.  The resulting ensemble is represented for each $x\in (\mathbb{R}^{d_x})^{\mathbb{N}}$ at every time $t\in \mathbb{N}$ by
% \begin{equation}
% \label{eq:enbsemble_server__predictions}
% \hat{F}(x)_t \eqdef 
% \overbrace{
% \sum_{i=1}^N\, 
%     \colorwblk{w_t^i}\, 
%     \underbrace{
%         \hat{f}^i\big(x_{[0:t]}\big)_t
%     }_{i^{th} \text{Agent (Expert)}}
% }^{\text{Mixture of Experts}}
% \end{equation}
% where each \textit{mixture coefficients} $w_t$ belonging to the $N$-simplex $\Delta_N$.  
% Observe that, by construction, the server's mixture prediction is also \textit{causal}; that is, $\hat{F}(x)_t$ only depends on $x_{[0:t]}$ and not $x_s$ for any $s>t$.

% \paragraph{The Proprietary Constraint}
% \add{
% Each \textit{agent} can dynamically update, or \textit{control}, its sequence of linear residual update parameters $(\beta_t)_{t=0}^{\infty}$ in~\eqref{eq:residual_update}, while the central \textit{server} dynamically updates its own parameters in~\eqref{eq:enbsemble_server__predictions}. In standard federated or online optimization problems, there are no restrictions on how agents and the server update their trainable parameters, apart from the requirement that updates be causal—that is, they must not depend on inaccessible future information.  
% \hfill\\
% However, the \textit{proprietary} nature of each model introduces an additional layer of structure-based complexity. Specifically, neither the server nor any agent has access to the internal structure of any other model, including its architecture, parameter values, or (partial) gradient information. Together, the \textit{causality} and \textit{proprietary} constraints imply that: 
% at every time $t\in \mathbb{N}_+$ the $i^{th}$ \textit{agent/client-side} parameter updates $\beta_t^{(i)}$ in~\eqref{eq:residual_update} are of the form
% \begin{equation}
% \label{eq:PROPRIETARY_CONSTRAINT__Agent}
%     \beta_t^{(i)} = b_t\Big(
%             % \overbrace{
%                 (Y_{[0:t]}^{(j)})_{j=1}^N
%             % }^{\text{Expert Predictions}}
%         ,
%                 y_{[0:t]}
%         ,
%             % \underbrace{
%                 x_{[0:t]}
%             % }_{\text{Input series}}
%         ,
%             % \overbrace{
%             w_{[0:t+1]}
%             % }^{\text{Server Weights}}
%         ,
%             % \underbrace{
%                 \beta_{[0:t]}^{(i)}
%             % }_{\text{Own } i^{th} \text{ Parameters}}
%     \Big)
% \end{equation}
% for each $t\in \mathbb{N}_+$, where $b_t:\mathbb{R}^{d_y(1+t)\times (N-1)}\times \mathbb{R}^{d_y(1+t)}\times \mathbb{R}^{d_x(1+t)}\times \mathbb{R}^{N(1+t)} \times \mathbb{R}^{d_z(1+t)}\to \mathbb{R}^{d_z\times 1}$ is a continuous function that may depend on the current time $t$ and various observed quantities, including all expert predictions $Y^{(1)}_{[0:t]}, \dots, Y_{[0:t]}^{(N)}$, the server weights $w_{[0:t]}$, and the input data $x_{[0:t]}$.  We highlight that the $i^{th}$ agent’s parameter updates $\beta_{[0:t]}^{(i)}$ are known to themselves and can therefore be incorporated into their own decisions%
% \footnote{The expression~\eqref{eq:PROPRIETARY_CONSTRAINT__Agent} could be extended to include the agent's internal parameters if the hidden layers were trainable, but they are not here.}.  
% \hfill\\
% Similarly, as the server does not have black-box access to any other proprietary model then: 
% at each time $t\in \mathbb{N}_+$ the server-side mixture coefficients $w_t$, in~\eqref{eq:enbsemble_server__predictions}, are of the form
% \begin{equation}
% \label{eq:PROPRIETARY_CONSTRAINT__Server}
%     w_t = \varpi_t\Big(
%             % \overbrace{
%                 (Y_{[0:t+1]}^{(j)})_{j=1}^N
%             % }^{\text{Expert Predictions}}
%         ,
%                 y_{[0:t]}
%         ,
%             % \underbrace{
%                 x_{[0:t]}
%             % }_{\text{Input series}}
%         ,
%             % \overbrace{
%             w_{[0:t]}
%             % }^{\text{Server Weights}}
%     \Big)
% \end{equation}
% where $\varpi_t:\mathbb{R}^{d_y(1+t)\times (N-1)}\times \mathbb{R}^{d_y(1+t)}\times \mathbb{R}^{d_x(1+t)}\times \mathbb{R}^{N(1+t)} \to \mathbb{R}^{d_z\times 1}$ is a continuous function that may depend on the current time $t \in \mathbb{N}_+$.  
% Note that, since the agents each predict first, then the server's update can leverage the information in $Y_{t+1}^{(1)},\dots,Y_{t+1}^{(N)}$. 
% \hfill\\
% We emphasize that each client-side mixture weight $\beta_t^{(i)}$ is computed using strictly more information the sever-side weights $w_t$. This distinction arises because each agent has access to its own internal parameters, whereas the server does not, as these parameters are proprietary and remain inaccessible to the server. 
% }



% %\begin{equation}
% %\label{eq:ridge_local}
% %    \beta_t^i\in \operatorname{argmin}\, 
% %        \sum_{s=t-T\vee 0}^t\,
% %        e^{-\alpha^i(t-s)}
% %        \,\|
% %            (y_s-\hat{Y}_s^i)
% %        -\beta_t^i\,Z_s^i\|^2
% %        +
% %        \gamma^i\|\beta_t^i\|^2.
% % \end{equation}

% \section{Main Results}
% \label{s:Main_Resuls}
% \add{Our first result formalizes and derives the optimal server-side update (Theorem~\ref{thm:OptimalWeights}).  Next, we derive the optimal client-side update in (Theorem~\ref{thm:NashEqmExistence}) at pre-defined synchronization times, which can be at each time $t$.  We also provide a greedy scheme which each client can use between these synchronization times (Proposition~\ref{prop:localgreedyupdates}) for an added speedup at the cost of sub-optimal descisions.}

% \subsection{Optimal Server-Side Weights}
% \label{s:Main_Results__Server}
% \add{
% Let $t\in \mathbb{N}$ and fix regularization hyperparameters $\kappa,\lambda>0$.  
% Given any $(Y_{[0:t+1]}^{(j)})_{j=1}^N\in L^1(\mathbb{R}^{d_y})^{N(1+t)}$, $y_{[0:t]}\in \mathbb{R}^{d_y(1+t)}$, $x_{[0:t]}\in \mathbb{R}^{d_x(1+t)}$, and $w_{[0:t]}\in \mathbb{R}^{N(1+t)}$ we define the server-side objective as
% \begin{equation}
% \label{eq:server}
% \begin{aligned}
%     \min_{w_t\in \mathbb{R}^N}\,
%     &
%     % \mathbb{E}  \, 
%     % \biggl[  
%         \Big\| y_{t+1}  - \sum_{j=1}^N w^j_t \hat{Y}^j_{t+1} \Big\|^2 
%     + 
%         \sum_{j=1}^N \kappa | w^j_t |^2 
%     % \biggr]  
% \\
% \mbox{s.t.} & \,
% w^1_t+\dots+w^N_t = \eta
% .
% \end{aligned}
% \end{equation}
% The normalization constraint $w^1_t+\dots+w^N_t = \eta$ ensures that the \textit{average weight size} is equal to $\eta$. When $\eta=1$, this condition serves as a \textit{signed} variant of the usual probabilistic normalization constraint found in the PAC-Bayes literature (e.g.,~\cite{alquier2024user}), where $w_t$ belongs to the $N$-simplex, meaning each weight must satisfy $0 \leq w^i_t \leq 1$ for each $i$.   However, since we are not \textit{sampling} agent predictions but rather \textit{combining} them, we remove this additional constraint. Doing so allows the central server to make “negative bets against” an agent’s predictions. Even if an agent consistently performs poorly, its signed opposite prediction may still be useful. This added degree of freedom enables the server to better exploit available information across all agents.}
% \hfill\\
% In essence, the hyperparameter $\kappa$ controls the amount we allow the server to \textit{leverage} borrow its investment level in any given expert to leverage it towards the predictive influence of any other expert, and $\eta$ controls the total investment level of the server into each agent.
% \begin{theorem}[Server: Optimal Mixture Weights]
% \label{thm:OptimalWeights}
% Let $\kappa,\eta>0$, $t\in \mathbb{N}$, $(Y_{[0:t+1]}^{(j)})_{j=1}^N\in L^1(\mathbb{R}^{d_y})^{N(1+t)}$, $y_{[0:t]}\in \mathbb{R}^{d_y(1+t)}$, $x_{[0:t]}\in \mathbb{R}^{d_x(1+t)}$, and $w_{[0:t]}\in \mathbb{R}^{N(1+t)}$ with $\sum_{i=1}^N w^{(i)}_t =\eta$ for each $t\in [0:t]$.  
% Then
% \[
%         w_t^{\star}  
%     = 
%          A^{-1}\,
%          \biggl(
%              b -  
%              % \biggl(
%                 \frac{
%                     \mathbf{1}_N^{\top}A^{-1}\,b-
%                     \eta%1
%                 }{
%                     \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N
%                 }
%             \cdot
%              % \biggr)
%              \,\mathbf{1}_N
%          \biggr)
% \]
% is the \textit{unique} optimal solution $w^{\star}_\cdot=(w^1_\cdot, \cdots, w^N_\cdot)^\top$ to~\eqref{eq:server}; 
% where $A\eqdef 2 ( \hat{\mathbf{Y}}^\top_{t} \hat{\mathbf{Y}}_{t} + \kappa I_N )$, $b\eqdef 2 (y^\top_{t}  \hat{\mathbf{Y}}_{t})^{\top}$, $\hat{\mathbf{Y}}_{t} = (\hat{Y}^1_{t}, ..., \hat{Y}^N_{t})$.
% \end{theorem}

% \subsection{Optimal Client-Side Updates}
% \label{s:Main_Results__Client}

% Each generative expert model $\hat{f}^i$ is stored locally on a different machine in the computational network.  The $i^{th}$ machine communicates with the server using two different mechanisms at two different frequencies.  Fix a \textit{synchronization frequency} $T\in \mathbb{N}_+$.  For each time $t\in \mathbb{N}$ not divisible by $T$, each expert model greedily optimizes its linear readout layer without communicating with any other expert by optimizing 
% \begin{align} 
% \label{eq:ridge_local}
% \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=(t-T)\vee 0}^{t-1}\,
%         e^{-\alpha_i(t-1-s)} 
%         \big\| y_{s+1} - ( \hat{Y}_{s}^i 
%         + Z_{s}^i \beta^i_t ) \big\|^2
%         +
%         \gamma_i\big\|\beta_t^i\big\|^2  . 
% \end{align} 

% \begin{comment} 
% \begin{equation}
%     \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=t-T\vee 0}^{t}\,
%         e^{-\alpha_i(t-s)} 
%         \| y_{s} - ( \hat{Y}_{s-1}^i 
%         + Z_{s-1}^i \beta^i_t ) \|^2
%         +
%         \gamma_i\|\beta_t^i\|^2  .
% \end{equation} 
% \end{comment} 

% This allows for rapid and fully parallelized online optimization of each model but has the drawback that the ensemble may deviate from its optimum.  
% The following gives the well-known optimal solution of the exponential-weighed ridge-regression problem in Equation \eqref{eq:ridge_local}.
% \begin{proposition}[Experts: Optimal Linear Decoder With No Expert Communication]
% \label{prop:localgreedyupdates}
% Let $\alpha_i\ge 0$ and $\gamma_i>0$.  Then the unique solution to Equation \eqref{eq:ridge_local} is given by
% %\begin{align} 
% %\beta^i_t = \Big[ \sum_{s=t-T\vee 0} e^{\alpha_i (t-s)} Z_s^{i\top} Z_s^i + \gamma_i I_{d_z} \Big]^{-1} 
% % \sum_{s=t-T\vee 0} e^{\alpha_i (t-s)} Z^{i\top}_s ( y_s - \hat{Y}^i_s )  \notag 
% %\end{align} 
% \begin{align} 
%    \beta_t^i =
%         \big(
%             X^{i \top}_{t-1} X^i_{t-1} + \gamma_i I_{d_z}
%         \big)^{-1}\, X_{t-1}^{i \top} \, \bar{y}^i_t  ,   \notag 
% \end{align} 
% where
% \begin{align} 
% & X^i_{t-1}  = \big[ e^{ - \alpha_i (t-1-0)/2} Z^{i\top}_0 , \ldots, e^{-\alpha_i (t-1-s)/2} Z^{i \top }_s, \ldots,  Z^{i \top }_{t-1} \big]^\top ,  \notag  \\ 
% & \bar{y}^i_t  = \big[ e^{-\alpha_i (t-1-0)/2} (y_1 - \hat{Y}^i_{0} )^\top, \ldots, e^{-\alpha_i (t-1-s)/2} (y_{s+1} - \hat{Y}^i_{s} )^\top, \ldots,  (y_{t} - \hat{Y}^i_{t-1} )^\top \big]^\top . \notag  
% \end{align} 
% \end{proposition}
% Each expert then immediately communicates their prediction $\hat{Y}_{t+1}^i$ to the central server. 
% The central server's objective is to mix the expert predictions to maximize the predictive power of the ensemble by minimizing 
% \begin{equation}
% \label{eq:primitive_energy}
%     % \min_{w}
%     % \mathbb{E}  \, 
%     % \biggl[  
%         \Big\| y_{t+1}  - \sum_{j=1}^N w^j_t \hat{Y}^j_{t+1} \Big\|^2 
%     % \biggr]  
% \end{equation}
% over mixture weights in $(w^1_t, ..., w^N_t) \in \mathbb{R}^N$.
% The server does this under the \textit{constraint} that it cannot over-leverage any one expert prediction.  
% The role of the server is then to aggregate the predictions of each expert into a weighted prediction of the form $\sum_{j=1}^N\, w_t^j\,\hat{Y}_{t+1}^j$ in such a way that no one expert is \textit{over-leveraged} and all weights are not overly large.
% Typically, in the PAC-Bayesian literature, see e.g.~\cite{alquier2024user}, one constrains the weights to lie in the $N$-simplex and interprets the mixture weights as probabilities that any one expert is active; see~\eqref{eq:NSimplexDef}.

% Though this approach is often solved using a Gibbs-measure associated to the problem, see e.g.~\cite{xxx}. Even without a probabilistic interpretation, Constraint~\eqref{c1:netting} is easily interpretable as requiring the overall investments of the server into each expert to ``net;'' meaning that if the server chooses to invest more into any one expert is must necessarily reduce its investment in any other expert's predictions.  From this perspective, Constraint~\eqref{c2:leveraging} prohibits the servers from \textit{over-leveraging} its investments into the prediction generated by any given expert by thresholding the minimal and maximal possible values of ascribable by any given weights; i.e.\ for each $n$ we have 
% $0\le w^i_\cdot \le 1-\sum_{j\neq i}\,w^j_\cdot \le 2-N$.

% If one does not take a probabilistic interpretation then Constraint~\eqref{c2:leveraging} can be restrictive as it does not allow the server to use one expert's (potentially poor) prediction to cancel out any residuals predictions of the entire mixture.  We instead replace~\eqref{c2:leveraging} with the the energy constraint in~\eqref{eq:primitive_energy} and consider the following penalized optimization problem for the server
% \begin{equation}
% \label{eq:server}
% \begin{aligned}
%     \min_{w_t\in \mathbb{R}^N}\,
%     &
%     % \mathbb{E}  \, 
%     % \biggl[  
%         \Big\| y_{t+1}  - \sum_{j=1}^N w^j_t \hat{Y}^j_{t+1} \Big\|^2 
%     + 
%         \sum_{j=1}^N \kappa | w^j_t |^2 
%     % \biggr]  
% \\
% \mbox{s.t.} & \,
% w^1_t+\dots+w^N_t = \eta
% \end{aligned}
% \end{equation}
% where $\kappa,\eta>0$.  The parameter $\kappa$ controls the amount we allow the server to \textit{leverage} borrow its investment level in any given expert in order to leverage it towards the predictive influence of any other expert and $\eta$ controls the total investment level of the server into each agent.
% \begin{theorem}[Server: Optimal Mixture Weights]
% \label{thm:OptimalWeights}
% Let $\kappa,\eta>0$.  Then, there is a unique optimal solution $w^{\star}_\cdot=(w^1_\cdot, \cdots, w^N_\cdot)^\top$ to Equation \eqref{eq:server} given by
% \[
%         w_t^{\star}  
%     = 
%          A^{-1}\,
%          \biggl(
%              b -  
%              % \biggl(
%                 \frac{
%                     \mathbf{1}_N^{\top}A^{-1}\,b-
%                     \eta%1
%                 }{
%                     \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N
%                 }
%             \cdot
%              % \biggr)
%              \,\mathbf{1}_N
%          \biggr)
% \]
% where $A\eqdef 2 ( \hat{\mathbf{Y}}^\top_{t} \hat{\mathbf{Y}}_{t} + \kappa I_N )$, $b\eqdef 2 (y^\top_{t}  \hat{\mathbf{Y}}_{t})^{\top}$, $\hat{\mathbf{Y}}_{t} = (\hat{Y}^1_{t}, ..., \hat{Y}^N_{t})$, 
% and $\mathbf{1}_N\in \mathbb{R}^N$ has all its entries equal to $1$. 
% \end{theorem}

% \begin{comment}
% \newpage
% In an ideal situation, this means that the server must weight the mixture of expert predictions, with the mixture weights at any given time $t$ belonging to the $N$ simplex and optimizing
% % \add{\textit{shifted first orthant} $\mathbb{R}_{\eta}^N\eqdef [\eta,\infty)^N$, where $\eta \ge 0$}; comprised of non-negative weights.  
% % We then control the maximum value of the weights using a weighted $\|\cdot\|_2$-norm penalty.
% % The optimal weight $w_t$ is chosen such that it optimizes the following penalized \textit{regret functional}
% % \begin{align} 
% %     J_0(w) 
% %  = 
% %      % \sum_{s=(t-T)\vee 0}^t 
% %      % e^{-\alpha(t-s)}
% %          \mathbb{E}  \, 
% %        \Big[  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
% %           + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big]  
% % , 
% % \label{DTJ0}
% % \end{align} 
% % where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  
% % \textit{Intuitively, we are asking that our weights belong to a ``round simplex'' rescaled by the factors $\kappa_1,\dots,\kappa_N$.}
% % Ideally, we would like to minimize the energy
% \add{the objective
% \[
%  %    J_0(w) 
%  % = 
%     \mathbb{E}  \, 
%     \biggl[  
%         \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%           % + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 
%     \biggr]  
% , 
% \]
% subject to the constraints 
% \begin{align}
%     \underbrace{
%         % \sum_{n=1}^N\, w_n  
%         w^1+\dots+w^N
%         = 1
%     }_{\term{c1:netting}}
% \mbox{ and }
%     \underbrace{
%         w^2,\dots,w^N  \ge 0
%     }_{\term{c2:leveraging}}
% .
% \end{align}
% Observe that,~\eqref{c1:netting} implies that $w^1 = 1- \sum_{n=2}^N\,w^n$ and therefore,~\eqref{c2:leveraging} implicitly has constrained $w^1$ to satisfy 
% $
% w^1 = 1- \sum_{n=2}^N\, w^n \le 1- (N-1)%\,\eta 1_{N>1}
% .
% $
% % where $1_{N>1}=1$ if $N>1$ and $0$ otherwise.  
% We highlight this to emphasize that there is no need to constraint $w^1$ further, as with $w^n$ for $n>1$, and doing so would lead to an over-determined system.
% % 
% For analytic traceability, we proceed using the following relaxation of~\eqref{c1:netting}, which must hold whenever the weights belong to the $N$-simplex
% \begin{equation}
% \label{c1:netting_relaxed}
% w_1 \le 1- (N-1)
% % \,\eta 1_{N>1}
% .
% \end{equation}
% With this relaxation, we would need to penalize the norm of the weights which we are optimizing over, in order to ensure that the mixture of experts does not ``overleverage'' any one expert.  That is, we would like to constrain the magnitude of the weights by instead considering the following regularized objective function
% \begin{equation}
% \label{DTJ0}
%     J_0(w) 
%  = 
%     \mathbb{E}  \, 
%     \biggl[  
%         \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%     + 
%         \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 
%     \biggr]  
% \end{equation}
% where $\kappa_1,\dots,\kappa_N> 0$ are hyperparameters implicitly controlling the size of the weight vector.  For each $N\in \mathbb{N}_+$, we thus optimize $J_0$ over the following relaxation of the $N$-simplex defined by a hyperparameter $\eta\le 1$
% \begin{equation}
% \label{eq:Generalized_Simplex_Constraint}
%         \Delta_{\eta,N}
%     \eqdef 
%     \big\{
%         w\in \mathbb{R}^N
%         :
%         \,
%         w_1 \le 1 +\eta - \eta N
%         \mbox{ and }
%         (\forall n>1)\, w_n\ge \eta
%     \big\}
% .
% \end{equation}
% }
% We compute the optimizer of~\eqref{DTJ0} in the following closed-loop form.
% \begin{theorem}[Server: Optimal Mixture Weights]
% \label{thm:OptimalWeights}
% Let $\eta\le 1$.  
% There is a unique optimizer 
% $w^{\star}_{\cdot} = (w^{1,\star}_{\cdot}, ..., w^{N,\star}_{\cdot} )$ 
% of $J_0$ over the generalized simplex $\Delta_{\eta,N}$ given by 
% % \begin{align}  
% %   w^{\star}_t & \eqdef  \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
% %   -\tilde{w}^{\star}_t , 
% %     \label{eqn:OptimalWeights}  
% %   \\
% %   \tilde{w}^{\star}_t   & \eqdef \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
% %   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
% %   % \\
% %   % &\times 
% %  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t  -  \mathbf{c} \Big] ,  \notag 
% %   \end{align}   
% \begin{align}
%     \label{eqn:OptimalWeights}  
%     w^{\star}_t
%     =
%     %%% Annie Relaxation
%         \big(
%             1-
%             % \frac1{k^2}
%             e^{-2\alpha(t-s)}
%         \big)
%         \big(
%             %% A
%             \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}
%         \big)^{-1}
%         \,
%         \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         % \frac1{k^2}
%         e^{-2\alpha(t-s)}
%         \,
%         \Big(
%             (1-\eta N) \,e_1 + \eta \mathbf{1}_N
%         \Big)
% \end{align}
% where $\mathrm{K} = \diag[\kappa_1, ..., \kappa_N]$ and 
% \begin{align} 
% %%% Annie Relaxation
%     G 
% \eqdef 
%     \begin{pmatrix}
%         1 & \mathbf{0}_{1\times N} \\
%         \mathbf{0}_{ (N \times 1) } & -I_{(N-1\times N-1)} 
%     \end{pmatrix}
%  % \mathrm{K} = \diag[\kappa_1, ..., \kappa_N]
%  % \in \mathbb{R}^{N\times N}
%  % , 
%  % \quad 
%  % G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  % G = -I_N
%  % \quad \mbox{and} \quad 
%  % \quad 
%  %  
%  % \mathbf{c} = 0_{N\times 1}
%  % \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%   \label{eq:Gc_Def}
% \end{align} 
% \end{theorem} 
% \end{comment}

% \textit{Synchronization rounds} occur periodically at pre-specified period $T\in \mathbb{N}_+$.  
% In each such round
% % During short communication rounds, 
% the $N$ machines communicate their past $T$ predictions with one another; however, they do not communicate their entire model with one another since that would take an infeasible bandwidth due to the size of each local model.  
% Instead, the local machines are only aware of the predictions generated by one another with the objective of maximizing their predictive power.  

% Consequentially, each local machine can be interpreted as an agent competing with the optimal behaviour, i.e.\ value of $\beta_t^i$, as a solution to a Nash \textit{equilibrium} between these machines.  Thus, given the weight $w_1,\dots,w_T$, each local machine $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^{T-1}$ non-cooperatively to minimize its local objective function
% % \allowdisplaybreaks 
% \begin{align} 
% \label{eq:Objective_nth_expert}   
%  J_i(\beta^i, \beta^{-i}) = 
%  \mathbb{E} \Bigg\{ \sum_{t=0}^{T-1} 
%     e^{ -\alpha_i (T - 1 - t)} 
%  \,
%   \Big[    
%  \Big\| y_{t+1} - \sum_{j=1}^N w^j_t \hat{Y}^j_{t+1} \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2    
%   \Big] 
%   \Bigg\}
% \end{align} 
% %\begin{align} 
% % J_i(\beta^i, \beta^{-i}) &= 
% % \mathbb{E} \Bigg\{ \sum_{t=0}^{T-1} 
% %    e^{ -\alpha_i (T - t)}  \,
% %  \Big[  \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
% %  + \gamma_i \| \beta^i_t \|^2    
% %  \Big] + \ \Big\| y_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 \Bigg \},   \notag 
% %\end{align} 
% for $i = 1, ..., N$, where $\beta^{-i}=
% (\beta^j)_{j=1; j\neq i}^N$
% % (\beta^1, ..., \beta^{i-1}, \beta^{i+1}, ..., \beta^N)
% and $\alpha^i\ge 0$ is a pre-specified hyperparameter controlling the impact of distant past observations on the current game the local machines are playing with one another.  
% The optimal value for the $i^{th}$ machine, which we denote by $(\beta^i_{t:\text{sync}})_{t=0}^T$, is given in closed-form as follows. 


% \begin{comment} 
% Denote 
% $%\begin{align} 
%  \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top$, $\hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top 
%  % . 
%  % \notag 
% $.%\end{align} 
% Then the costs in Equation \eqref{eq:Objective_nth_expert} for the $N$ agents can be written as  
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = 
%  \mathbb{E} \Bigg\{ \sum_{t=0}^{T-1} 
%     e^{ -\alpha_i (T - 1 - t)} 
%  \,
%   \Big[    
%  \big\| y_{t+1} -  \mathbf{w}^\top_t \hat{Y}_{t+1} \big\|^2 
%   + \gamma_i \| \beta^i_t \|^2    
%   \Big] 
%   \Bigg\},
%   \label{eq:Objective_nth_expertcompact}
% \end{align}
% for $i = 1, ..., N$. The optimal value for the $i^{th}$ machine, which we denote by $(\beta^i_{t:\text{sync}})_{t=0}^T$, is given in closed-form as follows.
% \end{comment}


% % The following proposition links the existence of a Nash equilibrium of \eqref{DTRCsystem} and \eqref{eq:Objective_nth_expert} to the solvability of the system \eqref{eqn:Pi}. 
% \begin{theorem}[Experts: Optimal Re-synchronization via The Nash Equilibrium]
% \label{thm:NashEqmExistence}
% Suppose the system \eqref{eqn:Pi} for $(P_i)_{i=1}^N$ admits a solution for $t=0$, $1$, ..., $T$.  
% Then the $N$-agent Nash game \eqref{eq:Objective_nth_expert} admits a unique feedback Nash equilibrium for $t=0$, $1$, ..., $T-1$
% \begin{align} 
%  \boldsymbol{\beta}_{t} =  [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top  
% =  \mathbf{G}(t) \hat{Y}_t + \mathbf{H}(t) , 
% %= &  \big[  e^{ - \boldsymbol\alpha (T-1-t)}  ( \Gamma + \widehat{\mathbf{A}}(t) ) + \mathbf{A}(t)  \big]^{-1}   
% % \big[  e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top \hat{Y}_t ) 
% %- \mathbf{B}(t) \hat{Y}_t - \mathbf{C}(t) \big]  , 
% \label{eqmvecbeta}   
% \end{align} 
% where the matrix-valued coefficients $\mathbf{G}(\cdot)$ and $\mathbf{H}(\cdot)$ are determined by the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% $t=0$, $1$ ..., $T$, 
% %\begin{equation} 
% %\begin{split} 
% %\left \{ 
% %\begin{aligned}
% %  P_i(t) &= 
% % \Big(\big[ \mathbf{D}(t)(  e^{-\boldsymbol{\alpha}(T-t)}  \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I \big]^\top
% %  \\
% %  &\qquad \qquad \qquad \cdot P_i(t+1)\big[  \mathbf{D}(t)( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} 
% % \mathbf{B}(t) - I \big] \Big)  \\ 
% %  & \qquad + \Big(e^{ - \alpha_i (T-t) } \gamma_i \big[  ( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} %\mathbf{B}(t) \big]^\top \\ 
% % & \qquad \qquad \qquad \cdot \big[  ( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) \big] \Big) \\ 
% % &\qquad + e^{ - \alpha_i (T-t)} \mathbf{w}_t \mathbf{w}_t^\top  \\ 
% %  P_i(T) &=  \mathbf{w}_T \mathbf{w}_T^\top  ,
% %\end{aligned}
% %\right.
% %\end{split}
% %\label{eqn:Pi}
% %\end{equation} 
% \begin{equation} 
% \begin{split} 
% \left \{ 
% \begin{aligned}
%   P_i(t)  = &   
%   \mathbf{G}(t)^\top 
%   \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] 
%    \mathbf{G}(t)  
%    \\ 
%    & + \big[ e^{-\alpha_i(T-1-t)}\mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big] 
%    \mathbf{D}(t) \mathbf{G}(t) \\ 
%    & + \mathbf{G}(t)^\top \mathbf{D}(t)^\top \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big]^\top  \\ 
%    & + e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  , \\ 
%   & \hspace{-0.6cm} e^{ - \boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{ - \boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t) 
%    \, \text{is invertible} , 
%   \\ 
%   P_i(T)   = &    0  ,
% \end{aligned}
% \right.
% \end{split}
% \label{eqn:Pi}
% \end{equation} 
% %where $e^{ - \boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{ - \boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)$ 
% % is assumed to be invertible. 
% \begin{equation}  
% \begin{split} 
% \left \{ 
% \begin{aligned}
%   S_i(t)  = &  \mathbf{G}^\top(t) \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) 
%    + e^{-\alpha_i(T-1-t)} \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] \mathbf{H}(t) \\ 
% & + \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  \big] \mathbf{D}(t) \mathbf{H}(t) \\  
% & + \mathbf{G}^\top(t) \mathbf{D}^\top(t) \big[ - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) \big] \\ 
% & - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) , \\ 
%  S_i(T) = & 0   . 
% \end{aligned}
% \right.
% \end{split} 
% \label{eqn:Si}
% \end{equation} 
% %\begin{equation}  
% %\begin{split} 
% %\left \{ 
% %\begin{aligned}
% %  S_i(t) &=   \Big(\mathbf{B}(t)^\top \big( e^{ - \boldsymbol{\alpha}(T-t)}  \Gamma + \mathbf{A}(t)\big)^{-1} 
% % \big[ e^{ - \alpha_i(T-t)} \gamma_i I +  \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t) \big] \\
% % & \qquad \qquad \qquad \cdot \big( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t)\big)^{-1} \mathbf{C}(t) \Big)    \\ 
% %  &\qquad - P_i(t+1) \mathbf{D}(t)\big( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t)\big)^{-1} \mathbf{C}(t) \\ 
% % &\qquad - \mathbf{B}(t)^\top \big( e^{ -\boldsymbol{\alpha} (T-t)} \Gamma + \mathbf{A}(t)\big)^{-1}\mathbf{D}(t)^\top S_i(t+1) \\ 
% % & \qquad + S_i(t+1) - e^{ - \alpha_i(T-t)} \mathbf{w}_t y_t, \\ 
% % S_i(T)&= - \mathbf{w}_T y_T   . 
% %\end{aligned}
% %\right.
% %\end{split} 
% %\label{eqn:Si}
% %\end{equation} 
% %
% %
% %
% %\allowdisplaybreaks 
% %\begin{align} 
% %& \mathbf{A}(t) = [ A_{ij}(t) ]_{i, j=1}^N \in \mathbb{R}^{ N dz \times  N dz} , \quad   
% % A_{ij}(t) =  \mathbb{E} [ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t ] \in \mathbb{R}^{dz \times dz}   \notag \\  
% %& \mathbf{B}(t) = [ B_i(t) ]_{i=1}^N   \quad 
% % B_i(t) = \mathbb{E} [ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) ] \notag \\ 
% % & \mathbf{C}(t) = [ C_i(t) ]_{i=1}^N , \quad 
% % C_i(t) = \mathbb{E} Z^{i\top}_t \mathbf{e}_i^\top  S_i(t+1) \notag \\ 
% % & \mathbf{D}(t) = [ D_i(t) ]_{i=1}^N , \quad 
% % D_i(t) =  \mathbb{E}(  \mathbf{e}_i  Z^i_t ) \notag 
% %\end{align} 
% %\begin{comment} 
% %\begin{align} 
% %& \mathbf{A}(t) = \overline{\mathbf{A}}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t) 
% %\notag 
% %\end{align} 
% The matrix-valued coefficients in \eqref{eqn:Pi} and \eqref{eqn:Si} are defined by  
% \allowdisplaybreaks 
% %\begin{align} 
% %& \mathbf{A}(t) = \mathbb{E} \begin{bmatrix} 
% %   Z^{1\top}_t \mathbf{e}_1^\top  P_1(t+1)  \mathbf{e}_1 Z^1_t  & 
% %   Z^{1\top}_t \mathbf{e}_1^\top  P_1(t+1)  \mathbf{e}_2 Z^2_t  
% % & \cdots & 
% %   Z^{1\top}_t \mathbf{e}_1^\top  P_1(t+1)  \mathbf{e}_N Z^N_t   \\ 
% %   Z^{2\top}_t \mathbf{e}_2^\top P_2(t+1) \mathbf{e}_1 Z^1_t   & 
% %   Z^{2\top}_t \mathbf{e}_2^\top P_2(t+1) \mathbf{e}_2 Z^2_t  
% % & \cdots & 
% %   Z^{2\top}_t \mathbf{e}_2^\top P_2(t+1) \mathbf{e}_N Z^N_t  \\ 
% % \vdots & \vdots & \ddots & \vdots \\ 
% %  Z^{N\top}_t \mathbf{e}_N^\top P_N(t+1) \mathbf{e}_1 Z^1_t  & 
% %  Z^{N\top}_t \mathbf{e}_N^\top P_N(t+1) \mathbf{e}_2 Z^2_t 
% % & \cdots & 
% %  Z^{N\top}_t \mathbf{e}_N^\top P_N(t+1) \mathbf{e}_N Z^N_t 
% %\end{bmatrix} \notag \\ 
% %\end{align} 
% %\begin{align} 
% %&\widehat{\mathbf{A}}(t) = 
% % \mathbb{E} \begin{bmatrix} 
% %   Z^{1\top}_t \mathbf{e}_1^\top  \mathbf{w}_t \mathbf{w}_t^\top   \mathbf{e}_1 Z^1_t  & 
% %  Z^{1\top}_t \mathbf{e}_1^\top  \mathbf{w}_t \mathbf{w}_t^\top   \mathbf{e}_2 Z^2_t  
% % & \cdots & 
% %  Z^{1\top}_t \mathbf{e}_1^\top  \mathbf{w}_t \mathbf{w}_t^\top   \mathbf{e}_N Z^N_t   \\ 
% % Z^{2\top}_t \mathbf{e}_2^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_1 Z^1_t   & 
% %  Z^{2\top}_t \mathbf{e}_2^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_2 Z^2_t  
% % & \cdots & 
% %  Z^{2\top}_t \mathbf{e}_2^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_N Z^N_t  \\ 
% % \vdots & \vdots & \ddots & \vdots \\ 
% %  Z^{N\top}_t \mathbf{e}_N^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_1 Z^1_t  & 
% %  Z^{N\top}_t \mathbf{e}_N^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_2 Z^2_t 
% % & \cdots & 
% %  Z^{N\top}_t \mathbf{e}_N^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_N Z^N_t 
% %\end{bmatrix} 
% %\notag \\
% %& \mathbf{B}(t) = 
% %\mathbb{E} 
% % \begin{bmatrix} 
% %   Z^{1\top}_t \mathbf{e}_1^\top P_1(t+1)  \\ 
% %  Z^{2\top}_t \mathbf{e}_2^\top P_2(t+1)   \\ 
% % \vdots \\  
% %  Z^{N\top}_t \mathbf{e}_N^\top P_N(t+1)  
% % \end{bmatrix} ,  
% % \qquad 
% % \mathbf{C}(t) = 
% % \mathbb{E} 
% % \begin{bmatrix} 
% %  Z^{1\top}_t \mathbf{e}_1^\top S_1(t+1)   \\ 
% %  Z^{2\top}_t \mathbf{e}_2^\top S_2(t+1)   \\ 
% % \vdots \\ 
% %  Z^{N\top}_t \mathbf{e}_N^\top S_N(t+1)   
% % \end{bmatrix} , 
% % \notag \\ 
% %\end{align} 
% \begin{align} 
%  & \mathbf{A}(t) = 
% \mathbb{E} \big\{ \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \cdots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top 
% \big[ \mathbf{e}_1 Z^1_t, \cdots,  \mathbf{e}_N Z^N_t  \big]  \big\}  , 
% \notag \\ 
% & \widehat{\mathbf{A}}(t) = 
% \mathbb{E} \big\{ \big[ \mathbf{e}_1 Z^1_t, \cdots, \mathbf{e}_N Z^N_t \big]^\top 
% \mathbf{w}_t \mathbf{w}_t^\top 
% \big[ \mathbf{e}_1 Z^1_t, \cdots,  \mathbf{e}_N Z^N_t  \big]  \big\} , 
% \notag \\ 
% & \mathbf{B}(t) = \mathbb{E} \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \cdots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top ,
%  \notag \\ 
% & \mathbf{C}(t) = \mathbb{E} \big[ S_1^\top(t+1) \mathbf{e}_1 Z^1_t, \cdots, S_N^\top(t+1) \mathbf{e}_N Z^N_t \big]^\top ,  \notag \\ 
% & \mathbf{D}(t) 
%  = \mathbb{E}  
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix} , \notag \\ 
%  & 
%  \mathbf{D}_i(t) 
%  = \mathbb{E} \Big\{   
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix}^\top 
%   P_i(t+1) 
%   \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix} 
%  \Big\} , \quad i = 1, ..., N, 
%  \notag \\ 
%  &  \mathbf{G}(t) = - \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma 
%   + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} 
%  \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t \mathbf{w}_t^\top + \mathbf{B}(t) \big] , 
%  \notag \\ 
%  & \mathbf{H}(t) = \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} 
%   \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t y_{t+1} - \mathbf{C}(t) \big] , 
%  \notag 
% \end{align} 
% %\end{comment} 
% where $\{e_1, \cdots, e_N\}$ is the standard basis of $\mathbb{R}^N$ with each $e_i$ being a column vector, and 
% \begin{align} 
%  & \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top, \quad \hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top, \quad   
%   \Gamma = \diag[ \gamma_1 I_{d_z} , ..., \gamma_N I_{d_z} ] ,
%   \notag \\ 
%  & 
%   \boldsymbol{\alpha} = \diag [\alpha_1 I_{d_z} , ..., \alpha_N I_{d_z} ] , 
%   \notag \\ 
% &  \mathbf{e}_i = e_i \otimes I_{d_y} = [0, ..., I_{d_y} , ..., 0]^\top , \quad 
%  \hat{\mathbf{e}}_i = e_i \otimes I_{d_z} = [0, ..., I_{d_z} , ..., 0]^\top , 
%   \quad i=1, \ldots, N . 
%  \notag 
% \end{align} 
% \end{theorem}

% Theorem~\ref{thm:NashEqmExistence} leads to the following synchronization subroutine (Algorithm~\ref{alg:sync_subroutine}).




% If the number of experts $N$ is too large for the matrix operators in Theorem~\ref{thm:NashEqmExistence} to be tractable, then one (uniformly) randomly samples a batch of size $1\le b\le N$, with $b\in \mathbb{N}$, amongst all the $N$ experts and that subset of experts plays the Nash game.  The remaining experts continue to update their linear readout layers using the exponentially weighted ridge-repression problem~\eqref{prop:localgreedyupdates}.


% In this \textit{general formulation}, the computational bottleneck in our federated learning algorithm is the computation of the matrices in Theorem~\ref{thm:NashEqmExistence}.  Nevertheless, in Examples~\ref{ex:finte_tine} and~\ref{ex:Random_NeuralNetwork}, they can be explicitly computed in a simple closed form.  We now exhibit these simplified closed-form expressions.

% \subsection{Discussion}
% Every $T$ round, the server synchronizes a (uniformly) randomly selected batch of $ b \le N$ experts from all the available experts.  
% Since each expert is working on a separate machine, which may not be large enough to load the states of all the experts simultaneously, they must reach a consensus with limited communication.  The optimal consensus can be framed as a \textit{non-cooperative game} amongst the randomly chosen $b$ experts, each of which seeks to exert predictive influence on the ensemble, to the proportion allotted by the server according to $w_t$.  The optimal direction which the ensemble can take can be formulated as a Nash equilibrium, in which no expert can improve their predictive influence on the mixture by further modifying their linear decoder~\eqref{eq:Objective_nth_expert}.
% The subroutine in Algorithm~\ref{alg:sync_subroutine} computes precisely this Nash equilibrium using $T$ iterations.

% %\AK{Xuwei: Write Proposition in Algo 2 Format}
% %\begin{algorithm}[H]%[ht!]%
% %\caption{Synchronization Subroutine}
% %\label{alg:sync_subroutine}
% %\begin{algorithmic}
% %\SetAlgoLined
% %\Require {\color{blue}{Copy and paste Proposition 2}} 
% %\DontPrintSemicolon 
% %\State  
% %\end{algorithmic}
% %\end{algorithm}


% We now summarize our federated learning algorithm.



% Next, we present several use-cases of our federated optimization pipeline.  We derive simplified expressions for each of the update rules in Theorem~\ref{thm:NashEqmExistence}, by leveraging the structure of several standard models; with the exception of the reservoir computer.  Each use-case is complemented with a series of experimental ablation studies across a variety of datasets, showing that our proposed federated learning algorithms (Algorithm~\ref{alg:FedMain}-\ref{alg:sync_subroutine}) surpasses the available state-of-the-art.

% \section{From Echo-State to Transformers Agents in Practice}
% \label{s:Examples}
% This section shows how our theory can be put into practice for various FL agents ranging from static kernel learners to sequential deep learning models with hidden states.  In each case, we derive simplified and specialized expressions of our main Theorems, yielding streamlined algorithms.  Critically, we find an undeniable advantage 
% of our game-theoretic FL pipeline on a range of real-world benchmark datasets.

% \paragraph{Experiment Details}
% Numerical experiments are conducted across five distinct time-series datasets. three are synthetically generated but provide various time-series modeling challenges. Two represent natural time-series commonly used to benchmark state-of-the-art time series models. These datasets are described in detail in Section \ref{datasets}. In addition, the three distinct model types are described in Section \ref{xx}. These are ESN, RFN, and pre-trained models. In the pre-trained model experiments, a causal transformer was trained to make predictions based on previously seen data in the time-series. These models were chosen due to their ability to easily incorporate past data into predictions, as well as their ease of training. See Section \ref{xx} for additional details on transformer pre-training. A discussion of the choice to use Hard Sigmoid activation functions for the RFN and ESN models appears in Section \ref{activation_discussion}.  Time series performance is measured in mean-squared error (MSE) relative to the reference sequence. For a sequence of length $T\in \mathbb{N}$.

% Each experiment involves several distributed clients (experts) and a single server. The present set of experiments considers predictions from two or five collaborating experts. Each experiment. In each configuration, the periodic use of synchronization steps leveraging the Nash game described in Section \ref{xx} for server predictions is compared with the simpler weight ensemble optimization described in Section \ref{xx}. These are referred to throughout this section as the Game and Non-Game settings, respectively. 



% In each experiment presented below, the optimal hyperparameters are reported for both the Nash and non-Nash game settings. While doing so is computationally expensive, it was advantageous to play the Nash game at each step in all experiments. Studies considering the effects of less frequent synchronization are reported in Section \ref{sync_freq_studies}. Detailed results for various agent types 
% across each dataset are reported in Sections \ref{esn_results}-\ref{transformer_results}, respectively. For brevity, visualizations are only considered for the five client settings.
% Here, we consider a variety ranging from ``static'' kernel models, such as random feature networks (RFN)~\cite{mei2022generalization}, to sequential learners with no hidden state, such as transformers. and ultimately to reservoir computers such as the \textit{Echo-State Networks} (ESN), which leverage hidden states for expressive recursions.  Definitions and worked-out details of how our main algorithm (described by Theorems~\ref{thm:OptimalWeights} and ~\ref{thm:NashEqmExistence}) simplifies for each of these models are provided in this section.   

% Before diving into each detailed case study, we provide an overall snapshot summarizing the concrete gain obtained from our methodology.  
% These main results are straightaway reported in Table \ref{tab:summary_results}. For all datasets and all models, application of Nash game synchronization improves MSE, sometimes by an order of magnitude. The Nash game is especially helpful for the Concept Shift, BoC Exchange Rate, and ETT time-series. For both ESN and RFN models, there is also typically an improvement in prediction accuracy, both with and without the Nash game, with more experts contributing to the mixture. Such improvement is generally expected, especially since these models incorporate randomness in their feature representations.

% \begin{table}[ht]
% \centering
% \caption{Summary of experimental results for ESN, RFN, and Transformer models across datasets. The reported MSE is the mean of three separate runs with different random seeds for ESNs and RFNs. For Transformers, the reported MSE is for a pretrained model. Thus, fluctuations due to randomness are not incorporated.}
% \label{tab:summary_results}
% \resizebox{0.99\linewidth}{!}{\begin{tabular}{cclccc}
% \toprule
% Model & \# of Experts & Dataset & Nash Game & No Nash Game & Better With 5 \\
% \midrule
% \multirow{10}{*}{ESN} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{1.02870\mathrm{e}{\text{-}1}}$ & $5.62155\mathrm{e}{\text{-}1}$ & \\
% & & Logistic Map & $\mathbf{4.71543\mathrm{e}{\text{-}2}}$ & $5.30976\mathrm{e}{\text{-}2}$ & \\
% & & Concept Shift & $\mathbf{1.30703\mathrm{e}{\text{-}1}}$ & $1.98226\mathrm{e}{\text{-}0}$ & \\
% & & BoC Exchange Rate & $\mathbf{5.15198\mathrm{e}{\text{-}5}}$ & $2.18067\mathrm{e}{\text{-}4}$ & \\
% & & ETT Series & $\mathbf{7.13503\mathrm{e}{\text{-}4}}$ & $1.11331\mathrm{e}{\text{-}3}$ & \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{3.22272\mathrm{e}{\text{-}2}}$ & $5.57315\mathrm{e}{\text{-}1}$ & (Yes, Yes) \\
% & & Logistic Map & $\mathbf{4.65061\mathrm{e}{\text{-}2}}$ & $5.28456\mathrm{e}{\text{-}2}$ & (Yes, Yes) \\
% & & Concept Shift & $\mathbf{8.86346\mathrm{e}{\text{-}2}}$ & $4.85359\mathrm{e}{\text{-}0}$ & (Yes, No) \\
% & & BoC Exchange Rate & $\mathbf{1.15900\mathrm{e}{\text{-}4}}$ & $ 4.08432\mathrm{e}{\text{-}4}$ & (No, No) \\
% & & ETT Series & $\mathbf{7.15441\mathrm{e}{\text{-}4}}$ & $1.08915\mathrm{e}{\text{-}3}$ & (No, Yes) \\
% \midrule
% \multirow{10}{*}{RFN} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{2.56902\mathrm{e}{\text{-}1}}$ & $6.28833\mathrm{e}{\text{-}1}$ & \\
% & & Logistic Map & $\mathbf{4.97284\mathrm{e}{\text{-}2}}$ & $5.54874\mathrm{e}{\text{-}2}$ & \\
% & & Concept Shift & $\mathbf{7.85654\mathrm{e}{\text{-}3}}$ & $9.45541\mathrm{e}{\text{-}0}$ & \\
% & & BoC Exchange Rate & $\mathbf{7.86047\mathrm{e}{\text{-}5}}$ & $2.10533\mathrm{e}{\text{-}3}$ & \\
% & & ETT Series & $\mathbf{1.19513\mathrm{e}{\text{-}3}}$ & $3.51060\mathrm{e}{\text{-}3}$ & \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{ 5.96514\mathrm{e}{\text{-}2}}$ & $6.15566\mathrm{e}{\text{-}1}$ & (Yes, Yes) \\
% & & Logistic Map & $\mathbf{4.64415\mathrm{e}{\text{-}2}}$ & $5.50781\mathrm{e}{\text{-}2}$ & (Yes, Yes) \\
% & & Concept Shift & $\mathbf{1.01067\mathrm{e}{\text{-}2}}$ & $1.28812\mathrm{e}{\text{-}0}$ & (No, Yes) \\
% & & BoC Exchange Rate & $\mathbf{7.65036\mathrm{e}{\text{-}5}}$ & $3.15237\mathrm{e}{\text{-}3}$ & (Yes, No) \\
% & & ETT Series & $\mathbf{7.11836\mathrm{e}{\text{-}4}}$ & $2.26659\mathrm{e}{\text{-}3}$ & (Yes, Yes) \\
% \midrule
% \multirow{10}{*}{Transformer} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{1.78749\mathrm{e}{\text{-}1}}$ & $5.86464\mathrm{e}{\text{-}1}$ & \\
% & & Logistic Map & $\mathbf{4.53782\mathrm{e}{\text{-}2}}$ & $5.46232\mathrm{e}{\text{-}2}$ & \\
% & & Concept Shift & $\mathbf{6.45116\mathrm{e}{\text{-}2}}$ & $6.77600\mathrm{e}{\text{-}1}$ & \\
% & & BoC Exchange Rate & $\mathbf{4.48450\mathrm{e}{\text{-}5}}$ & $8.06623\mathrm{e}{\text{-}5}$ & \\
% & & ETT Series & $\mathbf{7.50786\mathrm{e}{\text{-}4}}$ & $1.05523\mathrm{e}{\text{-}3}$ & \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{6.95994\mathrm{e}{\text{-}2}}$ & $5.86337\mathrm{e}{\text{-}1}$ & (Yes, Yes) \\
% & & Logistic Map & $\mathbf{3.88076\mathrm{e}{\text{-}2}}$ & $6.99996\mathrm{e}{\text{-}2}$ & (Yes, No) \\
% & & Concept Shift & $\mathbf{5.56220\mathrm{e}{\text{-}2}}$ & $3.25625\mathrm{e}{\text{-}1}$ & (Yes, Yes) \\
% & & BoC Exchange Rate & $\mathbf{4.48687\mathrm{e}{\text{-}5}}$ & $8.35143\mathrm{e}{\text{-}5}$ & (No, No) \\
% & & ETT Series & $\mathbf{7.27732\mathrm{e}{\text{-}4}}$ & $1.26992\mathrm{e}{\text{-}3}$ & (Yes, No) \\
% \bottomrule
% \end{tabular}}
% \end{table}


% \subsection{{Pre-Trained Transformer with Fine-Tunable Linear Decoder}}
% Consider the setting of Example~\ref{ex:finte_tine}.  Then, the matrices $\mathbf{A}(\cdot)$, $\widehat{\mathbf{A}}(\cdot)$,   
% $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, $\mathbf{D}(\cdot)$, and $\{\mathbf{D}_i(\cdot)\}_{i=1}^N$ in
% \eqref{eqn:Pi} and \eqref{eqn:Si} can be dramatically simplified, and all expectations can be removed.  
% In this setting they reduce to
% \allowdisplaybreaks 
% \begin{align} 
% & \mathbf{A}(t) = 
% \begin{bmatrix} 
% \phi^{(i)}(x_t)^{\top} \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j\phi^{(j)}(x_t) 
% \end{bmatrix}_{i,j=1}^N , 
% \notag \\ 
% & \widehat{\mathbf{A}}(t) = 
% \begin{bmatrix} 
% \phi^{(i)}(x_t)^{\top} \mathbf{e}_i^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_j\phi^{(j)}(x_t) 
% \end{bmatrix}_{i,j=1}^N , 
% \notag \\ 
% & \mathbf{B}(t) = 
%  \begin{bmatrix} 
%      P_1(t+1)  \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots,  P_N(t+1) \mathbf{e}_N \phi^{(N)}(x_t)
%  \end{bmatrix}^\top  
%  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%     S_1(t+1)^\top  \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots, S_N(t+1)^\top  \mathbf{e}_N \phi^{(N)}(x_t)
%  \end{bmatrix}^\top  
%  , 
%  \notag \\ 
% & \mathbf{D}(t) 
%  = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots , \mathbf{e}_N \phi^{(N)}(x_t) 
%  \end{bmatrix} , 
%  \notag \\ 
% &  \mathbf{D}_i(t) 
%  =    
%  \big[
%     \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots , \mathbf{e}_N \phi^{(N)}(x_t) 
%   \big]^\top 
%   P_i(t+1) 
%   \big[
%     \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots , \mathbf{e}_N \phi^{(N)}(x_t) 
%   \big] ,
%   \quad i = 1, \dots, N. 
%  \notag 
% \end{align} 

% \begin{example}[Pre-Trained Transformer with Fine-Tunable Linear Decoder]
% \label{ex:finte_tine}
% For $i=1,\dots,N$, let $\phi^{(i)}:\mathbb{R}^{%(1+t)
% d_x
% \times 1}\to \mathbb{R}^{d_z\times 1}$ be all but the final linear decoder layer $\beta_t\in \mathbb{R}^{d_z\times 1}$ of a pre-trained transformer
% \begin{equation*}
%     \varphi^{(i)}(x_{[0:t]}^i,Z_{t-1}^i, \epsilon_t^i ) \eqdef \phi^{(i)}(x_t).
% \end{equation*}
% \end{example}


% \subsection{Generative Random Feature Networks (RFNs)}
% \label{s:Analysis__ss:ELN}

% \begin{example}[A Generative Model: Random Feature Network]
% \label{ex:Random_NeuralNetwork}
% For each $i=1,\dots,N$, fix random matrices, $A^{i} \in \mathbb{R}^{d_y \times d_x}$ and $b^{i} \in \mathbb{R}^{d_y \times d_z}$. Define
% \begin{equation}
% \hat{Y}^i_{t+1} = \hat{Y}^i_t +
%             \big[ \operatorname{ReLU}\bullet\big(
%                 A^{i} x_t + b^{i} + \sigma^i \, W_t^i
%             \big) \big]  \beta^{i}_{t} , 
% \notag 
% \end{equation}
% where $W_t^i\sim \mathcal{N}_{1\times d_z}(0,1)$ are independent of $A$ and $b$, $x_t \in \mathbb{R}^{d_x\times d_z}$, $\beta^i_t\in \mathbb{R}^{d_z \times 1}$, $\sigma_t^i \in \mathbb{R}^{d_y \times 1}$, and $\bullet$ denotes the element-wise application of the function $\operatorname{ReLU}$. 
% Here, $\varepsilon_t^i\eqdef \sigma_t^i \, W_t^i$, 
% $\varphi^{(i)}(x_{[0:t]}^i,Z_{t-1}^i, \varepsilon_t^i)\eqdef \operatorname{ReLU}\bullet\big(A^{i} x_t + b^{i} + \sigma_t^i \, W_t^i\big) = Z_{t+1}^i$. 
% %$\varphi(x_{[0:t]},\varepsilon_t,z_t)\eqdef 
% %\operatorname{ReLU} \bullet (Ax_t +b + \varepsilon_t)$, and $Z_t^i\eqdef \operatorname{ReLU}\bullet\big(
% %                A^{i} x_t + b^{i} + \sigma_t^i \, W_t^i
% %            \big)$.
% \end{example}


% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}; meaning that: for all $i=1,\dots,N$ and $t\in \mathbb{N}$
% \begin{equation}
% \label{DTRCsystemReLU}
% \begin{aligned} 
% \hat{Y}_{t+1}^i & = \hat{Y}_t^i + 
%    \big[ \operatorname{ReLU}\bullet\big(
%         A^{i}x_t+b^{i}
%         + \sigma^i\, W_t^i
%     \big) 
% \big] \beta^i_t . 
% \end{aligned} 
% \end{equation} 

% \begin{comment} 
% \begin{equation}
% \label{DTRCsystemReLU}
% \begin{aligned} 
% \hat{Y}_{t+1}^i & = \hat{Y}_t^i + \beta_t^{i\top}\,
%     \operatorname{ReLU}\bullet\big(
%         A^{(i)}x_t+b^{(i)}
%         + 
%         \sqrt{\sigma_t^{i}}\, W_t^i
%     \big) 
% \big)
% .
% \end{aligned} 
% \end{equation} 
% \end{comment} 

% We first consider the case $d_y=1$.  
% \begin{corollary} 
% \label{cor:Random_NN}
% In the setting of Example~\ref{ex:Random_NeuralNetwork} with $d_y=1$, we have
% \begin{align*}
% & \mathbf{A}(t)
%  = 
% \big(A^{(i,j)}(t)\big)_{i,j=1}^N , 
% \hspace{2.05cm} 
% \widehat{\mathbf{A}}(t) = \big( \widehat{A}^{(i,j)}(t) \big)_{i, j = 1}^N , 
% \notag \\  
%  & \mathbf{B}(t)  = 
%  \begin{bmatrix} 
%   P_1(t+1) \mathbf{e}_1 a(t, 1), \cdots, P_N(t+1) \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%   S_1(t+1)^\top \mathbf{e}_1 a(t, 1), \cdots, S_N(t+1)^\top  \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top , 
%   \notag \\   
% & \mathbf{D}(t) 
%   = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 a(t,1), \cdots  , \mathbf{e}_N a(t, N) 
%  \end{bmatrix} , 
%  \notag \\ 
%  & \mathbf{D}_i(t) = ( D_i^{(j,k)}(t) )_{j,k = 1}^N , \quad i = 1, ..., N . \notag 
% % \big( D_i^{(j,k)} \big)_{j,k=1}^N , \quad i = 1, ..., N. \notag 
% \end{align*}
% where for $t=1,\dots,N$ and $t\in \mathbb{N}_+$, each $a(t,i)$ is defined as follows
% \begin{align} 
% & a^i_t\eqdef A^{i}x_t+b^{i} , \notag \\ 
% & a(t,i)
% \eqdef 
%    a^i_t 
%         \odot
%         \left(
%             \bar{1} 
%             - 
%             \Phi\bullet\left(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a^i_t
%             \right)
%         \right)
%         +
%             \frac{\sigma_t^i}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\left(
%             \frac{-1}{2\, (\sigma_t^i)^2 }
%             % \,
%             \left(a^i_t \odot a^i_t \right)
%         \right)  , \notag 
% \end{align} 
% and $\odot$ and $\Phi$ are defined in Lemma~\ref{lem:Mean_Cov_ResModel}. 
% %and $\cdot^2$ is applied componentwise; i.e.\ $x^2\eqdef (x_i^2)_{i=1}^N$ for any $x\in \mathbb{R}^N$. 
% %$a^i_t\eqdef A^{(i)}x_t+b^{(i)}$. 

% The submatrices 
% $\big(A^{(i,j)}(t)\big)_{i,j=1}^N$, $\big(\widehat{A}^{(i,j)}(t)\big)_{i,j=1}^N$, 
% and $\big(D_i^{(j,k)}(t)\big)_{j,k=1}^N$ of $\mathbf{A}(t)$, $\widehat{\mathbf{A}}(t)$, 
% and $\{ \mathbf{D}_i(t) \}_{i=1}^N$,  respectively, in the setting of Example~\ref{ex:Random_NeuralNetwork},  
% are given by
% \begin{align} 
%  A^{(i,j)}(t) =
% \begin{cases} 
% \big[  ( A^{(i,i)}(t) )_{jk} \big]_{j,k=1}^{d_z} , \quad & \mbox{if} \quad i = j , \\
%   a(t, i)^\top  (P_i(t+1))_{ij} a(t, j) , \quad & \mbox{if} \quad i \neq j  , 
%  \end{cases} 
%  \notag 
%  \end{align} 

% \begin{align} 
%  & \widehat{A}^{(i,j)}(t) = 
%  \begin{cases} 
%    \big[ ( \widehat{A}^{(i,i)}(t) )_{jk} \big]_{j,k=1}^{d_z}  , \quad & \mbox{if} \quad i = j , \\ 
%  a(t, i)^\top  w^i_t w^j_t a(t, j) , \quad & \mbox{if} \ i \neq j   , 
% \end{cases} 
% \notag 
% \end{align} 


% \begin{align} 
% & D_i^{(j,k)}(t) = 
% \begin{cases}
%   \big[ (D_i^{(j,j)})_{l m} \big]_{l,m=1}^{d_z} , \quad & \mbox{if} \quad j=k , \\ 
% a(t,j)^\top (P_i(t+1))_{jk} a(t, k) , \quad & \mbox{if} \, j\neq k , 
% \notag 
% \end{cases} 
% \end{align} 
% where the submatrices $A^{(i,i)}(t)= \big[ (A^{(i,i)}(t))_{jk}  \big]_{j,k=1}^{d_z}$, 
% $\widehat{A}^{(i,i)}(t)=\big[ ( \widehat{A}^{(i,i)}(t))_{jk}  \big]_{j,k=1}^{d_z}$, 
% and $ D_i^{(j,j)} = \big[ (D_i^{(j,j)})_{lm} \big]_{l,m=1}^{d_z}$ are
% given by
% \begin{align}  
% \big( A^{(i,i)}(t) \big)_{jk} %\notag \\
%  & 
%  % \hspace{1.2cm} 
%  =
%         ( P_i(t+1) )_{ii} \cdot
%     \begin{cases}
%             \Big( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 \Big)
%             \cdot
%             \left(
%                 1 
%                 - 
%                 \Phi\left(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 \right)
%             \right) \\
%             \hspace{2.5cm}+
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big) ,
%     & 
%         \mbox{ if } j=k , 
% \\ 
%       a(t, i)_j a(t,i)_k , 
%     & \mbox{ if }   j \neq k ,
%     \end{cases} 
%     \notag 
% \end{align} 

% \begin{align}  
% \big( \widehat{A}^{(i,i)}(t) \big)_{jk} %\notag \\
%  & 
%  % \hspace{1.2cm} 
%  =
%         (w^i_t)^2 \cdot
%     \begin{cases}
%             \Big( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 \Big)
%             \cdot
%             \left(
%                 1 
%                 - 
%                 \Phi\left(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 \right)
%             \right) \\
%             \hspace{2.5cm}+
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big) ,
%     & 
%         \mbox{ if } j=k , 
% \\ 
%       a(t, i)_j a(t,i)_k , 
%     & \mbox{ if }   j \neq k , 
%     \end{cases} 
%     \notag 
% \end{align} 


% \begin{align}  
% \big( D_i^{(j,j)}(t) \big)_{lm} %\notag \\
%  & 
%  % \hspace{1.2cm} 
%  =
%         (P_i(t+1))_{jj} \cdot
%     \begin{cases}
%             \Big( (a^j_t \odot a^j_t )_l + (\sigma^j_t)^2 \Big)
%             \cdot
%             \left(
%                 1 
%                 - 
%                 \Phi\left(
%                     \frac{-(a^j_t)_l}{\sigma_t^j}
%                 \right)
%             \right) \\
%             \hspace{2.5cm}+
%             (a^j_t)_l\,
%                 \frac{\sigma_t^j}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^j_t \odot a^j_t )_l }{2\,(\sigma_t^j)^2 }
%             \Big) ,
%     & 
%         \mbox{ if } l = m ,  
% \\ 
%       a(t, j)_l a(t,j)_m , 
%     & \mbox{ if }   l \neq m , 
%     \end{cases} 
%     \notag 
% \end{align} 
% \end{corollary} 



% \subsubsection{Periodic Signal}
% \label{s:ESN_PS}

% As in the ESN experiments, the predictions produced by the RFN models without Nash synchronization tend towards the mean of the of the Periodic Signal time series. On the other hand, those with Nash synchronization more closely incorporate the periodic behaviour. Consider the ratio of squared errors in Figure \ref{fig:rfn_periodic_figures}. The predictions with Nash game remain significantly better, though there are more examples below the critical threshold of $1.0$ than seen in the ESN experiments.
% The best hyperparameter choices are recorded in Table~\ref{tab:ESN_P} in Appendix~\ref{s:OptimalParamterChoices}.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 3$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 3$.
% %     \item Client $T = 3$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 3$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 3$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% %     \item Client $T = 3$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% % \end{itemize}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/periodic/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/periodic/relative_squared_server_errors.pdf}
% %     \caption{Periodic Signal results using RFN Models with and without Nash game synchronization.}
% %     \label{fig:rfn_periodic_figures}
% % \end{figure}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/logistic/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/logistic/relative_squared_server_errors.pdf}
% %     \caption{Logistic Map results using RFN Models with and without Nash game synchronization.}
% %     \label{fig:rfn_logistic_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/rfn/periodic/overlaid_server_predictions.pdf}
%             \caption{Periodic - Overlaid Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/rfn/periodic/relative_squared_server_errors.pdf}
%             \caption{Periodic - Relative Squared Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/rfn/logistic/overlaid_server_predictions.pdf}
%             \caption{Logistic - Overlaid Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/rfn/logistic/relative_squared_server_errors.pdf}
%             \caption{Logistic - Relative Squared Errors}
%         \end{subfigure}
%     \end{tabular}
%     \caption{Comparison of RFN Models with/without Nash game synchronization for different signals.}
%     \label{fig:rfn_comparison}
% \end{figure}

% \subsubsection{Logistic Map}
% \label{s:ESN_LM}

% Due to its periodic and sometimes unstable nature, the Logistic Map series poses challenges for the RFN models in both settings, just as it did for the ESNs. Predictions with Nash game synchronization are significantly better at matching the periodic behavior of the series. As in previous periodic settings, predictions without Nash synchronization settle near the mean of the of the series with smaller modulations in the prediction magnitude. During regions of more unstable behavior, occurring, for example, between $t=45$ to $t=65$, this approach tends to produce a better fit, due to its conservative nature. See the aforementioned time span in the ratio of squared errors plot in Figure \ref{fig:rfn_logistic_figures}. However, over the course of the series, the Nash game synchronization approach proves to provide much more accurate predictions.
% The best hyperparameter choices are recorded in Table~\ref{tab:ESN_LM} in Appendix~\ref{s:OptimalParamterChoices}.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 5$, Game $T=3$, $\alpha = 0.0001$, $\gamma = 15.0$, $\sigma = 0.01$, $d_z = 5$.
% %     \item Client $T = 3$, Game $T=3$, $\alpha = 0.0001$, $\gamma = 15.0$, $\sigma = 0.1$, $d_z = 5$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 3$.
% %     \item Client $T = 3$, $\alpha = 0.01$, $\gamma = 15.0$, $\sigma = 0.01$, $d_z = 3$.
% % \end{itemize}

% \subsubsection{Concept Drift}
% \label{RFN_CD}

% For simplicity in the RFN experiments, the concept drift time series target dimensionality is reduced such that $d_y = 1$. In this case, the $y_2$ series is retained. As in the ESN experiments, predictions made with Nash game synchronization outperform those without by a large margin. As seen in Figure \ref{fig:rfn_concept_figures}, at the beginning of the time series, both approaches perform quite well. Predictions with the Nash game remain of higher quality, but the non-Nash game setting is competitive. However, after the transition and especially later in the series, prediction errors appear to compound for the non-Nash setting, causing heavy oscillations and poor predictions. Given that the series transitions from a lower to higher frequency pattern in its oscillations, it's possible that the hyper-parameters for the non-Nash setting are well fitted to the lower frequency setting, but less so for the higher regime.

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/concept/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/concept/relative_squared_server_errors.pdf}
% %     \caption{Concept Drift results using RFN Models with and without Nash game synchronization.}
% %     \label{fig:rfn_concept_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/concept/overlaid_server_predictions.pdf}
%         \caption{Overlaid Server Predictions}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/concept/relative_squared_server_errors.pdf}
%         \caption{Relative Squared Server Errors}
%     \end{subfigure}
%     \caption{Concept Drift results using RFN Models with and without Nash game synchronization.}
%     \label{fig:rfn_concept_figures}
% \end{figure}

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, Game $T=2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 5$.
% %     \item Client $T = 5$, Game $T=2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 6$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 3$.
% %     \item Client $T = 2$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 3$.
% % \end{itemize}

% \subsubsection{BoC Exchange Rate}
% \label{s:RFN_BoCX}

% Provided with additional input variables and lagged target data, the RFN models produce fairly accurate predictions for the BoC Exchange Rate series. In spite of this improvement, considering the ratio of squared errors in Figure \ref{fig:rfn_boc_figures}, predictions with the Nash game tend to be of significantly higher quality. This is especially true in the later stages of the series. As with the ESN models, the vast majority of predictions throughout the time series are above the ratio threshold of $1.0$ in the figure.
% The best hyperparameter choices are recorded in Table~\ref{tab:RFN_BoCX} in Appendix~\ref{s:OptimalParamterChoices}.


% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, Game $T=2$, $\alpha = 1.0$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% %     \item Client $T = 5$, Game $T=2$, $\alpha = 0.01$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 6$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 0.01$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% %     \item Client $T = 5$, $\alpha = 1.0$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% % \end{itemize}

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/boc/overlaid_server_predictions.pdf}
%         \caption{Overlaid Server Predictions}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/boc/relative_squared_server_errors.pdf}
%         \caption{Relative Squared Server Errors}
%     \end{subfigure}
%     \caption{Boc Exchange Rate results using RFN Models with and without Nash game synchronization.}
%     \label{fig:rfn_boc_figures}
% \end{figure}


% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/boc/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/boc/relative_squared_server_errors.pdf}
% %     \caption{Boc Exchange Rate results using RFN Models with and without Nash game synchronization.}
% %     \label{fig:rfn_boc_figures}
% % \end{figure}

% \subsubsection{ETT Series}

% As with the ESN experiments, the RFN models, in both settings, produce relatively good predictions for the oil temperature target variable. For the server predictions, displayed in Figure \ref{fig:rfn_ett_figures}, those with the Nash game synchronization appear to do a better job matching the magnitudes of the time series. This is also borne out in the ratio of squared errors plots in the same Figure. The bulk of predictions are well above the line at $1.0$. Interestingly, it appears that the predictions for the RFN models are more heavily distributed in favor of the Nash synchronization process than in the ESN setting.
% The best hyperparameter choices are recorded in Table~\ref{tab:ESN_ETT} in Appendix~\ref{s:OptimalParamterChoices}.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 5$, Game $T=2$, $\alpha = 5.0$, $\gamma = 15.0$, $\sigma = 0.1$, $d_z = 2$.
% %     \item Client $T = 2$, Game $T=3$, $\alpha = 5.0$, $\gamma = 10.0$, $\sigma = 0.1$, $d_z = 1$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 3$, $\alpha = 0.01$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 2$.
% %     \item Client $T = 3$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 2$.
% % \end{itemize}



% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/ett/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/rfn/ett/relative_squared_server_errors.pdf}
% %     \caption{ETT Series results using RFN Models with and without Nash game synchronization.}
% %     \label{fig:rfn_ett_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/ett/overlaid_server_predictions.pdf}
%         \caption{Overlaid Server Predictions}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/ett/relative_squared_server_errors.pdf}
%         \caption{Relative Squared Server Errors}
%     \end{subfigure}
%     \caption{ETT Series results using RFN Models with and without Nash game synchronization.}
%     \label{fig:rfn_ett_figures}
% \end{figure}


% \subsection{Transformer Experiments} \label{s:transformer_results}

% % \subsubsection{Periodic Signal}
% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 7$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 5$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $d_z = 2$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 4$, $\alpha = 0.1$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 4$, $\alpha = 0.1$, $\gamma = 10.0$, $d_z = 2$.
% % \end{itemize}

% % \subsubsection{Logistic Map}

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 4$, Game $T=1$, $\alpha = 1.0$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 4$, Game $T=1$, $\alpha = 1.0$, $\gamma = 10.0$, $d_z = 2$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 4$, $\alpha = 0.01$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 6$, $\alpha = 0.001$, $\gamma = 15.0$, $d_z = 2$.
% % \end{itemize}

% % \subsubsection{Concept Shift}

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 4$, Game $T=2$, $\alpha = 1.0$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 4$, Game $T=2$, $\alpha = 1.0$, $\gamma = 10.0$, $d_z = 2$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 6$, $\alpha = 1.0$, $\gamma = 1.0$, $d_z = 2$.
% %     \item Client $T = 8$, $\alpha = 1.0$, $\gamma = 1.0$, $d_z = 2$.
% % \end{itemize}

% % \subsubsection{BoC Exchange Rate}

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 6$, Game $T=2$, $\alpha = 5.0$, $\gamma = 10.0$, $d_z = 2$.
% %     \item Client $T = 3$, Game $T=2$, $\alpha = 5.0$, $\gamma = 1.0$, $d_z = 2$.
% % \end{itemize}


% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 6$, $\alpha = 5.0$, $\gamma = 1.0$, $d_z = 2$.
% %     \item Client $T = 6$, $\alpha = 5.0$, $\gamma = 1.0$, $d_z = 2$.
% % \end{itemize}

% % \subsubsection{ETT Series}

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 3$, Game $T=2$, $\alpha = 1.0$, $\gamma = 1.0$, $d_z = 2$.
% %     \item Client $T = 3$, Game $T=4$, $\alpha = 1.0$, $\gamma = 1.0$, $d_z = 2$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 3$, $\alpha = 5.0$, $\gamma = 1.0$, $d_z = 2$.
% %     \item Client $T = 6$, $\alpha = 5.0$, $\gamma = 1.0$, $d_z = 2$.
% % \end{itemize}









% \subsection{Reservoir Computing via Echo-State Agents}
% \label{s:Examples_ReservoirComputer}
% Lastly, we apply our results to reservoir computers.
% \begin{example}[A Generative Model: Reservoir Computer]
% \label{ex:ResComp}
% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}.  Let $B \in \mathbb{R}^{d_y \times d_y}$ be a random matrix, independent of the $W_t^i$, for all $t$ and $i$.  
% If we allow for a hidden state $Z_t$ generated at any time to be remembered, then we obtain an Echo State Network (ESN), which is a special case of a general reservoir computer
% \begin{equation}
% \label{eq:reservoir}
% \begin{aligned}
% Z_{t}^i\eqdef & \operatorname{ReLU}\bullet\big(
%     A^i x_t + B^i Z_{t-1}^i + b^i + \sigma^i \, W_t^i
% \big) , 
% \\
% \hat{Y}^i_{t+1} \eqdef & \hat{Y}^i_t +  Z_t^i \beta^{i}_t
% .
% \end{aligned}
% \end{equation}
% Two subtle differences between~\eqref{eq:reservoir} and standard ESN formulations is that we allow for the final layer of the ESN to be dynamically updated, which is not usually the case in reservoir computing.  Further,~\eqref{eq:reservoir} updates the residuals unlike standard ESNs. 
% \end{example}

% Unlike the previous types of agents, namely pre-trained transformers and RFN, in this case, there is no simple closed-form available for the expected matrices in Theorem~\ref{thm:NashEqmExistence}.  Rather, we estimate these quantities using standard Monte-Carlo sampling.

% \subsubsection{Periodic Signal}
% \label{s:Experiments__ss:ESN_PS}

% As seen in Figure \ref{fig:esn_periodic_figures}, predictions leveraging the Nash game produce significantly better modeling than those without for the Periodic Signal time series. Without the Nash game, predictions for each time step essentially settle into an average type of behavior without really replicating the periodic dynamics of the series. On the other hand, while not quite reaching the full amplitude, predictions incorporating the game match the oscillations well. As seen in the mixture weights graphs, the server settles into a stable and repeating set of weights without the Nash game after a warm up period. On the other hand, the weights with the Nash game are somewhat more adaptive.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% %     \item Client $T = 2$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
% % \end{itemize}
% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 5$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 3$.
% %     \item Client $T = 5$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 3$.
% % \end{itemize}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/esn/periodic/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/esn/periodic/relative_squared_server_errors.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/periodic/mixture_weights_plot_nash.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/periodic/mixture_weights_plot.pdf}
% %     \caption{Periodic Signal results using ESN Models with and without Nash game synchronization.}
% %     \label{fig:esn_periodic_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/overlaid_server_predictions.pdf}
%             \caption{Overlaid Server Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/relative_squared_server_errors.pdf}
%             \caption{Relative Squared Server Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot_nash.pdf}
%             \caption{Mixture Weights (Nash)}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot.pdf}
%             \caption{Mixture Weights (Standard)}
%         \end{subfigure}
%     \end{tabular}
%     \caption{Periodic Signal results using ESN Models with and without Nash game synchronization.}
%     \label{fig:esn_periodic_figures}
% \end{figure}


% \subsubsection{Logistic Map}

% The Logistic Map time series is quite challenging, especially with a single lag input from which to make predictions. In Figure \ref{fig:esn_logistic_figures}, predictions not incorporating the Nash synchronization step tend to damp out any oscillations, similar to the results for the Periodic Signal series. Nash synchronization helps provide better matching behavior, especially during the more stable periodic behavior spans. 

% However, during periods of instability in the series, the largely damped predictions produced without Nash synchronization outperform those including such synchronization. This phenomenon can be seen, for example, between $t=50$ and $t=65$ or $t=85$ to $t=105$. In spite of this, Nash game synchronization produces notable reductions in prediction error. The distribution of the ratio of squared errors at each time step,
% \begin{align*}
% \frac{(Y^n_{i, t} - y_{i, t})^2}{(Y^g_{i, t} - y_{i, t})^2},
% \end{align*}
% where $i$ is the dimension of the variable and $t$ is the time step. The superscripts $n$ and $g$ denote non-game and game predictions, respectively. In Figure \ref{fig:esn_logistic_figures}, a majority of these ratios are above $1.0$.

% The best hyper-parameters for the game setting with two and five experts, respectively, are:
% \begin{itemize}
%     \item Client $T = 2$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 3$.
%     \item Client $T = 5$, Game $T=3$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 6$.
% \end{itemize}

% The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% \begin{itemize}
%     \item Client $T = 2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 3$.
%     \item Client $T = 2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 3$.
% \end{itemize}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/esn/logistic/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/esn/logistic/relative_squared_server_errors.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/logistic/mixture_weights_plot_nash.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/logistic/mixture_weights_plot.pdf}
% %     \caption{Logistic Map results using ESN Models with and without Nash game synchronization.}
% %     \label{fig:esn_logistic_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/overlaid_server_predictions.pdf}
%             \caption{Overlaid Server Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/relative_squared_server_errors.pdf}
%             \caption{Relative Squared Server Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot_nash.pdf}
%             \caption{Mixture Weights (Nash)}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot.pdf}
%             \caption{Mixture Weights (Standard)}
%         \end{subfigure}
%     \end{tabular}
%     \caption{Periodic Signal results using ESN Models with and without Nash game synchronization.}
%     \label{fig:esn_periodic_figures}
% \end{figure}


% \subsubsection{Concept Shift}

% The Concept Drift dataset incorporates multidimensional inputs and targets. As in previous results, use of the Nash game provides a significant advantage for this dataset. As shown in Figure \ref{fig:esn_concept_figures}, the predictions produced by the server using Nash synchronization are much more tightly bound to the target curves. This is even more evident when examining the ratio of squared errors between the two methods. 

% As discussed in Section \ref{datasets}, the Concept Drift time series goes through an abrupt, but smooth, transition in the relationship between the input and output variables. This transition occurs between time step $88$ and $112$. The onset of this transition is evident in the mixture weights computations of both methods. The dynamics of these weights changes significantly during this period. The transition also appears to briefly impact the efficacy of the Nash synchronization, evidenced by a degradation and eventual recovery of the ratio of errors between the non-game and game predictions during this time-frame.

% It is interesting to note that, for this dataset, there are clearly experts in the ensemble that struggle to produce helpful predictions. Two of the clients in the Nash-game setting hover around zero weight in the ensemble, while three experts in the non-game setting are assigned weights near zero a various points in the series.  All hyperparameter choices are recorded in Appendix~\ref{s:OptimalParamterChoices__a:TransExpHyper}.

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/esn/concept/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/esn/concept/relative_squared_server_errors.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/concept/mixture_weights_plot_nash.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/concept/mixture_weights_plot.pdf}
% %     \caption{Concept Drift results using ESN Models with and without Nash game synchronization.}
% %     \label{fig:esn_concept_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/overlaid_server_predictions.pdf}
%             \caption{Overlaid Server Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/relative_squared_server_errors.pdf}
%             \caption{Relative Squared Server Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/mixture_weights_plot_nash.pdf}
%             \caption{Mixture Weights (Nash)}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/mixture_weights_plot.pdf}
%             \caption{Mixture Weights (Standard)}
%         \end{subfigure}
%     \end{tabular}
%     \caption{Concept Drift results using ESN Models with and without Nash game synchronization.}
%     \label{fig:esn_concept_figures}
% \end{figure}


% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 10$, Game $T=3$, $\alpha = 0.1$, $\gamma = 1.0$, $\sigma = 0.01$, $d_z = 3$.
% %     \item Client $T = 5$, Game $T=2$, $\alpha = 0.001$, $\gamma = 1.0$, $\sigma = 0.01$, $d_z = 3$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 6$.
% %     \item Client $T = 2$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 3$.
% % \end{itemize}

% \subsubsection{BoC Exchange Rate}

% As outlined in Section \ref{datasets}, the BoC Exchange Rate series incorporates a number of lagged input currency exchange rates and lagged target currency exchange rates. With these additional inputs, the server predictions for both the Nash game and non-Nash game settings closely follow the target exchange rate. Considering the ratios of squared errors exhibited in Figure \ref{fig:esn_boc_figures}, the bulk of time steps have ratios above $1.0$, indicating better performance from predictions leveraging Nash game synchronization than those without.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 5$, Game $T=3$, $\alpha = 0.001$, $\gamma = 1.0$, $\sigma = 1.0$, $d_z = 6$.
% %     \item Client $T = 5$, Game $T=2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 6$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 0.001$, $\gamma = 10.0$, $\sigma = 0.01$, $d_z = 6$.
% %     \item Client $T = 3$, $\alpha = 0.1$, $\gamma = 10.0$, $\sigma = 1.0$, $d_z = 6$.
% % \end{itemize}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/esn/boc/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/esn/boc/relative_squared_server_errors.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/boc/mixture_weights_plot_nash.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/boc/mixture_weights_plot.pdf}
% %     \caption{BoC Dataset results using ESN Models with and without Nash game synchronization.}
% %     \label{fig:esn_boc_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/boc/overlaid_server_predictions.pdf}
%             \caption{Overlaid Server Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/boc/relative_squared_server_errors.pdf}
%             \caption{Relative Squared Server Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/boc/mixture_weights_plot_nash.pdf}
%             \caption{Mixture Weights (Nash)}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/boc/mixture_weights_plot.pdf}
%             \caption{Mixture Weights (Standard)}
%         \end{subfigure}
%     \end{tabular}
%     \caption{BoC Dataset results using ESN Models with and without Nash game synchronization.}
%     \label{fig:esn_boc_figures}
% \end{figure}


% \subsubsection{ETT Series}
% \label{s:ESN_ETT}

% As with the Boc Exchange Rate series, the ETT series incorporates several informative input variables and lagged values of the target oil temperature. As such, both the Nash and non-Nash game predictions follow the target fairly closely. However, as in other oscillatory series, predictions without the Nash game are more smoothed. The predictions incorporating Nash synchronization tend to produce better matches to the magnitudes of the various spikes in the oil temperature throughout the series. The squared-error ratios are more evenly distributed around $1.0$ than in other settings. However, the majority remains above the critical threshold of $1.0$.

% % The best hyper-parameters for the game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, Game $T=2$, $\alpha = 5.0$, $\gamma = 1.0$, $\sigma = 1.0$, $d_z = 1$.
% %     \item Client $T = 2$, Game $T=2$, $\alpha = 5.0$, $\gamma = 1.0$, $\sigma = 1.0$, $d_z = 1$.
% % \end{itemize}

% % The best hyper-parameters for the non-game setting with two and five experts, respectively, are:
% % \begin{itemize}
% %     \item Client $T = 2$, $\alpha = 5.0$, $\gamma = 1.0$, $\sigma = 1.0$, $d_z = 3$.
% %     \item Client $T = 3$, $\alpha = 5.0$, $\gamma = 1.0$, $\sigma = 1.0$, $d_z = 3$.
% % \end{itemize}

% % \begin{figure}[ht!]
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/esn/ett/overlaid_server_predictions.pdf}
% %     \includegraphics[width=0.95\linewidth]{figures/esn/ett/relative_squared_server_errors.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/ett/mixture_weights_plot_nash.pdf}
% %     \includegraphics[width=0.475\linewidth]{figures/esn/ett/mixture_weights_plot.pdf}
% %     \caption{ETT Series results using ESN Models with and without Nash game synchronization.}
% %     \label{fig:esn_ett_figures}
% % \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/ett/overlaid_server_predictions.pdf}
%             \caption{Overlaid Server Predictions}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/ett/relative_squared_server_errors.pdf}
%             \caption{Relative Squared Server Errors}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/ett/mixture_weights_plot_nash.pdf}
%             \caption{Mixture Weights (Nash)}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.48\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/ett/mixture_weights_plot.pdf}
%             \caption{Mixture Weights (Standard)}
%         \end{subfigure}
%     \end{tabular}
%     \caption{ETT Series results using ESN Models with and without Nash game synchronization.}
%     \label{fig:esn_ett_figures}
% \end{figure}




% % \begin{algorithm}[H]%[ht]
% % \caption{Synchronization Subroutine}
% % \label{alg:sync_subroutine}
% % \begin{algorithmic}
% % \SetAlgoLined
% % \Require Observed target values $\{ ( y^1_t, ..., y^N_t ) \}_{t=0}^T$. 
% % \State Mixture weights $w_\cdot = \{ (w^1_t, ..., w^N_t) \}_{t=0}^T$ $\leftarrow$ Run: Algorithm~\ref{alg:FedMain}
% % \DontPrintSemicolon
% % \State \SetKwBlock{ForParallel}{for $i:1,\dots,N$ in parallel}{end}
% %     \State 
% %     \tcp{Initialize Updates} 
% % \State    $\mathbf{w}_T=(w^1_T I_{d_{y}}, ..., w^N_T I_{d_{y}})^\top$
% %   \State \ForParallel{
% %     \State $P_i(T)  = \mathbf{w}_T \mathbf{w}_T^\top$ 
% %     \State $S_i(T) = - \mathbf{w}_T y_T$ 
% % }


% %     \State \tcp{Generate Iterates}
% %     \State \For{$t=T-1,\dots,0$}{
% %         \State \tcp{Update Driving Parameters} 

% % \State $\mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top$ 
% % \State $\mathbf{A}(t)=  \big[ \mathbb{E} \big( Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big) \big]_{i,j=1}^N$ 
% % \State $\mathbf{B}(t)= \big[ \mathbb{E} \big( Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \big) \big]_{i=1}^N$ 
% % \State $\mathbf{C}(t)= \big[ \mathbb{E} \big( Z^{i\top}_t \mathbf{e}_i^\top S_i(t+1) \big) \big]_{i=1}^N$ 
% % \State $\mathbf{D}(t)= \big[ \mathbb{E}( \mathbf{e}_i Z^i_t ) \big]_{i=1}^N$


% % \ForParallel{
% % \State 
% % \hspace{-0.3cm}
% % $P_i(t)=  e^{-\alpha_i (T-t)} \mathbf{w}_t \mathbf{w}_t^\top $ 
% % $ + [ \mathbf{D}(t)(  e^{-\boldsymbol{\alpha}(T-t)}  \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]^\top P_i(t+1) [  \mathbf{D}(t)( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]$
% % $ + e^{-\alpha_i (T-t) } \gamma_i [ \mathbf{e}_i^\top ( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ]^\top  [ \mathbf{e}_i^\top ( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ] $  

% % \vspace{0.3cm}
% % \State 
% % \hspace{-0.3cm}
% % $S_i(t) = e^{-\alpha_i(T-t)} \gamma_i \mathbf{B}(t)^\top ( e^{-\boldsymbol{\alpha}(T-t)}  \Gamma + \mathbf{A}(t))^{-1} 
% %    \mathbf{e}_i \mathbf{e}_i^\top   
% %  ( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{C}(t)  $

% % $+ \mathbf{B}(t)^\top ( e^{-\boldsymbol{\alpha}(T-t)}  \Gamma + \mathbf{A}(t))^{-1} 
% %    \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t)  
% %  ( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{C}(t) $ 

% %  $ - P_i(t+1) \mathbf{D}(t)( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{C}(t)$  
 
% %  $-  \mathbf{B}(t)^\top ( e^{ -\boldsymbol{\alpha} (T-t)} \Gamma + \mathbf{A}(t))^{-1}\mathbf{D}(t)^\top S_i(t+1) 
% %  +  S_i(t+1)   - e^{-\alpha_i(T-t)} \mathbf{w}_t y_t $ 
% %  }
% % }


% % \State\For{$t=0, ..., T-1$}{
% %   \State\tcp{Update Game Strategy} 

% % \State 
% % $\boldsymbol{\beta}_t = [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top 
% % = - \big[  e^{ -\boldsymbol\alpha (T-t)}  \Gamma + \mathbf{A}(t) \big]^{-1} 
% % \big( \mathbf{B}(t) \hat{Y}_t + \mathbf{C}(t) \big)$ 


% % }

% % \State \Return $\boldsymbol{\beta}_t$ for $t=0, 1, ..., T-1$
% % \end{algorithmic}
% % \end{algorithm} 





% % Next, we analyze Algorithm~\ref{alg:FedMain} and the subroutine in Algorithm~\ref{alg:sync_subroutine}.
% % \section{Theoretical Analysis}
% % \label{s:Analysis}

% % Our theoretical analysis of Algorithms~\ref{alg:FedMain} and~\ref{alg:sync_subroutine} is broken tinto two steps.  First, we analyze the optimality of the server/(major agent), which mixes the prediction generated by the $N$ experts (minor agents).  Then, we analyze the optimality of the prediction generated by each agent either in the (slow) synchronization phase, where a random subset of $b$ agents plays a Nash game to synchronize their linear encoders, or in the (fast) intermediate times, where each expert selfishly optimizes their linear readout layer independently of the behaviour of the other experts.

% % \subsubsection{The Server's Optimal Mixting Problem}
% % \label{s:Optimal_Server__akaMajoragent}

% % Consider the objective of the major agent/central planner is to optimize 
% % \begin{align} 
% %     \min_{w_{\cdot}}\,
% %  J_0(w) = \mathbb{E}  \sum_{t=1}^T e^{-\alpha^0 t } \Big[  
% %  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{y}^j_t \Big\|^2 
% %   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] .  
% %   \label{DTJ0}
% % \end{align} 
% % where the minimization is taken over all decision rules $w_{\cdot} \eqdef \{w_t\}_{t=1}^T = \{(w^1_t, ..., w^N_t)\}_{t=1}^T$ whose paths lie in the $N$-simplex $\Delta_N \eqdef  \{w\in [0,1]^N:\, \sum_{n=1}^N\, w_n=1\}$.  
% % Our first main result shows that there exists a unique solution to the optimization problem~\eqref{DTJ0}.
% % \begin{theorem}[Optimal Coordination]
% % \label{thm:OptimalWeights}
% % The quadratic programming problem \eqref{Majoragent:QP} admits a unique solution $w^\star = (w^{1, \star}, ..., w^{N, \star})$ given by 
% % \begin{align} 
% % \notag
% %   w^\star   =   \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_t^\top  y_t 
% % % \\    
% %   % &
% %   -  & \Big[ N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big]^{-1}   G^\top 
% %   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
% %   \\
% %   &\times 
% %  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \mathrm{K} \Big)^{-1} \hat{Y}^\top_t  y_t  -  \mathbf{c} \Big] . 
% %   \label{eqn:OptimalWeights}  
% % \end{align} 
% % where we denote 
% % \begin{align} 
% %  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N}, 
% %  \quad 
% %  G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
% %  \mbox{ and }
% %  \quad 
% %   \mathbf{c} =  \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
% %   \label{eq:Gc_Def}
% % \end{align} 

% % \end{theorem} 




% \begin{comment}
% We consider a model with $N$ agents $\{\mathcal{A}_i\}_{i=1}^N$. 
% Let each agent $\mathcal{A}_i$ has input signal sequence $\{Z^i_t\}_{t\geq 0}$ and a linear decoder.  
% \AK{This needs to be updated, but only at the end.}[.]
% \begin{equation}
% \begin{aligned} 
% & X^i_{t+1} =  A_i X^i_t + \sigma W^i_t , \quad X^i_\cdot \in \mathbb{R}^{dx \times 1} , \\  
% & Z^i_{t+1} =  \varphi(Z^i_t, X^i_{t+1}) ,  \quad Z^i_\cdot \in \mathbb{R}^{d_{z} \times 1} ,  \\ 
% & \hat{Y}^i_{t+1} = \hat{Y}^i_t + \beta^{i\top}_t Z^i_t , \quad \hat{Y}^i_\cdot \in \mathbb{R}^{d_{y} \times 1} , \ i = 1, ..., N ,   
% \end{aligned} 
% \label{DTRCsystem}
% \end{equation} 
% where $W^i_t$, $i=1$, ..., $N$, $t=0$, ..., $T$ are identically independently distributed standard normal random variables. 
% \end{comment}

% \begin{comment}
% Consider a central planner/major agent who also acts as a central planner and chooses weight vector sequence on the $N$-simplex   
% \begin{align} 
% w_t= (w^1_t, ..., w^N_t)^\top \in \Delta_N , \quad t = 0, 1, ..., T \notag  
% \end{align} 
% for the minor agents' output $\hat{Y}^i$ in order to minimize the total loss  
% \begin{align} 
%  J_0(w) = \mathbb{E}  \sum_{t=1}^T \Big[ 
%  \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j_t \big\|^2 \Big] ,  
%   \notag 
%   \label{DTJ0}
% \end{align} 
% where $y^i_\cdot$, $i=1$, ..., $N$ are the observed target values, and all $\kappa_j>0$.  

% Given the weight $w_t = (w^1_t, ..., w^N_t)$, $t=0$, $1$, ..., $T$, each minor agent $\mathcal{A}_i$ 
% chooses $\{\beta^i_t\}_{t=0}^T$ non-cooperatively to minimize the individual cost 
% \allowdisplaybreaks
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y^i_T - \sum_{j=1}^N w^j_T \hat{Y}^j_T \Big\|^2 \Big\}   , \quad i = 1, ..., N ,  \label{eq:Objective_nth_expert}  
%   \end{align} 
%  where $\beta^{-i}=(\beta^1, ..., \beta^{i-1}, \beta{i+1}, ..., \beta^N)$. 
% \end{comment}



% \begin{comment} 
% \subsection{The Nash Equilibrium between the Minor agents}
% Denote 
% \begin{align} 
%  & \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top, \quad \hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top, \quad   
% \mathbf{e}^N_i = e^N_i \otimes I_{d_{z}} = [0, ..., I_{d_{z}} , ..., 0]^\top,  \notag \\ 
%  & \Gamma = \diag[\gamma_1, ..., \gamma_N] \notag 
% \end{align} 
% then the costs \eqref{eq:Objective_nth_expert} for the $N$ agents can be written as  
% \begin{align} 
%  & J_i(\beta^i, \beta^{-i}) = \mathbb{E} \Big\{  \sum_{t=0}^{T-1} \Big[ \Big\| y_t - \mathbf{w}^\top_t \hat{Y}_t \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2  \Big]  + \Big\| y_T - \mathbf{w}_T^\top \hat{Y}_T \Big\|^2 \Big\}   , \quad i = 1, ..., N. 
%   \label{eq:Objective_nth_expertcompact}
%  \end{align} 

%  We aim to find a set of Nash equilibrium strategies $(\beta^1, ..., \beta^N)$ for the $N$ agent such that 
%  \begin{align} 
%  J_i(\beta^i, \beta^{-i}) 
%  \leq J_i(u, \beta^{-i}), 
%  \quad \forall u \in \mathbb{R}^{d_{z} \times d_{y}} , 
%  \quad  \forall i = 1, ..., N. \label{NEbeta}
%  \end{align} 
% \end{comment} 


% % We introduce the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% % $t=0$, $1$ ..., $T$. 
% % \begin{equation} 
% % \begin{cases}  
% %   P_i(t) = 
% %  [ \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]^\top P_i(t+1) [  \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I ]  \\ 
% %   \hspace{2cm} + [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ]^\top 
% %  [ \mathbf{e}_i^\top \mathbf{D}(t)( \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) ] 
% %  + \mathbf{w}_t \mathbf{w}_t^\top  \\ 
% %   \Gamma + \mathbf{A}(t) \, \text{is invertible}  \\ 
% %   P_i(T) =  \mathbf{w}_T \mathbf{w}_T^\top  , \quad i = 1, 2, ..., N , 
% %  \end{cases}
% %  \label{eqn:Pi}
% %  \end{equation} 

% % \allowdisplaybreaks 
% % \begin{equation}  
% %  \begin{cases} 
% %   S_i(t) =   \mathbf{B}(t)^\top (I + \mathbf{A})^{-1} 
% %  [\mathbf{e}_i \mathbf{e}_i^\top + \mathbf{D}(t)^\top P_i(t+1) \mathbf{D}(t) ] (I+\mathbf{A})^{-1} \mathbf{C}   \\ 
% %   \hspace{1cm} - P_i(t+1) \mathbf{D}(I+\mathbf{A})^{-1} \mathbf{C} 
% %  - \mathbf{B}^\top (I + \mathbf{A})^{-1}\mathbf{D} S_i(t+1) 
% %  - \mathbf{w}_t y_t 
% %  + S_i(t+1) , 
% %   \\ 
% %  S_i(T) = - \mathbf{w}_T y_T   . 
% % \end{cases}   
% % \label{eqn:Si}
% % \end{equation} 
% % %
% % %
% % %
% % In \eqref{eqn:Pi} and \eqref{eqn:Si}, the matrices $\mathbf{A}(\cdot)$,  
% % $\mathbf{B}(\cdot)$, $\mathbf{C}(\cdot)$, and $\mathbf{D}(\cdot)$ are defined by  
% % \allowdisplaybreaks 
% % \begin{align} 
% % &\mathbf{A}(t) = \begin{bmatrix} 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_1 Z^{1\top}_t ] & 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_1 Z^{1\top}_t)^\top P_1(t+1) e_N Z^{N\top}_t ] \\ 
% %  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_1 Z^{1\top}_t ] & 
% %  \mathbb{E} [(e_2 Z^{1\top}_t)^\top P_2(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_2 Z^{2\top}_t)^\top P_2(t+1) e_N Z^{N\top}_t ] \\ 
% %  \vdots & \vdots & \ddots & \vdots \\ 
% %  \mathbb{E}[ (e_N Z^{N\top}_t)^\top P_N(t+1) e_1 Z^{1\top}_t ]& 
% %  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_2 Z^{2\top}_t ]
% %  & \cdots & 
% %  \mathbb{E} [ (e_N Z^{N\top}_t)^\top P_N(t+1) e_N Z^{N\top}_t ]
% % \end{bmatrix} \notag \\ 
% % & \mathbf{B}(t) = 
% %  \begin{bmatrix} 
% %  \mathbb{E} (e_1 Z^{1\top}_t )^\top P_1(t+1) \\ 
% %  \mathbb{E}(e_2 Z^{2\top}_t )^\top P_2(t+1) \\ 
% %  \vdots \\  
% %  \mathbb{E} (e_N Z^{N\top}_t) P_N(t+1) 
% %  \end{bmatrix} ,  
% %  \qquad 
% %  \mathbf{C}(t) = 
% %  \begin{bmatrix} 
% %  \mathbb{E}(e_1 Z^{1\top}_t )^\top S_1(t+1) \\ 
% %  \mathbb{E}(e_2 Z^{2\top}_t )^\top S_2(t+1) \\ 
% %  \vdots \\ 
% %  \mathbb{E}(e_N Z^{N\top}_t) S_N(t+1) 
% %  \end{bmatrix} , 
% %  \notag \\ 
% % & \mathbf{D}(t) 
% %  = 
% %  \begin{bmatrix} 
% %  \mathbb{E}( e_1 Z^{1\top}_t ) , \, 
% % \mathbb{E} ( e_2 Z^{2\top}_t ) ,  \,
% %  \cdots , \, 
% % \mathbb{E} ( e_N Z^{N\top}_t )
% %  \end{bmatrix} . 
% %  \notag 
% % \end{align} 

% % The following proposition links the existence of a Nash equilibrium of \eqref{DTRCsystem} and \eqref{eq:Objective_nth_expert} to the solvability of the system \eqref{eqn:Pi}. 
% % \begin{proposition}[Nash Equilibrium of Minor agents]
% % \label{prop:NashEqmExistence}
% % Suppose the system \eqref{eqn:Pi} for $(P_i)_{i=1}^N$ admits a solution for $t=0$, $1$, ..., $T$.  
% % Then the $N$-agent Nash game \eqref{eq:Objective_nth_expert} admits a unique feedback Nash equilibrium 
% % \begin{align} 
% % \boldsymbol{\beta}_t = [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top = - ( \Gamma + \mathbf{A}(t) )^{-1} 
% % \big( \mathbf{B}(t) \hat{Y}_t + \mathbf{C}(t) \big) , \quad t = 0, 1, ..., T. 
% % \label{eqmvecbeta} 
% % \end{align} 
% % \end{proposition}




% % \subsection{Parallelized Selfish Expert Optimization}
% % \label{s:ShortComm}
% % We first express the optimal control of the local model, when optimizing their predicting performance before the synchronization time $T$.

% \subsection{Ablation Studies}
% \label{s:Experiments__ss:Ablation}
% In this section, we examine the effects of the principal knobs and hyperparameters driving the behaviour of our online federated learning algorithm. Specifically, we examine the impact of the lookback parameter ($T$) in the Nash games and the effect of varying the game frequency (especially on the trade-off between run-time of our FL algorithm and its predictive power).


% \subsubsection{Effect of Nash Game Lookback Length}
% \label{s:Experiments__ss:Ablation___sss:Lookback}

% The ``lookback'' length, or number of steps backwards in time considered in the Nash game calculations, is an important hyper-parameter. This length not only affects prediction accuracy but also the computational cost, as the longer the lookback, the more calculations are necessary. In this section, the effect of increasing lookback length is considered for RFN models applied to the BoC Exchange Rate and ETT datasets in the 5-client setting. The optimal hyper-parameters discussed in Section \ref{rfn_results} are applied with the exception of variation in the Game $T$, which takes values in the set $\{2, 3, 4, 5, 6, 7, 8, 9, 10, 15, 25\}$.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.49\linewidth]{figures/lookback/min_mses_over_lookback_boc_5c.pdf}
%     \includegraphics[width=0.49\linewidth]{figures/lookback/min_mses_over_lookback_ett_5c.pdf}
%     \caption{Variations in Minimum MSE for RFN models with varying Nash game lookback lengths for the BoC Exchange Rate (left) and ETT (right) time series using 5 experts.}
%     \label{fig:lookback_results}
% \end{figure}

% Similar to the Client $T$ value for local ridge regression, the optimal lookback length is dataset specific, dependent on the decay parameter $\alpha$, and not monotonic in nature. Results of the experiments are displayed in Figure \ref{fig:lookback_results}. Departing slightly from previous results, the figure reports the minimum MSE seen across three separate RFN models with different seeds. As lookback length increases, it is likely that the optimal hyper-parameters differ significantly from those found in Section \ref{rfn_results}. As such, the time series predictions sometimes become unstable with longer lookback lengths. If none of the three runs produced an MSE less than $1.0$, they are excluded from the figure. The optimal lookback length for the BoC Exchange Rate and ETT time series are $5$ and $3$, respectively, with the minimum MSE growing steadily thereafter. Encouragingly, there are other lookback values near the optimum with good performance.


% \subsubsection{Nash Game Frequency and Run-Time/Performance Trade-off}
% \label{s:Experiments__ss:Ablation___sss:Runtime}

% Given the computational overhead associated with computing the Nash equilibrium, increasing the frequency with which the Nash computations are performed increases prediction latency. In this section, the run time overhead imposed by playing the Nash game is measured. As discussed above, synchronizing predictions at every step is optimal in the experiments, but this comes at a cost of increased run time. ESN models are expected to incur the largest run time overhead as solutions to the Nash system require the approximation of a number of expectations. These approximations are computed with Monte-Carlo simulations using $100$ samples for each expectation when performing synchronization. The computational cost is considerably less for RFN models due to the analytical expressions for such expectations. Pretrained models impose the least run time overhead when playing the Nash game. Table \ref{tab:runtime} reports the mean run times over the three random seeds for the Period and Boc Exchange Rate time series using ESN, RFN, and Transformer models with and without Nash synchronization. The optimal hyper-parameters, outlined in Sections \ref{esn_results}-\ref{transformer_results} are applied and Nash synchronization occurs at each step, when it is used.

% Total time for RFN model predictions is shorter than that of ESN models by approximately a factor of $40$. Subsequently, transformer models are faster than RFNs by roughly a factor of $2$, making these models a good choice when prediction latency is important. On the other hand, without the Nash game, Transformers have the longest run time compared to other models due to their computational overhead. It should be noted that significant computation optimizations have not been pursued in solving the Nash game systems. For example, the Monte Carlo simulations are sequential but are embarrassingly parallelizable in practice.

% \begin{table}[ht!]
%     \centering
%     \caption{Run time measurements in seconds for simulations with five experts. Nash synchronization occurs each step when the technique is applied, and all optimal hyper-parameters are used.}
%     \begin{tabular}{llcccc}
%     \toprule
%      & & \multicolumn{2}{c}{Nash Game} & \multicolumn{2}{c}{No Nash Game} \\
%     Model & Dataset & Total (s) & Per Step (s) & Total (s) & Per Step (s) \\
%     \midrule
%      \multirow{2}{*}{ESN} & Periodic & $1.88\mathrm{e}{\text{+}3}$s & $9.41\mathrm{e}{\text{-}0}$s & $4.24\mathrm{e}{\text{-}1}$s & $ 2.12\mathrm{e}{\text{-}3}$s\\
%      & BoC & $2.00\mathrm{e}{\text{+}4}$s & $1.00\mathrm{e}{\text{-}1}$s & $4.24\mathrm{e}{\text{-}0}$s & $2.11\mathrm{e}{\text{-}3}$s\\
%      \multirow{2}{*}{RFN} & Periodic & $5.28\mathrm{e}{\text{+}1}$s & $2.64\mathrm{e}{\text{-}1}$s & $3.68\mathrm{e}{\text{-}1}$s & $1.84\mathrm{e}{\text{-}3}$s\\
%      & BoC & $5.08\mathrm{e}{\text{+}2}$s & $2.54\mathrm{e}{\text{-}1}$s & $4.07\mathrm{e}{\text{-}0}$s & $2.03\mathrm{e}{\text{-}3}$s \\
%      \multirow{2}{*}{Transformer} & Periodic & $1.96\mathrm{e}{\text{+}1}$s & $9.80\mathrm{e}{\text{-}2}$s & $1.67\mathrm{e}{\text{-}0}$s & $8.34\mathrm{e}{\text{-}3}$s\\
%      & BoC & $1.59\mathrm{e}{\text{+}2}$s & $7.93\mathrm{e}{\text{-}2}$s & $1.81\mathrm{e}{\text{+}1}$s & $9.03\mathrm{e}{\text{-}3}$s \\
%      \bottomrule
%     \end{tabular}
%     \label{tab:runtime}
% \end{table}

% A considerable performance advantage when synchronizing with the Nash game may be preserved by performing such synchronizations less frequently. Consider the BoC Exchange Rate dataset and an RFN model. With optimal hyper-parameters, tuned for the synchronization frequency, if Nash synchronization occurs every $10$ steps, instead of every step, the run time is reduced by a factor of more than $7.5$, and the resulting MSE remains below that of the non-game setting. Specifically, a synchronization frequency of $10$ results in an average MSE of $5.82080\mathrm{e}{\text{-}4}$ over $67.027$s compared with the non-game mean MSE of $3.15237\mathrm{e}\text{-}3$ and average run time of $4.069$s.


% % \bibliographystyle{spmpsci}      % mathematics and physical sciences
% %\bibliographystyle{spphys}       % APS-like style for physics
% %\bibliographystyle{plain} %plain
% \bibliography{Refs}   % name your BibTeX data base

% % \newpage


% \appendix
% \section{Proofs}
% \label{s:Proofs}

% This section contains the proofs of our main results.

% \subsection{{Proof of Proposition~\ref{prop:localgreedyupdates}}}
% \begin{proof}%[{Proof of Proposition~\ref{prop:localgreedyupdates}}]
% Observe that the loss function in~\eqref{eq:ridge_local} can be re-written as
% \allowdisplaybreaks
% \begin{align}
% \label{eq:redux_ridge}
% \begin{aligned}
%         & \sum_{s=0}^t\,
%             e^{ -\alpha_i(t-s)}
%             \,\big\|(y_s-\hat{Y}_s^i) - Z_s^i \beta_t^i \big\|^2
%             +
%             \gamma_i\big\|\beta_t^i\big\|^2
%     \\
%     & =
%         \sum_{s=0}^t\,
%             \,\big\| e^{-\alpha_i(t-s)/2}
%                 (y_s-\hat{Y}_s^i)
%              - (e^{-\alpha_i(t-s)/2} Z_s^i) \beta^i_t \big\|^2
%      +
%             \gamma_i\big\|\beta_t^i\big\|^2  \\ 
%     & = \big( \bar{y}^i_t - X^i_t \beta^i_t \big)^\top \big( \bar{y}^i_t - X^i_t \beta^i_t \big) 
%      + \gamma_i \beta^{i\top}_t \beta^i_t 
% \end{aligned}
% \end{align}
% and the last line of~\eqref{eq:redux_ridge} is simply a standard ridge-regression problem.  Since this is a strictly convex problem, there is a unique $\beta_t^i\in \mathbb{R}^{d_y\times d_x}$ minimizing the last line of~\eqref{eq:redux_ridge}.  The desired closed-form expression is given in \citep[Equation (3.44)]{HastieTibshiraniFriedman_2001ESLBook}.
% \end{proof}




% \begin{comment}
% \subsection{{Proof of Theorem~\ref{thm:OptimalWeights}}}
% \label{s:Proofs__ss:OptimalWeights}
% Fix a hyperparameter $\eta\le 0$ and consider a time $s\in \mathbb{N}$.
% We will now optimize the objective in~\eqref{DTJ0} over the constraint set defined in~\eqref{eq:Generalized_Simplex_Constraint}.  
% Observe that the major agent thus seeks to solve the nonlinear programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N) }  e^{-\alpha(t-s)} \Big\{ \big\| y_s - \sum_{j=1}^N w^j \hat{y}^j_s \big\|^2 
%  + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 \Big\} \\ 
% & \text{subject to} 
% \,\,
% \mathbf{g}(w)=
% % (w^1-1, ..., w^N-1, -w^1, ..., -w^N)
% % ( -w^{\add{2}}, ..., -w^N)
% %%% AK Relaxation
% (\add{w^{1}}, -w^{\add{2}}, ..., -w^N)
% \leq 
% (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
% \eqdef \mathbf{c}
% % , 
% % \\ 
% % & \hspace{1.45cm}
% % \,\,
%  % h(w) = w^1 + ... + w^N - 1 = 0 
% ,
% \end{aligned} 
% \label{Majoragent:NLoptim}
% \end{equation} 
% where, for any $m\in \mathbb{N}_+$ we denote $\mathbf{1}_m\in \mathbb{R}^m$ given for each $i=1,\dots,m$ by $(\mathbf{1}_m)_i=1$.
% % \AK{Check if notation still needed:} 
% % Denote 
% % \begin{align} 
% % % \hat{\mathbf{Y}}_t = \big[ \hat{y}^1_t, \cdots , \hat{y}^N_t \big] , \quad 
% %   \mathbf{1}_{1\times N} = \big[ 1, ..., 1 \big] \in \mathbb{R}^{1\times N} , \quad 
% %  % \hat{\boldsymbol{\lambda}} = \big[ \hat{\lambda}_1, ..., \hat{\lambda}_N \big]^\top , \quad 
% %  % \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N} . \notag 
% % \end{align} 



% Since the objective function of the nonlinear programming problem \eqref{Majoragent:NLoptim} can be written as 
% \begin{align} 
%  & e^{-\alpha(t-s)} \Big\{ \Big\| y_s - \sum_{j=1}^N w^j \hat{y}^j_s \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2  \Big\}  \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ \Big( y^\top_s - \sum_{j=1}^N w^j \hat{y}^{j\top}_s \Big) 
%  \Big( y_s - \sum_{j=1}^N w^j \hat{y}^j_s \Big) + \sum_{j=1}^N \kappa_j w^{j 2} \Big\}   \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ N \sum_{i,j=1}^N w^i \hat{y}^{i\top}_s \hat{y}^j_s w^j 
%   - 2  y^\top_s   \sum_{j=1}^N w^j \hat{y}^j_s 
%    +  y^\top_s y_s + \sum_{j=1}^N \kappa_j w^{j 2} \Big\}  \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ w^\top \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) w 
%   - 2  y^\top_s  \hat{\mathbf{Y}}_s w 
%    + y^\top_s y_s \Big\} . \notag 
% \end{align} 
% Therefore the nonlinear programming problem \eqref{Majoragent:NLoptim} is equivalent to the following quadratic programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N)^\top }  \frac{1}{2}  w^\top e^{-\alpha(t-s)}\big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s     + \mathrm{K} \big) w 
%   - e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s w  , \\ 
% & \text{subject to} \ G w \leq \mathbf{c} ,
% \end{aligned} 
% \label{Majoragent:QP}
% \end{equation} 
% where $G$ and $\boldsymbol{c}$ are defined in~\eqref{eq:Gc_Def}; whose definition we recall here
% \begin{align} 
%  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N]
%  % \in \mathbb{R}^{N\times N}
%  , 
%  \,
%  % Shifted Orthant
%   % G = -I_N
%   %% Full Simplex
%  % G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  % Hyperplane containing simplex
%  % G = \begin{bmatrix} 
%  % \mathbf{1}_{1\times N} \\
%  % - \mathbf{1}_{1\times N}  
%  % \end{bmatrix} 
%  %%% Annie Relaxation
%  G = 
%  \begin{pmatrix}
%      1 & \mathbf{0}_{1\times N} \\
%      \mathbf{0}_{ (N \times 1) } & -I_{(N-1\times N-1)} 
%  \end{pmatrix}
%  \,\mbox{ and }\,
%  % \quad 
%  %  
%  \mathbf{c} = 
%  % Shifted Orthant
%  % 0_{N\times 1}
%  % \bar{\eta}
%  %% Full Simplex
%  % \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%  % Hyperplane containing simplex
%  % \begin{bmatrix} 
%  % 1 
%  % \\ 
%  % -1   
%  % \end{bmatrix}
%  %%% Annie Relaxation
%  (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
%   \label{eq:Gc_Def}
% \end{align} 
% \add{where for each $n,m\in \mathbb{N}_+$, $\mathbf{0}_{n,m}$ denotes the $n\times m$ zero matrix and $I_n$ the $n\times n$ identity matrix.
% Likewise, $\operatorname{diam}(\kappa_1,\dots,\kappa_N)$ denotes the $N\times N$-diagonal matrix whose diagonal is given, for each $i=1,\dots,N$, by $K_{i,i}=\kappa_i$.
% }



% To prove Theorem~\ref{thm:OptimalWeights}, we need to use the results of the following Theorems~\ref{thm:NSQP} and \ref{thm:QPdual} from \cite{Berkovitz2001}. 
% According to \cite[Theorem V.6.1]{Berkovitz2001}, the following theorem gives a necessary and sufficient condition for solutions of \eqref{Majoragent:QP}. 
% \begin{theorem} 
% \label{thm:NSQP}
% A necessary and sufficient condition for a point $w^\star=(w^{1, \star}, ..., w^{N, \star})^\top$ to be a solution of the quadratic programming problem \eqref{Majoragent:QP} is that 
% \begin{align} 
% G w^\star \leq \mathbf{c} \label{NSQP:Gw<=c} 
% \end{align} 
% and there exists a vector $\boldsymbol{\lambda} \geq 0$ in $\mathbb{R}^{2N+2}$ such that 
% \begin{align} 
%  & e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
%   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
%   + G^\top \boldsymbol{\lambda} = 0 , \label{NSQP:w+lambda} \\ 
%  & \boldsymbol{\lambda}^\top (G w^\star - \mathbf{c}) = 0 . \label{NSQP:wlambda}  
% \end{align} 
% \end{theorem}

% Introduce the dual quadratic programming problem: 
% \begin{equation} 
% \begin{aligned}  
% & \max \big\{ \theta (\boldsymbol{\lambda}) : \ \boldsymbol{\lambda} \geq 0 , \ \theta(\boldsymbol{\lambda}) > -\infty \big\} , 
%  \\ 
% & \theta(\boldsymbol{\lambda}) = \inf \{ L( \mathbf{x}, \boldsymbol{\lambda}) : \ \mathbf{x} \in \mathbb{R}^N \} ,  \\ 
% & L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}  
%   - e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) .   
% \end{aligned} 
% \label{Majoragent:DQP} 
% \end{equation} 

% By \cite[Theorem V.6.2]{Berkovitz2001}, we have the following relation between the quadratic programming problem \eqref{Majoragent:QP} and the dual problem \eqref{Majoragent:DQP}. 
% \begin{theorem} 
% \label{thm:QPdual}
% Let the quadratic programming problem \eqref{Majoragent:QP} has a solution $w^\star=(w^{1, \star}, ..., w^{N, \star})$. Then the dual problem \eqref{Majoragent:DQP} has a solution $\boldsymbol{\lambda}_\star$, and the solution $\boldsymbol{\lambda}_\star$ is exactly the multiplier $\boldsymbol{\lambda}$ in Theorem~\ref{thm:NSQP} corresponding to $w^\star$. 
% \end{theorem} 

% With Theorems~\ref{thm:NSQP} and \ref{thm:QPdual}, we are ready to prove Theorem~\ref{thm:OptimalWeights}. 

% \begin{proof}[Proof of Theorem~\ref{thm:OptimalWeights}]  

% By Theorem~\ref{thm:NSQP}, we can determine the optimal weights $w^\star=(w^{1,\star}, ..., w^{N,\star})$ from 
% \eqref{NSQP:w+lambda}. The multiplier $\boldsymbol{\lambda}$ in \eqref{NSQP:w+lambda} is the solution of the dual problem \ref{Majoragent:DQP}. 

% We first solve the dual problem \eqref{Majoragent:DQP} for the optimal $\boldsymbol{\lambda}$. 
% The function $L(\mathbf{x}, \boldsymbol{\lambda})$ in \eqref{Majoragent:DQP} can be rewritten as  
% \begin{align} 
%  L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = & \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  \mathbf{x}  
%   - e^{-\alpha(t-s)} y^\top_s \hat{\mathbf{Y}}_s \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) \notag \\ 
%    = &  \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}  
%   - \Big[ e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s - \boldsymbol{\lambda}^\top G \Big] \mathbf{x} 
%    - \boldsymbol{\lambda}^\top \mathbf{c} . 
%    \label{L(x,lambda)2}   
% \end{align} 
% For each $\boldsymbol{\lambda}$ fixed, the function $L(\cdot, \boldsymbol{\lambda})$ given by \eqref{L(x,lambda)2} is a $C^1$ convex function on $\mathbb{R}^N$. Then $\mathbf{x}_{\boldsymbol{\lambda}}$ is a minimizer of $L(\cdot, \boldsymbol{\lambda})$ if and only if $\nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda}) = 0$. 
% It then follows from \eqref{L(x,lambda)2} that 
% \begin{align} 
%  0 = & \nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda})  \notag \\ 
%  = & e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s y_s - G^\top \boldsymbol{\lambda}  \Big] , 
%  \notag 
% \end{align} 
% which further gives that 
% \begin{align} 
% 0 = &   \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big(   N\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s 
%  + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \mathbf{x}_{\boldsymbol{\lambda}}^\top \Big[  e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] .  
%   \label{0=<x,gradL>}  
% \end{align} 
% Substituting \eqref{0=<x,gradL>} into \eqref{Majoragent:DQP}, we obtain an explicit form of $\theta(\boldsymbol{\lambda})$
% \begin{align} 
%  \theta(\boldsymbol{\lambda}) = & L(\mathbf{x}_{\boldsymbol{\lambda}}, \boldsymbol{\lambda}) \notag \\ 
%  =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%   e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  
%   \mathbf{x}_{\boldsymbol{\lambda}}   
%   - \Big[ e^{-\alpha(t-s)} y^\top_s \hat{\mathbf{Y}}_s - \boldsymbol{\lambda}^\top G \Big] 
%    \mathbf{x}_{\boldsymbol{\lambda}}  
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s  + \mathrm{K} \big) 
%     \mathbf{x}_{\boldsymbol{\lambda}}   
%   -  \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big( N\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s 
%    + \mathrm{K} \big)    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =&  - \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%    e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  
%    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} . \notag 
% \end{align}  

% With the above explicit form of $\theta(\boldsymbol{\lambda})$, the dual quadratic programming problem \eqref{Majoragent:DQP} is then equivalent to 
% \begin{equation} 
% \begin{aligned} 
% & \max_{\mathbf{x}, \ \boldsymbol{\lambda}} \ 
% - \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} ,   \\ 
% & \text{subject to:} \ 
%  e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x} 
%   - \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] = 0 .  
% \end{aligned} 
% \label{Majoragent:DQPequiv} 
% \end{equation} 
% Since $\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s$ is positive semi-definite, $N>0$, and $K$ is a diagonal matrix with positive diagonal entries, then $N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}$ is positive definite and thus it is invertible.  
% Whence, the equality constraint in \eqref{Majoragent:DQPequiv} 
% implies that 
% \begin{align} 
%    \mathbf{x} 
% = e^{\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1} 
%  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] . 
% \label{xsublambda}
% \end{align} 
% With \eqref{xsublambda} substituted into \eqref{Majoragent:DQPequiv}, 
% the dual problem \eqref{Majoragent:DQPequiv} is then equivalent to the following unconstrained optimization problem: 
% \begin{align} 
%  \max_{\boldsymbol{\lambda}} \ -\frac{1}{2}  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s 
%    y_s - G^\top \boldsymbol{\lambda}  \Big]^\top 
%    e^{\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1} 
%  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] 
%  - \boldsymbol{\lambda}^\top \mathbf{c} . 
% \label{Majoragent:DQPunconstrained} 
% \end{align} 
% We reduce the unconstrained optimization problem \eqref{Majoragent:DQPunconstrained} to deduce that $\boldsymbol{\lambda}_\star$ satisfies
% \begin{align} 
% e^{\alpha(t-s)}\,
%  \Big[ G 
%  % e^{\alpha(t-s)}
%  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]
%  \boldsymbol{\lambda}_\star 
%  =
%  \Big[ G  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
%  y_s  -  \mathbf{c} \Big] . 
%  \label{lambdasubstar_almost} 
% \end{align} 
% Observe that $G$ (and thus $G^{\top}$) is invertible \add{since it is an $N\times N$ matrix with $\operatorname{det}(G)=1\cdot (-1)^{N-1}\neq  0$.
% Furthermore, notice that $G=G^{\top}$, $G$ commutes with all other matrices (when matrix multiplying), $G^2= I_N$, and the inverse of $G$ is given by
% \[
% \tilde{G}\eqdef 
%  \begin{pmatrix}
%      -1 & \mathbf{0}_{1\times N} \\
%      \mathbf{0}_{ (N \times 1) } & I_{(N-1\times N-1)} 
%  \end{pmatrix}
% .
% \]
% We use these remarks in the following computation.
% }  
% %is a diagonal matrix with non-zero diagonal values.  

% \noindent 
% Since we have already seen that $N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ is positive-define, and thus invertible, then $G\,N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} G^{\top}$.  
% \add{For legibility, set $A\eqdef \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ and $k\eqdef e^{\alpha(t-s)}>0$.}
% Thus, we may simplify~\eqref{lambdasubstar_almost} to obtain
% \begin{align} 
%  \boldsymbol{\lambda}_\star 
%  = & \Big[ G e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
%  y_s  -  \mathbf{c} \Big] 
%  \\
%   = & 
% %   \add{
% %       \Big[ 
% %       e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \Big]^{-1} 
% %      \Big[ -\Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %      y_s  
% %      -
% %      (-\eta \bar{1}_N)
% %      \Big] 
% %  }
% %  \\
% %   = & 
% %   \add{
% %   e^{\alpha(t-s)} 
% %   \,
% %       \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %      \Big[ 
% %         \eta \bar{1}_N
% %          -
% %          \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %          y_s  
% %      \Big] 
% %  }
% %  \\
% %   = & 
% %   \add{
% %   e^{\alpha(t-s)} 
% %   \Big[
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N
% %   -
% %     \hat{Y}^\top_s y_s  
% % \Big]
%  % }
%  %%% Annie Relaxation
%  \add{
%      \Big[ G k A^{-1} G^\top \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
% }
%  \\
%  &=
% \add{
%      \Big[ G k A^{-1} G \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%   \\
%  &=
% \add{
%      \Big[ G^2 k A^{-1} \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%    \\
%  &=
% \add{
%      \Big[ k A^{-1} \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%     \\
%  &=
% \add{
%      \frac1{k}\, A
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%      \\
%  &=
% \add{
%      \frac1{k}\, 
%         G AA^{-1} \hat{Y}^\top_s y_s  
%      -
%      \frac1{k}\,
%         A\mathbf{c} 
%  }
%       \\
%  &=
% \add{
%     \big(
%             \frac1{k}\, 
%                 G \hat{Y}^\top_s y_s  
%         -
%             \frac1{k}\,
%                 A\mathbf{c} 
%     \big)
%  }
%  . 
%  \label{lambdasubstar_almost} 
% \end{align} 
% Then we substitute $\boldsymbol{\lambda}_\star$ into \eqref{NSQP:w+lambda} to solve for the optimal weight vector $w^\star=(w^{1,\star}, ..., w^{N,\star})^\top$: 
% \allowdisplaybreaks
% %%% Annie Relaxation
% \add{
% \begin{align}
% % &\,\,
%   %   e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
%   % - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
%   % + G^\top \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + G \boldsymbol{\lambda}_{\star}  = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + G
%   \big(
%         \frac1{k}\, 
%             G \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%             A\mathbf{c} 
%     \big)
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k}\,
%         G
%         G \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k}\,
%         \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% A  w^\star 
%   - 
%     \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k^2}\,
%         \hat{Y}^\top_s y_s  
%     -
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% A  w^\star 
% =
%     \hat{\mathbf{Y}}_s^\top y_s 
%   - 
%         \frac1{k^2}\,
%         \hat{Y}^\top_s y_s  
%     +
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     A  w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         A^{-1}
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%         A^{-1}A\mathbf{c} 
% \\
% \label{eq:final_simplification__Gc}
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%         \mathbf{c} 
% .
% \end{align}
% By definition of $G$ and $\mathbf{c}$, given in~\eqref{eq:Gc_Def}, we find that
% \allowdisplaybreaks
% \begin{align} 
% \nonumber
%         G \mathbf{c} 
%         \,
%     = &
%         \begin{pmatrix}
%             1 & \mathbf{0}_{1\times N} \\
%             \mathbf{0}_{ (N \times 1) } & -I_{(N-1\times N-1)} 
%         \end{pmatrix}
%         \,
%         (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
% \\
% \nonumber
% =& 
%         (1+\eta - \eta N, \, \eta \mathbf{1}_{N-1})
% \\
% \nonumber
% =& 
%         (1-\eta N) \,e_1 + \eta \mathbf{1}_N
% \end{align} 
% where $e_1$ is the first standard basis vector in $\mathbb{R}^N$.
% Consequentially, the right-hand side of~\eqref{eq:final_simplification__Gc} further simplifies to
% \begin{equation}
% \label{eq:pre_final_weights}
%     w^\star 
% =
%         \Big(
%             1-\frac1{k^2}
%         \Big)
%         A^{-1}
%         \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         \Big(
%             (1-\eta N) \,e_1 + \eta \mathbf{1}_N
%         \Big)
% .
% \end{equation}
% Plugging in the definitions of $A$ and of $k$ back into~\eqref{eq:pre_final_weights} yields
% $A\eqdef \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ and $k\eqdef e^{\alpha(t-s)}>0$
% \[
%     w^\star 
% =
%         \big(
%             1-
%             % \frac1{k^2}
%             e^{-2\alpha(t-s)}
%         \big)
%         \big(
%             %% A
%             \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}
%         \big)^{-1}
%         \,
%         \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         % \frac1{k^2}
%         e^{-2\alpha(t-s)}
%         \,
%         \Big(
%             (1-\eta N) \,e_1 + \eta \mathbf{1}_N
%         \Big)
% \]
% % This conclude the proof.
% }
% %%%% Shifted Orthant
% % \add{
% % \begin{align}
% % &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   + G^\top \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% % \therefore & 
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   - \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% % \therefore &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   = 
% %   -e^{\alpha(t-s)}\mathbf{Y}_s^{\top}y_s  
% %   +
% %   e^{\alpha(t-s)} 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N
% % \\
% % \therefore &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   % - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   = 
% %   % -e^{\alpha(t-s)}\mathbf{Y}_s^{\top}y_s  
% %   % +
% %   e^{\alpha(t-s)} 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   = 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     w^\star 
% %   = 
% %   \eta\,
% %   \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1}
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     w^\star 
% %   = 
% %   \eta\,\bar{1}_N 
% % \end{align}
% % }
% % \begin{align} 
% %    w^\star = &  e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}  \Big)^{-1} 
% %     \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top  y_s 
% %   - G^\top \boldsymbol{\lambda}_\star \Big]  \notag  \\ 
% %   = &  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_s^\top  y_s 
% %   \notag \\    
% %   & -  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1}   G^\top 
% %   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
% %  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %   y_s -  \mathbf{c} \Big] , 
% %   \notag  
% % \end{align} 
% which is \eqref{eqn:OptimalWeights}.  
% \end{proof} 
% \end{comment}

% \subsection{{Proof of Theorem~\ref{thm:OptimalWeights}}}

% \begin{proof}%[{Proof of Theorem~\ref{thm:OptimalWeights}}]
% Define $A\eqdef 2\,
%  ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \kappa I_N)$, where $I_N$ is the $N\times N$ identity matrix, and set $b\eqdef 2  \big(
% y^\top_t  \hat{\mathbf{Y}}_t\big)^{\top}$. 
% The matrix $\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t$ is positive semi-definite.  Since $\kappa>0$ then $\det(\kappa I_N)=\kappa^N>0$ and thus, the matrix $A$ is positive definite.  

% Let $B\eqdef \mathbf{1}_N\in \mathbb{R}^{N\times 1}$, where for $i=1,\dots,N$ we have $B_i=1$.  
% Note that $B$ has rank $1\le N$.

% Observe that the loss function $\Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 + \sum_{j=1}^N \kappa\, | w^j_t|^2 $ can be written as
% \allowdisplaybreaks
% \begin{align}
%     \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%     + 
%     \sum_{j=1}^N \kappa\, | w^j_t|^2 
% = &
%     \frac1{2}\, 
%     w^\top A w 
%   - b^{\top} w 
%    + y_t^\top y_t
% \eqdef Q(w)
% .
% \end{align}
% Therefore, the server's optimization problem~\eqref{eq:server} can be written as a quadratic program with linear constraint 
% \begin{equation}
% \label{eq:server__QPLC}
% \begin{aligned}
%     \min_{w\in \mathbb{R}^N}\,
%     &
%     \frac1{2} \,
%     w^{\top} A w - b^{\top} w
% \\
% \mbox{s.t.} & \,\,
% B^{\top} w = \eta .%1.
% \end{aligned}
% \end{equation}
% Since $A$ is positive definite and since $\operatorname{rank}(B)=1\le N$ then~\eqref{eq:server__QPLC} is a non-degenerate quadratic program with a feasible linear constraint set.
% By \citep[Proposition 6.3]{gallier2020linear}, there exists a unique solution to the constrained quadratic program~\eqref{eq:server__QPLC} and it is given by the Karush-Kuhn-Tucker (KKT) system
% \begin{align}
% \label{eq:KKT_1}
% A\,w + B\lambda & = b
% \\
% \label{eq:KKT_2}
% B^{\top} w & = \eta .%1.
% \end{align}
% Since $A$ is positive definite, it is invertible.  Therefore,~\eqref{eq:KKT_1} allows us to isolate $w$
% \begin{align}
% \label{eq:KKT_1__manip1}
% w  = A^{-1}\,(b - B\lambda)
% .
% \end{align}
% Plugging the expression for $w$, which we just obtained in~\eqref{eq:KKT_1__manip1}, back into~\eqref{eq:KKT_2} yields
% \allowdisplaybreaks
% \begin{align}
% \nonumber
% % 1
% \eta
% = & B^{\top} \big(A^{-1}\,(b - B\lambda)\big)
% \\
% \nonumber
% \therefore \,
% % 1 
% \eta
% = & B^{\top} \big(A^{-1}\,b - A^{-1}B\lambda \big) 
% = B^{\top}A^{-1}\,b - \lambda B^{\top}A^{-1}B
% \\
% \nonumber
% \therefore \,
%     \lambda B^{\top}A^{-1}B
% = & 
%     B^{\top}A^{-1}\,b-
%     \eta%1
% \\
% \label{eq:KKT_2__manip1}
% \therefore \,
%     \lambda 
% = & 
%     \frac{
%         B^{\top}A^{-1}\,b-
%         \eta%1
%     }{
%         B^{\top}A^{-1}B
%     }
% .
% \end{align}
% Plugging the value for $\lambda$, just obtained in~\eqref{eq:KKT_2__manip1}, back into~\eqref{eq:KKT_1__manip1} yields the optimizer $w^{\star}\in \mathbb{R}^N$ to~\eqref{eq:server__QPLC}
% \allowdisplaybreaks
% \begin{align}
% \nonumber
% w^{\star}   & = A^{-1}\,\big(b - B\lambda\big)
% \\
% \nonumber
% & = 
%  A^{-1}\,b -  \lambda\, A^{-1}B
% \\
% \nonumber
% & = 
%  A^{-1}\,b -  
%  \biggl(
%     \frac{
%         B^{\top}A^{-1}\,b-
%         \eta%1
%     }{
%         B^{\top}A^{-1}B
%     }
%  \biggr)
%  \, A^{-1}B
% \\
% \label{eq:KKT_1__manip2}
% \therefore \,
% w^{\star} & = 
%  A^{-1}\,
%  \Biggl(
%      b -  
%      \biggl(
%         \frac{
%             B^{\top}A^{-1}\,b-
%             \eta%1
%         }{
%             B^{\top}A^{-1}B
%         }
%      \biggr)B
%  \Biggr)
% .
% \end{align}
% Plugging in our definitions for $A$, $b$, and $B$ back into~\eqref{eq:KKT_1__manip2} yields the conclusion.
% \end{proof}


% \subsection{{Proof of Theorem~\ref{thm:NashEqmExistence}}}
% \label{s:Proofs__ss:thm:NashEqmExistence}
% \begin{proof} 
% The proof is carried out in a similar manner as~\cite[Corollary 6.1]{BO1998}.  
% Let $V_i(t,\hat{\mathbf{y}})$, $i=1$,...,$N$ be the value functions of the $N$ agents associated with \eqref{eq:latent_state}, 
% \eqref{eq:residual_update}, and \eqref{eq:Objective_nth_expert}. 
% %\begin{align}  
% % & V_i(t, \hat{\mathbf{y}}) 
% %=  \sup_{\beta^i} \mathbb{E} \Big\{  
% % \Big\| y^i_t - \sum_{i=1}^N w^i 
% % \hat{y}^i \Big\|^2 
% %  + \| \beta^i \|^2    
% %+ V_i(t+1, \hat{\mathbf{y}} + 
% % \sum_{j=1}^N  e_j Z^{j\top}_t\beta^j) 
% %  \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
% %   & V_i(T, \hat{\mathbf{y}}) 
% %   = \notag 
% %\end{align} 
% From \eqref{eq:Objective_nth_expert}, the value functions at time $T$ with $\hat{Y}_T=\hat{\mathbf{y}}$ satisfy 
% $V_i(T, \hat{\mathbf{y}}) = 0$. 
% %\begin{align} 
% % V_i(T, \hat{\mathbf{y}})  = 0 . 
% % \label{Vi(T)}
%  %=  \big\| y_T -  \mathbf{w}_T^\top \hat{\mathbf{y}} \big\|^2 
%  %= \hat{\mathbf{y}}^\top \mathbf{w}_T \mathbf{w}_T^\top \hat{\mathbf{y}} 
%  %- 2 y_T^\top \mathbf{w}_T^\top \hat{\mathbf{y}} + \| y_T \|^2 .  
% %\end{align} 
% By the dynamic programming principle, the value functions at $T-1$ with $\hat{Y}_{T-1}= \hat{\mathbf{y}}=(\hat{y}^{1\top}, ..., \hat{y}^{N\top})^\top$ satisfy  
% \begin{align} 
% V_i(T-1, \hat{\mathbf{y}}) 
% = & \min_{\beta^i} \mathbb{E} \Big\{   \Big\| y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2     
%   \notag \\ 
%  & \hspace{5cm} +  V_i(T, \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_{T-1} \beta^j ) 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
% = & \min_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    \Big\} , 
%    \label{DPeqnVi(T-1)}
% \end{align} 
% where the condition $\hat{Y}_{T-1}=\hat{\mathbf{y}}$ can be removed from the expectation because $Z^j_{T-1}$, $j=1$, ..., $N$ are independent of $\hat{Y}_{T-1}$. 
% By the first order condition for the right side of \eqref{DPeqnVi(T-1)}, the equilibrium strategy $\boldsymbol{\beta}=(\beta^{1 \top}, \cdots, \beta^{N \top} )^\top$ should satisfy  
% \begin{align} 
%  & \mathbb{E} \Big\{  \gamma_i \beta^i + Z^{j\top}_{T-1} \mathbf{e}_j^\top \mathbf{w}_{T-1} 
%   \Big[ y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j    \Big] 
%   \Big\}   = 0,  
%  \quad i = 1, ..., N ,  \notag 
% \end{align} 
% which can be written in the compact form 
% \begin{align} 
%  & \big( \Gamma + \widehat{\mathbf{A}}(T-1) +  \mathbf{A}(T-1) \big) \boldsymbol{\beta}_{T-1} \notag \\ 
% = &   \big[  \mathbf{D}(T-1)^\top \mathbf{w}_{T-1} (y_T - \mathbf{w}_{T-1}^\top \hat{Y}_{T-1} ) - \mathbf{B}(T-1) \hat{Y}_{T-1} - \mathbf{C}(T-1) \big]     .  
% \notag 
% \end{align} 
% Since \eqref{eqn:Pi} admits a solution by the hypothesis of the proposition, we have that 
% $\Gamma + \widehat{\mathbf{A}}(T-1) +  \mathbf{A}(T-1)$ is positive definite, and hence 
% \begin{align} 
%   \boldsymbol{\beta}_{T-1} 
%   = & - (  \Gamma  + \widehat{\mathbf{A}}(T-1) + \mathbf{A}(T-1) )^{-1} \cdot \notag \\  
%   & \big[  \mathbf{D}(T-1)^\top \mathbf{w}_{T-1} (y_T - \mathbf{w}_{T-1}^\top \hat{Y}_{T-1} ) - \mathbf{B}(T-1) \hat{Y}_{T-1} - \mathbf{C}(T-1) \big]   . 
% \label{eqmbetaT-1}
% \end{align} 

% Substituting \eqref{eqmbetaT-1} into \eqref{DPeqnVi(T-1)}, 
% we obtain that $V_i(T-1, \hat{\mathbf{y}})$ take the form 
% \begin{align} 
%   V_i(T-1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(T-1) \hat{\mathbf{y}}  
%   + 2 S_i(T-1)^\top \hat{\mathbf{y}} + r_i(T-1) , \quad i = 1, ..., N. \notag  
%  \end{align} 
%  where $P_i(T-1)$ and $S_i(T-1)$ satisfy \eqref{eqn:Pi} and \eqref{eqn:Si}. 

% Assume by induction that at $t+1$ the value functions $\{V_i(t+1, \hat{\mathbf{y}})\}_{i=1}^N$ take the affine-quadratic form 
% \begin{align} 
%   V_i(t+1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t+1) \hat{\mathbf{y}}  
%   + 2 S_i(t+1)^\top \hat{\mathbf{y}} + r_i(t+1) , \quad i = 1, ..., N , \notag  
%  \end{align} 
% with $P_i$ and $S_i$ determined from \eqref{eqn:Pi} and \eqref{eqn:Si}, respectively. 
% We show that at $t$ with $\hat{Y}_t=\hat{\mathbf{y}}$ the value functions $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ also take the form 
% \begin{align} 
%   V_i(t, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) , \quad i = 1, ..., N . 
%   \label{vi(t,y)ansatz}
%  \end{align} 
% %and the equilibrium strategy $\boldsymbol{\beta}=[\beta^{1\top}, ..., \beta^{N\top} ]$ is indeed given by \eqref{eqmvecbeta}. 

 
% By the dynamic programming principle, $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ satisfy the system of dynamic programming equations:  
% \begin{align} 
% V_i(t, \hat{\mathbf{y}}) 
% = & \min_{\beta^i} \mathbb{E} \Big\{  e^{-\alpha_i (T-1-t)} 
%  \Big[ \Big\| y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2   \Big]   \notag \\ 
%   & \hspace{5cm} +   V_i(t+1, \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_t \beta^j ) 
%    \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
%   = & \min_{\beta^i} \mathbb{E} 
%   \Big\{   e^{-\alpha_i (T-1-t)} 
%  \Big[ \Big\| y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2   \Big]    \notag \\ 
%  & \hspace{2cm}  +   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big]^\top P_i(t+1) 
%   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big] \notag \\ 
%  &   \hspace{2cm}  + 2    S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big] 
%   +   r_i(t+1)      \Big\} , \quad 
%    i = 1, ..., N . 
%   \label{DPeqnVi(t)}  
% \end{align} 
% The first order condition for the right side of \eqref{DPeqnVi(t)} is given by  
% \begin{align} 
% & \mathbb{E} \Big\{   - e^{-\alpha_i (T-1-t)} Z^{i\top}_t \mathbf{e}_i^\top \mathbf{w}_t 
%  \Big[ y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)   \Big] 
%  + e^{-\alpha_i (T-1-t)} \gamma_i \beta^i    \notag \\  
% & \qquad +  Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \Big( \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_t \beta^j \Big) 
%   + Z^{i\top}_t \mathbf{e}_i^\top S_i(t+1) \Big\}  =0 , 
%   \quad i = 1, ..., N , \notag 
% % \label{betaifirstorderV(y)} 
% \end{align} 
% which can be written in the compact form  
% \begin{align} 
%  &  \big[ e^{-\boldsymbol{\alpha}(T -1 - t)}  \Gamma  
%   + e^{-\boldsymbol{\alpha}(T -1 - t)} \widehat{\mathbf{A}}(t) 
%    + \mathbf{A}(t) \big] \boldsymbol{\beta}_t  \notag \\ 
%  & + \mathbf{B} (t) \hat{\mathbf{y}} + \mathbf{C}(t) 
%   - e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top  \hat{\mathbf{y}} ) 
%  = 0 . \notag 
% \end{align} 
% The equilibrium strategy at time $t$ is determined by 
% \begin{align} 
%  \boldsymbol{\beta}_t = &  \big[ e^{-\boldsymbol{\alpha} (T-1-t) } \Gamma 
%   + e^{-\boldsymbol{\alpha}(T -1 - t)} \widehat{\mathbf{A}}(t)  + \mathbf{A}(t) \big]^{-1} \cdot \notag \\  
% & \big[  e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top  \hat{\mathbf{y}} ) 
% - \mathbf{B}(t) \hat{\mathbf{y}} - \mathbf{C}(t) 
%   \big]  \notag \\ 
% = & \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t).   
% \label{eqmbetat}   
% \end{align} 
% Substituting \eqref{eqmbetat} and \eqref{vi(t,y)ansatz} into \eqref{DPeqnVi(t)}, we obtain 
% \begin{align} 
%  & \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) \notag \\ 
%   = & \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big]^\top  
%  \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top \big]  \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big]  
%  \notag \\ 
%  & + 2 \big[  - e^{-\alpha_i(T-1-t)} (y_{t+1} - \mathbf{w}_t^\top \hat{\mathbf{y}} )^\top \mathbf{w}_t^\top \mathbf{D}(t) 
%   + \hat{\mathbf{y}}^\top P_i(t+1) \mathbf{D}(t) + S_i^\top(t+1) \mathbf{D}(t) \big] 
%    \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big] 
%  \notag \\ 
%  & + e^{-\alpha_i(T-1-t)} \big\| y_{t+1} - \mathbf{w}_t^\top \hat{\mathbf{y}} \big\|^2 + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}} 
%  + 2 S_i^\top(t+1) \hat{\mathbf{y}} + r_i(t+1) . 
%  \notag 
% \end{align} 
% By matching the coefficients of quadratic terms of $\hat{\mathbf{y}}$, we obtain \eqref{eqn:Pi} for $P_i(t)$;  
% matching the coefficients of the linear terms of $\hat{\mathbf{y}}$, we obtain \eqref{eqn:Si} for $S_i(t)$. 

 
% \end{proof} 

% \subsection{Proofs of Corollaries} 


% \begin{proof} [{Proof of Corollary~\ref{cor:Random_NN}}]
% %Set $a^i_t\eqdef A^{(i)}x_t+b^{(i)}$.  By Theorem~\ref{thm:OptimalWeights}, for $i,j=1,\dots,N$ we have
% From Theorem~\ref{thm:NashEqmExistence}, the submatrices of $\mathbf{A}(t)=\big( A^{(i,j)}(t) \big)_{1\leq i,j \leq N}$ 
% are 
% \begin{align} 
% A^{(i,j)}(t) 
% =
%  & \mathbb{E} \big[ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big]  
%   \notag 
% \end{align} 
% By Lemma~\ref{lem:Mean_Cov_ResModel}, the entries in the diagonal submatrices $A^{(i,i)}(t)$ of $\mathbf{A}(t)$ are given by  
% \begin{align} 
% ( A^{(i,i)}(t) )_{jk} = &
%   \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii}\,
%     \begin{cases}
%             ( ( a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 ) 
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j   \,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big(
%                 \frac{-(a^i_t \odot a^i_t )_j}{2\, (\sigma_t^i)^2 }
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = a(t, i)_j a(t,i)_k 
%     & \mbox{ if }   j \neq k
%     \end{cases} 
%     \notag 
% \end{align} 


% Since the white noises $\{W^i_t\}_{i, t}$, are independent, \eqref{DTRCsystemReLU} implies that 
% $Z^i_t$ and $Z^j_t$ are independent for $i\neq j$. 
% The off-diagonal submatrices of $\mathbf{A}(t)$ can be written as   
% \begin{align} 
% A^{(i,j)}(t) 
%  %= & \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_j Z^{j\top}_t ] \notag \\ 
%  %= & \mathbb{E} [  Z^i_t ]  e_i^\top P_i(t+1) e_j  \mathbb{E} [ Z^{j\top}_t ] \notag \\ 
%  = & \mathbb{E} [  Z^{i\top}_t ]  ( P_i(t+1) )_{ij}  \mathbb{E} [ Z^j_t ] 
% \notag \\ 
%  = & a(t, i)^\top ( P_i(t+1) )_{ij} a(t, j) 
% \end{align} 
% where $\mathbb{E} [  Z^i_t ]$ and $\mathbb{E} [  Z^j_t ]$ where computed explicitly using Lemma~\ref{lem:Mean_Cov_ResModel}. 
% \end{proof} 


% \begin{comment} 
% \begin{proof} [{Proof of Corollary~\ref{cor:Random_NN}}]
% %Set $a^i_t\eqdef A^{(i)}x_t+b^{(i)}$.  By Theorem~\ref{thm:OptimalWeights}, for $i,j=1,\dots,N$ we have
% From Proposition~\ref{prop:NashEqmExistence}, the submatrices of $\mathbf{A}(t)=\big( A^{(i,j)}(t) \big)_{1\leq i,j \leq N}$ 
% are 
% \begin{align} 
% A^{(i,j)}(t) 
% =
%  & \mathbb{E} \big[ Z^i_t e_i^\top P_i(t+1) e_j Z^{j\top}_t \big]  
%  =  \mathbb{E} \big[ Z^i_t  ( P_i(t+1) )_{ij}  Z^{j\top}_t \big] \notag 
% \end{align} 
% By Lemma~\ref{lem:Mean_Cov_ResModel}, the entries in the diagonal submatrices $A^{(i,i)}(t)$ of $\mathbf{A}(t)$ are given by  
% \begin{align} 
% ( A^{(i,i)}(t) )_{jk} = &
%   \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii}\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma^i_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = a(t, i)_j a(t,i)_k 
%     & \mbox{ if }   j \neq k
%     \end{cases} 
%     \notag 
% \end{align} 


% Since the white noises $\{W^i_t\}_{i, t}$, are independent, \eqref{DTRCsystemReLU} implies that 
% $Z^i_t$ and $Z^j_t$ are independent for $i\neq j$. 
% The off-diagonal submatrices of $\mathbf{A}(t)$ can be written as   
% \begin{align} 
% A^{(i,j)}(t) 
%  %= & \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_j Z^{j\top}_t ] \notag \\ 
%  %= & \mathbb{E} [  Z^i_t ]  e_i^\top P_i(t+1) e_j  \mathbb{E} [ Z^{j\top}_t ] \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  ( P_i(t+1) )_{ij}  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & a(t, i) ( P_i(t+1) )_{ij} a(t, j)^\top
% \end{align} 
% where $\mathbb{E} [  Z^i_t ]$ and $\mathbb{E} [  Z^j_t ]$ where computed explicitly using Lemma~\ref{lem:Mean_Cov_ResModel}. 
% \end{proof} 
% \end{comment} 



% Under these dynamics, the following lemma gives enough information to compute the relevant matrices in Theorem~\ref{thm:NashEqmExistence}.
% \begin{lemma}[Mean and Covariance of $Z_{\cdot}^i$ in the Example~\ref{ex:Random_NeuralNetwork} for the case of $d_y=1$]
% \label{lem:Mean_Cov_ResModel}
% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[Z_{t+1}^i] 
%     = &
%         a^i_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a^i_t
%             )
%         \Big)
%         +
%             \frac{\sigma_t^i}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\, (\sigma_t^i)^2 }
%             % \,
%             (a^i_t \odot a^i_t )
%         \Big)
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 )
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the row vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of Example~\ref{ex:Random_NeuralNetwork}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion. 

% \end{proof}

% The multi-dimensional version of Corollary~\ref{cor:Random_NN} is relegated to the appendix.  Overall it is of a similar form with some additional technicalities.
% \begin{corollary} 
% \label{cor:Random_NN_dy>1}
% In the setting of Example~\ref{ex:Random_NeuralNetwork} with $d_y>1$, we have 
% \begin{align*}
% & \mathbf{A}(t)
%  = 
% \big(A^{(i,j)}(t)\big)_{i,j=1}^N , 
% \hspace{2.05cm} 
% \widehat{\mathbf{A}}(t) = \big( \widehat{A}^{(i,j)}(t) \big)_{i, j = 1}^N , 
% \notag \\  
%  & \mathbf{B}(t)  = 
%  \begin{bmatrix} 
%   P_1(t+1) \mathbf{e}_1 a(t, 1), \cdots, P_N(t+1) \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%   S_1(t+1)^\top \mathbf{e}_1 a(t, 1), \cdots, S_N(t+1)^\top  \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top , 
%   \notag \\   
% & \mathbf{D}(t) 
%   = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 a(t,1), \cdots  , \mathbf{e}_N a(t, N) 
%  \end{bmatrix} , 
%  \notag \\ 
%  & \mathbf{D}_i(t) = ( D_i^{(j,k)}(t) )_{j,k = 1}^N , \quad i = 1, ..., N . \notag 
% % \big( D_i^{(j,k)} \big)_{j,k=1}^N , \quad i = 1, ..., N. \notag 
% \end{align*}
% where for $t=1,\dots,N$ and $t\in \mathbb{N}_+$, each $a(t,i)$ is defined as follows
% \begin{align} 
% & a^i_t\eqdef A^{i}x_t+b^{i} = \big[ (a^i_t)_1^\top , \cdots, (a^i_t)_{d_y}^\top \big]^\top \in \mathbb{R}^{d_y \times d_z} , \notag \\ 
% & a(t,i)
% \eqdef 
%    \big[ a(t, i)_1^\top , \cdots, a(t, i)_{d_y}^\top \big]^\top , \notag \\ 
% & a(t, i)_k = (a^i_t)_k 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{(\sigma_t^i)_k}%\cdot 
%                 (a^i_t)_k
%             )
%         \Big)
%         +
%             \frac{(\sigma_t^i)_k}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\, ( (\sigma_t^i)_k )^2 }
%             % \,
%             ( (a^i_t)_k \odot (a^i_t)_k )
%         \Big)  , \quad 
%         k = 1, ... , d_y \notag 
% \end{align} 
% and $\odot$ and $\Phi$ are defined in Lemma~\ref{lem:Mean_Cov_ResModel}. 
% The submatrices 
% $\big(A^{(i,j)}(t)\big)_{i,j=1}^N$, $\big(\widehat{A}^{(i,j)}(t)\big)_{i,j=1}^N$, 
% and $\big(D_i^{(j,k)}(t)\big)_{j,k=1}^N$ of $\mathbf{A}(t)$, $\widehat{\mathbf{A}}(t)$, 
% and $\{ \mathbf{D}_i(t) \}_{i=1}^N$,  respectively, in the setting of Example~\ref{ex:Random_NeuralNetwork},  
% are given by

% \begin{align} 
%  A^{(i,j)}(t) =
% \begin{cases} 
% \sum_{k, l = 1 }^{d_y} \mathbb{E} \Big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \Big] , \quad & \mbox{if} \quad i = j , \\
%   a(t, i)^\top \mathbf{e}_i^\top  P_i(t+1) \mathbf{e}_j a(t, j) , \quad & \mbox{if} \quad i \neq j  , 
%  \end{cases} 
%  \notag 
%  \end{align} 





% \end{corollary} 



% \begin{proof}[{Proof of Corollary~\ref{cor:Random_NN_dy>1}}]
% Now we present the result for the general case $d_y>1$. 
% \begin{align} 
%  a^i_t = \big[ (a^i_t)_1^\top , \cdots, (a^i_t)_{d_y}^\top \big]^\top \in \mathbb{R}^{d_y \times d_z} , \quad 
%  \sigma^i_t = \big[ (\sigma^i_t)_1 , \cdots , (\sigma^i_t)_{d_y} \big]^\top \in \mathbb{R}^{d_y \times 1} , \notag 
% \end{align} 
% where $(a^i_t)_1$, ..., $(a^i_t)_{d_y}$ are $d_z$-dimensional row vectors and $(\sigma^i_t)_1$, ..., $(\sigma^i_t)_{d_y}$ are non-negative scalars. 
% \begin{align} 
%  Z^i_t = \operatorname{ReLU} \big( A^i x_t + b^i + \sigma^i_t W^i_t \big)  
%  = \big[ (Z^i_t)_1^\top , \cdots , (Z^i_t)_{d_y}^\top \big]^\top \notag  
% \end{align} 
% with $(Z^i_t)_k = (a^i_t)_k + (\sigma^i_t)_k W^i_t$, $k=1$, ..., $d_y$. 
% \begin{align} 
%  a(t, i) = \big[ a(t, i)_1^\top , \cdots, a(t, i)_{d_y}^\top \big]^\top \notag 
% \end{align} 

% For $k=1$, ..., $d_y$, 
% \begin{align} 
%  a(t, i)_k = (a^i_t)_k 
%         \odot
%         \left(
%             \bar{1} 
%             - 
%             \Phi\bullet \left(
%                 \frac{-1}{(\sigma_t^i)_k}%\cdot 
%                 (a^i_t)_k
%             \right)
%         \right)
%         +
%             \frac{(\sigma_t^i)_k}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\, ( (\sigma_t^i)_k )^2 }
%             % \,
%             \left( (a^i_t)_k \odot (a^i_t)_k \right)
%         \Big)  
%     \notag 
% \end{align} 

% \begin{align} 
%  \mathbb{E}[Z^i_t] = a(t, i) = \big[ a(t, i)_1^\top , \cdots, a(t, i)_{d_y}^\top \big]^\top  
%  \notag 
% \end{align} 



% For $i\neq j$, $Z^i_t$ and $Z^j_t$ are independent since the random noises $W^i_t$ and $W^j_t$ are independent, 
% then $A^{(i,j)}(t)$ can be represented as 
% \begin{align} 
%   A^{(i,j)}(t) = &
%  \mathbb{E} [ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t ] \notag \\ 
%  =& \mathbb{E} [ Z^{i\top}_t ] \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j \mathbb{E} [ Z^j_t ] \notag \\ 
%  =& a(t, i)^\top \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j a(t,j) 
%  \notag 
% \end{align} 

% For $i=j$, 
% \begin{align} 
%  A^{(i,i)}(t) = &
%  \mathbb{E} [ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i Z^i_t ]   \notag  \\ 
%  = & \mathbb{E} \Big[ \sum_{k, l = 1 }^{d_y} (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \Big]  
%  \notag \\ 
%  = & \sum_{k, l = 1 }^{d_y} \mathbb{E} \Big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \Big] ,  
%  \notag 
% \end{align} 

% For $k=l$, 
% \begin{align} 
%  \mathbb{E} \Big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kk} (Z^i_t)_k \Big] 
%  \notag 
% \end{align} 

% For $k\neq l$, 
% \begin{align} 
%  \mathbb{E} \Big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \Big] 
%  \notag 
% \end{align} 
% \end{proof} 

% \begin{lemma}[Mean and Covariance of $Z_{\cdot}^i$ in the Example~\ref{ex:Random_NeuralNetwork}]
% \label{lem:Mean_Cov_ResModel(dy>1)}
% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[ (Z_{t+1}^i)_k ] 
%     = &
%         (a^i_t)_k 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{(\sigma_t^i)_k}%\cdot 
%                 (a^i_t)_k
%             )
%         \Big)
%         +
%             \frac{\sigma_t^i}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\, (\sigma_t^i)_k^2 }
%             % \,
%             ( (a^i_t)_k \odot (a^i_t)_k )
%         \Big) , 
%         \quad k = 1, ..., d_y
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 )
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}




% \newpage




% \begin{comment} 
% \begin{lemma}[{Mean and Covariance of $Z_{\cdot}^i$ in the Example~\ref{ex:Random_NeuralNetwork}}]
% \label{lem:Mean_Cov_ResModel}
% Consider the setting of Example~\ref{ex:Random_NeuralNetwork}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[Z_{t+1}^i] 
%     = &
%         a^i_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a^i_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             (a^i_t)^2
%         \Big)
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a^i_t)_j^2 + \sigma^i_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a^i_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of Example~\ref{ex:Random_NeuralNetwork}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion.
% \end{proof}
% \end{comment} 




% \section{The Algorithm}
% \label{s:AlgoMain}

% \begin{algorithm}[H]%[hbp!]%
% \SetKwInOut{Require}{Require}
% \caption{Synchronization Subroutine}
% \label{alg:sync_subroutine}
% \SetAlgoLined
% \LinesNumberedHidden
% \Require{Observed target values $\{ ( y^1_t, ..., y^N_t ) \}_{t=0}^T$. \\
% Mixture weights $w_\cdot = \{ (w^1_t, ..., w^N_t) \}_{t=0}^T$ $\leftarrow$ Run: Algorithm~\ref{alg:FedMain}}
% \DontPrintSemicolon
% \vspace{0.2cm}
% \DontPrintSemicolon
% \tcp{Initialize Updates} 
% $\mathbf{w}_T=(w^1_T I_{d_{y}}, ..., w^N_T I_{d_{y}})^\top$\\
% \For{$i:1,\dots,N$ in parallel}{
% $P_i(T)  = 0$ \\
% $S_i(T) = 0$ 
% }
% \tcp{Generate Iterates}
% \For(){$t=T-1,\dots,0$}{
% \tcp{Update Driving Parameters} 
% $\mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top$ \\
% %$\mathbf{A}(t)=  \big[ \mathbb{E} \big( Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big) \big]_{i,j=1}^N$ \\
% $\mathbf{A}(t) = \mathbb{E} \big\{ [ P_1(t+1) \mathbf{e}_1 Z^1_t, \, \cdots, \, P_N(t+1) \mathbf{e}_N Z^N_t ]^\top 
%  [ \mathbf{e}_1 Z^1_t, \cdots, \mathbf{e}_N Z^N_t ] \big\}$ \\  
%  $\widehat{\mathbf{A}}(t) = \mathbb{E} \big\{ [ \mathbf{e}_1 Z^1_t, \, \cdots, \, \mathbf{e}_N Z^N_t ]^\top \mathbf{w}_t \mathbf{w}_t^\top  
%  [ \mathbf{e}_1 Z^1_t, \cdots, \mathbf{e}_N Z^N_t ] \big\}$ \\  
% $\mathbf{B}(t)= \mathbb{E} [ P_1(t+1) \mathbf{e}_1 Z^1_t, \, \cdots, \, P_N(t+1) \mathbf{e}_N Z^N_t ]^\top $ \\
% $\mathbf{C}(t)= \mathbb{E} [ S_1^\top(t+1) \mathbf{e}_1 Z^1_t, \, \cdots, \, S_N^\top(t+1) \mathbf{e}_N Z^N_t ]^\top$ \\
% $\mathbf{D}(t)  
%  = \mathbb{E}  
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix}$ \\ 
%    $\mathbf{G}(t) = - \big[ e^{-\boldsymbol{\alpha}(T-1-t)} ( \Gamma + \widehat{\mathbf{A}}(t) ) 
%   + \mathbf{A}(t)    \big]^{-1} 
%  \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t \mathbf{w}_t^\top + \mathbf{B}(t) \big] $ 
%  \notag \\ 
%   $\mathbf{H}(t) = \big[ e^{-\boldsymbol{\alpha}(T-1-t)} (\Gamma + \widehat{\mathbf{A}}(t) ) + \mathbf{A}(t)   \big]^{-1} 
%   \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t y_{t+1} - \mathbf{C}(t) \big] $
%  \notag \\
% \For{$i:1,\dots,N$ in parallel}{
% \vspace{-0.2cm}
% \begin{align*} 
% & \hspace{-1.2cm} \mathbf{D}_i(t) 
%  =  \mathbb{E} \big\{   
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix}^\top 
%   P_i(t+1) 
%   \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix} 
%  \big\}  
%  \notag \\ 
%   P_i(t) = &  
%   \mathbf{G}(t)^\top 
%   \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] 
%    \mathbf{G}(t) \\   
%   &  + \big[ e^{-\alpha_i(T-1-t)}\mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big] 
%    \mathbf{D}(t) \mathbf{G}(t)  \\ 
%   &  + \mathbf{G}(t)^\top \mathbf{D}(t)^\top \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big]^\top
%   \\ 
% & + e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  \\
% %%%%%
%  S_i(t)  = &   \mathbf{G}^\top(t) \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) 
%    + e^{-\alpha_i(T-1-t)} \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] \mathbf{H}(t) \\ 
% & + \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  \big] \mathbf{D}(t) \mathbf{H}(t) \\  
% & + \mathbf{G}^\top(t) \mathbf{D}^\top(t) \big[ - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) \big]  \\
% & - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1)
% \end{align*}
% }
% }
% \tcp{Update Game Strategy} 
% $\hat{Y}_0 = (y^{1\top}_0, ..., y^{N\top}_0)^\top$ \\
% \For{$t=0, ..., T-1$}{
% $\boldsymbol{\beta}_t 
% %= [\beta^{1\top}_t, ..., \beta^{N \top}_t ]^\top 
% =  \mathbf{G}(t) \hat{Y}_t + \mathbf{H}(t)$ \\
% $\hat{Y}_{t+1} = \hat{Y}_t + \diag[Z^1_t, ..., Z^N_t ] \boldsymbol{\beta}_t$
% }

% \Return $\boldsymbol{\beta}_t$ for $t=0, 1, ..., T-1$
% \end{algorithm} 

% We now summarize our federated learning algorithm.

% \begin{algorithm}[H]%[hpt!]%
% \SetKwInOut{Require}{Require}
% \caption{Proposed Federated Learning Algorithm}
% \label{alg:FedMain}
% \SetAlgoLined
% \LinesNumberedHidden
% \Require{Current time $t\in \mathbb{N}$, Hidden States $\{Z_t^i\}_{i=1}^N$, expert models $\{\varphi^i\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$, Batch size $1\le b\le N$.}
% \DontPrintSemicolon
% \vspace{0.2cm}
% \For(\tcp*[f]{Update Experts in Parallel}){$t:1,\dots,T$ in parallel} 
%  {
% \For(\tcp*[f]{Update Experts in Parallel}){$i:1,\dots,N$ in parallel}{
% $\beta_{t-1}^i \leftarrow \big( X^{i \top}_{t-1} X^i_{t-1} + \gamma_i I_{d_z} \big)^{-1}\, X_{t-1}^{i \top} \bar{y}^i_{t} $
% \tcp*{Local Weighted Regression}
% Generate $\varepsilon_{t-1}^i$
% \tcp*{Generate Random State}
% $Z_{t-1}\leftarrow \varphi(x_{[0:t-1]},\varepsilon_{t-1}^i,Z_{t-2}^i)$
% \tcp*{Update Hidden State}
% $\hat{Y}^i_t \leftarrow \hat{Y}_{t-1}^i + Z_{t-1} \, \beta_{t-1}^i $
% \tcp*{Update Residual Prediction}
% } 
% %%% Get Mixture Weights
% \tcp{Compute Mixture Weights} 
% % \For(\tcp*[f]{Update Experts in Parallel}){$t:1,\dots,T$ in parallel}{
% $\hat{\mathbf{Y}}_{t-1} \leftarrow  (\hat{Y}^{1\top}_{t-1}, ..., \hat{Y}^{N\top}_{t-1})^\top$ \\
% $A \leftarrow 2\,N \hat{\mathbf{Y}}^\top_{t-1} \hat{\mathbf{Y}}_{t-1} + \kappa I_N$ \\
% $b\leftarrow 2 (y^\top_{t-1}  \hat{\mathbf{Y}}_{t-1})^{\top}$ \\
% $ w_t \leftarrow  A^{-1}\, \left( b - \frac{\mathbf{1}_N^{\top}A^{-1} b \, - \, \eta}{\strut \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N} \cdot\,\mathbf{1}_N
% \right)$ \\
% } 
% %%%% Synchronization Step
% \If{$t \bmod T =  0$ and $t>0$}{
% \tcp{Synchronize Local Experts via Nash Game}
% $\boldsymbol{\beta}^{\text{sync}}_{t-1} \leftarrow $ Run Synchronize Sub-Routine: Algorithm~\ref{alg:sync_subroutine}
% \tcp*{Synchronized Weights}
% \For(\tcp*[f]{Compute New Predictions}){$i:1,\dots,N$ in parallel}{
% $\beta_{t}^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_{t-1})_i$\;
% Generate $\varepsilon_{t-1}^i$ 
% \tcp*{Generate Random State}
% $\hat{Y}^i_{t+1} \leftarrow \hat{Y}^i_{t} + \varphi(x_{[0:t]},\varepsilon_{t}^i,Z_{t-1}^i)  \beta^i_{t}$ \;
% }
% }
% \tcp{Server Synchronizes Local Expert Predictions}
% \Return{$w_T^\top \hat{\mathbf{Y}}_{T+1}$}
% \tcp*{Ensemble Prediction}
% \end{algorithm}

% % \begin{algorithm}[H]%[ht!]%
% % \caption{Proposed Federated Learning Algorithm}
% % \label{alg:FedMain}
% % \begin{algorithmic}
% % \SetAlgoLined
% % \Require Current time $t\in \mathbb{N}$, Hidden States $\{Z_t^i\}_{i=1}^N$, expert models $\{\varphi^i\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$, Batch size $1\le b\le N$.
% % \DontPrintSemicolon
% %         \tcp*{Update Mixture Weights}
% %         % \State \eIf{$t \bmod T\neq 0$}{
% %             \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
% %                 \State \tcc{Update Experts in Parallel}
% %                 \State \ForParallel{\State $\beta_t^i \leftarrow 
% %         \big( X^{i \top}_t X^i_t + \gamma_i I_{d_z} \big)^{-1}\, X_t^{i \top} \bar{y}^i_t $
% %                     \tcp*{Local Weighted Regression}
% %                     \State Generate $\varepsilon_t^i$
% %                     \tcp*{Generate Random State}
% %                     \State $Z_{t+1}\leftarrow \varphi(x_{[0:t]},\varepsilon_t^i,Z_{t+1}^i)$
% %                     \tcp*{Update Hidden State}
% %                     \State 
% %                       $\hat{Y}^i_t
% %                       \leftarrow
% %                       \hat{Y}_{t-1}^i
% %                       + 
% %                       \beta_t^i \,
% %                       Z_t$
% %                       \tcp*{Update Residual Prediction}
% %                         }
% %                    % }{
% %         %%% Get Mixture Weights
% %         \State \tcc{Compute Mixture Weights} 
% %         \State $\hat{\mathbf{Y}}_t \leftarrow  (\hat{Y}^1_t, ..., \hat{Y}^N_t)$ 
% %         \State $A \leftarrow 2\,N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \kappa I_N$ 
% %         \State $b\leftarrow 2 (y^\top_t  \hat{\mathbf{Y}}_t)^{\top}$, 
% %         \State $ w_t  
% %         \leftarrow  
% %              A^{-1}\,
% %              \big(
% %                  b -  
% %                  % \biggl(
% %                     \frac{
% %                         \mathbf{1}_N^{\top}A^{-1} b \, - \, \eta 
% %                     }{
% %                         \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N
% %                     }
% %                 \cdot
% %                  % \biggr)
% %                  \,\mathbf{1}_N
% %              \big)$
% %             %%%% Synchronization Step
% %             % \State \eIf{$t \bmod T\neq 0$}{
% %             \State \tcc{Synchronize Local Experts via Nash Game}
% %             \State \eIf{$t \bmod T =  0$ and $t>0$}{
% %                 \State $\boldsymbol{\beta}^{\text{sync}}_t \leftarrow $ Run Synchronize Sub-Routine: Algorithm~\ref{alg:sync_subroutine}
% %                 \tcp*{Synchronized Weights}
% %                 \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
% %                     \State \ForParallel{
% %                     \State $\beta_t^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_t)_i$\;
% %                     \State Generate $\varepsilon_t^i$ \tcp*{Generate Random State}
% %                     \State $
% %                     \hat{Y}^i_t
% %                     \leftarrow
% %                     \hat{Y}^i_{t-1}
% %                     + 
% %                     (\beta_t^i)^{\top}\,
% %                     \varphi(x_{[0:t]},\varepsilon_t^i,Z_t^i)
% %                     $\;
% %                 }
% %               }
% %     \State \tcc{Server Synchronizes Local Expert Predictions}
% %     %%
% %     \State \Return $\hat{\mathbf{Y}}_t w_t$.
% %     \tcp*{Ensemble Prediction}
% % \end{algorithmic}
% % %\textbf{Note:} The helper functions $\mathbf{A},\mathbf{B},\mathbf{C},\Gamma$, and $\boldsymbol{\alpha}$ are defined in %circa Proposition~\ref{prop:NashEqmExistence} and the matrices $K$, $G$, and $\mathbf{c}$ are defined in~\eqref{eq:Gc_Def}.
% % \end{algorithm}

% \section{Experiment Details}
% \label{s:ExperimentDetials}


% This appendix contains additional technical details on our experiments.
% \subsection{Experiment Design}
% Time series performance is measured in mean-squared error (MSE) relative to the reference sequence. For a sequence of length $T$, predictions $\hat{y}_i \in \mathbb{R}^n$, and targets $y_i \in \mathbb{R}^n$, MSE is computed as 
% \begin{align*}
%     \text{MSE} = \frac{1}{T} \sum_{i=1}^T \Vert \hat{y}_i - y_i \Vert_2.
% \end{align*}
% For all simulations, unless otherwise stated, a hyper-parameter search is performed to find the best set of hyper-parameters minimizing the MSE for the time series in question. The set of hyper-parameters considered for both the Game and Non-Game settings are detailed in Tables \ref{tab:esn_hyperparams}-\ref{tab:transformer_hyperparams}. The hyper-parameter optimization is done post-hoc. However, the results compare the best possible performance of the two approaches in this idealized setting. In addition, several experiments in Section \ref{validation_studies} compare performance after hyper-parameter tuning on validation time-series. Sections \ref{sync_freq_studies} and \ref{lookback_studies} consider the effect of synchronization frequency and lookback length on the performance of the Nash game.

% Experiments considering ESN and RFN models demonstrate an inherent randomness due, for example, to the construction of their affine maps and perturbative noise. Thus, for these models, simulations are run with three random seeds ($2024$, $2025$, $2026$) in all settings and results are averaged over the three runs. This is done for both hyper-parameter tuning and reporting of final results.


% \subsection{Datasets} 
% \label{datasets}

% In this section, the details for each of the time-series datasets considered in the numerical experiments are laid out. In all, five unique time series are considered. Each incorporates different complexities for time-series prediction, varying length scales, and dimensionalities. Throughout this section, time series inputs are denoted as $\vec{x}$, targets as $\vec{y}$, and predictions as $\hat{\vec{y}}$

% \subsubsection{Periodic Signal}

% The Periodic Signal series is the simplest in terms of construction, but can be challenging for time series prediction due to its highly oscillatory nature. The series has $200$ data points taking on a minimum value of -0.9 and a maximum value of 0.9. The target regularly oscillates a number of times between these two values throughout the series. At each time step, $t$, a single target lag is used to make model predictions such that $x_{t-1} = y_{t-1}$ in predicting $y_t$. Figure \ref{fig:periodic_series} displays the target values of the series.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/periodic_series.pdf}
%     \caption{Periodic time series with 200 target values.}
%     \label{fig:periodic_series}
% \end{figure}

% \subsubsection{Logistic Map}

% The logistic map dataset is a synthetic time series based on the dynamics of the logistic map. The generating function from the EchoTorch library \cite{echotorch} is used to produce a time series with $200$ total data points. The default parameters for the EchoTorch dataset are applied, namely $\alpha=5$, $\beta=11$, $gamma=13$, $c=3.6$, and $b=0.13$. Figure \ref{fig:logistic_map_dataset} shows the resulting series. The target variable, $y$ has a single dimension. As with the Periodic dataset, a single step lag is provided as input for model predictions. That is, for time step $t$ and target $y_t$, the input is $x_{t-1} = y_{t-1}$.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/logistic_map_dataset.pdf}
%     \caption{Logistic map series progressing over $200$ time steps.}
%     \label{fig:logistic_map_dataset}
% \end{figure}

% \subsubsection{Concept Shift}

% The concept drift dataset considers and rapid change in the relationship of $\vec{x}$ and $\vec{y}$ halfway through. The series consists of $200$ points drawn from the following analytical relationship. Let $p$ be evenly spaced in the interval $[0, 2\pi]$. Then
% \begin{align*}
%     x_1 = p, && x_2 = p, && x_3 = \sqrt{p}.
% \end{align*}
% For $p \in [0, \frac{7}{8}\pi]$, $\vec{y} \in \mathbb{R}^2$ is
% \begin{align*}
%     y_{1, 1}(x_1, x_2, x_3) &= x_1^2 + \sin x_2 + x_1  x_3 + \frac{1}{2} \cos(10 x_1), \\
%     y_{2, 1}(x_1, x_2, x_3) &= x_1  \cos x_2 + x_3 - e^{-x_2}.
% \end{align*}
% For $p \in [\frac{9}{8} \pi, 2\pi]$,
% \begin{align*}
%     y_{1, 2}(x_1, x_2, x_3) &= x_1 + x_2 - \sin x_3 \\
%     y_{2, 2}(x_1, x_2, x_3) &= \cos x_1  \sin x_2 + x_3^2 + \frac{1}{4} \cos(10 x_1)
% \end{align*}
% The phase transition, where $p \in [\frac{7}{8} \pi, \frac{9}{8} \pi]$ is facilitated by the piecewise function
% \begin{align*}
%     \alpha(x) = \begin{cases}
%       1.0 & x < \frac{7}{8} \pi, \\
%       \cos(2(x_1 - \frac{7}{8}\pi) & \frac{7}{8} \pi \geq x \leq \frac{9}{8} \pi, \\
%       0.0 & x > \frac{9}{8} \pi. \\
%     \end{cases}
% \end{align*}
% Then the final series is written
% \begin{align*}
%     y_1(x_1, x_2, x_3) &= \alpha(x_1) \cdot y_{1, 1}(x_1, x_2, x_3) + (1-\alpha(x_1)) \cdot y_{1, 2}(x_1, x_2, x_3), \\
%     y_2(x_1, x_2, x_3) &= \alpha(x_1) \cdot y_{2, 1}(x_1, x_2, x_3) + (1-\alpha(x_1)) \cdot y_{2, 2}(x_1, x_2, x_3).
% \end{align*}
% Figure \ref{fig:concept_drift} provides a visualization of the series as a function of $x_1$.
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/concept_drift_plot.pdf}
%     \caption{Visualization of the concept drift time-series as a function of $x_1$.}
%     \label{fig:concept_drift}
% \end{figure}

% \subsubsection{Bank of Canada Exchange Rate}

% The Bank of Canada (BoC) Exchange Rate dataset \cite{boc_exchange_rates} records the daily exchange rates for $12$ different currencies, relative to the Canadian dollar (CAD), from May, 1, 2007 to April, 28, 2017. This constitutes $3,651$ observations per currency. Any one of the exchange rates may be used as a target with lagged currency values used as inputs. 

% In the numerical experiments, the target exchange rate is USD and inputs for model predictions at a given time step $t$ are $\{\text{USD}_{t-1}$, $\text{USD}_{t-2}$, $\text{AUD}_{t-1}$, $\text{AUD}_{t-2}$, $\text{EUR}_{t-1}$, $\text{EUR}_{t-2}$, $\text{GBP}_{t-1}$, $\text{GBP}_{t-2}$, $\text{JPY}_{t-1}$, $\text{JPY}_{t-2}\}$. Here, for example, $\text{JPY}_{t-1}$ is the exchange rate for the Japanese Yen from the previous time step. The experiments below consider the first $2000$ rates.

% Figure \ref{fig:boc_dataset} provides a visualization of the dataset for a subset of currencies over the entire time range.
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.45\linewidth]{figures/boc_exchange_rates.pdf}
%     \caption{Exchange rates relative to the Canadian dollar for a subset of the $12$ currencies tracked in the BoC exchange rate time series.}
%     \label{fig:boc_dataset}
% \end{figure}

% \subsubsection{Electricity Transformer Temperature} \label{ett_dataset}

% The Electricity Transformer Temperature (ETT) datasets were first introduced in \cite{haoyietal-informer-2021} as a difficult benchmark for the Informer time series model. The ETT-Small dataset is chosen for this work. The target value for prediction in each dataset is the oil temperature (OT) at a given time within one of two electricity transformers. The datasets span a time-frame from July 1, 2016 to June 26, 2018. In particular, the ETT-small-h1 time series is studied, which records temperature measurements every hour during this date-span along with measurements of six other input features.

% In the experiments below, the first $2000$ data points are used. All six input features (HUFL, HULL, MUFL, MULL, LUFL, LULL) are used to make predictions. When predicting $\text{OT}_t$, inputs include $\text{OT}_{t-1}$, $\text{OT}_{t-2}$, along with $\text{X}_{t-1}$, $\text{X}_{t-2}$, $\text{X}_{t-3}$, where $\text{X}$ is represents an aforementioned input feature. Finally, all values in the dataset have been normalized to by dividing the input and target sequences by the maximum value seen across the time series of interest. As discussed in Section \ref{normalization_study}, this is an important pre-processing step, as large input and target values tend to cause instabilities in the numerical computations and/or saturate the activation functions of the ESN and RFN models. While an exact normalization value may not be available during online prediction, an approximate normalizing scalar is likely sufficient.

% Figure \ref{fig:ett_dataset} exhibits a slice of the first $3$k steps in the time series along with the value of the input features at that time.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/ett_dataset.pdf}
%     \caption{A snapshot of the normalized ETT-Small-h1 dataset with target value OT overtime, along with the corresponding features used to help make predictions.}
%     \label{fig:ett_dataset}
% \end{figure}

% \subsection{Best Hyperparameter Choices in Each Experiment}
% \label{s:OptimalParamterChoices__a:TransExpHyper}

% The full set of hyper-parameters explored for each dataset, model combination, and Nash game setting are recorded in Tables \ref{tab:esn_hyperparams}-\ref{tab:transformer_hyperparams}. In each experiment, the parameters $\kappa$ and $\eta$ are each fixed to $1.0$. Additionally, for the transformer experiments, $d_z$ is fixed at $2$ for simplicity and empirical observations of better performance. Note that $\sigma$ is also not used in transformer models and is therefore irrelevant in hyper-parameter tuning.

% \subsubsection{Static Agents - Random Feature Networks}
% \label{s:OptimalParamterChoices__a:RFNs}

% \begin{table}[H]
% \centering
% \caption{Summary of hyper-parameters searched for RFN models across datasets and whether Nash game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$ and $\eta=1.0$, regardless of other hyper-parameters.}
% \label{tab:rfn_hyperparams}
% \resizebox{0.99\linewidth}{!}{\begin{tabular}{llccccccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & $\sigma$ & $d_z$ & Client $T$ & Game $T$ & Sync Freq. \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.0001}, 0.001, 0.01, 0.1, 1\}$ & $\{0.1, 1, 10, \mathbf{15}\}$ & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{3, 4, \mathbf{5}, 6, 7\}$ & $\{2, 3, 4, \mathbf{5}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.0001}, 0.001, 0.01, 0.1, 1\}$ & $\{0.1, 1, 10, \mathbf{15}\}$ & $\{0.01, \mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 4, 5, 6, 7\}$ & $\{\mathbf{2}, 3, 4, 5, 6\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 0.1, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $\{\mathbf{2}, 3, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, \mathbf{0.01}, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{0.1}, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.01, 0.1, \mathbf{1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{10, \mathbf{15}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{1, \mathbf{2}\}$ & $\{2, 3, 4, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{\mathbf{0.01}, 0.1, 1, 5\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, \mathbf{1}\}$ & $\{1, \mathbf{2}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.0001}, 0.001, 0.01\}$ & $\{10, \mathbf{15}\}$ & $\{0.01, \mathbf{0.1}\}$ & $\{3, 4, \mathbf{5}\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.0001, 0.001, \mathbf{0.01}\}$ & $\{10, \mathbf{15}\}$ & $\{\mathbf{0.01}, 0.1\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, 0.1, \mathbf{1.0}\}$ & $\{3, \mathbf{6}\}$ & $\{2, 3, \mathbf{5}\}$ & $\{\mathbf{2}, 3, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{0.1}, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{2, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.01, 0.1, \mathbf{1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, 1\}$ & $\{\mathbf{1}, 2\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{2, \mathbf{3}\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, \mathbf{0.1}, 1, 5\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, \mathbf{1}\}$ & $\{1, \mathbf{2}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}


% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{\sigma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 2 & 2 & 0.001 & 10.0 & 0.01 & 5 \\
% %                                            & 5 & 5 & 2 & 0.001 & 10.0 & 1.0  & 6 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 2 & - & 0.1   & 10.0 & 0.1  & 3 \\
% %                                            & 5 & 2 & - & 0.1   & 10.0 & 0.1  & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{random feature model} agents, in the Concept Drift dataset: two and five experts - Section~\ref{s:RFN_CD}.}
% % \label{tab:RFN_CD}
% % \end{table}

% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{\sigma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 2 & 2 & 1.0   & 10.0 & 1.0  & 3 \\
% %                                            & 5 & 5 & 2 & 0.01  & 10.0 & 1.0  & 6 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 2 & - & 0.01  & 10.0 & 1.0  & 3 \\
% %                                            & 5 & 5 & - & 1.0   & 10.0 & 1.0  & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{random feature model} agents, in the Bank of Canada Exchange dataset: two and five experts - Section~\ref{s:RFN_BoCX}.}
% % \label{tab:RFN_BoCX}
% % \end{table}

% \subsubsection{Semi-dynamic Agents - Pre-Trained Transformers}
% \label{a:TransExpHyper}

% \begin{table}[H]
% \centering
% \caption{Summary of hyper-parameters searched for Transformer models across datasets and whether Nash game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$, $\eta=1.0$, $d_z = 2$, and $\text{synchronization frequency} = 1$, regardless of other hyper-parameters.}
% \label{tab:transformer_hyperparams}
% \resizebox{0.65\linewidth}{!}{\begin{tabular}{llcccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & Client $T$ & Game $T$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{\mathbf{3}, 4, 5, 6, \mathbf{7}\}$ & $\{2, \mathbf{3}, 4\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $\{\mathbf{1}, 2, 3, 4\}$ \\
% & False & $\{0.001, \mathbf{0.01}, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{1, \mathbf{10}\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, 4, \mathbf{5}, 6\}$ & $\{2, \mathbf{3}, 4\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, 10, \mathbf{15}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $\{\mathbf{1}, 2, 3, 4\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, 6, 7, \mathbf{8}\}$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{2, 3, \mathbf{4}\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

% Before listing the hyperparameters for the ESN agents, we overview some important additional training details for the transformer netwoks.
% \paragraph{Additional Training Details}

% During the pre-training phase of the transformer model, the encoder and the final linear decoder layer are trained to predict the target sequence given the input sequence. This is achieved using a causal mask, which ensures that the transformer relies only on the current and previous time step inputs to predict  $\hat{y}_{t+1}$. The output of the transformer’s encoder is then passed to a final trainable linear layer to predict the target at $t+1$. After pre-training for a few epochs, the encoder of the transformer, excluding the final linear layer, is used as the encoder model in the main experiments.

% The first layer of the transformer is an embedding layer that maps the input dimension to the transformer's hidden dimension. A positional encoding layer is then added to the input. The resulting input is then passed to the transformer encoder.  The transformer encoder consists of two transformer layers, each consisting of self-attention and feed-forward networks. The number of expected features is set to $d_z \times d_y$, the number of heads is set to $2$, and the dimension of the feed-forward network is set to $16$, which are selected based on some initial hyper-parameter tuning of the model. The dropout is set to $0.1$ for all experiments. The decoder layer is the final linear layer that transforms the encoder’s output $Z_t$ from a dimension of $d_y \times d_z$ to $d_y$.  This final layer is dropped and trained again in the main algorithm.


% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 7 & 3 & 0.001   & 10.0 & 2 \\
% %                                            & 5 & 5 & 3 & 0.001   & 10.0 & 2 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 4 & - & 0.1     & 10.0 & 2 \\
% %                                            & 5 & 4 & - & 0.1     & 10.0 & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the Periodic Signal dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \end{table}

% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 4 & 1 & 1.0   & 10.0 & 2 \\
% %                                            & 5 & 4 & 1 & 1.0   & 10.0 & 2 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 4 & - & 0.01  & 10.0 & 2 \\
% %                                            & 5 & 6 & - & 0.001 & 15.0 & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the Logistic Map dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \end{table}

% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 4 & 2 & 1.0   & 10.0 & 2 \\
% %                                            & 5 & 4 & 2 & 1.0   & 10.0 & 2 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 6 & - & 1.0   & 1.0  & 2 \\
% %                                            & 5 & 8 & - & 1.0   & 1.0  & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the Concept Shift dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \end{table}

% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 6 & 2 & 5.0   & 10.0 & 2 \\
% %                                            & 5 & 3 & 2 & 5.0   & 1.0  & 2 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 6 & - & 5.0   & 1.0  & 2 \\
% %                                            & 5 & 6 & - & 5.0   & 1.0  & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the BoC Exchange Rate dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \end{table}

% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 3 & 2 & 1.0   & 1.0  & 2 \\
% %                                            & 5 & 3 & 4 & 1.0   & 1.0  & 2 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 3 & - & 5.0   & 1.0  & 2 \\
% %                                            & 5 & 6 & - & 5.0   & 1.0  & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the ETT Series dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \end{table}



% \subsubsection{Fully Dynamic Agents - Echo State Networks}
% \label{s:OptimalParamterChoices__a:ESNs}

% \begin{table}[ht]
% \centering
% \caption{Summary of hyper-parameters searched for ESN models across datasets and whether Nash game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$ and $\eta=1.0$, regardless of other hyper-parameters. Bolded numbers correspond to the optimal parameters based on mean MSE in the experiments.}
% \label{tab:esn_hyperparams}
% \resizebox{0.99\linewidth}{!}{\begin{tabular}{llccccccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & $\sigma$ & $d_z$ & Client $T$ & Game $T$ & Sync Freq. \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2, 3\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, \mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{2, 5, \mathbf{10}\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{3, \mathbf{6}, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{1}, 2, 3\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{1, 2, \mathbf{3}\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $-$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 10\}$ & $\{0.01, 0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2, 3\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 10\}$ & $\{0.01, 0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{1\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}\}$ & $\{\mathbf{2}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{3, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{\mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{\mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{1}, 2, 3\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{1, 2, \mathbf{3}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

% % \begin{table}[!htbp]%
% % \centering
% % \begin{tabular}{@{}llccc@{}}
% % \toprule
% %  & & \textbf{2 Experts} & \textbf{5 Experts} \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game setting}} & Client $T$ & 2 & 2 \\
% % & Game $T$ & 3 & 3 \\
% % & $\alpha$ & 0.001 & 0.001 \\
% % & $\gamma$ & 10.0 & 10.0 \\
% % & $\sigma$ & 1.0 & 1.0 \\
% % & $d_z$ & 3 & 3 \\[2mm]

% % \multirow{2}{*}{\textbf{Non-game setting}} & Client $T$ & 5 & 5 \\
% % & $\alpha$ & 0.1 & 0.1 \\
% % & $\gamma$ & 10.0 & 10.0 \\
% % & $\sigma$ & 0.01 & 0.01 \\
% % & $d_z$ & 3 & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the Periodic Signal dataset: two and five experts - Section~\ref{s:Experiments__ss:ESN_PS}.}
% % \label{tab:best_hyperparameters_game_non_game_PS}
% % \end{table}


% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{\sigma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 3 & 3 & 0.001 & 10.0 & 0.1 & 3 \\
% %                                            & 5 & 3 & 3 & 0.001 & 10.0 & 0.1 & 3 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 3 & - & 0.1   & 10.0 & 1.0 & 3 \\
% %                                            & 5 & 3 & - & 0.1   & 10.0 & 1.0 & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{echo state network} agents, in the Periodic Signal dataset: with two and five experts - Section~\ref{s:ESN_PS}}
% % \label{tab:ESN_P}
% % \end{table}


% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{\sigma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 5 & 3 & 0.0001 & 15.0 & 0.01 & 5 \\
% %                                            & 5 & 3 & 3 & 0.0001 & 15.0 & 0.1  & 5 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 2 & - & 0.001  & 10.0 & 0.1  & 3 \\
% %                                            & 5 & 3 & - & 0.01   & 15.0 & 0.01 & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{echo state network} agents, in the Logistic Map dataset: two and five experts.}
% % \label{tab:ESN_LM}
% % \end{table}

% % \begin{table}[!htbp]%
% % \centering
% % \begin{tabular}{@{}llccc@{}}
% % \toprule
% %  & & \textbf{2 Experts} & \textbf{5 Experts} \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game setting}} & Client $T$ & 5 & 5 \\
% % & Game $T$ & 3 & 2 \\
% % & $\alpha$ & 0.001 & 0.001 \\
% % & $\gamma$ & 1.0 & 10.0 \\
% % & $\sigma$ & 1.0 & 1.0 \\
% % & $d_z$ & 6 & 6 \\[2mm]

% % \multirow{2}{*}{\textbf{Non-game setting}} & Client $T$ & 2 & 3 \\
% % & $\alpha$ & 0.001 & 0.1 \\
% % & $\gamma$ & 10.0 & 10.0 \\
% % & $\sigma$ & 0.01 & 1.0 \\
% % & $d_z$ & 6 & 6 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the Bank of Canada dataset: two and five experts - Section~\ref{s:Experiments__ss:transformer_results}.}
% % \label{tab:best_hyperparameters_game_non_game}
% % \end{table}


% % \begin{table}[!htbp]
% % \centering
% % \begin{tabular}{@{}lccccccc@{}}
% % \toprule
% % \textbf{Setting} & \textbf{Experts} & \textbf{Client $T$} & \textbf{Game $T$} & $\boldsymbol{\alpha}$ & $\boldsymbol{\gamma}$ & $\boldsymbol{\sigma}$ & $\boldsymbol{d_z}$ \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game Setting}}     & 2 & 5 & 2 & 5.0   & 15.0 & 0.1 & 2 \\
% %                                            & 5 & 2 & 3 & 5.0   & 10.0 & 0.1 & 1 \\[2mm]
% % \multirow{2}{*}{\textbf{Non-Game Setting}} & 2 & 3 & - & 0.01  & 10.0 & 1.0 & 2 \\
% %                                            & 5 & 3 & - & 0.1   & 10.0 & 1.0 & 2 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{echo state network} agents, in the ETT Series dataset: two and five experts - Section~\ref{s:ESN_ETTSeries}.}
% % \label{tab:ESN_ETT}
% % \end{table}

% % \begin{table}[!htbp]%
% % \centering
% % \begin{tabular}{@{}llccc@{}}
% % \toprule
% %  & & \textbf{2 Experts} & \textbf{5 Experts} \\
% % \midrule
% % \multirow{2}{*}{\textbf{Game setting}} & Client $T$ & 2 & 2 \\
% % & Game $T$ & 2 & 2 \\
% % & $\alpha$ & 5.0 & 5.0 \\
% % & $\gamma$ & 1.0 & 1.0 \\
% % & $\sigma$ & 1.0 & 1.0 \\
% % & $d_z$ & 1 & 1 \\[2mm]

% % \multirow{2}{*}{\textbf{Non-game setting}} & Client $T$ & 2 & 3 \\
% % & $\alpha$ & 5.0 & 5.0 \\
% % & $\gamma$ & 1.0 & 1.0 \\
% % & $\sigma$ & 1.0 & 1.0 \\
% % & $d_z$ & 3 & 3 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Best hyper-parameters for game and non-game \textit{pre-trained transformer} agents, in the ETT Series dataset: two and five experts - Section~\ref{s:ESN_ETT}.}
% % \label{tab:best_hyperparameters_game_non_game}
% % \end{table}






% \newpage

% \subsection{Further Ablation Studies}
% \label{s:Ablations}

% This section contains additional, relevant ablation studies whose information can be useful for the successful deployment of our FL pipeline.


% \subsubsection{ReLU Activations and ESN Recursion} \label{activation_discussion}

% Recently, it has been shown that ESN models with ReLU activations have desirable properties, including Universality \cite{Gonon1}. A natural question then is why use Hard Sigmoid activations in the models explored here. Peripherally, the work in \cite{Li6} extends many of the properties proven in \cite{Gonon1} to ESNs for general activation function. However, the primary motivation is the unbounded nature of the ReLU activation function can result in significant growth in the Froebenius norm of the latent representations, $Z_t$. Such growth produces poorly conditioned matrices. This can be problematic for both the numerical solution of the ridge regression problems required for predictions without the Nash game and the more complex systems required for the proposed Nash game synchronization.

% Consider the following code to replicate the recurrence relationship for the latent space of the ESN. 

% \begin{minted}[bgcolor=white]{python}
% import torch
% from torch.nn import ReLU
% from typing import Tuple
% import statistics

% def generate_random_tensor(
%     shape: Tuple[int, ...], device: torch.device = torch.device("cpu")
% ) -> torch.Tensor:
%     return torch.randn(shape, device=device)

% def generate_linalg_components(
%     x_dim: int, y_dim: int, z_dim: int
% ) -> Tuple[torch.Tensor, torch.Tensor, torch.Tensor]:
%     A = generate_random_tensor((y_dim, x_dim))
%     B = generate_random_tensor((y_dim, y_dim))
%     b = generate_random_tensor((y_dim, z_dim))
%     return A, B, b

% def generate_random_state(
%     sigma_t: torch.Tensor, z_dim: int, y_dim: int
% ) -> torch.Tensor:
%     W_t = torch.normal(mean=torch.zeros((1, z_dim)), std=1.0)
%     random_state = torch.matmul(sigma_t, W_t)
%     return random_state

% torch.manual_seed(42)
% x_0_sequence = torch.arange(0.1, 1.1, 0.1)
% x_1_sequence = torch.arange(0.2, 2.2, 0.2)
% x_sequence = torch.stack([x_0_sequence, x_1_sequence], dim=1)
% z_dim, y_dim, x_dim = 5, 3, 2
% sigma_t = torch.Tensor([0.1, 0.2, 0.3]).reshape(-1, 1)
% largest_values = []

% for _ in range(100):
%     A, B, b = generate_linalg_components(x_dim, y_dim, z_dim)
%     Z = torch.zeros((y_dim, z_dim))
%     for x_t in x_sequence:
%         input = x_t.reshape(-1, 1)
%         input_matrix = input.repeat(1, z_dim)
%         random_state = generate_random_state(sigma_t, z_dim, y_dim)
%         AX = torch.matmul(A, input_matrix)
%         BZ = torch.matmul(B, Z)
%         Z = ReLU()(AX + BZ + b + random_state)
%     largest_values.append(torch.max(Z).item())

% print(f"Mean: {statistics.mean(largest_values)}")
% print(f"Max: {max(largest_values)}")
% \end{minted}

% In the above, the input features are quite reasonable and the length of the time series is only 10 time steps long. In spite of this, for unlucky draws, the magnitude of elements for $Z$ grow extremely rapidly. The largest of which is $87025$ in this simulation. Over the $100$ simulation trajectories, the mean value for the largest element in $Z$ is $1937$. While the distribution is fairly skewed by outliers, this example demonstrates the potential hazard in using ReLU activations in ESNs over long time series. Using a bounded activation function, such as the Hard Sigmoid used in the experiments above, largely mitigates this issue.

% \subsubsection{ESN and RFN Models on Unnormalized Data} \label{normalization_study}

% In Section \ref{ett_dataset}, the importance of normalizing the inputs and outputs of the ETT time series is briefly mentioned. In this section, some studies considering the impact of failing to scale data when using ESN or RFN models with Hard Sigmoid functions. Consider a toy dataset composed of three Brownian motion trajectories with drift \cite{Glasserman1}. For each trajectory, the Brownian motion has a $\mu = 1.0$ and $\sigma = 1.0$. At each time step, the target is simply the sum of $x_t = 0.1\cdot t$ and the value of trajectory $i$ at that time step, $b_{i, t}$. The inputs are simply $x_t$ and $b_{i, t}$. So the model need only learn to properly add these two values together to make an accurate prediction. In the examples below, a time series of length $200$ is used, three trajectories are sampled as targets, two experts are present for the mixture, and ESN models are used.

% As seen in Figure \ref{fig:normalization}, the values of the Brownian trajectories quickly grow fairly large, implying that the model inputs also grow steadily. Examining the server predictions without Nash synchronization, it is clear that the server is unable to mix predictions from the two clients to make predictions for target variable $y_2$. The root cause of this failure is seen in considering the predictions produced by the individual clients. Both clients fail to produce meaningful predictions for $y_2$. Furthermore, Client 1 produces extremely poor predictions for all target dimensions. Thus, the server must rely exclusively on predictions from Client 0 to produce any meaningful predictions at all. Note that these issues remain present, even after significant hyper-parameter tuning.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/normalization/server_predictions_plot.pdf}
%     \includegraphics[width=0.95\linewidth]{figures/normalization/client_predictions_plot.pdf}
%     \caption{Predictions for the server (top) and individual clients (bottom) for the synthetic Brownian motion dataset. Due to the large input and target values, the clients, especially Client 1, fail to produce good predictions using ESN models.}
%     \label{fig:normalization}
% \end{figure}

% The driver of these failures is a collapse in the latent representations, $Z$, from which clients derive their predictions. Recall that, for ESN models, 
% \begin{align*}
%     Z_t^i &= \text{Hard Sigmoid}\left (A^i x_t + B^i Z_{t-1}^i b^i + \sigma^i W_t^i \right) \\
%     \hat{Y}_{t+1}^i &= \hat{Y}_t^i + Z_t^i \beta_t^i.
% \end{align*}
% If a row of $Z_t^i$ were to become zero, the previous prediction $\hat{Y}_t^i$ remains constant in that dimension, regardless of $\beta_t^i$. If the inputs to the Hard Sigmoid become negative enough, this can happen repeatedly. In the case of Figure \ref{fig:normalization}, after a few steps, the latent matrix $Z$ becomes zero across the board for Client 1 and the second row becomes zero for Client 0. 

% This deficiency may be addressed in several ways. For example, a $\tanh$ function might be substituted for the Hard Sigmoid activation. Thereby removing the vanishing representation problem. However, the issue of saturating the extremes of the activation function remains present. Experimentally, a suitable solution for the ETT time series is normalization of the input and output variables by some computed maximum. This approach was applied for all experiments. However, it is likely that an ideal setup would be a combination of the $\tanh$ activation and normalization.



% \newpage
% ~
% \newpage
% \pagebreak
% David's na\"{i}ve questions and suggestions. \\
% \underline{Section 1.1} \\
% \begin{enumerate}
%     % \item Should $\mathbb{N}_{+}$ be defined? Not sure how common the notation is, so wanted to ask.
%     % \AK{@X pls define} 
%     % \Xuwei{done in the first paragraph of Section 1.1}
    
%     % \item $d_x$, $d_z$, $d_\epsilon$ are not explicitly defined. That is, as the dimensionality of the respective variables $\geq 1$.
%     % \AK{@X pls define} 
%     %  \Xuwei{done in the first paragraph of Section 1.1}
%     \item For the general setup (Defined in and near Equation (1)), we have 
%     \begin{align*}
%     Z^i_{t+1} &= \varphi^{(i)}(x^i_{[0:t]}, Z_t^i, \epsilon_t^i), \\
%     \hat{Y}_{t+1}^i &= \hat{Y}^i_t + Z_t^i \beta_t.
%     \end{align*}
%     This implies that when generating the prediction for the next time step $t+1$, $Z_t^i$ is based on $x^i_{[0:(t-1)]}$, which seems strange. Would we not also use $x_t$ in computing the $Z_t^i$ off of which we're basing our predictions? It seems like we should instead have the relationship 
%     \begin{align*}
%     Z^i_{t} &= \varphi^{(i)}(x^i_{[0:t]}, Z_{t-1}^i, \epsilon_t^i), \\
%     \hat{Y}_{t+1}^i &= \hat{Y}^i_t + Z_t^i \beta_t.
%     \end{align*}

%     \item In Equation (5), I don't think we have the right residual relationship, at least based on my understanding of the minimization we're trying to do. For a given $s$, we have the update equation $\hat{Y}^i_{s+1} = \hat{Y}^i_{s} + Z^i_{s} \beta^i_t$, if we're optimizing over a fixed $\beta_t^i$. So shouldn't the residual relationship that we want to minimize be $\Vert (y_{s+1} - \hat{Y}_{s}^i) - Z^i_{s} \beta^i_t\Vert$? If this is correct, this causes some issues about how things are computing in the first steps, since, for example, we don't have a residual for $t=0$.

%     \item In Equation (3), is $\sigma_t^i$ fixed and random like $A^i$ and $b^i$ or does it vary with time? The use of the subscript $t$ seems to suggest it varies with time. However, we don't explicitly state that anywhere. A similar distribution question as in the question above would also apply.
    
%     \item I think, throughout, we could simplify the notation for vectors by stating that $x \in \mathbb{R}^n$ for integer $n$ is assumed to be a column vector throughout rather than using the heavier notation $x \in \mathbb{R}^{n \times 1}$. If we want to specify a row vector, we could either use transpose or use the heavier notation $x \in \mathbb{R}^{1 \times n}$
%     \AK{I agree} 
    
%     % \item Should $\epsilon_r^i$ be $\epsilon_t^i$ above Equation (1)? 
    
%     % \Xuwei{Yes, it's corrected now.}
    
%     \item The range space for the encoder $\varphi^{(i)}$ is denoted as $\mathbb{R}^{d_z \times 1}$ above Equation (1) but then $Z^i$ is said to be in $\mathbb{R}^{d_y \times d_z}$ in defining $\hat{Y}_{t+1}^i$, which is incompatible.
%     \AK{either we transpose or, better, Y's dimension should be fixed}
%     \item I'm not sure the notation $\mathbb{R}^{\mathbb{N}}$ is well-defined, since $\mathbb{N}$ is a vector space. Maybe it's standard notation, but I think maybe defining $f^{(i)}: \mathbb{R}^{d_x} \rightarrow \mathbb{R}^{d_y}$ is more clear?
%     \AK{Sure I agree; but $\mathbb{R}^{\mathbb{N}}$ is well-defined as a TVS (actually as a Frechet space; but not as a Banach space), its $\prod_{t=0}^{\infty}\,\mathbb{R}$ with Fr\'{e}chet metric $d(x_{\cdot},y_{\cdot})\eqdef 
%     \sum_{t=0}^{\infty}\, \frac1{2^t}\,\frac{|x_t-y_t|}{1+|x_t-y_t|}
%     $; recall that $(x,y)\mapsto \frac{|x-y|}{1+|x-y|}$ generates the norm topology on $\mathbb{R}$; but it has the nice property of being bounded :)
%     }
%     % \item For $x_. \rightarrow \hat{Y}_t^i$ should that . be $x_{[0:t]}^i$ as in definition (1)?
%     % \AK{yes} 
%     % \Xuwei{$x_\cdot$ is changed to $x^i_{[0:t]}$}
    
%     % \item In Example 1.1, is there a reason we use $\beta_0$ for the decoder layer instead of $\beta_t$?
%     % \AK{should be $\beta_t$} 
%     % \Xuwei{corrected.}
    
% %     \item We don't define the bullet notation (used in Equation (3) for example) before its use. I think it's for element-wise application of the function? Maybe its very standard, so disregard if so. 

% % \Xuwei{The definition of $\bullet$ is added to Example 1.2.}
    
%     \item For $A^i$ and $b^i$ are there any restrictions on these matrices distributions? I.e. can we draw them uniformly from [0, 1] (for example) or are they truly random and unbounded?
%     \AK{In the context of this paper, no; but for good (E.g. univerality) properties one may take random Gaussian (as in https://arxiv.org/abs/2104.13669 similarly this paper https://bmild.github.io/fourfeat/) or with uniformly distributed columns (as in https://arxiv.org/abs/2002.05933).}

%     \item The time indices in Equation (4) don't seem to match those of other settings (Equation (3) for example). That is, to be consistent I think $\hat{Y}^i_{t+1} \eqdef \hat{Y}^i_{t} + Z_t \beta_t$?
    
%     % \item There is a bit of redundancy in the definitions of $\varphi$ and $Z_t^i$ near Equation (3). Would it perhaps be simpler to just write $\varphi^{(i)}(x_{[0:t]}^i,Z_t^i, \varepsilon_t^i)\eqdef \operatorname{ReLU}\bullet\big(A^{i} x_t + b^{i} + \sigma_t^i \, W_t^i\big) = Z_{t+1}^i$?
%     % \AK{Agreed :)} 
%     % \Xuwei{Done.}
    
%     % \item For the definitions in Equation (4), we seem to be using the old notation of $(\beta_{t+1}^i)^T$. Maybe we should make it consistent with (3)?
%     % \AK{Yes} 
%     % \Xuwei{Done.}
    
%     % \item We seem to be taking the square root of $\sigma_t^i$ in Equation (4), but not doing so in Equation (3). We should probably be consistent? Are there any implications for this mismatch in the downstream calculations?
%     % \AK{Thanks, yes :)} 
%     % \Xuwei{Now we use $\sigma^i_t W^i_t$ without taking square root of $\sigma^i_t$.}
%     \item Above Equation (1), we are defining our general decoder $\varphi^{(i)}: \mathbb{R}^{d_x} \times \mathbb{R}^{d_z} \times \mathbb{R}^{d_{\epsilon}} \rightarrow \mathbb{R}^{d_y \times d_x}$. However, given our definitions below, should this be revised to be $\varphi^{(i)}: \mathbb{R}^{d_x \times d_z} \times \mathbb{R}^{d_y \times d_z} \times \mathbb{R}^{d_y \times d_z}$? This sort of "narrows" how these pieces can be put together. For example, the noise doesn't technically \emph{have} to be of this dimensionality. It just does in our examples. Maybe there is a more generic notation we can use for the domain and range spaces of $\varphi^{(i)}$?
% \end{enumerate}
% \underline{Section 1.2}
% \begin{enumerate}
% \item As in the previous section $(\mathbb{R}^{d_{x}})^{\mathbb{Z}}$, is a little unorthodox given the integers are a vector space. Could we use the notation $(\mathbb{R}^{d_{x}})^N$?
% \item In the equation for $\hat{F}$, we don't really define the $.$ notation on $x.$ I think we're using it as shorthand for $x^i_{[0:t]}$? If so, we could either write that explicitly or define the notation somewhere?
% \item In the equation for $\hat{F}$, we haven't defined an $\hat{f}^i$ that I'm aware of at this point? Perhaps we can just drop the hat notation? It seems like we could also drop it for $F$ as well for brevity?
% \item In the definition $w_{\cdot}\eqdef (w_t)_{t\in \mathbb{Z}}$, I think we want to define t as being in $\mathbb{N}$ rather than $\mathbb{Z}$, to match our definition in Secton 1.1? Also, I may be wrong, but I'm not sure we use the $w_{\cdot}$ notation elsewhere, except in the phrase ...optimizes the $w_{.}$ and $\beta_{i}$... So we might just drop the notation and write something like: ...for mixture coefficients $w_t \in \mathbb{R}^N$ for all $t \in \mathbb{N}_+$... and ...optimizes the $w_t$ and $\beta_t$...
% \item In defining the simplex $\Delta_N$, we use a subscript $i$ rather than a superscript, which we use in other places. Maybe we should change it to be consistent?
% \item For Equation 5, we don't state what values $\alpha_i$ (same for $\gamma_i$) can take on. It's constraint is in Proposition 1, namely $\alpha_i \geq 0$ (and $\gamma_i$), but it seems like we should state that directly before or after the definition of Equation (5). It would likely also be helpful to state that we are, in essence, discounting past errors in favor of higher weights on more recent errors (or something of that kind)
% \item There are a few places, for example in the definition of $\Delta_N$, where we're implying that the mixture weights $w^i_t$ need to be $\geq 0$. However, in Equation (8), that constraint is relaxed. We might want to mention that it is relaxed "below" in these places so someone doesn't get confused when the definition of $\Delta_N$ becomes slightly different.
% \item While it is sort of implied to be the l2-norm, we don't strictly define the norm we're using for $\Vert \cdot \Vert$. I think any norm is likely valid. So we could also state that.
% \item Immediately following Proposition 1, we have the phrase ``Each expert then immediately communicates their prediction $\hat{Y}_t^i$.'' However, in Equation (5), we are optimizing using predictions and labels up to $t$. So I think the prediction we're communicating with the server is properly indexed as $\hat{Y}_{t+1}^i$?
% \item Similar to the question above, we want the server to be making a prediction for $t+1$ (I think). So we would rephrase ...to aggregate the predictions of
% each expert into a weighted prediction of the form $\sum_{i=1}^N w_t^i \hat{Y}^i_{t+1}$ in such a way...?
% \item We have the commentary "In each such round the $N$ machines communicate their past $T$ predictions with one another; however, they do not communicate their entire model with one another since that would take an infeasible bandwidth due to the size of each local model. Instead, the local machines are only aware of the predictions generated by one another with the objective of maximizing their predictive power." Two thoughts.
% \begin{itemize}
%     \item We're already communicating these predictions to the server and it's the server computing the Nash game. So if the server stores the old predictions in a buffer, then there is no additional communication overhead (which is a benefit).
%     \item Even if the models are small, avoiding full weight communication is beneficial from a privacy perspective, as it means the server never sees the full individual models. It might be worth including these? 
% \end{itemize}
% \item One other thing that does need to be communicated with the server (I think) that we haven't stated is the value of $Z_0^i$ if expectations with respect to the latent variable are required. I think we want to state that, along with how the expectations are computed to make it easier on the reader? It's also potentially worth noting for the reader that the $Z_t^i$ are independent of $\beta_t^i$?
% \item Are the $alpha_i$ in Equation (9) necessarily the same $\alpha_i$ from Equation (5)? It sort of makes sense that they would be the same, but maybe we can make that explicit with a statement?
% \item In defining (9), we don't explicitly state anywhere that, for notational simplicity, we're denoting t=0 to be the time of the last sync. That is, it is a stand-in for $s=t-T \vee 0$
% \item In some places, we use parenthesis to denote matrices or vectors (see definitions of $\mathbf{w}_t$ and $\hat{Y}_t$) and others we use square brackets, see Equation (11) definition of $\boldsymbol{\beta}$. We probably want to be consistent?
% \end{enumerate}
% \underline{Section 1.3}
% \begin{enumerate}
% \item We aren't quite consistent with when we use $\varphi$ vs. $\phi$ to denote the encoder function. For example, in Section 1.1 we predominantly use $\varphi$, but in Section 1.3.1 we use $\phi$. Maybe I'm missing a reason for that though?
% \item We might want to state explicitly that the defintion of A(t) is a blockwise indexed definition (i.e. versus specifying an element at a time)? I was initially confused when tracing the dimensionality
% \item In Corollary 1, in the definition of $a(t, i)$ we have $\bar{1}$, which isn't defined here. I see we have a definition in Lemmas 1,2 but those come much later.
% \item In Lemmas (1) and (2), are we missing a transpose on $(Z^i_{t+1})_j$ in $\mathbb{E}[(Z^i_{t+1})_jb(Z^i_{t+1})_k]$? It doesn't match the shapes that I expected.
% \item We define $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$ in both Lemmas (1) and (2). However, it doesn't look like it appears anywhere in the equations? It's also unclear to me what $(a_{t\,j}^2)_{j=1}^{d_z}$ actually means when $(a_t^i)_j \in \mathbb{R}^{1\times d_z}$ and $a_t \in \mathbb{R}^{d_y \times d_z}$. Is $a_t^2$ equivalent to $(a_t^i)_j \odot (a_t^i)_j$? We do have $(\sigma_j^i)^2$ in there. Does this have the same meaning? 
% \item In Algorithm 1, I think the update equation for $Z_{t+1}$ needs a bit of a fix. To match previous notation, I think $Z^i_{t+1} \leftarrow \varphi^{(i)}\left(x^i_{[0:t]}, Z_t^i, \epsilon^i_t\right)$ might be the right fit?
% \item In Algorithm 1, it seems like the time indices for the lines of // update hidden state and // update residual prediction are not in sync. It seems like we should be updating $\hat{Y}^i_{t+1}$ as $\hat{Y}^i_{t+1} \leftarrow \hat{Y}^i_{t} + Z_t \beta_t$? Also note the update to the $Z_t \beta_t$ part.
% \item In the prediction after the Nash synchronization, we have the old $\beta_t^i$ shape and (as above), I think we want to write $\hat{Y}^i_{t+1} \leftarrow \hat{Y}^i_{t} + \varphi^{(i)}\left(x^i_{[0:t]}, Z_t^i, \epsilon^i_t\right)\beta_t$? The reasoning here is that starting at $t=0$ and predicting for $t=1$ this makes the definition of $\bar{y}_t$ and others work with the present indexing etc.
% \item In Algorithm 1, we have the comment ``Server Synchronizes Local Expert Predictions.'' Is this just a comment about the return value of $\hat{\mathbf{Y}}_t w_t$ or is another calculation happening, like re-optimizing the $w_t$?
% \item For the Nash calculations, rather than doing an all-to-all communication of predictions, server weights, etc. between the clients, might we just use the server to compute the Nash game for everyone? It's already receiving the predictions from each client and producing the mixture weights. So the communication overhead would be smaller.
% \item It seems like, based on the numbering in Algorithm 2, the indices are out of sync with Algorithm 1. That is, if we're at time step $T$ (for simplicity the first sync step) we want to compute $\beta^i_T$ via the Nash game, where $\beta^i_T$ is one component of $\boldsymbol{\beta}_T^{\text{sync}}$. However, in Algorithm 2, it looks like $\boldsymbol{\beta}_t$ is only computed up to $T-1$? How do we get the final $\boldsymbol{\beta}_T$?
% \end{enumerate}


% \end{document} 

==> Historical_Versions/2025_04_28.tex <==
% \documentclass[twoside,11pt]{article}

% \usepackage{blindtext}

% % Any additional packages needed should be included after jmlr2e.
% % Note that jmlr2e.sty includes epsfig, amssymb, natbib and graphicx,
% % and defines many common macros, such as 'proof' and 'example'.
% %
% % It also sets the bibliographystyle to plainnat; for more information on
% % natbib citation styles, see the natbib documentation, a copy of which
% % is archived at http://www.jmlr.org/format/natbib.pdf

% % Available options for package jmlr2e are:
% %
% %   - abbrvbib : use abbrvnat for the bibliography style
% %   - nohyperref : do not load the hyperref package
% %   - preprint : remove JMLR specific information from the template,
% %         useful for example for posting to preprint servers.
% %
% % Example of using the package with custom options:
% %
% % \usepackage[abbrvbib, preprint]{jmlr2e}

% \usepackage{jmlr2e}
% \usepackage{subcaption}
% \input{packages}
% \input{mathcommands}
% \input{Commenting}
% \usepackage{booktabs}
% \usepackage{longtable}
% \usepackage{multirow}
% \usepackage{geometry}
% \geometry{margin=1in}
% \usepackage{lastpage}
% % \jmlrheading{23}{2024}{1-\pageref{LastPage}}{1/21; Revised 5/22}{9/22}{21-0000}{Xuwei Yang, Fatemeh Tavakoli, Anastasis Kratsios, and David B. Emerson}

% \ShortHeadings{Online Federation For Mixtures of Proprietary Agents with Black-Box Access}{Xuwei Yang, Fatemeh Tavakoli, Anastasis Kratsios, and David B. Emerson}
% \firstpageno{1}

% \begin{document} 

% \title{Online Federation For Mixtures of Proprietary Agents\\ with Black-Box Encoders}

% \author{\name Xuwei Yang 
%   \email yangx212@mcmaster.ca \\
% \addr Department of Mathematics\\
%   McMaster University\\
%   Ontario, Canada 
%   \AND
%    \name
%    Fatemeh Tavakoli
%    \email 
% fatemeh.tavakoli@vectorinstitute.ai
%    \\
% \addr Vector Institute\\
%     Ontario, Canada 
%   \AND
%   Anastasis Kratsios\thanks{Corresponding Author. 
%   Funded by NSERC DG No.\ RGPIN-2023-04482.} 
%   \email 
%   kratsioa@mcmaster.ca
%   \\
%  \addr  Department of Mathematics\\
%   McMaster University and the Vector Institute\\
%   Ontario, Canada 
%   \AND
%   \name David B. Emerson 
%   \email 
% david.emerson@vectorinstitute.ai \\ 
% \addr  Vector Institute\\
%     Ontario, Canada 
% }

% \editor{}

% \maketitle

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract} 
% Most industry-standard generative AIs and feature encoders are proprietary, offering only black-box access: their outputs are observable, but their internal parameters and architectures remain hidden from the end-user.  This black-box access is especially limiting when constructing mixture-of-expert type ensemble models since the user cannot optimize each proprietary AI's internal parameters.  Our problem naturally lends itself to a non-competitive game-theoretic lens where each proprietary AI (agent) is inherently competing against the other AI agents, with this competition arising naturally due to their obliviousness of the AI's to their internal structure.  In contrast, the user acts as a central planner trying to synchronize the ensemble of competing AIs.  

% We show the existence of the unique Nash equilibrium in the online setting, which we even compute in closed-form by eliciting a feedback mechanism between any given time series and the sequence generated by each (proprietary) AI agent.  Our solution is implemented as a decentralized, federated-learning algorithm in which each agent optimizes their structure locally on their machine without ever releasing any internal structure to the others.  We obtain refined expressions for pre-trained models such as transformers, random feature models, and echo-state networks.  Our ``proprietary federated learning'' algorithm is implemented on a range of real-world and synthetic time-series benchmarks. It achieves orders-of-magnitude improvements in predictive accuracy over natural benchmarks, of which there are surprisingly few due to this natural problem still being largely unexplored.
% \end{abstract}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%% Section 1: Instruction %%%%%%
% %\section{Introduction}
% %\label{chp:intro}

% %Input data $x=(x_1, ..., x_d)\in \mathbb{R}^d$. 
% % \begin{comment}

% \section{Introduction} 
% \label{s:Intro}

% % What is Propreitary setting and why its important
% The modern era of mainstream deep learning has witnessed the emergence of ensembles of proprietary models with public \textit{black-box} access; that is, the users do not know nor can they modify the inner structure of these AIs used to build their ensemble models. 
% Examples include standard large pre-trained language and image encoders such as CLIP \citep{radford2021learning}, purely image-based encoders like DINO(v2) \citep{caron2021emerging,oquab2024dinov2learningrobustvisual}, pre-trained large language encoders SLIP(v2) \citep{mu2022slip,tschannen2025siglip}, or directly using the outputs of proprietary LLMs, e.g. \citep{chatgpt} or \citep{guo2024deepseek} as deep features. 
% A similar scenario arises within organizations where different teams -- for example, trading desks in a financial institution -- employ distinct models whose structures are not disclosed to one another. In such cases, only the predictions are shared, rendering traditional machine-learning techniques inapplicable since the user does not have access to, and thus \textit{cannot train}, these models.

% % Why FL, but why not classical FL
% Our problem naturally lends itself to a \textit{federated learning} (FL) approach, where a single computational task is distributed among many decentralized agents. These models are synchronized by the user/server.  This is because, in this setting, each agent can hold their own model's information locally while only releasing their predictions to the ensemble. Though the FL view may be natural when optimizing an ensemble of proprietary AIs, the black-box constraint pulls it out of the standard FL toolbox. This is because traditional FL setups, e.g. \citep{Even22SampleOptimalityFL,Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}, work by (partially) averaging local model parameters on the central server or their (partial) gradients, requiring full (white-box) access to each agent.

% It is, thus, natural to approach our \textit{proprietary federated learning (PFL)} problem through a non-cooperative game-theoretic lens, recognizing that each agent can optimize their own predictions but they are constrained to act non-cooperatively by virtue of them not knowing the structure of any other agent.  Instead, the agents are guided towards cooperation by the user, acting as a central planner, who continually re-weights the contributions of each expert’s prediction to maximize the ensemble’s overall predictive performance.  This non-cooperative game-theoretic perspective provides a meaningful notion of an \textit{optimal} PFL algorithm, namely one which achieves a Nash equilibrium among the agents.

% % {
% % This paper develops the \textit{kernelized} setting, where after an initial full training phase--during which each agent fully optimizes its model using an initial segment of training data--the agents are then restricted to dynamically updating only their final learned layer. Each agent’s utility function is quantified by its running mean squared error (MSE) based on how well the ensemble predicts the target time series, penalized by a term that discourages irregular "bang-bang" strategies, which involve rapid switches between states or decisions.
% % }
% % The approach involves training local models on the agents and periodically exchanging model parameters, rather than data, to construct a global model shared across all agents. 


% \paragraph{Main Contribution}
% Though a solution to the general PFL problem is yet elusive, we have completely solved it within the generative pre-trained online setting. Each AI agent and the user/server have access to the same dynamically evolving time series and the corresponding outputs generated by each AI.   Using the information in these evolving input-output pairs, we can construct a feedback mechanism, enabling every agent to optimize their ensemble while preserving the proprietary nature of each AI (Algorithm \ref{alg:sync_subroutine}).  

% Our non-cooperative game-theoretic approach precisely quantifies what ``optimality'' means: the agent's act in a \textit{Nash Equilibrium}.  This Nash equilibrium not only exists, but our PFL algorithm implements the unique \textit{closed-form} solution to this game (Theorem \ref{thm:NashEqmExistence}).  

% \paragraph{Secondary Contributions}
% We further focus on three classes of online deep learning models, where our algorithm’s updates can be streamlined for improved computational efficiency. First, we examine deterministic (non-generative) pre-trained deep learning models -- such as those commonly used for feature encoding -- which have no latent memory (Corollary \ref{cor:PreTrainedTransformer}). Further, we consider a class of generative extreme learning machines, specifically random shallow neural networks with continuously re-generated random biases (Corollary \ref{cor:Random_NeuralNetwork}), motivated by their theoretical interest propelled by the NTK literature. Unlike the first class, these models are generative but lack latent memory. Finally, in Section \ref{s:Examples_ReservoirComputer}, we explore echo-state networks as an example of deep learning models leveraging randomized internal states and latent memory. Each model class is supported by numerical studies demonstrating the effectiveness of our PFL algorithm across a range of online prediction tasks, using both real-world and synthetic datasets. Our PFL algorithm outperforms the benchmark by orders of magnitude in all cases.


% \begin{comment} 
% In this paper, we introduce a game-theoretic approach to FL that incorporates proprietary black-box agents, each of which periodically synchronizes at fixed time intervals. 
% Between synchronization rounds, each agent independently makes predictions based on its local data and transmits them to a central server. 
% During synchronization, agents utilize these optimized weights to make non-cooperative predictions, while also gaining access to the predictions of other agents. This structured interaction among agents is modelled using a Nash game, providing a mechanism to balance the privacy of individual agents and the accuracy of the ensemble model. %and computational efficiency. 
% By utilizing the proprietary models of individual agents, our game-theoretic synchronization scheme alleviates the computational workload on the central server and improves prediction accuracy of the ensemble.
% Our framework ensures efficient cooperation between proprietary agents while maintaining optimal predictive performance over evolving time series data.
% Through numerical experiments, we demonstrate that our method outperforms conventional FL approaches that do not leverage game-theoretic strategies. To the best of our knowledge, this is the first study to apply the game theory to improve the ensemble prediction accuracy by leveraging the computational power of proprietary agents.
% \end{comment}

% \begin{comment} 
% In this paper, we introduce a game-theoretic approach to FL that incorporates multiple generative experts, each of which periodically synchronizes. Our FL framework operates through synchronization rounds occurring at fixed time intervals. Between synchronization rounds, each agent independently makes predictions based on its local data and transmits them to a central server. The server then computes optimal weights for these individual predictions to minimize the overall ensemble prediction error. During synchronization, agents utilize these optimized weights to make non-cooperative predictions, while also gaining access to the predictions of other agents. This structured interaction among agents is modeled using Nash game theory, providing a mechanism to balance accuracy and computational efficiency. 
% By distributing the learning task across clients, our game-theoretic synchronization scheme alleviates the computational workload on the central server.  
% Through numerical experiments, we demonstrate that our method outperforms conventional FL approaches that do not leverage game-theoretic strategies. To the best of our knowledge, this is the first study to apply the game theory to improve the ensemble prediction accuracy by leveraging the computational power of local agents.
% \end{comment} 


% \begin{comment}
% \AK{I moved this here, please intergrate naturally into contributions \textit{with} links to corollaries}

% We will focus on the following three classes of examples.  
% (1) The first is a pre-trained deep learning model that allows for dynamically fine-tuning the final linear decoder layer.  (2) The next example is a particular instance of a \textit{generative} extreme learning machine; a random feature network with continually regenerated random biases. Finally, (3) we consider recurrent models such as \textit{reservoir computers} where one can regenerate a small source of randomness at each time increment, allowing for generative modelling. 
% \end{comment}

% \paragraph{Organization of the Paper}
% % The paper is organized as follows.  
% In Section \ref{s:Setup}, we introduce the generative sequential learning models and the FL scheme. Section \ref{s:Main_Resuls} contains our main theoretical guarantees. In Section \ref{s:Examples}, we examine various FL agents and demonstrate, through numerical experiments, the advantage of our game-theoretic FL approach.   All proofs and additional supporting experimental details are relegated to comprehensive appendices.


% \subsection{Related Work}
% \label{s:Introduction__ss:RelatedWork}

% % \AK{Compress to like 2 paragraphs tops}
% %Though this decentralization reduces the computational burden placed on a single machine, 
% %Federated learning (FL) is a decentralized machine learning paradigm that enables multiple clients to collaboratively train models while preserving data privacy. 
% Traditional FL methods, such as FedAvg \citep{mcmahan2017FedAvg}, 
% aggregate locally-optimized parameters or gradient updates on a central server, which periodically synchronizes local models \citep{Even22SampleOptimalityFL}. 
% %Standard FL schemes rely on idealized assumptions such as homogeneous clients, identically and independently distributed (i.i.d.) datasets, and synchronized updates from clients.  
% %These methods rely on the assumptions that individual agents have i.i.d. datasets, similar system capacities, and uniform data accessibility. 
% These methods rely on idealized assumptions such as homogeneous agents, identically and independently distributed datasets, and synchronized updates from clients.  However, these stylized assumptions tend not to match real-world use cases, wherein agents face heterogeneous data distributions, different system capacities, and de-synchronized updates  \citep{Kairouz21AdvancesFL, Li20FLfuture}.  
% %\citep{kairouz2021advances, li2020federated}. 
% %The heterogeneity and de-synchronization leads to biased global models and lower accuracy of prediction. 
% %It immediately introduces several challenges due to competing heterogeneities between the individual agents' objectives, resulting in a de-synchronization of the system's overall objective. 
% %To address these challenges, asynchronous FL techniques allow clients to update the global model independently based on their availability \citep{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}. 
% %This is typically resolved by periodically synchronizing agents \citep{Even22SampleOptimalityFL}, with the idea being that the agent's optimal policies are in a game-theoretic equilibrium.  
% %Although there are several general FL guarantees, showing that various types of policies are eventually in equilibrium \citep{EqmOptmCollaborationFL}. 
% %This paper focuses precisely allowing the training of machine learning models across multiple local datasets residing on individual agents without sharing raw data \citep{FL:ConceptApplications}. 


% % One major issue in FL is the weights that aggregating agents’ updates (predictions). 
% Due to heterogeneity between agents, averaging of model weights as a means of synchronizing distributed model training \citep{mcmahan2017FedAvg} leads to biased global models and lower prediction accuracy \citep{Zhao22nonIID}. 
% %To address heterogeneity, 
% %change the weights of aggregation.
% Some robust optimization strategies have been designed to address this issue. For example, FedProx \citep{FedOptimHeteroNet} incorporates regularization to stabilize updates across heterogeneous agents, while SCAFFOLD \citep{Karimireddy20Scaffold} employs variance reduction to mitigate local drift. Another challenge in FL is desynchronization of updates from agents due to varying computational speeds and capacity. Asynchronous FL methods address this by allowing each agent to update the global model independently as soon as it completes its local computation \citep{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}. 
% %The lens through which we will examine asynchronous FL pipelines is that of optimization through a game-theoretic perspective, though several other important lenses are natural when studying different, e.g. statistical or XXX, aspects which we will not consider here. 



% %Traditional federated learning (FL) methods, such as FedAvg \citep{mcmahan2017FedAvg}, aggregate locally-optimized parameters or gradient updates on a central server, which periodically synchronizes the local models \citep{SampleOptimalityFL}. These approaches crucially assume that individual agents have i.i.d.\ datasets, similar system capacities, and uniform data accessibility. However, these stylized assumptions tend not to match real-world use cases, wherein agents face heterogeneity via their individual data distributions and system capacities, among other differences. Asynchronous FL methods, e.g. \citep{Fraboni23FO-AsynchronHetero, FedOptimHeteroNet, FL:all-in-one}, address this heterogeneity by allowing each agent to update the global model independently as soon as it completes its local computation.  
% %The lens through which we will examine asynchronous FL pipelines is that of \textit{optimization} through a \textit{game theoretic} perspective, though several other important lenses are natural when studying different, e.g.\ statistical or XXX, aspects which we will not consider here. 
% %Another issue in FL is the weights that aggregating agents' updates (predictions). 
% %Due to heterogeneity between agents, the weights of the clients to update the global model are not uniform as \citep{mcmahan2017FedAvg} which assume that all clients are homogeneous. \citep{Karimireddy20Scaffold} to reduce the affects of sampling heterogeneity of clients. 
% %For FL with non-i.i.d. data, \citep{Zhao22}



% \paragraph{Game-Theoretic Approaches to Machine Learning}
% % \AK{Populate}
% Federated learning can be naturally cast as an interactive multi-agent system wherein optimal control and game theory can be applied.  
% %where participants may act collaboratively or non-cooperatively depending on constraints such as communication costs, computational resources, and privacy considerations. 
% %Game theory provides a framework for analyzing these strategic interactions and optimizing model aggregation, synchronization frequency, and client participation incentives. 
% %Recent works have begun incorporating game-theoretic perspectives into FL, modelling interactions among clients and the central server as multi-agent strategic games. %These approaches enable incentive-aware optimization, but they often focus on static formulations rather than dynamic adaptation.
% In collaborative FL settings, agents share their data and update local models to achieve better performance of the global model \citep{Blum21EqmOptmFL, Donahue21OptimalityStability, Huang23Collaboration, Murhekar23Incentives}. 
% Several challenges arise in collaborative FL, such as privacy leakage \citep{Wei20DiffPrivacy}, communication costs \citep{Yoon25LessCommunication}, and conflicting objectives \citep{Yin24PrivacyAccuracyEnergy}. 
% %agents operate non-cooperatively to update the global model, due to factors such as communication %costs \citep{Yoon25LessCommunication}, privacy constraints, and conflicting objectives \citep{Yin24PrivacyAccuracyEnergy}.  
% %lead agents to update the model non-cooperatively. 
% %In this context, we can leverage a game-theoretic approach to FL.   
% %The game-theoretic approach can be applied to various aspects of FL. Agents collaborate by sharing datasets for collective learning, with the goal of minimizing the total sample size while ensuring that each agent meets the lower bound of individual error. 
% %\citep{Blum21EqmOptmFL} introduces the notions of stable equilibrium and envy-free equilibrium. 
% %In hedonic games agents choose to join different federating groups to achieve better performance \citep{CollaborationEqmFL},
% %\citep{OptimalityStabilityFL:Game}, \citep{HedonicGamesShareData25}. 
% %\citep{Murhekar:23} finds an optimal trade-off between FL learning payoff and data sharing cost. 
% %\citep{Xie24mixed} game between the central server and adversarial clients, in which the adversary aims to attack the training % while the server aims to achieve low overall training error. 
% %Several works have formalized equilibrium concepts in FL. 
% %\citep{Blum21EqmOptmFL} introduce the notions of stable equilibrium and envy-free equilibrium to ensure fairness in FL model aggregation. 
% %In hedonic games, agents self-organize into federated coalitions to optimize their predictive performance \citep{CollaborationEqmFL, Donahue21OptimalityStability, HedonicGamesShareData25}. 
% %Other works investigate the trade-offs between FL learning performance and data-sharing costs \citep{Murhekar23Incentives},  ensuring that clients benefit from collaboration without incurring excessive privacy risks.
% %Moreover, game-theoretic modeling can be applied to robust FL against adversarial threats \citep{Xie24mixed, Zhang23RobustGameFL}. \citep{Blanco-Justicia21SecurityPrivacy}
% Non-cooperative game-theoretic models have been used to address challenges such as adversarial threats \citep{Zhang23RobustGameFL,Xie24mixed} and privacy protection \citep{Blanco-Justicia21SecurityPrivacy, Yin21PrivacyPreserving}. Utilizing non-cooperative game theory to formulate and improve multi-agent model performance, especially with proprietary AI agents, remains an emerging area of research.
% %In robust FL against adversarial threats, \citep{Xie24mixed} model FL as a mixed-strategy game between a central server and adversarial clients, where the server aims to optimize model accuracy, while the adversary strategically perturbs updates to degrade performance. 
% %Game-theoretic approaches are used  %\citep{Yin24FLprivacy,}. 


% %Since FL participants operate under constraints such as communication costs, computational limitations, and privacy concerns, their interactions can be either collaborative or non-cooperative. Cooperative game is used to incentivize data-sharing \citep{Huang23Collaboration}. Non-cooperative game is used in the scenarios with privacy concerns \citep{Murhekar23Incentives}.  


% % \subsection{Sequential Deep Learning - Causality/Adaptedness Constraints}
% % \AK{I add}
% % %In FL schemes, clients focus on individual objectives 


% \subsection{Notation and Conventions} 
% \label{s:notation}
% In this section, the notation used throughout the manuscript is gathered for clarity and accessibility. We denote $\mathbb{N} \eqdef \{0, 1, 2, \cdots \}$ and $\mathbb{N}_+\eqdef \{x\in \mathbb{N}:\, x>0\}$.  
% %For any $N\in \mathbb{N}_+$, the \textit{simplex} $\Delta_N$ is the set of $w\in \mathbb{R}^N$ satisfying the following positivity and normalization constraints
% %\begin{align}
% %\label{eq:NSimplexDef}
% %    \underbrace{
% %       w^1_\cdot + \dots + w^N_\cdot 
% %        = 1
% %    }_{\term{c1:netting}}
% %\mbox{ and }
% %    \underbrace{
% %        w^1_\cdot , w^2_\cdot ,\dots,w^N_\cdot   \ge 0 
% %    }_{\term{c2:leveraging}}.
% %\end{align}
% We henceforth fix a latent, complete probability space $(\Omega,\mathcal{F},\mathbb{P})$.  For any $d,D\in \mathbb{N}_+$ and $1\le p<\infty$, use $L^p(\mathbb{R}^d)$ (resp.\ $L^p(\mathbb{R}^{d\times D})$) to denote the space of $\mathbb{R}^d$ (resp.\ $\mathbb{R}^{d\times D})$) valued random variables $X$ whose expected $p^{\text{th}}$ power of their Euclidean $\|\cdot\|_2$ (resp.\ Frobenius $\|\cdot\|_F$) norm is finite $\mathbb{E}[\|X\|^p_2]<\infty$ (resp.\ $\mathbb{E}[\|X\|_F^p]<\infty$), where the expectation is taken with respect to $\mathbb{P}$. As shorthand for an arbitrary Cartesian product of a single space $X$, $X \times \ldots \times X$, we write $(X)^{\mathbb{N}}$.

% \paragraph{Row and Column Vectors and Matrices}
% We will nearly always specify if a vector is a row or column vector and its dimensions.  However, when clear from the context, we identify the space of row vectors $\mathbb{R}^{d\times 1}\cong \mathbb{R}^d$ and the space of column vectors $\mathbb{R}^{1\times d}\cong \mathbb{R}^d$ (for the relevant $d\in \mathbb{N}_+$) to keep notation light.  
% For each $d\in \mathbb{N}_+$, $I_d$ is the $d \times d$-identity matrix.  Moreover, $\bar{1}_d\in \mathbb{R}^d$ has all its entries equal to $1$. 
% We denote by $0$ the zero scalar, zero vector, or zero matrix with dimensions specified in the context. 
% The Kronecker product of any two matrices $A$ and $B$ is denoted by $A\otimes B$. 
% The Euclidean ($\ell^2$) norm of any vector $x\in \mathbb{R}^d$, for any given dimension $d\in \mathbb{N}_+$, is denoted by $\| \cdot \|$. 
% % The absolute value of any real number $x\in \mathbb{R}$ is denoted by $x|$.  

% \section{The Online Proprietary Federated Setting}
% \label{s:Setup}

% \paragraph{The Agents - Online Sequential Learners}
% % \label{s:Setup__ss:EnsembleModel}
% We consider $N\in \mathbb{N}_+$ generative \textit{proprietary} sequential learners $f^{1},\dots,f^{N}$ with at most three inputs at any time $t\in \mathbb{N}$.  For each such $t\in \mathbb{N}_+$, the $i^{\text{th}}$ expert model takes the (common) historical input sequence $x_{[0:t]}\in \mathbb{R}^{d_x \, (1+t)}$, an individual source of randomness $\epsilon_t^i$ which is an integrable $d_y \times d_z$-valued random variable, and an individual hidden state $Z_t^i\in \mathbb{R}^{d_y\times d_z}${; where $d_x, d_y, d_z \in \mathbb{N}_+$}.  
% These three inputs are used to generate the latent state $Z^i_{t+1}$ using a \textit{static} \textbf{encoder} $\varphi^{i}:\mathbb{R}^{d_x(1+t)} \times \mathbb{R}^{d_y \times d_z}\times 
%  \mathbb{R}^{d_y\times d_z }\to \mathbb{R}^{d_y 
% \times d_z}$ via
% \begin{equation}
% % \tag{ENC}
% \label{eq:ENCODER}
%     Z_{t}^i 
% \eqdef 
%     \underbrace{
%         \varphi^{i}\big(x_{[0:t]}
%         ,Z_{t-1}^i,\epsilon_t^i\big)
%     }_{\text{(Deep) Feature Encoder}}
% .
% \end{equation}
% The (deep) feature encoder is either pre-trained or trained on an initial segment of time-series data, formally regarded as before the time when prediction begins to roll out online; i.e.\ $t=0$ and any negative times are considered part of an offline pre-training phase not considered here.  Thus, on and after time $t>0$, the feature encoder is no longer updated in this paper, and the (deep) learning model effectively becomes a kernel function.  We require that $Z_t^{i}\in L^1(\mathbb{R}^{d_y\times d_z})$ for each $t\in \mathbb{N}$.
% Once the latent state is generated, it is used to update the \textit{residual} of the prediction generated at the previous time $t$ via a \textit{dynamically updating} linear \textbf{decoder} parameterized by $\beta^i$.
% %\begin{equation}
% %\label{eq:DECODER_RESIDUALS}
% % \hat{Y}^i_{t+1} = 
% % \hat{Y}^i_t + \beta^{i\top}_t Z^i_t 
% %\end{equation} 
% \begin{equation} 
% % \tag{DEC}
% \label{eq:DECODER_RESIDUALS}
% % \smash{
%     \underbrace{
%         \hat{Y}^i_{t+1}
%     }_{\text{Prediction}}
% = 
%         \underbrace{
%             \hat{Y}^i_t 
%         }_{\text{Historical State (Memory)}}
%     +  
%     \underbrace{
%         \overbrace{Z^i_t 
%         }^{\text{feature}}
%         % \overbrace{ 
%             \beta^{i}_t
%             %\colorwblk{\beta^{i}_t}
%         ,
%         % }^{\text{linear}}
%     }_{\text{Residual (Update)}}
% % }
% \end{equation} 
% where $\hat{Y}_t^i \in \mathbb{R}^{d_y \times 1}$, $Z_t^i\in \mathbb{R}^{d_y \times d_z}$, and $\beta_t^i \in \mathbb{R}^{d_z \times 1}$. Both initial states $\hat{Y}_0^i\in \mathbb{R}^{d_y\times 1}$ and $Z_0^i\in \mathbb{R}^{d_y \times d_z}$ are fixed a priori.  

% Following the theoretical reservoir computing literature, e.g. \citep{grigoryeva2018echo}, each generative sequential is a \textit{causal} deep learning agent defined by
% \begin{equation*}
% \begin{aligned}
%     f^{i}: (\mathbb{R}^{d_{x}})^{\mathbb{N}}&\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{N}}, \\
%     (x_t)_{t=0}^{\infty} & \to \big(\hat{Y}^i_t\big)_{t=0}^{\infty}.
% \end{aligned}
% \end{equation*}
% where, for each $t\in \mathbb{N}$, $\hat{Y}^{i}_{t+1}$ is computed recursively  by first encoding the input path $x_{[0:t]}$ via Equation \eqref{eq:ENCODER}, and then updating the residual via Equation \eqref{eq:DECODER_RESIDUALS}.  By \textit{causality}, we mean that for each time $t\ge 0$, the prediction $\hat{Y}_{t+1}^i$ only depends on the input sequence as \textit{observed thus far}, i.e.\ on $x_{[0:t]}$, and not on any of its future realizations, i.e.\ not on $x_s$ for any $s>t$.
  

% For example, in echo-state networks (ESNs) \citep{jaeger2001echo,maass2002real} or extreme learning machines such as random feature networks (RFNs) \citep{huang2006universal,rahimi2008weighted}, the deep features in Equation \eqref{eq:ENCODER} are randomly initialized and left untrained and residual updates, parameterized by $(\beta_t)_{t=0}^{\infty}$, in Equation \eqref{eq:DECODER_RESIDUALS} are trained before the online-time $t=0$ and then frozen (thus are constant) for all times $t \ge 0$.  In pre-trained models, such as transformers \citep{vaswani2017attention}, the deep features are pre-trained on an offline dataset, i.e.\ before time $t=0$, and the residual decoding/readout layer in Equation \eqref{eq:DECODER_RESIDUALS} is also typically left fixed.


% \paragraph{The Server - Adaptive Mixture of Experts/Agents}
% % \label{s:Setup__ss:Federated}
% We assume that $N>1$, with the case of $N=1$ being trivial, as no multi-agent coordination is required. The objective of the server is to adaptively \textit{synchronize} these $N$ generative models, into a single generative ensemble model $F:(\mathbb{R}^{d_{x}})^{\mathbb{N}}\to L^1(\mathbb{R}^{d_{y}})^{\mathbb{N}}$ to maximize their performance.  The resulting ensemble is represented for each $x \in (\mathbb{R}^{d_x})^{\mathbb{N}}$ at every time $t\in \mathbb{N}$ by
% \begin{equation} 
% \label{eq:enbsemble_server__predictions}
% F(x_{[0:t]})_t \eqdef 
% \overbrace{
% \sum_{i=1}^N\, 
%     %\colorwblk{w_t^i}\, 
%     w_t^i 
%     % \,
%     \underbrace{
%         f^{i} \big(x_{[0:t]}\big)_t
%     \,
%     ,
%     }_{i^{\text{th}} \text{Agent (Expert)}}
% }^{\text{Mixture of Experts}}
% \end{equation}
% where the \textit{mixture coefficients} $w_t$ belongs to $\mathbb{R}^N$. %the $N$-simplex $\Delta_N$.  
% Observe that, by construction, the server's mixture prediction is also \textit{causal}; that is, $F(x_{[0:t]})_t$ only depends on $x_{[0:t]}$ and not $x_s$ for any $s>t$.

% \paragraph{The Proprietary Constraint}
% {
% Each \textit{agent} can dynamically update, or \textit{control}, its sequence of linear residual update parameters $(\beta_t)_{t=0}^{\infty}$ in Equation \eqref{eq:DECODER_RESIDUALS}, while the central \textit{server} dynamically updates its own parameters in Equation \eqref{eq:enbsemble_server__predictions}. In standard federated or online optimization problems, there are no restrictions on how agents and the server update their trainable parameters, apart from the requirement that updates be causal. That is, they must not depend on inaccessible future information.  

% However, the \textit{proprietary} nature of each model introduces an additional layer of structural complexity. Specifically, neither the server nor any agent has access to the internal structure of any other model, including its architecture, parameter values, or (partial) gradient information. Together, the \textit{causality} and \textit{proprietary} constraints imply that, 
% at every time $t\in \mathbb{N}_+$, the $i^{\text{th}}$ \textit{agent/client-side} parameter updates to $\beta_t^{i}$ in Equation \eqref{eq:DECODER_RESIDUALS} are of the form
% \begin{equation}
% \label{eq:PROPRIETARY_CONSTRAINT__Agent}
%     \beta_t^{i} = b_t\Bigg(
%             % \overbrace{
%                 \left(\hat{Y}_{[0:t]}^{j}\right)_{j=1}^N
%             % }^{\text{Expert Predictions}}
%         , 
%             \left(Z_{[0:t]}^{j}\right)_{j=1}^N
%         ,
%                 y_{[0:t]}
%         ,
%             % \underbrace{
%                 x_{[0:t]}
%             % }_{\text{Input series}}
%         ,
%             % \overbrace{
%             w_{[0:t]}
%             % }^{\text{Server Weights}}
%             % \underbrace{
%             %    \beta_{[0:t]}^{i}
%             % }_{\text{Own } i^{\text{th}} \text{ Parameters}}
%     \Bigg),
% \end{equation}
% for each $t\in \mathbb{N}_+$, where $b_t:\mathbb{R}^{d_y(1+t)\times N }\times \mathbb{R}^{(d_y \times d_z)(1+t)\times N }\times \mathbb{R}^{d_y(1+t)}\times \mathbb{R}^{d_x(1+t)}\times \mathbb{R}^{N(1+t)} \to \mathbb{R}^{d_z \times 1}$ is a continuous function that may depend on the current time $t$ and various observed quantities, including all historical expert predictions $\hat{Y}^{1}_{[0:t]}, \dots, \hat{Y}_{[0:t]}^{N}$, their historical deep features $Z_{[0:t]}^{1},\dots,Z_{[0:t]}^{N}$ the server weights $w_{[0:t]}$, and the input data $x_{[0:t]}$.  We highlight that the $i^{\text{th}}$ agent’s parameter updates $\beta_{[0:t]}^{i}$ are known to themselves and can therefore be incorporated into their own decisions.%
% \footnote{Expression \eqref{eq:PROPRIETARY_CONSTRAINT__Agent} could be extended to include the agent's internal parameters if the hidden layers were trainable, but they are not here.}

% Similarly, as the server does not have black-box access to any other proprietary model, then, 
% at each time $t\in \mathbb{N}_+$, the server-side mixture coefficients $w_t$ in Equation \eqref{eq:enbsemble_server__predictions}, are of the form
% \begin{equation}
% \label{eq:PROPRIETARY_CONSTRAINT__Server}
%     w_t = \varpi_t\Bigg(
%             % \overbrace{
%                 \left(\hat{Y}_{[0:t+1]}^{j}\right)_{j=1}^N
%             % }^{\text{Expert Predictions}}
%         ,
%             \left(Z_{[0:t]}^{j}\right)_{j=1}^N
%         ,
%                 y_{[0:t]}
%         ,
%             % \underbrace{
%                 x_{[0:t]}
%             % }_{\text{Input series}}
%         ,
%             % \overbrace{
%             w_{[0:t]}
%             % }^{\text{Server Weights}}
%     \Big),
% \end{equation}
% where $\varpi_t:\mathbb{R}^{d_y(2+t)\times N}\times \mathbb{R}^{ ( d_y \times d_z)(1+t)\times N}\times \mathbb{R}^{d_y(1+t)}\times \mathbb{R}^{d_x(1+t)}\times \mathbb{R}^{N(1+t)} \to \mathbb{R}^N$ is a continuous function that may depend on the current time $t \in \mathbb{N}_+$.  
% Note that, since the agents each predict first, then the server's update can leverage the information in $\hat{Y}_{t+1}^{1},\dots,\hat{Y}_{t+1}^{N}$. 

% We emphasize that each client-side parameter $\beta_t^{i}$ is computed using strictly more information than the server-side weights $w_t$. This distinction arises because each agent has access to its own internal parameters, whereas the server does not, as these parameters are proprietary and remain inaccessible to the server. 
% \begin{remark}[The Proprietary Constraint is a Measurability Restriction]
% \label{rem:adapedness}
% If $b_t$ and $\varpi$ were only required to be Borel measurable, then Conditions \eqref{eq:PROPRIETARY_CONSTRAINT__Agent} and \eqref{eq:PROPRIETARY_CONSTRAINT__Server} could be formulated as \textit{adaptedness} conditions. Specifically, $\beta_t^{i}$ would be measurable with respect to the $\sigma$-algebra generated by $\{\hat{Y}_{s}^{j},\,w_{u}, \beta_{s}^{i},Z_s^{i}\}_{s,u,j=1}^{t,t+1,N}$, while $w_t$ would be required to be measurable with respect to the $\sigma$-algebra generated by $\{\hat{Y}_{s}^{j},\,w_{u},Z_s^{i}\}_{s,j=1}^{t,N}$.   However, imposing additional continuity constraints on $b_t$ and $w_t$ enhances the structural regularity of the problem.  
% \end{remark}



% %\begin{equation}
% %\label{eq:ridge_local}
% %    \beta_t^i\in \operatorname{argmin}\, 
% %        \sum_{s=t-T\vee 0}^t\,
% %        e^{-\alpha^i(t-s)}
% %        \,\|
% %            (y_s-\hat{Y}_s^i)
% %        -\beta_t^i\,Z_s^i\|^2
% %        +
% %        \gamma^i\|\beta_t^i\|^2.
% % \end{equation}

% \section{Main Results}
% \label{s:Main_Resuls}
% {Our first result formalizes and derives the optimal server-side update (Theorem \ref{thm:OptimalWeights}).  We derive the optimal client-side update in (Theorem \ref{thm:NashEqmExistence}).  We additionally provide a greedy scheme which each client can use between these synchronization times (Proposition \ref{prop:localgreedyupdates}) for an added speedup at the cost of sub-optimal decisions.}

% \subsection{Optimal Server-Side Weights}
% \label{s:Main_Results__Server}

% Let $t\in \mathbb{N}_+$ and fix a regularization parameter $\kappa>0$.  
% Given any $\left(\hat{Y}_{t}^{j}\right)_{j=1}^N\in L^1(\mathbb{R}^{d_y})^{N}$ and $y_t\in \mathbb{R}^{d_y}$, 
% %$y_{[0:t]}\in\mathbb{R}^{d_y(1+t)}$, 
% %$x_{[0:t]}\in \mathbb{R}^{d_x(1+t)}$, and %$w_{[0:t]}\in \mathbb{R}^{N(1+t)}$, 
% we define the server-side objective as
% \begin{equation}
% \label{eq:server}
% \begin{aligned}
%     \min_{w_t\in \mathbb{R}^N}\,
%     &
%     % \mathbb{E}  \, 
%     % \biggl[  
%         \Big\| y_{t}  - \sum_{j=1}^N w^j_t \hat{Y}^{j}_{t} \Big\|^2 
%     + 
%         \sum_{j=1}^N \kappa | w^j_t |^2,
%     % \biggr]
% \\
% \mbox{s.t.} & \,
% w^1_t+\dots+w^N_t = \eta
% .
% \end{aligned}
% \end{equation}
% The normalization constraint $w^1_t+\dots+w^N_t = \eta$ ensures that the \textit{total weight size} is equal to $\eta$. When $\eta=1$, this condition serves as a \textit{signed} variant of the usual probabilistic normalization constraint found in the PAC-Bayes literature \citep{alquier2024user} optimized by a Gibbs-type measure, where instead there $w_t$ is constrained to the $N$-simplex, meaning each weight must satisfy $0 \leq w^i_t \leq 1$ for each $i$.   However, this additional constraint is removed since we are not \textit{sampling} agent predictions but rather \textit{combining} them. Doing so allows the central server to make “negative bets against” an agent’s predictions. Even if an agent consistently performs poorly, its signed opposite prediction may still be useful. This added freedom enables the server to better exploit available information across all agents.

% In essence, the hyperparameter $\kappa$ controls the amount we allow the server to borrow its investment level in any given expert to leverage it towards the predictive influence of any other expert, and $\eta$ controls the total investment level of the server into each agent.
% \begin{theorem}[Server: Optimal Mixture Weights]
% \label{thm:OptimalWeights}
% Let $\kappa,\eta>0$, $t\in \mathbb{N}_+$, $\left(\hat{Y}_{t}^{j}\right)_{j=1}^N\in L^1(\mathbb{R}^{d_y})^{N}$, $y_{[0:t]}\in \mathbb{R}^{d_y(1+t)}$, $x_{[0:t]}\in \mathbb{R}^{d_x(1+t)}$, and $w_{[0:t]}\in \mathbb{R}^{N(1+t)}$.  
% Then
% \[
%         w_t^{\star}  
%     = 
%          A^{-1}\,
%          \biggl(
%              b -  
%              % \biggl(
%                 \frac{
%                     \mathbf{1}_N^{\top}A^{-1}\,b-
%                     \eta%1
%                 }{
%                     \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N
%                 }
%             \cdot
%              % \biggr)
%              \,\mathbf{1}_N
%          \biggr)
% \]
% is the \textit{unique} solution $w^{\star}_t=[ w^1_t, \dots, w^N_t]^\top$ 
% to System \eqref{eq:server}, where $A\eqdef 2 ( \hat{\mathbf{Y}}^\top_{t} \hat{\mathbf{Y}}_{t} + \kappa I_N )$, $b\eqdef 2 (y^\top_{t}  \hat{\mathbf{Y}}_{t})^{\top}$, $\hat{\mathbf{Y}}_{t} = [ \hat{Y}^1_{t}, \dots, \hat{Y}^N_{t} ]$.
% \end{theorem}

% Having settled the optimal server-side behaviour in Theorem~\ref{thm:OptimalWeights}, we now turn our attention to the optimal agent/client-side behaviour given the weights produced by the server.
% \subsection{Optimal Client-Side Behaviour} \label{nash_sync}

% Since each agent is unaware of the internal parameters and models of other agents, the best they can do is optimize their contribution to the ensemble mixture, $\sum_{j=1}^N w_t^j \hat{Y}_{t+1}^{j}$, given the mixture weight assigned by the central server and the observable predictions of other agents over a look-back window of length $T \in \mathbb{N}_+$. An exponentially weighted average, where recent predictive accuracy is deemed more important than historical predictions up to pre-specified weights $\alpha_i$ for $i=1,\dots,N$, is used. 
% %$s\in [(t-T)\vee 0:t-1]$. 
% For notational simplicity, we denote $t=0$ to be the start of the look-back window; that is, it serves as a stand-in for $s=t-T \vee 0$.  
% The objective function is written
% % \allowdisplaybreaks 
% \begin{align} 
% \label{eq:Objective_nth_expert}
%  J_i(\beta^i, \beta^{-i}) = 
%  \mathbb{E} \Bigg\{ \sum_{t=0}^{T-1} 
%     e^{ -\alpha_i (T - 1 - t)} 
%  \,
%   \Big[    
%  \Big\| y_{t+1} - \sum_{j=1}^N w^j_t \hat{Y}^j_{t+1} \Big\|^2 
%   + \gamma_i \| \beta^i_t \|^2    
%   \Big] 
%   \Bigg\},
% \end{align} 
% for $i = 1, \dots, N$, $\beta^{-i}=
% (\beta^j)_{j=1; j\neq i}^N$ and $\alpha_i\ge 0$.
% % is a pre-specified hyperparameter controlling the impact of distant past observations on the current game the local machines are playing with one another. 


% Thus, each agent/client is naturally in \textit{competition} with all other agents to maximize their influence on the mixture $\sum_{j=1}^N\, w_t^j\hat{Y}_{t+1}^{j}$.  Thus, the \textit{optimal} behaviour of each agent is that of a \textit{Nash equilibrium}; that is, the action of each agent at any time cannot reduce the value of their running cost function $J_i$ in Equation \eqref{eq:Objective_nth_expert}. The following is our main theoretical contribution, which identifies and computes the \textit{unique} Nash equilibrium behaviour for all agents in \textit{closed-form}.

% \begin{theorem}[Agents: Optimal Re-synchronization via The Nash Equilibrium]
% \label{thm:NashEqmExistence}
% Let $T, t \in \mathbb{N}_+$ with $t\ge T$, $\left(\hat{Y}_{[0:t]}^{j}\right)_{j=1}^N\in L^1(\mathbb{R}^{d_y})^{N(1+t)}$, $y_{[0:t]}\in \mathbb{R}^{d_y(1+t)}$, $x_{[0:t]}\in \mathbb{R}^{d_x(1+t)}$, and $w_{[0:t]}\in \mathbb{R}^{N(1+t)}$ with $\sum_{i=1}^N w^{i}_t =\eta$ for each $t\in [0:t]$. 
% %%%
% Suppose the system in Equation \eqref{eqn:Pi} for $( P_i )_{i=1}^N$ admits a solution for $t=0$, $1$, $\dots$, $T$.  
% Then the $N$-agent Nash game with cost functions defined in Equation \eqref{eq:Objective_nth_expert} admits a unique feedback Nash equilibrium for $t=0$, $1$, $\dots$, $T-1$
% \begin{align} 
% \label{eqmvecbeta}
%  \boldsymbol{\beta}_{t} =  [\beta^{1\top}_t, \dots, \beta^{N \top}_t ]^\top  
% =  \mathbf{G}(t)  [ \hat{Y}^{1\top}_t, \dots, \hat{Y}^{N\top}_t ]^\top + \mathbf{H}(t) , 
% %= &  \big[  e^{ - \boldsymbol\alpha (T-1-t)}  ( \Gamma + \widehat{\mathbf{A}}(t) ) + \mathbf{A}(t)  \big]^{-1}   
% % \big[  e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top \hat{Y}_t ) 
% %- \mathbf{B}(t) \hat{Y}_t - \mathbf{C}(t) \big]  ,    
% \end{align} 
% where the matrix-valued coefficients $\mathbf{G}(t)$ and $\mathbf{H}(t)$ are determined by the following system of matrix-valued equations for $(P_i, S_i)_{i=1}^N$ on the time span 
% $t=0$, $1$ $\dots$, $T$, 
% %\begin{equation} 
% %\begin{split} 
% %\left \{ 
% %\begin{aligned}
% %  P_i(t) &= 
% % \Big(\big[ \mathbf{D}(t)(  e^{-\boldsymbol{\alpha}(T-t)}  \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) - I \big]^\top
% %  \\
% %  &\qquad \qquad \qquad \cdot P_i(t+1)\big[  \mathbf{D}(t)( e^{-\boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} 
% % \mathbf{B}(t) - I \big] \Big)  \\ 
% %  & \qquad + \Big(e^{ - \alpha_i (T-t) } \gamma_i \big[  ( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} %\mathbf{B}(t) \big]^\top \\ 
% % & \qquad \qquad \qquad \cdot \big[  ( e^{ - \boldsymbol{\alpha}(T-t)} \Gamma +\mathbf{A}(t))^{-1} \mathbf{B}(t) \big] \Big) \\ 
% % &\qquad + e^{ - \alpha_i (T-t)} \mathbf{w}_t \mathbf{w}_t^\top  \\ 
% %  P_i(T) &=  \mathbf{w}_T \mathbf{w}_T^\top  ,
% %\end{aligned}
% %\right.
% %\end{split}
% %\label{eqn:Pi}
% %\end{equation} 
% \begin{equation} 
% \begin{split} 
% \left \{ 
% \begin{aligned}
%   P_i(t)  = &   
%   \mathbf{G}(t)^\top 
%   \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \widehat{\mathbf{e}}_i \widehat{\mathbf{e}}_i^\top  \big] 
%    \mathbf{G}(t)  
%    \\ 
%    & + \big[ e^{-\alpha_i(T-1-t)}\mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big] 
%    \mathbf{D}(t) \mathbf{G}(t) \\ 
%    & + \mathbf{G}(t)^\top \mathbf{D}(t)^\top \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big]^\top  \\ 
%    & + e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  , \\ 
%   & \hspace{-0.6cm} e^{ - \boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{ - \boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t) 
%    \, \text{is invertible} , 
%   \\ 
%   P_i(T)   = &    0  ,
% \end{aligned}
% \right.
% \end{split}
% \label{eqn:Pi}
% \end{equation} 
% %where $e^{ - \boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{ - \boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)$ 
% % is assumed to be invertible. 
% \begin{equation}  
% \begin{split} 
% \left \{ 
% \begin{aligned}
%   S_i(t)  = &  \mathbf{G}^\top(t) \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) 
%    + e^{-\alpha_i(T-1-t)} \gamma_i \widehat{\mathbf{e}}_i \widehat{\mathbf{e}}_i^\top  \big] \mathbf{H}(t) \\ 
% & + \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  \big] \mathbf{D}(t) \mathbf{H}(t) \\  
% & + \mathbf{G}^\top(t) \mathbf{D}^\top(t) \big[ - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) \big] \\ 
% & - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) , \\ 
%  S_i(T) = & 0   . 
% \end{aligned}
% \right.
% \end{split} 
% \label{eqn:Si}
% \end{equation} 
% The matrices in Equations \eqref{eqn:Pi} and \eqref{eqn:Si} are defined in Table \ref{tab:matricesEqnPiSi}.  
% \begin{comment} 
% \allowdisplaybreaks 
% \begin{align} 
%  & \mathbf{A}(t) = 
% \mathbb{E} \big\{ \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \cdots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top 
% \big[ \mathbf{e}_1 Z^1_t, \cdots,  \mathbf{e}_N Z^N_t  \big]  \big\}  , 
% \notag \\ 
% & \widehat{\mathbf{A}}(t) = 
% \mathbb{E} \big\{ \big[ \mathbf{e}_1 Z^1_t, \cdots, \mathbf{e}_N Z^N_t \big]^\top 
% \mathbf{w}_t \mathbf{w}_t^\top 
% \big[ \mathbf{e}_1 Z^1_t, \cdots,  \mathbf{e}_N Z^N_t  \big]  \big\} , 
% \notag \\ 
% & \mathbf{B}(t) = \mathbb{E} \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \cdots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top ,
%  \notag \\ 
% & \mathbf{C}(t) = \mathbb{E} \big[ S_1^\top(t+1) \mathbf{e}_1 Z^1_t, \cdots, S_N^\top(t+1) \mathbf{e}_N Z^N_t \big]^\top ,  \notag \\ 
% & \mathbf{D}(t) 
%  = \mathbb{E}  
%  \big[ \mathbf{e}_1 Z^1_t , \, \mathbf{e}_2 Z^2_t ,  \, \cdots , \, \mathbf{e}_N Z^N_t  \big] , \notag \\ 
%  & 
%  \mathbf{D}_i(t) 
%  = \mathbb{E} \Big\{   
%  \big[ 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \big]^\top 
%   P_i(t+1) 
%   \big[ \mathbf{e}_1 Z^1_t, \, \mathbf{e}_2 Z^2_t , \,\cdots , \, \mathbf{e}_N Z^N_t \big]  
%  \Big\} , \quad i = 1, ..., N, 
%  \notag \\ 
%  &  \mathbf{G}(t) = - \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma 
%   + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} 
%  \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t \mathbf{w}_t^\top + \mathbf{B}(t) \big] , 
%  \notag \\ 
%  & \mathbf{H}(t) = \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} 
%   \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t y_{t+1} - \mathbf{C}(t) \big] , 
%  \notag 
% \end{align} 
% where $\{e_1, \cdots, e_N\}$ is the standard ordered basis of $\mathbb{R}^N$ and 
% \begin{align} 
%  & \mathbf{w}_t=(w^1_t I_{d_{y}}, ..., w^N_t I_{d_{y}})^\top , \quad \hat{Y}_t=(\hat{Y}^{1\top}_t, ..., \hat{Y}^{N\top}_t)^\top, \quad   
%   \Gamma = \diag[ \gamma_1 I_{d_z} , ..., \gamma_N I_{d_z} ] ,
%   \notag \\ 
%  & 
%   \boldsymbol{\alpha} = \diag [\alpha_1 I_{d_z} , ..., \alpha_N I_{d_z} ] , 
%   \notag \\ 
% &  \mathbf{e}_i = e_i \otimes I_{d_y} = [0, ..., I_{d_y} , ..., 0]^\top , \quad 
%  \hat{\mathbf{e}}_i = e_i \otimes I_{d_z} = [0, ..., I_{d_z} , ..., 0]^\top , 
%   \quad i=1, \ldots, N . 
%  \notag 
% \end{align} 
% \end{comment} 
% \end{theorem} 
% \begin{table}[H] 
% \caption{The matrices defining the closed-form updates in Theorem \ref{thm:NashEqmExistence}.}
% % , in Equations \eqref{eqn:Pi} and \eqref{eqn:Si}.}
% \label{tab:matricesEqnPiSi}
% \begin{tabular}{ll}
% % \hline
% \toprule
% \textbf{Matrix} & \textbf{Closed-Form Expression}
% \\
% \midrule
% % \multicolumn{2}{l}{
% $\mathbf{A}(t)$ & $\mathbb{E} \big\{ \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \dots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top \big[ \mathbf{e}_1 Z^1_t, \dots,  \mathbf{e}_N Z^N_t  \big]  \big\}$ 
% % }                                                            
% \\
% % \multicolumn{2}{l}{
% $\widehat{\mathbf{A}}(t)$ & $\mathbb{E} \big\{ \big[ \mathbf{e}_1 Z^1_t, \dots, \mathbf{e}_N Z^N_t \big]^\top \mathbf{w}_t \mathbf{w}_t^\top \big[ \mathbf{e}_1 Z^1_t, \dots,  \mathbf{e}_N Z^N_t  \big]  \big\}$                               \\
% $\mathbf{B}(t)$ & $ \mathbb{E} \big[ P_1(t+1) \mathbf{e}_1 Z^1_t, \dots, P_N(t+1) \mathbf{e}_N Z^N_t \big]^\top$                    
% % &
% \\
% $\mathbf{C}(t) $ & $\mathbb{E} \big[ S_1^\top(t+1) \mathbf{e}_1 Z^1_t, \dots, S_N^\top(t+1) \mathbf{e}_N Z^N_t \big]^\top$                                                                                                                                              
% % &  
% \\
% $\mathbf{D}(t)$ & $ \mathbb{E} \big[ \mathbf{e}_1 Z^1_t , \, \mathbf{e}_2 Z^2_t ,  \, \dots , \, \mathbf{e}_N Z^N_t  \big]$                                                                                                                                          
% % & 
% \\
% $\mathbf{D}_i(t) $ & $\mathbb{E} \big\{  \big[ \mathbf{e}_1 Z^1_t  ,  \,\dots , \, \mathbf{e}_N Z^N_t    \big]^\top P_i(t+1) \big[ \mathbf{e}_1 Z^1_t, \,\dots , \, \mathbf{e}_N Z^N_t \big]  \big\} , \quad i = 1, \dots, N,$                                            
% % &  
% \\
% $\mathbf{G}(t)$ & $ - \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma   + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t \mathbf{w}_t^\top + \mathbf{B}(t) \big]$ 
% % &
% \\
% $\mathbf{H}(t) $ & $ \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \Gamma + \mathbf{A}(t) + e^{-\boldsymbol{\alpha}(T-1-t)} \widehat{\mathbf{A}}(t)  \big]^{-1} \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t y_{t+1} - \mathbf{C}(t) \big]$               
% % & 
% \\ 
% % \cline{1-1}
% % $\{e_1, \cdots, e_N\}$: the standard ordered basis of $\mathbb{R}^N$                                                                                                                                                                                                   &  \\
% % $\mathbf{e}_i = e_i \otimes I_{d_y} = [0, \cdots, I_{d_y} , ..., 0]^\top , \quad \hat{\mathbf{e}}_i = e_i \otimes I_{d_z} = [0, \cdots, I_{d_z} , \cdots, 0]^\top , \quad i=1, \ldots, N$                                                                                       &  \\
% % $\mathbf{w}_t=(w^1_t I_{d_{y}}, \cdots, w^N_t I_{d_{y}})^\top$ $\quad$ $\Gamma = \diag[ \gamma_1 I_{d_z} , \cdots, \gamma_N I_{d_z}]$ $\quad$  $\boldsymbol{\alpha} = \diag [\alpha_1 I_{d_z} , \cdots, \alpha_N I_{d_z} ]$                                                   &  \\ \cline{1-1}
% \bottomrule
% \end{tabular}
% % \caption*{}

% Here $e_i$ is the $i^{\text{th}}$ standard basis vector in $\mathbb{R}^N$,  $\mathbf{e}_i = e_i \otimes I_{d_y} = [0, \dots, I_{d_y} , \dots, 0]^\top , \quad \widehat{\mathbf{e}}_i = e_i \otimes I_{d_z} = [0, \dots, I_{d_z} , \dots, 0]^\top$, and 
% $\mathbf{w}_t=[ w^1_t I_{d_{y}}, \dots, w^N_t I_{d_{y}} ]^\top$,  $\Gamma = \diag[ \gamma_1 I_{d_z} , \dots, \gamma_N I_{d_z}]$, and $\boldsymbol{\alpha} = \diag [\alpha_1 I_{d_z} , \dots, \alpha_N I_{d_z} ]$; where $i=1,\dots,N$.
% \end{table}

% % If the number of experts $N$ is too large for the matrix operators in Theorem \ref{thm:NashEqmExistence} to be tractable, then one (uniformly) randomly samples a batch of size $1\le b\le N$, with $b\in \mathbb{N}$, amongst all the $N$ experts and that subset of experts plays the Nash game.  The remaining experts continue to update their linear readout layers using the exponentially weighted ridge-repression problem \eqref{prop:localgreedyupdates}.

% {
% In the most general form of our main result, as stated in Theorem \ref{thm:NashEqmExistence}, the computational bottleneck in the FL algorithm lies in computing the matrices described therein. However, explicit closed-form expressions are derived for deterministic (non-generative) feature encoders in Section \ref{s:Analysis__ss:PreTrained} and for RFNs in Section \ref{s:Analysis__ss:ELN}.  
% The algorithmic formulation of Theorem \ref{thm:NashEqmExistence} is recorded in Algorithm \ref{alg:sync_subroutine}. Before detailing these simplified cases, we first illustrate a variant of our procedure where experts are temporarily restricted in the information governing their actions, leading to sub-optimal behaviour. This relaxation enables a more rapid computational throughput of their optimal actions at the cost of a controllable degree of sub-optimal behaviour.}

% \subsubsection{Speedy and Greedy: Client Acceleration via Infrequent Games} \label{greedy_algorithm}
% {Though the optimal behaviour of each agent, in the proprietary setting, is now known explicitly in closed-form due to Theorem \ref{thm:NashEqmExistence}, the optimal strategy does involve several large matrix computations which can be computationally intensive.  Therefore, one can consider a more efficient \textit{variant} of the client-side procedure, which only computes the optimal updates in Equation \eqref{eqmvecbeta} periodically with a frequency of $\tau\in \mathbb{N}_+$.\footnote{Note when $\tau=1$ then both this section and the previous sections' strategies are identical.} We call these times $\{\tau t\}_{t=0}^{\infty}$ \textit{synchronization times} where the system of proprietary agents synchronize.  This is because the agents act greedily, and thus Nash-sub-optimally, for all other times, then their behaviour is \textit{de-synchronizing} for the optimal behaviour given by the Nash equilibrium computed in Theorem \ref{thm:NashEqmExistence}.

% We consider the following \textit{greedy} objective for each agent between synchronization times.  We emphasize that this greedy objective ignores the prediction of all other agents and the weights issued/used by the central server.  For each $t\in \mathbb{N}_+$ not divisible by $\tau$, the $i^{\text{th}}$ expert's greedy objective is defined to be
% \begin{align} 
% \label{eq:ridge_local}
%         \tilde{J}_i(\beta_t^{i})
%     \eqdef 
% % \beta_t^i\in \operatorname{argmin}\, 
%         \sum_{s=(t-T)\vee 0}^{t-1}\,
%         e^{-\alpha_i(t-1-s)} 
%         \big\| y_{s+1} - ( \hat{Y}_{s}^i 
%         + Z_{s}^i \beta^i_t ) \big\|^2
%         +
%         \gamma_i\big\|\beta_t^i\big\|^2  , 
% \end{align} 
% where the parameters $\alpha_i$ and $\gamma_i$ are the same as Equation \eqref{eq:Objective_nth_expert}. 
% This allows for rapid and fully parallelized online optimization of each model but has the drawback that the ensemble may deviate from its optimum. Note that the $T$ in Equation \eqref{eq:ridge_local} need not be the same as that in Equation \eqref{eq:Objective_nth_expert}. When required, the former is referred to as the Client $T$ while the later is the Game $T$.  
% The following is a variant of the well-known optimal solution to the exponentially-weighted ridge-regression problem of Equation \eqref{eq:ridge_local}.

% \begin{proposition}[Agents: Optimal Linear Decoder With No Communication] 
% \label{prop:localgreedyupdates} 
% The unique minimum for Objective \eqref{eq:ridge_local} is
% \begin{align} 
%    \beta_t^i =
%         \big(
%             X^{i \top}_{t-1} X^i_{t-1} + \gamma_i I_{d_z}
%         \big)^{-1}\, X_{t-1}^{i \top} \, \bar{y}^i_t  ,   \notag 
% \end{align} 
% where
% \begin{align} 
% & X^i_{t-1}  = \big[ e^{ - \alpha_i (t-1-0)/2} Z^{i\top}_0 , \ldots, e^{-\alpha_i (t-1-s)/2} Z^{i \top }_s, \ldots,  Z^{i \top }_{t-1} \big]^\top ,  \notag  \\ 
% & \bar{y}^i_t  = \big[ e^{-\alpha_i (t-1-0)/2} (y_1 - \hat{Y}^i_{0} )^\top, \ldots, e^{-\alpha_i (t-1-s)/2} (y_{s+1} - \hat{Y}^i_{s} )^\top, \ldots,  (y_{t} - \hat{Y}^i_{t-1} )^\top \big]^\top . \notag  
% \end{align} 
% \end{proposition}
% }

% % \subsection{Discussion}
% % Every $T$ round, the server synchronizes a (uniformly) randomly selected batch of $ b \le N$ experts from all the available experts.  
% % Since each expert is working on a separate machine, which may not be large enough to load the states of all the experts simultaneously, they must reach a consensus with limited communication.  The optimal consensus can be framed as a \textit{non-cooperative game} amongst the randomly chosen $b$ experts, each of which seeks to exert predictive influence on the ensemble, to the proportion allotted by the server according to $w_t$.  The optimal direction which the ensemble can take can be formulated as a Nash equilibrium, in which no expert can improve their predictive influence on the mixture by further modifying their linear decoder \eqref{eq:Objective_nth_expert}.
% % The subroutine in Algorithm \ref{alg:sync_subroutine} computes precisely this Nash equilibrium using $T$ iterations.

% % %\AK{Xuwei: Write Proposition in Algo 2 Format}
% % %\begin{algorithm}[H]%[ht!]%
% % %\caption{Synchronization Subroutine}
% % %\label{alg:sync_subroutine}
% % %\begin{algorithmic}
% % %\SetAlgoLined
% % %\Require {\color{blue}{Copy and paste Proposition 2}} 
% % %\DontPrintSemicolon 
% % %\State  
% % %\end{algorithmic}
% % %\end{algorithm}


% % We now summarize our federated learning algorithm.

% \subsection{Algorithmic Compute, Communication, and Privacy Trade-offs}

% Two computational, and subtly different, implementations of the proposed algorithm are possible, both of which minimize the agent objectives in Equation \eqref {eq:Objective_nth_expert} using the iterative method from Theorem \ref{thm:NashEqmExistence}. In the first, detailed in Algorithm \ref{alg:sync_subroutine}, each agent computes $\mathbf{D}_i(t)$, $P_i(t)$, and $S_i(t)$ in parallel. Alternatively, all computations can be centralized on the server. While both are mathematically equivalent, they differ regarding computational burden, communication overhead, and privacy implications.

% Computing the Nash equilibrium is resource-intensive. If the server is compute-constrained, one can parallelize the construction of $\mathbf{D}_i(t)$, $P_i(t)$, and $S_i(t)$ across agents to alleviate the bottleneck. However, this introduces trade-offs. Each agent must access $\{Z_t^i\}_{i=1}^N$, which exposes potentially proprietary model activations to other participants in the network. Moreover, while all required history $\{Z_t^i\}_{i=1}^N$ may be gather and shared once, quantities like $\mathbf{A}(t)$ and $\mathbf{B}(t)$ depend on $\{P_i(t+1)\}_{i=1}^N$ and must be updated and communicated at each time step -- incurring additional communication costs and privacy risks.

% Alternatively, if each agent transmits all required $\{Z_t^i\}_{i=1}^N$, either all at once or alongside predictions, to the server. Then all information needed to perform the iterative updates of Theorem \ref{thm:NashEqmExistence} exists at the server's disposal. This one-shot communication significantly reduces overhead and enhances privacy, as agents do not access potentially sensitive activations from others. Such concealment is standard, for example, in commercial LLM APIs to prevent model inversion or theft \citep{Oliynyk1}. The trade-off is that the server must now centrally perform the full linear algebra computations, which can be resource intensive. This centralized setup is used in the experiments below.

% \section{Use-Cases: From Pre-Trained Encoders to Echo-State Agents}
% \label{s:Examples}

% This section puts our theory into practice for various AI agents ranging from ``static'' kernel regressors to sequential deep learning models with internal latent ``memory states.'' In each case, we derive simplified and specialized expressions of the main result (Theorem \ref{thm:NashEqmExistence}), yielding streamlined algorithms.  We consider three cases: pre-trained feature encoders, RFNs, and ESNs. In each case, the proposed theoretical PFL algorithm is tested across multiple datasets, validating its reliability on synthetic and real-world data.

% \subsection{Experiment Details} 

% Before detailing each case, the experiments used to evaluate the quality of the proposed PFL algorithm are outlined. We consider five challenging time-series datasets. Three are synthetic and and two are drawn from real-world benchmarks. Each is discussed in detail in Appendix \ref{s:ExperimentDetials__ss::datasets}. The experiments involve multiple agents and a server, with predictions made using two or five collaborating agents. Periodic synchronization via the Nash game, defined in Section \ref{nash_sync}, is compared with purely greedy local optimization, detailed in Section \ref{greedy_algorithm}, forgoing any Nash computations. These two approaches are often referred to throughout as the game and non-game settings, respectively. Experimental results for the distinct model varieties are reported in Sections \ref{s:Analysis__ss:PreTrained}--\ref{s:Examples_ReservoirComputer}, with visualizations focusing on the five-client settings. These sections also derive how the main algorithm (Theorems \ref{thm:OptimalWeights} and \ref{thm:NashEqmExistence}) simplifies for each model. A model's predictive performance is primarily quantified by its predictive mean-squared error (MSE), with optimal hyperparameters reported for both Nash and non-Nash settings.  

% Various other quantitative tools and qualitative visualizations are also incorporated to provide a complete perspective on each model and algorithm's performance.  The first set of plots overlay the predictions made by the server in both the game and non-game settings with the ground truth signal for comparison. The second set of figures illustrates the distribution of relative squared errors between the game and non-game predictions at every time step,
% \begin{align*}
% \frac{(\hat{Y}^n_{i, t} - y_{i, t})^2}{(\hat{Y}^g_{i, t} - y_{i, t})^2},
% \end{align*}
% where $y_{i, t}$ is the $i^{\text{th}}$ dimension of the target variable at time step $t$. The corresponding predictions with and without the Nash-game are denoted $\hat{Y}^g_{i, t}$ and $\hat{Y}^n_{i, t}$, respectively. If the value of the ratio at a given time step is greater than one, the server's prediction error in the Nash setting is lower than that of the non-Nash setting.

% Thereafter, in Section \ref{s:Experiments__ss:Ablation}, three ablation studies are presented. First, the impact of the Nash game on a server's mixture weights over time is illustrated, highlighting its positive influence towards producing higher quality mixtures. In the second study, the impact of varying the look-back length on Nash game performance is analyzed, offering deeper insights into its internal mechanisms. Finally, the Nash game's performance under different synchronization frequencies is considered, along with runtime overhead measurements, including the total runtime incurred by playing the Nash game each round for all agent types across two datasets. For additional experimental details, hyperparameters, and further ablations, such as motivation for using Hard Sigmoid activations with ESNs, see Appendices \ref{s:ExperimentDetials__ss::datasets}--\ref{a:Ablations}.\footnote{All experimental code is found at: \url{https://github.com/fatemetkl/FedMOE}.}

% \subsection{Experimental Results Summary}

% The main results are reported in Table \ref{tab:summary_results}. For all datasets and all models, application of Nash-game synchronization improves MSE, sometimes by an order of magnitude. The Nash game is especially helpful for the Concept Shift, BoC Exchange Rate, and ETT time-series. For both ESN and RFN models, there is also typically an improvement in prediction accuracy, both with and without the Nash game, with more experts contributing to the mixture. Such improvement is largely expected, especially since these models incorporate randomness in their feature representations.

% \begin{table}[ht]
% \centering
% \caption{Summary of experimental results for feature encoder, RFN, and ESN models across datasets. The reported MSE is the mean of three separate runs with different random seeds for ESNs and RFNs. For the pre-trained encoder models, there are no fluctuations due to randomness.}
% \label{tab:summary_results}
% \resizebox{0.9\linewidth}{!}{\begin{tabular}{cclccc}
% \toprule
% Model & \# of Experts & Dataset & Nash game & No Nash game \\
% \midrule
% \multirow{10}{*}{Transformer} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{1.78749\mathrm{e}{\text{-}1}}$ & $5.86464\mathrm{e}{\text{-}1}$ \\
% & & Logistic Map & $\mathbf{4.53782\mathrm{e}{\text{-}2}}$ & $5.46232\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{6.45116\mathrm{e}{\text{-}2}}$ & $6.77600\mathrm{e}{\text{-}1}$ \\
% & & BoC Exchange Rate & $\mathbf{4.48450\mathrm{e}{\text{-}5}}$ & $8.06623\mathrm{e}{\text{-}5}$ \\
% & & ETT Series & $\mathbf{7.50786\mathrm{e}{\text{-}4}}$ & $1.05523\mathrm{e}{\text{-}3}$ \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{6.95994\mathrm{e}{\text{-}2}}$ & $5.86337\mathrm{e}{\text{-}1}$ \\
% & & Logistic Map & $\mathbf{3.88076\mathrm{e}{\text{-}2}}$ & $6.99996\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{5.56220\mathrm{e}{\text{-}2}}$ & $3.25625\mathrm{e}{\text{-}1}$ \\
% & & BoC Exchange Rate & $\mathbf{4.48687\mathrm{e}{\text{-}5}}$ & $8.35143\mathrm{e}{\text{-}5}$ \\
% & & ETT Series & $\mathbf{7.27732\mathrm{e}{\text{-}4}}$ & $1.26992\mathrm{e}{\text{-}3}$ \\
% \midrule
% \multirow{10}{*}{RFN} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{2.56902\mathrm{e}{\text{-}1}}$ & $6.28833\mathrm{e}{\text{-}1}$ \\
% & & Logistic Map & $\mathbf{4.97284\mathrm{e}{\text{-}2}}$ & $5.54874\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{7.85654\mathrm{e}{\text{-}3}}$ & $9.45541\mathrm{e}{\text{-}0}$ \\
% & & BoC Exchange Rate & $\mathbf{7.86047\mathrm{e}{\text{-}5}}$ & $2.10533\mathrm{e}{\text{-}3}$ \\
% & & ETT Series & $\mathbf{1.19513\mathrm{e}{\text{-}3}}$ & $3.51060\mathrm{e}{\text{-}3}$ \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{ 5.96514\mathrm{e}{\text{-}2}}$ & $6.15566\mathrm{e}{\text{-}1}$ \\
% & & Logistic Map & $\mathbf{4.64415\mathrm{e}{\text{-}2}}$ & $5.50781\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{1.01067\mathrm{e}{\text{-}2}}$ & $1.28812\mathrm{e}{\text{-}0}$ \\
% & & BoC Exchange Rate & $\mathbf{7.65036\mathrm{e}{\text{-}5}}$ & $3.15237\mathrm{e}{\text{-}3}$ \\
% & & ETT Series & $\mathbf{7.11836\mathrm{e}{\text{-}4}}$ & $2.26659\mathrm{e}{\text{-}3}$ \\
% \midrule
% \multirow{10}{*}{ESN} & \multirow{5}{*}{2} & Periodic Signal & $\mathbf{1.02870\mathrm{e}{\text{-}1}}$ & $5.62155\mathrm{e}{\text{-}1}$ \\
% & & Logistic Map & $\mathbf{4.71543\mathrm{e}{\text{-}2}}$ & $5.30976\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{1.30703\mathrm{e}{\text{-}1}}$ & $1.98226\mathrm{e}{\text{-}0}$ \\
% & & BoC Exchange Rate & $\mathbf{5.15198\mathrm{e}{\text{-}5}}$ & $2.18067\mathrm{e}{\text{-}4}$ \\
% & & ETT Series & $\mathbf{7.13503\mathrm{e}{\text{-}4}}$ & $1.11331\mathrm{e}{\text{-}3}$ \\
% \cmidrule{2-6}
% & \multirow{5}{*}{5} & Periodic Signal & $\mathbf{3.22272\mathrm{e}{\text{-}2}}$ & $5.57315\mathrm{e}{\text{-}1}$  \\
% & & Logistic Map & $\mathbf{4.65061\mathrm{e}{\text{-}2}}$ & $5.28456\mathrm{e}{\text{-}2}$ \\
% & & Concept Shift & $\mathbf{8.86346\mathrm{e}{\text{-}2}}$ & $4.85359\mathrm{e}{\text{-}0}$ \\
% & & BoC Exchange Rate & $\mathbf{1.15900\mathrm{e}{\text{-}4}}$ & $ 4.08432\mathrm{e}{\text{-}4}$ \\
% & & ETT Series & $\mathbf{7.15441\mathrm{e}{\text{-}4}}$ & $1.08915\mathrm{e}{\text{-}3}$ & \\
% \bottomrule
% \end{tabular}}
% \end{table}
% \subsection{{Pre-Trained Transformer with Fine-Tunable Linear Decoder}}
% \label{s:Analysis__ss:PreTrained}

% We first consider the setting in which each (deep) feature encoder $\varphi^{i}$ in Equation \eqref{eq:ENCODER} is pre-trained and deterministic. This is likely the most common case in our setting, occurring when $\varphi^{i}$ is, for instance, a pre-trained transformer or a foundation model such as  CLIP \citep{radford2021learning}, DINO(v2) \citep{caron2021emerging,oquab2024dinov2learningrobustvisual}, SLIP(v2) \citep{mu2022slip,tschannen2025siglip}, among many others. Beyond its prevalence in modern deep learning, this setup offers a key advantage. The dynamically-evolving matrices in Theorem \ref{thm:NashEqmExistence} simplify dramatically, yielding surprisingly straightforward expressions. This is largely due to all expectations vanishing, as the encoder has no remaining internal sources of randomness.

% \begin{corollary}[Pre-Trained Deterministic Feature Encoders]
% \label{cor:PreTrainedTransformer}
% In the setting of Theorem \ref{thm:NashEqmExistence}.  If additionally, for $i=1,\dots,N$, the map $\varphi^{i}:\mathbb{R}^{%(1+t)
% d_x
% \times 1}\to \mathbb{R}^{d_z\times 1}$ is of the form
% % be all but the final linear decoder layer $\beta_t\in \mathbb{R}^{d_z\times 1}$ of a pre-trained feature encoder (e.g. a transformer)
% \begin{equation*}
%     \varphi^{i}(x_{[0:t]},Z_{t-1}^i, \epsilon_t^i ) \eqdef \phi^{i}(x_t).
% \end{equation*}
% {Then the matrix-valued processes in Theorem \ref{thm:NashEqmExistence} are}
% \allowdisplaybreaks 
% \begin{align} 
% & \mathbf{A}(t) = 
% \begin{bmatrix} 
% \phi^{i}(x_t)^{\top} \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j\phi^{(j)}(x_t) 
% \end{bmatrix}_{i,j=1}^N , 
% \notag \\ 
% & \widehat{\mathbf{A}}(t) = 
% \begin{bmatrix} 
% \phi^{i}(x_t)^{\top} \mathbf{e}_i^\top \mathbf{w}_t \mathbf{w}_t^\top  \mathbf{e}_j\phi^{(j)}(x_t) 
% \end{bmatrix}_{i,j=1}^N , 
% \notag \\ 
% & \mathbf{B}(t) = 
%  \begin{bmatrix} 
%      P_1(t+1)  \mathbf{e}_1 \phi^{(1)}(x_t) , \dots,  P_N(t+1) \mathbf{e}_N \phi^{(N)}(x_t)
%  \end{bmatrix}^\top  
%  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%     S_1(t+1)^\top  \mathbf{e}_1 \phi^{(1)}(x_t) , \dots, S_N(t+1)^\top  \mathbf{e}_N \phi^{(N)}(x_t)
%  \end{bmatrix}^\top  
%  , 
%  \notag \\ 
% & \mathbf{D}(t) 
%  = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 \phi^{(1)}(x_t) , \dots , \mathbf{e}_N \phi^{(N)}(x_t) 
%  \end{bmatrix} , 
%  \notag \\ 
%  & \mathbf{D}_i(t) 
%  = \big[ \phi^{(j)}(x_t)^\top \mathbf{e}_j^\top P_i(t+1) \mathbf{e}_k \phi^{(k)}(x_t) \big]_{j,k=1}^N , 
%  \quad i = 1, \dots, N . 
%  \notag 
% %&  \mathbf{D}_i(t)  =    
% % \big[ \mathbf{e}_1 \phi^{(1)}(x_t) , \cdots , \mathbf{e}_N \phi^{(N)}(x_t) \big]^\top 
% %  P_i(t+1) 
% % \big[\mathbf{e}_1 \phi^{(1)}(x_t) , \cdots , \mathbf{e}_N \phi^{(N)}(x_t) \big] ,
% % \quad i = 1, \dots, N.  \notag 
% \end{align} 
% \end{corollary}

% In this section, the deep encoder considered is a pre-trained transformer-based encoder model. Pre-training details are outlined in Appendix \ref{a:TransExpHyper}. The final linear layer constitutes the trainable $\beta$. In subsequent sections, sources of randomness are incrementally incorporated into the models.

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/periodic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:transformer_periodic_overlaid_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/logistic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:transformer_logistic_overlaid_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/concept/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:transformer_concept_overlaid_predictions}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/boc/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:transformer_boc_overlaid_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/ett/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:transformer_ett_overlaid_predictions}
%     \end{subfigure}
%     \caption{Server predictions compared with ground truth targets for mixtures of encoder models with and without Nash-game synchronization for the Periodic (\subref{fig:transformer_periodic_overlaid_predictions}), Logistic (\subref{fig:transformer_logistic_overlaid_predictions}), Concept Drift (\subref{fig:transformer_concept_overlaid_predictions}), BoC Exchange Rates (\subref{fig:transformer_boc_overlaid_predictions}), and ETT (\subref{fig:transformer_ett_overlaid_predictions}) time series.}
%     \label{fig:transfomer_overlaid}
% \end{figure}

% \subsubsection{Transformer Experimental Results}
% \label{s:Examples__ss:PreTrained__sss:Results}

% As seen in Figure \ref{fig:transfomer_overlaid}, predictions leveraging the Nash game produce significantly better modelling than those without it. Qualitatively, this improvement is especially notable in high-frequency segments of the time series and following sudden changes in the trajectory of the signals. Figure \ref{fig:transfomer_relative} shows the squared-error ratio of the non-game setting to that of the Nash game, as described in Section \ref{s:Examples}, for transformer agents over different signals. Points above the red line indicate time steps for which the Nash game is outperforming the baseline. A high density of such points above the red line reflects the performance advantages of Nash-game synchronization.

% In the Periodic and Logistic time series, predictions produced by the transformer models without Nash synchronization tend towards the overall series mean. In contrast, models with Nash synchronization more effectively capture the amplitude of the underlying oscillations. While the non-game predictions for the Periodic signal may appear accurate at the beginning and end of the series, the ratio of squared errors in Figure \ref{fig:transfomer_relative}\subref{fig:transformer_periodic_squared_errors} shows that the error remains consistently and significantly higher than that of the Nash game predictions across the entire time span.
% The Logistic Map dataset is quite challenging, especially with only a single lagged input from which to make predictions. This series poses difficulties for the transformer models in both settings due to its oscillatory and occasionally unstable nature. However, as shown in Figures \ref{fig:transfomer_overlaid}\subref{fig:transformer_logistic_overlaid_predictions} and \ref{fig:transfomer_relative}\subref{fig:transformer_logistic_squared_errors}, predictions with Nash-game synchronization capture the series' behavior significantly better. Interestingly, for some time steps, the non-game settings tendency to follow the mean can reduce the risk of sharp deviations that lead to larger errors in the game-based model during changes in dynamics.

% % Concept drift
% The Concept Drift dataset incorporates multi-dimensional inputs and targets. In this series, a smooth shift in the relationship between the input and target variables occurs halfway through. As shown in Figure \ref{fig:transfomer_overlaid}\subref{fig:transformer_concept_overlaid_predictions}, the Nash game predictions more cleanly adapt to this change. In contrast, predictions without Nash synchronization struggle to adjust to the transition, resulting in a delayed alignment with the target signal and degraded fidelity. 

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/periodic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:transformer_periodic_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/logistic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:transformer_logistic_squared_errors}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/concept/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:transformer_concept_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/boc/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:transformer_boc_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/transformer/ett/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:transformer_ett_squared_errors}
%     \end{subfigure} 

%     \caption{Comparison of relative squared errors for encoder model predictions with and without Nash-game synchronization for the Periodic (\subref{fig:transformer_periodic_squared_errors}), Logistic (\subref{fig:transformer_logistic_squared_errors}), Concept Drift (\subref{fig:transformer_concept_squared_errors}), BoC Exchange Rates (\subref{fig:transformer_boc_squared_errors}), and ETT (\subref{fig:transformer_ett_squared_errors}) time series.}
%     \label{fig:transfomer_relative}
% \end{figure}

% % BoC and ETT
% Predictions for the BoC Exchange Rate and ETT datasets are generally of higher quality likely due, in part, to presence of more informative features as detailed in Appendices \ref{s:ExperimentDetials__ss::datasets__sss:::BoC} and \ref{s:ExperimentDetials__ss::datasets__sss:::ETT}. They are also much longer time series than the preceding three datasets. The BoC series incorporates a number of lagged covariate exchange rates. Similarly, the ETT series leverages several informative input variables and lagged values of the target oil temperature. With these additional inputs, the server predictions of the Nash and non-Nash settings closely follow the targets for both datasets. However, as seen in Figures \ref{fig:transfomer_overlaid}\subref{fig:transformer_boc_overlaid_predictions} and \ref{fig:transfomer_overlaid}\subref{fig:transformer_ett_overlaid_predictions}, the non-game model predictions still fail to match the target signal in several parts of the time series. These shortcomings are effectively addressed by incorporating the Nash game. This improvement is clearly evident in Figures \ref{fig:transfomer_relative}\subref{fig:transformer_boc_squared_errors} and \ref{fig:transfomer_relative}\subref{fig:transformer_ett_squared_errors}, where the bulk of error ratios favor predictions using Nash synchronization.

% \subsection{Generative Random Feature Networks (RFNs)}
% \label{s:Analysis__ss:ELN}

% In this section, the feature encoders of Equation \eqref{eq:ENCODER} are expanded to incorporate re-sampled randomness at every step. This places such encoders within the realm of extreme learning machines such as RFNs \citep{huang2006universal,rahimi2008weighted}, which have attracted significant attention recently due to their theoretical amenability; especially via NTK theory \citep{jacot2018neural,cheng2024characterizing}, or the wide neural network literature; see e.g. \citep{mei2022generalization,gonon2023approximation,dirksen2022separation,frei2023random,simchoni2023integrating,hanin2024random,parhi2025random,maillard2025injectivity}.  

% Focusing on the case where the encoder is a random shallow ReLU neural network, we are able to obtain explicit expressions for all matrix-valued processes. Corollary~\ref{cor:Random_NeuralNetwork} presents the results for the case $d_y=1$, while the general case with $d_y>1$ is detailed in Corollary~\ref{cor:Random_NN_dy>1}, located in Appendix~\ref{s:ProofCorollaries}.
% \begin{corollary}[Random Feature Network]
% \label{cor:Random_NeuralNetwork}
% Assume the setting of Theorem \ref{thm:NashEqmExistence} with $d_y=1$. For each $i=1,\dots,N$, fix random matrices, $A^{i} \in \mathbb{R}^{d_y \times d_x}$ and $b^{i} \in \mathbb{R}^{d_y \times d_z}$. Define
% \begin{equation}
% \hat{Y}^i_{t+1} = \hat{Y}^i_t +
%             \big[ \operatorname{ReLU}\bullet\big(
%                 A^{i} [x_t, \dots, x_t ] + b^{i} + \sigma_t^i \, W_t^i
%             \big) \big]  \beta^{i}_{t} , 
% \notag 
% \end{equation}
% where $W_t^i\sim \mathcal{N}_{1\times d_z}(0,1)$ are independent of $A^i$ and $b^i$, 
% $[x_t, \dots, x_t] \in \mathbb{R}^{d_x\times d_z}$, $\beta^i_t\in \mathbb{R}^{d_z \times 1}$, $\sigma^i_t \in \mathbb{R}^{d_y \times 1}$, and $\bullet$ denotes the element-wise application of the $\operatorname{ReLU}$ function. 
% Here, $\varepsilon_t^i\eqdef \sigma^i_t \, W_t^i$, 
% $\varphi^{i}(x_{[0:t]}^i,Z_{t-1}^i, \varepsilon_t^i)\eqdef \operatorname{ReLU}\bullet\big(A^{i} [x_t, \dots, x_t] + b^{i} + \sigma^i_t \, W_t^i\big) = Z_{t}^i$.  
% We have the block matrices 
% \begin{align*}
% & \mathbf{A}(t)
%  = 
% \big[ A^{(i,j)}(t)\big]_{i,j=1}^N , 
% \hspace{0.5cm} 
% \widehat{\mathbf{A}}(t) = \big[ \widehat{A}^{(i,j)}(t) \big]_{i, j = 1}^N , 
% \notag \\  
%  & \mathbf{B}(t)  = 
%  \begin{bmatrix} 
%   P_1(t+1) \mathbf{e}_1 a(t, 1), \dots, P_N(t+1) \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%   S_1(t+1)^\top \mathbf{e}_1 a(t, 1), \dots, S_N(t+1)^\top  \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top , 
%   \notag \\   
% & \mathbf{D}(t) 
%   = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 a(t,1), \dots  , \mathbf{e}_N a(t, N) 
%  \end{bmatrix} , 
%  \notag \\ 
%  & \mathbf{D}_i(t) = \big[ D_i^{(j,k)}(t) \big]_{j,k = 1}^N , \quad i = 1, \dots, N . \notag 
% % \big( D_i^{(j,k)} \big)_{j,k=1}^N , \quad i = 1, \dots, N. \notag 
% \end{align*}
% For $t=1,\dots,N$ and $t\in \mathbb{N}_+$, each $a(t,i)$ is defined as follows
% \begin{align} 
% % & 
% a^i_t\eqdef A^{i}[x_t, \dots, x_t] + b^{i} 
% % , \notag \\ 
% \mbox{ and }
% % & 
% a(t,i)
% % \eqdef 
% % \mathbf{E}\big[ Z^i_t \big] 
% = 
%    a^i_t 
%         \odot
%         \left(
%             \bar{1}_{d_z} 
%             - 
%             \Phi\bullet\left(
%                 \frac{-a^i_t}{\sigma^i_t}%\cdot 
%             \right)
%         \right)
%         +
%             \frac{\sigma_t^i}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\left(
%             \frac{- ( a^i_t \odot a^i_t )}{2\, (\sigma^i_t)^2 }
%             % \,
%         \right)  , \notag 
% \end{align} 
% and $\odot$ and $\Phi$ are as in Lemma \ref{lem:Mean_Cov_ResModel}. 
% %and $\cdot^2$ is applied componentwise; i.e.\ $x^2\eqdef (x_i^2)_{i=1}^N$ for any $x\in \mathbb{R}^N$. 
% %$a^i_t\eqdef A^{(i)}x_t+b^{(i)}$. 
% The sub-matrices of $\mathbf{A}(t)$, $\widehat{\mathbf{A}}(t)$, 
% and $\{ \mathbf{D}_i(t) \}_{i=1}^N$, 
% are given by
% \begin{align} 
% & A^{(i,j)}(t) =
% \begin{cases} 
%   \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i \mathbb{E} \big[  Z^{i\top}_t  Z^i_t  \big] , \quad & \mbox{if} \,\, i = j , \\
%   \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j a(t, i)^\top a(t, j) , \quad & \mbox{if} \,\, i \neq j  , 
%  \end{cases} 
%  \notag \\ 
% % \end{align} 
% % \begin{align} 
%  & \widehat{A}^{(i,j)}(t) = 
%  \begin{cases} 
%  w^i_t w^i_t  \mathbb{E} \big[ Z^{i\top}_t Z^i_t \big]  , \quad & \mbox{if} \,\, i = j , \\ 
%  w^i_t w^j_t a(t, i)^\top   a(t, j) , \quad & \mbox{if} \,\, i \neq j   , 
% \end{cases} 
% \notag \\ 
% %\end{align} 
% %\begin{align} 
% & D_i^{(j,k)}(t) = 
% \begin{cases}
%   \mathbf{e}_j^\top P_i(t+1) \mathbf{e}_j \mathbb{E} \big[  Z^{j\top}_t  Z^j_t  \big]  , \quad & \mbox{if} \,\, j=k , \\ 
%  \mathbf{e}_j^\top P_i(t+1) \mathbf{e}_k a(t,j)^\top  a(t, k) , \quad & \mbox{if} \,\, j\neq k , 
% \notag 
% \end{cases} 
% \end{align} 
% where the matrices $\mathbb{E}\big[ Z^{i\top}_t Z^i_t \big] = \big( \mathbb{E}\big[ Z^{i\top}_t Z^i_t \big]_{jk}  \big)_{j,k=1}^{d_z}$, $i=1, \dots, N$ are given by 
% \begin{align}  
% & \mathbb{E} \big[ Z^{i\top}_t Z^i_t \big]_{jk}  
%  =  
%     \begin{cases}
%             \Big( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 \Big)
%             \cdot
%             \left(
%                 1 
%                 - 
%                 \Phi\left(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 \right)
%             \right) 
%             % \\
%             % \hspace{2cm}
%             +
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big) ,
%     & 
%         \mbox{ if } j=k , 
% \\ 
%       a(t, i)_j a(t,i)_k , 
%     & \mbox{ if }   j \neq k . 
%     \end{cases} 
%     \notag 
% \end{align} 
% \end{corollary} 

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/periodic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:rfn_periodic_overlaid_server_predictions}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/logistic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:rfn_logistic_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/concept/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:rfn_concept_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/boc/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:rfn_boc_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/ett/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:rfn_ett_overlaid_predictions}
%     \end{subfigure}
%     \caption{Server predictions compared with ground truth targets for mixtures of RFN models with and without Nash-game synchronization for the Periodic (\subref{fig:rfn_periodic_overlaid_server_predictions}), Logistic (\subref{fig:rfn_logistic_overlaid_server_predictions}), Concept Drift (\subref{fig:rfn_concept_overlaid_server_predictions}), BoC Exchange Rates (\subref{fig:rfn_boc_overlaid_server_predictions}), and ETT (\subref{fig:rfn_ett_overlaid_predictions}) time series.}
%     \label{fig:rfn_overlaid_prediction}
% \end{figure}

% \subsubsection{RFN Experimental Results}
% \label{s:Examples__ss:RFN__sss:Results}

% Across all datasets, the predictions incorporating the Nash game remain significantly better. This is qualitatively evident in the various trajectories shown in Figure \ref{fig:rfn_overlaid_prediction}. The RFN models are simpler than the transformers models of Section \ref{s:Analysis__ss:PreTrained} in terms of expressiveness. As such, the predictions in the non-game setting tend to be of somewhat lower quality. This is quantitatively supported by the numerical results in Table \ref{tab:summary_results}. Nonetheless, Figure \ref{fig:rfn_squared_error} illustrates that, for all signals, over the majority of time steps, the Nash game achieves lower squared errors compared to the non-game approach. Moreover, use of Nash synchronization brings the predictions of such models into closer competition with those of the transformers. Note that the best hyperparameter choices are recorded in Table \ref{tab:rfn_hyperparams} of Appendix \ref{s:OptimalParamterChoices}.

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/periodic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:rfn_periodic_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/logistic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:rfn_logistic_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/concept/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:rfn_concept_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/boc/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:rfn_boc_relative_squared_server_rrrors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/rfn/ett/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:rfn_ett_rlative_squared_error}
%     \end{subfigure}
%     \caption{Comparison of relative squared errors for RFN model predictions with and without Nash-game synchronization for the Periodic (\subref{fig:rfn_periodic_relative_squared_errors}), Logistic (\subref{fig:rfn_logistic_relative_squared_errors}), Concept Drift (\subref{fig:rfn_concept_relative_squared_errors}), BoC Exchange Rates (\subref{fig:rfn_boc_relative_squared_server_rrrors}), and ETT (\subref{fig:rfn_ett_rlative_squared_error}) time series.}
%     \label{fig:rfn_squared_error}
% \end{figure}

% Similar to the transformer results, predictions without Nash synchronization settle near the mean of the Periodic and Logistic series with smaller modulations in the prediction magnitude. During regions of more unstable behavior, occurring, for example, between $t=45$ to $t=65$ in the Logistic time series, this approach can inadvertently produce a better fit due to its conservative nature, as seen in Figure  \ref{fig:rfn_squared_error}\subref{fig:rfn_logistic_relative_squared_errors}. However, over the course of the series, the Nash-game synchronization process provides much more accurate predictions for both datasets.

% For simplicity in the RFN experiments, the Concept Drift time series target dimensionality is reduced such that $d_y = 1$. In this case, the $y_2$ series is retained. Predictions made with Nash-game synchronization outperform those without by a large margin. As seen in Figures  \ref{fig:rfn_overlaid_prediction}\subref{fig:rfn_concept_overlaid_server_predictions} and \ref{fig:rfn_squared_error}\subref{fig:rfn_concept_relative_squared_errors}, at the beginning of the time series, both approaches perform quite well. Predictions with the Nash game are of relatively higher quality, but the non-Nash game setting is competitive. However, after the concept transition, and especially later in the series, prediction errors appear to compound for the non-Nash setting causing heavy oscillations and poor predictions. Given that the series transitions from a lower to higher frequency pattern in its oscillations, it's possible that the hyperparameters for the non-Nash setting are well-fitted to the lower frequency setting but less so for the higher regime, and it fails to adapt.

% The RFN models produce fairly accurate predictions for the BoC Exchange Rate series. Considering the squared errors in Figure \ref{fig:rfn_squared_error}\subref{fig:rfn_boc_relative_squared_server_rrrors}, the vast majority of predictions throughout the time series are above the threshold of $1.0$. This is especially true in the later stages of the series. For many of the time steps, predictions based on the Nash game are three to five orders of magnitude better fits. Likewise, the RFN models produce relatively good predictions for the ETT dataset. For the server predictions, displayed in Figure \ref{fig:rfn_overlaid_prediction}\subref{fig:rfn_ett_overlaid_predictions}, those with the Nash-game synchronization qualitatively do a better job matching the magnitudes of the time series. This is also borne out in the ratio of squared errors plots of Figure \ref{fig:rfn_squared_error}\subref{fig:rfn_ett_rlative_squared_error}. The bulk of predictions errors favor the Nash-game setting. Further, it appears that the predictions for the RFN models are more heavily distributed in favor of the Nash synchronization process than in the transformer model settings, see Figure \ref{fig:transfomer_overlaid}\subref{fig:transformer_ett_squared_errors}.

% \subsection{Echo-State Agents - The Classical Reservoir Computers}
% \label{s:Examples_ReservoirComputer}
% Lastly, the framework is applied to reservoir computers. The setting of Corollary \ref{cor:Random_NeuralNetwork} is augmented by considering an additional random matrix, $B^i \in \mathbb{R}^{d_y \times d_y}$, independent of the $W_t^i$, for all $t$ and $i$.  
% If we allow for the hidden state, $Z_t$, generated at time $t$ to be remembered, then we obtain an ESN, which is a special case of a general reservoir computer, with structure
% \begin{equation}
% \label{eq:reservoir}
% \begin{aligned}
% Z_{t}^i\eqdef & \text{Hard Sigmoid} \bullet \big(
%     A^i [x_t, \dots , x_t] + B^i Z_{t-1}^i + b^i + \sigma^i \, W_t^i
% \big) , 
% \\
% \hat{Y}^i_{t+1} \eqdef & \hat{Y}^i_t +  Z_t^i \beta^{i}_t
% .
% \end{aligned}
% \end{equation}
% There are two subtle differences between Equation \eqref{eq:reservoir} and standard ESN formulations. First, the final layer of the ESN, $\beta$, is allowed to be dynamically updated, which is not usually the case in reservoir computing. Second, the residual updates in Equation \eqref{eq:reservoir} differ from standard ESNs. Unlike the previous types of agents, namely pre-trained encoders and RFNs, no simple closed forms are available for the expectation matrices in Theorem \ref{thm:NashEqmExistence}.  Rather, these quantities are estimated in the experiments using standard Monte-Carlo sampling. While the approach can be computationally heavy, the process is also quite effective, as seen in the results to follow.

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/periodic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:esn_periodic_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/logistic/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:esn_logistic_overlaid_server_predictions}
%     \end{subfigure} 

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/concept/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:esn_concept_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/boc/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:esn_boc_overlaid_server_predictions}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.8\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/ett/overlaid_server_predictions.pdf}
%     \end{minipage}
%     \label{fig:esn_ett_overlaid_server_predictions}
%     \end{subfigure}
%     \caption{Server predictions compared with ground truth targets for mixtures of ESN models with and without Nash-game synchronization for the Periodic (\subref{fig:esn_periodic_overlaid_server_predictions}), Logistic (\subref{fig:esn_logistic_overlaid_server_predictions}), Concept Drift (\subref{fig:esn_concept_overlaid_server_predictions}), BoC Exchange Rates (\subref{fig:esn_boc_overlaid_server_predictions}), and ETT (\subref{fig:esn_ett_overlaid_server_predictions}) time series.}
%     \label{fig:esn_overlaid_prediction_comparison}
% \end{figure}

% \subsubsection{ESN Experimental Results}
% \label{s:Examples__ss:ESN__sss:Results}

% As in previous experiments, predictions incorporating the Nash synchronization procedure significantly outperform those without. This is seen both qualitatively, in Figure \ref{fig:esn_overlaid_prediction_comparison}, and quantitatively in Figure \ref{fig:esn_relative_squared_errors}. Consistent with previous results, predictions without the Nash game are largely damped towards the average of both the Periodic and Logistic time series. On the other hand, while not quite reaching the full amplitude, predictions incorporating the game match provide much better replication of the series dynamics. However, during periods of instability in the Logistic Map series, the damped predictions produced without Nash synchronization temporarily outperform those including such synchronization. This phenomenon can be seen, for example, between $t=50$ and $t=65$ or $t=85$ to $t=105$. In spite of this, Nash-game synchronization produces notable reductions in prediction error. In Figures \ref{fig:esn_relative_squared_errors}\subref{fig:esn_periodic_relative_squared_errors} and \ref{fig:esn_relative_squared_errors}\subref{fig:esn_logistic_relative_squared_errors}, the majority error ratios are above $1.0$.

% For the Concept Drift dataset, non-Nash predictions actually struggle to accurately model the target values in both phases of the series, as shown in Figure \ref{fig:esn_overlaid_prediction_comparison}\subref{fig:esn_concept_overlaid_server_predictions}. The fit produced by the ESN model in this setting for the second stage is generally more accurate than seen in preceding experiments, while predictions for the first half are worse. Nonetheless, as in previous results, the predictions produced by the server when leveraging Nash synchronization are much more tightly bound to the target curves. This is even more evident when examining the squared-error ratios in Figure \ref{fig:esn_relative_squared_errors}\subref{fig:esn_concept_relative_squared_error}. 

% Similar to the results from other model types, both Nash and non-Nash game predictions follow the target signal fairly closely in the BoC Exchange Rate and ETT datasets, due in part to the higher quality of input features. In the BoC Exchange Rate dataset, the non-game server prediction fails to match the target signal during several time periods, such as between $t=600$ to $t=700$. This is, overall, not the case for Nash-game predictions, which demonstrate better alignment with the target. For the ETT dataset, predictions incorporating Nash synchronization more accurately capture the magnitudes of various spikes in the oil temperature throughout the series. As shown in Figures \ref{fig:esn_relative_squared_errors}\subref{fig:esn_boc_relative_squared_errors} and \ref{fig:esn_relative_squared_errors}\subref{fig:esn_ett_rlative_squared_errors}, the bulk of time steps have squared-error ratios above $1.0$, indicating sustained performance improvements from predictions leveraging Nash-game synchronization than those without.

% % esn squared erros

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/periodic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:esn_periodic_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/logistic/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:esn_logistic_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/concept/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:esn_concept_relative_squared_error}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/boc/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:esn_boc_relative_squared_errors}
%     \end{subfigure}

%     \begin{subfigure}[b]{0.99\linewidth}
%     \centering
%     \begin{minipage}[c]{0.05\linewidth}
%     \caption{}
%     \end{minipage}
%     \begin{minipage}[c]{0.7\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/esn/ett/relative_squared_server_errors.pdf}
%     \end{minipage}
%     \label{fig:esn_ett_rlative_squared_errors}
%     \end{subfigure}
%     \caption{Comparison of relative squared errors for ESN model predictions with and without Nash-game synchronization for the Periodic (\subref{fig:esn_periodic_relative_squared_errors}), Logistic (\subref{fig:esn_logistic_relative_squared_errors}), Concept Drift (\subref{fig:esn_concept_relative_squared_error}), BoC Exchange Rates (\subref{fig:esn_boc_relative_squared_errors}), and ETT (\subref{fig:esn_ett_rlative_squared_errors}) time series.}
%     \label{fig:esn_relative_squared_errors}
% \end{figure}


% \subsection{Ablation Studies}
% \label{s:Experiments__ss:Ablation}
% In this section, the effects of adjusting the principal knobs and hyperparameters driving the behaviour of the proposed FL algorithm are examined. Specifically, we analyze the impact of the Nash game on the mixture weights optimized by the server, the look-back parameter ($T$) in the Nash games, and the influence of varying the frequency with which Nash synchronization occurs ($\tau$), with special focus on the trade-off between runtime of the FL algorithm and its predictive power.

% \subsubsection{Mixture weights Analysis}
% \label{s:Experiments__ss:Ablation___sss:MixtureWeights}

% The Concept Drift dataset goes through an abrupt, but smooth, transition in the relationship between the input and output variables approximately halfway through the series. More details are provided in Appendix \ref{concept_drift_description}. This shift occurs between time steps $88$ and $112$. The onset of this transition is evident in the mixture weights computations of both methods in Figure \ref{fig:mixture_weights_concept_drift}. During this period, the dynamics of these weights changes significantly. The transition also appears to briefly impact the efficacy of Nash synchronization, evidenced by a degradation and eventual recovery of the ratio of errors in Figure \ref{fig:esn_relative_squared_errors}\subref{fig:esn_concept_relative_squared_error} between the non-game and game predictions during this time-frame. Of note for this dataset, there are clearly agents in the ensemble that struggle to produce helpful predictions. For example, two of the clients in the Nash game setting hover around zero weight in the ensemble, while three experts in the non-game setting are assigned weights near zero at various points in the series. 

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/transformer/concept/mixture_weights_plot.pdf}
%             \caption{Mixture weights with transformer models.}
%             \label{transformer_concept_mixtures_no_nash}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/mixture_weights_plot.pdf}
%             \caption{Mixture weights with ESN models.}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/transformer/concept/mixture_weights_plot_nash.pdf}
%             \caption{Mixture weights with transformer models.}
%             \label{transformer_concept_mixtures_nash}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/concept/mixture_weights_plot_nash.pdf}
%             \caption{Mixture weights with ESN models.}
%         \end{subfigure}
%     \end{tabular}
% \caption{Concept Drift Dataset Mixture Weights}
% \label{fig:mixture_weights_concept_drift}
% \end{figure}

% As seen in the mixture weights graphs of Figure \ref{fig:mixture_weights_periodic_signal} for the Periodic signal, the non-game ESN server settles into a stable and repeating set of weights after a warm-up period. On the same dataset, the non-game transformer server assigns highly volatile mixture weights with rapid changes between positive and negative weights assigned to a single expert. Meanwhile, the weights with the Nash game are somewhat more adaptive while maintaining stability for both agent types. 

% For both datasets, application of Nash synchronization appears to yield more stable mixture weight trajectories and shorter periods of instability. For example, comparing the weights of Figures \ref{fig:mixture_weights_concept_drift}\subref{transformer_concept_mixtures_no_nash} and \subref{transformer_concept_mixtures_nash}, those associated with the Nash game maintain steady states during periods of stable relationships between the input and target variables, while those without the Nash game exhibit larger fluctuations. Similarly, between Figures \ref{fig:mixture_weights_concept_drift}\subref{fig:mixture_weights_periodic_esn_non_game} and \subref{fig:mixture_weights_periodic_esn_nash_game}, the Nash game weights reach their periodic state more quickly and with lower oscillation amplitude than those without Nash synchronization.

% \begin{figure}[ht!]
%     \centering
%     \begin{tabular}{cc}
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/transformer/periodic/mixture_weights_plot.pdf}
%             \caption{Mixture weights with transformer models.}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot.pdf}
%             \caption{Mixture weights with ESN models.}
%             \label{fig:mixture_weights_periodic_esn_non_game}
%         \end{subfigure} \\
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/transformer/periodic/mixture_weights_plot_nash.pdf}
%             \caption{Mixture weights with transformer models.}
%         \end{subfigure} &
%         \begin{subfigure}[b]{0.45\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/esn/periodic/mixture_weights_plot_nash.pdf}
%             \caption{Mixture weights with ESN models.}
%             \label{fig:mixture_weights_periodic_esn_nash_game}
%         \end{subfigure}
%     \end{tabular}
% \caption{Periodic Signal Mixture Weights}
% \label{fig:mixture_weights_periodic_signal}
% \end{figure}


% \subsubsection{Effect of Nash game look-back Length}
% \label{s:Experiments__ss:Ablation___sss:look-back}

% The ``look-back'' length, or number of steps backwards in time considered in the Nash game calculations, is an important hyperparameter, denoted by $T$. This length not only affects prediction accuracy but also the computational cost, as the longer the look-back, the more calculations are necessary in the backward and forward processes of the Nash system. In this section, the effect of increasing look-back length is examined using RFN models applied to the BoC Exchange Rate and ETT datasets in the 5-client setting. The optimal hyperparameters discussed in Appendix \ref{s:OptimalParamterChoices} are applied with the exception of variation in the Game $T$, which takes values in the set $\{2, 3, 4, 5, 6, 7, 8, 9, 10, 15, 25\}$.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.49\linewidth]{figures/lookback/min_mses_over_lookback_boc_5c.pdf}
%     \includegraphics[width=0.49\linewidth]{figures/lookback/min_mses_over_lookback_ett_5c.pdf}
%     \caption{Variations in Minimum MSE for RFN models with varying Nash game look-back lengths for the BoC Exchange Rate (left) and ETT (right) time series using 5 experts.}
%     \label{fig:look-back_results}
% \end{figure}

% Similar to the Client $T$ value for local ridge regression, the optimal look-back length is dataset specific, dependent on the decay parameter $\alpha$, and non-monotonic in nature. Results of the experiments are displayed in Figure \ref{fig:look-back_results}. Departing slightly from previous results, the figure reports the minimum MSE seen across three separate RFN models with different seeds. As look-back length increases, it is likely that the optimal hyperparameters differ significantly from those reported in Appendix \ref{s:OptimalParamterChoices}. As such, the time-series predictions sometimes become unstable with longer look-back lengths. If none of the three runs produced an MSE less than $1.0$, they are excluded from the figure. The optimal look-back length for the BoC Exchange Rate and ETT time series are $5$ and $3$, respectively, with the minimum MSE growing steadily thereafter. Encouragingly, there are other look-back values near the optimum with good performance.


% \subsubsection{Nash game Frequency and Runtime/Performance Trade-off}
% \label{s:Experiments__ss:Ablation___sss:Runtime}

% Given the computational overhead associated with computing the Nash equilibrium, increasing the frequency with which the Nash computations are performed increases prediction latency. In this section, the performance drop induced by playing the Nash game less frequently is investigated, along with the runtime overhead imposed by each synchronization round. As discussed above, synchronizing predictions at every step is optimal in the experiments, but this comes at a cost of increased runtime. Runtime measurements for each round of Nash synchronization with five agents are shown in Table \ref{tab:runtime}, as well as total runtime.

% MSE results when running Nash synchronization every $\tau$ steps are shown in Figure \ref{fig:nash_frequency} with a fixed set of hyperparameters matching those in Appendix \ref{s:OptimalParamterChoices}. Such hyperparameters are likely no longer optimal for different $\tau$ steps, where $\tau \in \{1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 15, 25\}$. As such they no longer outperform the hyperparameter optimized non-Nash predictions. Nonetheless, the relationship between $\tau$ and performance is informative, even in this regime. The divergence from optimal hyperparameters is acutely felt in the 5-client setting for the BoC Exchange Rate dataset. When synchronization happens less often than every four steps, predictions tend towards instability. As such, the results for these experiments are not reported in the figure. A potential way to reduce the reliance of frequent synchronization is to replace previous client predictions with the ideal trajectory computed by the Nash game. Investigation of this improvement is left to future work.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.49\linewidth]{figures/frequency/mses_frequency_boc_leg.pdf}
%     \includegraphics[width=0.49\linewidth]{figures/frequency/mses_frequency_ett_leg.pdf}
%     \caption{Variations in Mean MSE for RFN models with increasing $\tau$ for the BoC Exchange Rate (left) and ETT (right) time series. Note that the the 5-client setting for the BoC Exchange Rate dataset produces significant instabilities for the chosen hyperparameters when synchronization happens less than every four steps. Thus, it is excluded.}
%     \label{fig:nash_frequency}
% \end{figure}
 
% Comparing the runtime and performance differences between the Nash game and non-game settings provides an estimation of the extra time imposed by the algorithm per round of playing the game. ESN models are expected to incur the largest overhead, as solutions to the Nash system require the approximation of a number of expectations. These approximations are computed with Monte-Carlo simulations using $100$ samples for each expectation when performing synchronization. The computational cost is considerably less for RFN models due to the analytical expressions for such expectations. Pretrained models impose the least runtime overhead when playing the Nash game. Table \ref{tab:runtime} reports the mean runtimes over three random seeds for the Periodic and BoC Exchange Rate time series using ESN, RFN, and transformer models with and without Nash synchronization. 

% Total time for RFN model predictions is shorter than that of ESN models by a factor of approximately $40$. Subsequently, transformer models are faster than RFNs by roughly a factor of $2$, making these models a good choice when prediction latency is important. On the other hand, without the Nash game, transformers have the longest runtime compared to other models due to their computational overhead. It should be noted that significant computation optimizations have not been pursued in solving the Nash systems. For example, the Monte Carlo simulations are done sequentially but are embarrassingly parallelizable in practice.

% \begin{table}[ht!]
%     \centering
%     \caption{Runtime measurements in seconds for simulations with five experts. Nash synchronization occurs each step when the technique is applied, and all optimal hyperparameters are used.}
%     \begin{tabular}{llcccc}
%     \toprule
%      & & \multicolumn{2}{c}{Nash game} & \multicolumn{2}{c}{No Nash game} \\
%     Model & Dataset & Total (s) & Per Step (s) & Total (s) & Per Step (s) \\
%     \midrule
%      \multirow{2}{*}{ESN} & Periodic & $1.88\mathrm{e}{\text{+}3}$s & $9.41\mathrm{e}{\text{-}0}$s & $4.24\mathrm{e}{\text{-}1}$s & $ 2.12\mathrm{e}{\text{-}3}$s\\
%      & BoC & $2.00\mathrm{e}{\text{+}4}$s & $1.00\mathrm{e}{\text{-}1}$s & $4.24\mathrm{e}{\text{-}0}$s & $2.11\mathrm{e}{\text{-}3}$s\\
%      \midrule
%      \multirow{2}{*}{RFN} & Periodic & $5.28\mathrm{e}{\text{+}1}$s & $2.64\mathrm{e}{\text{-}1}$s & $3.68\mathrm{e}{\text{-}1}$s & $1.84\mathrm{e}{\text{-}3}$s\\
%      & BoC & $5.08\mathrm{e}{\text{+}2}$s & $2.54\mathrm{e}{\text{-}1}$s & $4.07\mathrm{e}{\text{-}0}$s & $2.03\mathrm{e}{\text{-}3}$s \\
%      \midrule
%      \multirow{2}{*}{Transformer} & Periodic & $1.96\mathrm{e}{\text{+}1}$s & $9.80\mathrm{e}{\text{-}2}$s & $1.67\mathrm{e}{\text{-}0}$s & $8.34\mathrm{e}{\text{-}3}$s\\
%      & BoC & $1.59\mathrm{e}{\text{+}2}$s & $7.93\mathrm{e}{\text{-}2}$s & $1.81\mathrm{e}{\text{+}1}$s & $9.03\mathrm{e}{\text{-}3}$s \\
%      \bottomrule
%     \end{tabular}
%     \label{tab:runtime}
% \end{table}

% It is important to note that a considerable performance advantage when synchronizing with the Nash game may be preserved by performing such synchronizations less frequently if using optimal parameters. Consider the BoC Exchange Rate dataset and an RFN model. With hyperparameters tuned for the specific synchronization frequency, if Nash synchronization occurs every $10$ steps, rather than every step, the runtime is reduced by a factor of more than $7.5$, and the resulting MSE remains well below that of the non-game setting. Specifically, a synchronization frequency of $10$ results in an average MSE of $5.82080\mathrm{e}{\text{-}4}$ over $67.027$s compared with the non-game mean MSE of $3.15237\mathrm{e}\text{-}3$ and average runtime of $4.069$s.

% \section{Conclusion and Future Work}

% In this work, the proprietary federated learning problem is viewed through a non-cooperative game-theoretic lens (Theorem \ref{thm:NashEqmExistence})
% and an efficient and decentralized algorithm (Algorithm \ref{alg:sync_subroutine}) enabling collaboration among black-box agents without revealing their internal structure is derived.  
% The method is successfully applied to transformers (Corollary \ref{cor:PreTrainedTransformer}), random feature networks (Corollary \ref{cor:Random_NeuralNetwork}), and echo-state networks (Equation \eqref{eq:reservoir}). Numerical experiments are conducted on challenging real-world and synthetic time series, demonstrating significant improvements in predictive accuracy over existing baselines. 

% This work opens as many possible future research questions as it answers. Two such questions which we emphasize are how to solve the static and non-linear settings, beyond the kernelized setup we currently have where the agents only control their linear readout layer in Equation \eqref{eq:DECODER_RESIDUALS}.  We also mention a possible asymptotically large-population version of this problems which we imagine can be approached using the mean-field game toolbox, in a vague analogy with the neural tangent kernel \citep{jacot2018neural}. 

% % \bibliographystyle{spmpsci}      % mathematics and physical sciences
% %\bibliographystyle{spphys}       % APS-like style for physics
% %\bibliographystyle{plain} %plain
% \bibliography{Refs}   % name your BibTeX data base

% % \newpage


% \appendix
% \section{Proofs of Propositions and Theorems}
% \label{s:Proofs}

% This section contains the proofs of our main results.

% \subsection{{Proof of Proposition \ref{prop:localgreedyupdates}}}
% \begin{proof}%[{Proof of Proposition \ref{prop:localgreedyupdates}}]
% Observe that the loss function in Equation \eqref{eq:ridge_local} can be re-written as
% \allowdisplaybreaks
% \begin{align}
% \label{eq:redux_ridge}
% \begin{aligned}
%         & \sum_{s=0}^t\,
%             e^{ -\alpha_i(t-s)}
%             \,\big\|(y_s-\hat{Y}_s^i) - Z_s^i \beta_t^i \big\|^2
%             +
%             \gamma_i\big\|\beta_t^i\big\|^2
%     \\
%     & =
%         \sum_{s=0}^t\,
%             \,\big\| e^{-\alpha_i(t-s)/2}
%                 (y_s-\hat{Y}_s^i)
%              - (e^{-\alpha_i(t-s)/2} Z_s^i) \beta^i_t \big\|^2
%      +
%             \gamma_i\big\|\beta_t^i\big\|^2  \\ 
%     & = \big( \bar{y}^i_t - X^i_t \beta^i_t \big)^\top \big( \bar{y}^i_t - X^i_t \beta^i_t \big) 
%      + \gamma_i \beta^{i\top}_t \beta^i_t,
% \end{aligned}
% \end{align}
% and the last line of Equation \eqref{eq:redux_ridge} is simply a standard ridge-regression problem.  Since this is a strictly convex problem, there is a unique $\beta_t^i\in \mathbb{R}^{d_z \times 1}$ minimizing the last line of Equation\eqref{eq:redux_ridge}.  The desired closed-form expression is given in \citep[Equation (3.44)]{HastieTibshiraniFriedman_2001ESLBook}.
% \end{proof}

% \begin{comment}
% \subsection{{Proof of Theorem \ref{thm:OptimalWeights}}}
% \label{s:Proofs__ss:OptimalWeights}
% Fix a hyperparameter $\eta\le 0$ and consider a time $s\in \mathbb{N}$.
% We will now optimize the objective in \eqref{DTJ0} over the constraint set defined in \eqref{eq:Generalized_Simplex_Constraint}.  
% Observe that the major agent thus seeks to solve the nonlinear programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N) }  e^{-\alpha(t-s)} \Big\{ \big\| y_s - \sum_{j=1}^N w^j \hat{y}^j_s \big\|^2 
%  + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2 \Big\} \\ 
% & \text{subject to} 
% \,\,
% \mathbf{g}(w)=
% % (w^1-1, ..., w^N-1, -w^1, ..., -w^N)
% % ( -w^{{2}}, ..., -w^N)
% %%% AK Relaxation
% ({w^{1}}, -w^{{2}}, ..., -w^N)
% \leq 
% (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
% \eqdef \mathbf{c}
% % , 
% % \\ 
% % & \hspace{1.45cm}
% % \,\,
%  % h(w) = w^1 + ... + w^N - 1 = 0 
% ,
% \end{aligned} 
% \label{Majoragent:NLoptim}
% \end{equation} 
% where, for any $m\in \mathbb{N}_+$ we denote $\mathbf{1}_m\in \mathbb{R}^m$ given for each $i=1,\dots,m$ by $(\mathbf{1}_m)_i=1$.
% % \AK{Check if notation still needed:} 
% % Denote 
% % \begin{align} 
% % % \hat{\mathbf{Y}}_t = \big[ \hat{y}^1_t, \cdots , \hat{y}^N_t \big] , \quad 
% %   \mathbf{1}_{1\times N} = \big[ 1, ..., 1 \big] \in \mathbb{R}^{1\times N} , \quad 
% %  % \hat{\boldsymbol{\lambda}} = \big[ \hat{\lambda}_1, ..., \hat{\lambda}_N \big]^\top , \quad 
% %  % \mathrm{K} = \diag[\kappa_1, ..., \kappa_N] \in \mathbb{R}^{N\times N} . \notag 
% % \end{align} 



% Since the objective function of the nonlinear programming problem \eqref{Majoragent:NLoptim} can be written as 
% \begin{align} 
%  & e^{-\alpha(t-s)} \Big\{ \Big\| y_s - \sum_{j=1}^N w^j \hat{y}^j_s \Big\|^2 
%   + \sum_{j=1}^N \kappa_j \big\| w^j \big\|^2  \Big\}  \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ \Big( y^\top_s - \sum_{j=1}^N w^j \hat{y}^{j\top}_s \Big) 
%  \Big( y_s - \sum_{j=1}^N w^j \hat{y}^j_s \Big) + \sum_{j=1}^N \kappa_j w^{j 2} \Big\}   \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ N \sum_{i,j=1}^N w^i \hat{y}^{i\top}_s \hat{y}^j_s w^j 
%   - 2  y^\top_s   \sum_{j=1}^N w^j \hat{y}^j_s 
%    +  y^\top_s y_s + \sum_{j=1}^N \kappa_j w^{j 2} \Big\}  \notag \\ 
%  = &  e^{-\alpha(t-s)} \Big\{ w^\top \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) w 
%   - 2  y^\top_s  \hat{\mathbf{Y}}_s w 
%    + y^\top_s y_s \Big\} . \notag 
% \end{align} 
% Therefore the nonlinear programming problem \eqref{Majoragent:NLoptim} is equivalent to the following quadratic programming problem 
% \begin{equation} 
% \begin{aligned}  
% & \min_{w=(w^1, ..., w^N)^\top }  \frac{1}{2}  w^\top e^{-\alpha(t-s)}\big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s     + \mathrm{K} \big) w 
%   - e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s w  , \\ 
% & \text{subject to} \ G w \leq \mathbf{c} ,
% \end{aligned} 
% \label{Majoragent:QP}
% \end{equation} 
% where $G$ and $\boldsymbol{c}$ are defined in \eqref{eq:Gc_Def}; whose definition we recall here
% \begin{align} 
%  \mathrm{K} = \diag[\kappa_1, ..., \kappa_N]
%  % \in \mathbb{R}^{N\times N}
%  , 
%  \,
%  % Shifted Orthant
%   % G = -I_N
%   %% Full Simplex
%  % G = \begin{bmatrix} I_N \\ -I_N \\ \mathbf{1}_{1\times N} \\ - \mathbf{1}_{1\times N}  \end{bmatrix} 
%  % Hyperplane containing simplex
%  % G = \begin{bmatrix} 
%  % \mathbf{1}_{1\times N} \\
%  % - \mathbf{1}_{1\times N}  
%  % \end{bmatrix} 
%  %%% Annie Relaxation
%  G = 
%  \begin{pmatrix}
%      1 & \mathbf{0}_{1\times N} \\
%      \mathbf{0}_{ (N \times 1) } & -I_{(N-1\times N-1)} 
%  \end{pmatrix}
%  \,\mbox{ and }\,
%  % \quad 
%  %  
%  \mathbf{c} = 
%  % Shifted Orthant
%  % 0_{N\times 1}
%  % \bar{\eta}
%  %% Full Simplex
%  % \begin{bmatrix} 1_{N\times 1} \\ 0_{N\times 1} \\ 1 \\ -1   \end{bmatrix} . 
%  % Hyperplane containing simplex
%  % \begin{bmatrix} 
%  % 1 
%  % \\ 
%  % -1   
%  % \end{bmatrix}
%  %%% Annie Relaxation
%  (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
%   \label{eq:Gc_Def}
% \end{align} 
% {where for each $n,m\in \mathbb{N}_+$, $\mathbf{0}_{n,m}$ denotes the $n\times m$ zero matrix and $I_n$ the $n\times n$ identity matrix.
% Likewise, $\operatorname{diam}(\kappa_1,\dots,\kappa_N)$ denotes the $N\times N$-diagonal matrix whose diagonal is given, for each $i=1,\dots,N$, by $K_{i,i}=\kappa_i$.
% }



% To prove Theorem \ref{thm:OptimalWeights}, we need to use the results of the following Theorems \ref{thm:NSQP} and \ref{thm:QPdual} from \citep{Berkovitz2001}. 
% According to \cite[Theorem V.6.1]{Berkovitz2001}, the following theorem gives a necessary and sufficient condition for solutions of \eqref{Majoragent:QP}. 
% \begin{theorem} 
% \label{thm:NSQP}
% A necessary and sufficient condition for a point $w^\star=(w^{1, \star}, ..., w^{N, \star})^\top$ to be a solution of the quadratic programming problem \eqref{Majoragent:QP} is that 
% \begin{align} 
% G w^\star \leq \mathbf{c} \label{NSQP:Gw<=c} 
% \end{align} 
% and there exists a vector $\boldsymbol{\lambda} \geq 0$ in $\mathbb{R}^{2N+2}$ such that 
% \begin{align} 
%  & e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
%   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
%   + G^\top \boldsymbol{\lambda} = 0 , \label{NSQP:w+lambda} \\ 
%  & \boldsymbol{\lambda}^\top (G w^\star - \mathbf{c}) = 0 . \label{NSQP:wlambda}  
% \end{align} 
% \end{theorem}

% Introduce the dual quadratic programming problem: 
% \begin{equation} 
% \begin{aligned}  
% & \max \big\{ \theta (\boldsymbol{\lambda}) : \ \boldsymbol{\lambda} \geq 0 , \ \theta(\boldsymbol{\lambda}) > -\infty \big\} , 
%  \\ 
% & \theta(\boldsymbol{\lambda}) = \inf \{ L( \mathbf{x}, \boldsymbol{\lambda}) : \ \mathbf{x} \in \mathbb{R}^N \} ,  \\ 
% & L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}  
%   - e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) .   
% \end{aligned} 
% \label{Majoragent:DQP} 
% \end{equation} 

% By \cite[Theorem V.6.2]{Berkovitz2001}, we have the following relation between the quadratic programming problem \eqref{Majoragent:QP} and the dual problem \eqref{Majoragent:DQP}. 
% \begin{theorem} 
% \label{thm:QPdual}
% Let the quadratic programming problem \eqref{Majoragent:QP} has a solution $w^\star=(w^{1, \star}, ..., w^{N, \star})$. Then the dual problem \eqref{Majoragent:DQP} has a solution $\boldsymbol{\lambda}_\star$, and the solution $\boldsymbol{\lambda}_\star$ is exactly the multiplier $\boldsymbol{\lambda}$ in Theorem \ref{thm:NSQP} corresponding to $w^\star$. 
% \end{theorem} 

% With Theorems \ref{thm:NSQP} and \ref{thm:QPdual}, we are ready to prove Theorem \ref{thm:OptimalWeights}. 

% \begin{proof}[Proof of Theorem \ref{thm:OptimalWeights}]  

% By Theorem \ref{thm:NSQP}, we can determine the optimal weights $w^\star=(w^{1,\star}, ..., w^{N,\star})$ from 
% \eqref{NSQP:w+lambda}. The multiplier $\boldsymbol{\lambda}$ in \eqref{NSQP:w+lambda} is the solution of the dual problem \ref{Majoragent:DQP}. 

% We first solve the dual problem \eqref{Majoragent:DQP} for the optimal $\boldsymbol{\lambda}$. 
% The function $L(\mathbf{x}, \boldsymbol{\lambda})$ in \eqref{Majoragent:DQP} can be rewritten as  
% \begin{align} 
%  L( \mathbf{x}, \boldsymbol{\lambda}) 
%  = & \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  \mathbf{x}  
%   - e^{-\alpha(t-s)} y^\top_s \hat{\mathbf{Y}}_s \mathbf{x} 
%    + \boldsymbol{\lambda}^\top (G \mathbf{x} - \mathbf{c} ) \notag \\ 
%    = &  \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}  
%   - \Big[ e^{-\alpha(t-s)} y^\top_s  \hat{\mathbf{Y}}_s - \boldsymbol{\lambda}^\top G \Big] \mathbf{x} 
%    - \boldsymbol{\lambda}^\top \mathbf{c} . 
%    \label{L(x,lambda)2}   
% \end{align} 
% For each $\boldsymbol{\lambda}$ fixed, the function $L(\cdot, \boldsymbol{\lambda})$ given by \eqref{L(x,lambda)2} is a $C^1$ convex function on $\mathbb{R}^N$. Then $\mathbf{x}_{\boldsymbol{\lambda}}$ is a minimizer of $L(\cdot, \boldsymbol{\lambda})$ if and only if $\nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda}) = 0$. 
% It then follows from \eqref{L(x,lambda)2} that 
% \begin{align} 
%  0 = & \nabla_{\mathbf{x}} L(\mathbf{x}_{\boldsymbol{\lambda}} , \boldsymbol{\lambda})  \notag \\ 
%  = & e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s y_s - G^\top \boldsymbol{\lambda}  \Big] , 
%  \notag 
% \end{align} 
% which further gives that 
% \begin{align} 
% 0 = &   \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big(   N\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s 
%  + \mathrm{K} \big) \mathbf{x}_{\boldsymbol{\lambda}} 
%   - \mathbf{x}_{\boldsymbol{\lambda}}^\top \Big[  e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] .  
%   \label{0=<x,gradL>}  
% \end{align} 
% Substituting \eqref{0=<x,gradL>} into \eqref{Majoragent:DQP}, we obtain an explicit form of $\theta(\boldsymbol{\lambda})$
% \begin{align} 
%  \theta(\boldsymbol{\lambda}) = & L(\mathbf{x}_{\boldsymbol{\lambda}}, \boldsymbol{\lambda}) \notag \\ 
%  =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%   e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  
%   \mathbf{x}_{\boldsymbol{\lambda}}   
%   - \Big[ e^{-\alpha(t-s)} y^\top_s \hat{\mathbf{Y}}_s - \boldsymbol{\lambda}^\top G \Big] 
%    \mathbf{x}_{\boldsymbol{\lambda}}  
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =& \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s  + \mathrm{K} \big) 
%     \mathbf{x}_{\boldsymbol{\lambda}}   
%   -  \mathbf{x}_{\boldsymbol{\lambda}}^\top e^{-\alpha(t-s)} \big( N\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s 
%    + \mathrm{K} \big)    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} \notag \\ 
%    =&  - \frac{1}{2}  \mathbf{x}_{\boldsymbol{\lambda}}^\top 
%    e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  
%    \mathbf{x}_{\boldsymbol{\lambda}}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} . \notag 
% \end{align}  

% With the above explicit form of $\theta(\boldsymbol{\lambda})$, the dual quadratic programming problem \eqref{Majoragent:DQP} is then equivalent to 
% \begin{equation} 
% \begin{aligned} 
% & \max_{\mathbf{x}, \ \boldsymbol{\lambda}} \ 
% - \frac{1}{2}  \mathbf{x}^\top e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x}   
%    - \boldsymbol{\lambda}^\top \mathbf{c} ,   \\ 
% & \text{subject to:} \ 
%  e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big) \mathbf{x} 
%   - \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] = 0 .  
% \end{aligned} 
% \label{Majoragent:DQPequiv} 
% \end{equation} 
% Since $\hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s$ is positive semi-definite, $N>0$, and $K$ is a diagonal matrix with positive diagonal entries, then $N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}$ is positive definite and thus it is invertible.  
% Whence, the equality constraint in \eqref{Majoragent:DQPequiv} 
% implies that 
% \begin{align} 
%    \mathbf{x} 
% = e^{\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1} 
%  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] . 
% \label{xsublambda}
% \end{align} 
% With \eqref{xsublambda} substituted into \eqref{Majoragent:DQPequiv}, 
% the dual problem \eqref{Majoragent:DQPequiv} is then equivalent to the following unconstrained optimization problem: 
% \begin{align} 
%  \max_{\boldsymbol{\lambda}} \ -\frac{1}{2}  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s 
%    y_s - G^\top \boldsymbol{\lambda}  \Big]^\top 
%    e^{\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1} 
%  \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}^\top_s  y_s  - G^\top \boldsymbol{\lambda}  \Big] 
%  - \boldsymbol{\lambda}^\top \mathbf{c} . 
% \label{Majoragent:DQPunconstrained} 
% \end{align} 
% We reduce the unconstrained optimization problem \eqref{Majoragent:DQPunconstrained} to deduce that $\boldsymbol{\lambda}_\star$ satisfies
% \begin{align} 
% e^{\alpha(t-s)}\,
%  \Big[ G 
%  % e^{\alpha(t-s)}
%  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]
%  \boldsymbol{\lambda}_\star 
%  =
%  \Big[ G  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
%  y_s  -  \mathbf{c} \Big] . 
%  \label{lambdasubstar_almost} 
% \end{align} 
% Observe that $G$ (and thus $G^{\top}$) is invertible {since it is an $N\times N$ matrix with $\operatorname{det}(G)=1\cdot (-1)^{N-1}\neq  0$.
% Furthermore, notice that $G=G^{\top}$, $G$ commutes with all other matrices (when matrix multiplying), $G^2= I_N$, and the inverse of $G$ is given by
% \[
% \tilde{G}\eqdef 
%  \begin{pmatrix}
%      -1 & \mathbf{0}_{1\times N} \\
%      \mathbf{0}_{ (N \times 1) } & I_{(N-1\times N-1)} 
%  \end{pmatrix}
% .
% \]
% We use these remarks in the following computation.
% }  
% %is a diagonal matrix with non-zero diagonal values.  

% \noindent 
% Since we have already seen that $N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ is positive-define, and thus invertible, then $G\,N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} G^{\top}$.  
% {For legibility, set $A\eqdef \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ and $k\eqdef e^{\alpha(t-s)}>0$.}
% Thus, we may simplify \eqref{lambdasubstar_almost} to obtain
% \begin{align} 
%  \boldsymbol{\lambda}_\star 
%  = & \Big[ G e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
%  \Big[ G  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
%  y_s  -  \mathbf{c} \Big] 
%  \\
%   = & 
% %   {
% %       \Big[ 
% %       e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \Big]^{-1} 
% %      \Big[ -\Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %      y_s  
% %      -
% %      (-\eta \bar{1}_N)
% %      \Big] 
% %  }
% %  \\
% %   = & 
% %   {
% %   e^{\alpha(t-s)} 
% %   \,
% %       \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %      \Big[ 
% %         \eta \bar{1}_N
% %          -
% %          \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %          y_s  
% %      \Big] 
% %  }
% %  \\
% %   = & 
% %   {
% %   e^{\alpha(t-s)} 
% %   \Big[
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N
% %   -
% %     \hat{Y}^\top_s y_s  
% % \Big]
%  % }
%  %%% Annie Relaxation
%  {
%      \Big[ G k A^{-1} G^\top \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
% }
%  \\
%  &=
% {
%      \Big[ G k A^{-1} G \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%   \\
%  &=
% {
%      \Big[ G^2 k A^{-1} \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%    \\
%  &=
% {
%      \Big[ k A^{-1} \Big]^{-1} 
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%     \\
%  &=
% {
%      \frac1{k}\, A
%      \Big[
%         G  A^{-1} \hat{Y}^\top_s y_s  
%         -  
%         \mathbf{c} 
%      \Big] 
%  }
%      \\
%  &=
% {
%      \frac1{k}\, 
%         G AA^{-1} \hat{Y}^\top_s y_s  
%      -
%      \frac1{k}\,
%         A\mathbf{c} 
%  }
%       \\
%  &=
% {
%     \big(
%             \frac1{k}\, 
%                 G \hat{Y}^\top_s y_s  
%         -
%             \frac1{k}\,
%                 A\mathbf{c} 
%     \big)
%  }
%  . 
%  \label{lambdasubstar_almost} 
% \end{align} 
% Then we substitute $\boldsymbol{\lambda}_\star$ into \eqref{NSQP:w+lambda} to solve for the optimal weight vector $w^\star=(w^{1,\star}, ..., w^{N,\star})^\top$: 
% \allowdisplaybreaks
% %%% Annie Relaxation
% {
% \begin{align}
% % &\,\,
%   %   e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
%   % - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
%   % + G^\top \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + G \boldsymbol{\lambda}_{\star}  = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + G
%   \big(
%         \frac1{k}\, 
%             G \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%             A\mathbf{c} 
%     \big)
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k}\,
%         G
%         G \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% k
% A  w^\star 
%   - k \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k}\,
%         \hat{Y}^\top_s y_s  
%     -
%         \frac1{k}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% A  w^\star 
%   - 
%     \hat{\mathbf{Y}}_s^\top y_s 
%   + 
%         \frac1{k^2}\,
%         \hat{Y}^\top_s y_s  
%     -
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
%   = 0
% \\
% \nonumber
% \therefore & \,\,
% A  w^\star 
% =
%     \hat{\mathbf{Y}}_s^\top y_s 
%   - 
%         \frac1{k^2}\,
%         \hat{Y}^\top_s y_s  
%     +
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     A  w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         A^{-1}
%         G
%             A\mathbf{c} 
% \\
% \nonumber
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%         A^{-1}A\mathbf{c} 
% \\
% \label{eq:final_simplification__Gc}
% \therefore & \,\,
%     w^\star 
% =
%     \big(
%         1-\frac1{k^2}
%     \big)
%     A^{-1}
%     \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         G
%         \mathbf{c} 
% .
% \end{align}
% By definition of $G$ and $\mathbf{c}$, given in \eqref{eq:Gc_Def}, we find that
% \allowdisplaybreaks
% \begin{align} 
% \nonumber
%         G \mathbf{c} 
%         \,
%     = &
%         \begin{pmatrix}
%             1 & \mathbf{0}_{1\times N} \\
%             \mathbf{0}_{ (N \times 1) } & -I_{(N-1\times N-1)} 
%         \end{pmatrix}
%         \,
%         (1+\eta - \eta N,-\eta \mathbf{1}_{N-1})
% \\
% \nonumber
% =& 
%         (1+\eta - \eta N, \, \eta \mathbf{1}_{N-1})
% \\
% \nonumber
% =& 
%         (1-\eta N) \,e_1 + \eta \mathbf{1}_N
% \end{align} 
% where $e_1$ is the first standard basis vector in $\mathbb{R}^N$.
% Consequentially, the right-hand side of \eqref{eq:final_simplification__Gc} further simplifies to
% \begin{equation}
% \label{eq:pre_final_weights}
%     w^\star 
% =
%         \Big(
%             1-\frac1{k^2}
%         \Big)
%         A^{-1}
%         \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         \frac1{k^2}\,
%         \Big(
%             (1-\eta N) \,e_1 + \eta \mathbf{1}_N
%         \Big)
% .
% \end{equation}
% Plugging in the definitions of $A$ and of $k$ back into \eqref{eq:pre_final_weights} yields
% $A\eqdef \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} $ and $k\eqdef e^{\alpha(t-s)}>0$
% \[
%     w^\star 
% =
%         \big(
%             1-
%             % \frac1{k^2}
%             e^{-2\alpha(t-s)}
%         \big)
%         \big(
%             %% A
%             \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}
%         \big)^{-1}
%         \,
%         \hat{\mathbf{Y}}_s^\top y_s 
%     +
%         % \frac1{k^2}
%         e^{-2\alpha(t-s)}
%         \,
%         \Big(
%             (1-\eta N) \,e_1 + \eta \mathbf{1}_N
%         \Big)
% \]
% % This conclude the proof.
% }
% %%%% Shifted Orthant
% % {
% % \begin{align}
% % &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   + G^\top \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% % \therefore & 
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   - \boldsymbol{\lambda}_{\star}  = 0 
% % \\
% % \therefore &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   = 
% %   -e^{\alpha(t-s)}\mathbf{Y}_s^{\top}y_s  
% %   +
% %   e^{\alpha(t-s)} 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N
% % \\
% % \therefore &
% %     e^{-\alpha(t-s)} \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   % - e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top y_s 
% %   = 
% %   % -e^{\alpha(t-s)}\mathbf{Y}_s^{\top}y_s  
% %   % +
% %   e^{\alpha(t-s)} 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)  w^\star 
% %   = 
% %   \eta\,
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     w^\star 
% %   = 
% %   \eta\,
% %   \big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \big)^{-1}
% %   \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)
% %   \bar{1}_N 
% % \\
% % \therefore &
% %     w^\star 
% %   = 
% %   \eta\,\bar{1}_N 
% % \end{align}
% % }
% % \begin{align} 
% %    w^\star = &  e^{\alpha(t-s)} \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K}  \Big)^{-1} 
% %     \Big[ e^{-\alpha(t-s)} \hat{\mathbf{Y}}_s^\top  y_s 
% %   - G^\top \boldsymbol{\lambda}_\star \Big]  \notag  \\ 
% %   = &  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1}  \hat{\mathbf{Y}}_s^\top  y_s 
% %   \notag \\    
% %   & -  \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1}   G^\top 
% %   \Big[ G \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} G^\top \Big]^{-1} 
% %  \Big[ G \Big( N \hat{\mathbf{Y}}^\top_s \hat{\mathbf{Y}}_s + \mathrm{K} \Big)^{-1} \hat{Y}^\top_s 
% %   y_s -  \mathbf{c} \Big] , 
% %   \notag  
% % \end{align} 
% which is \eqref{eqn:OptimalWeights}.  
% \end{proof} 
% \end{comment}

% \subsection{{Proof of Theorem \ref{thm:OptimalWeights}}}

% \begin{proof}%[{Proof of Theorem \ref{thm:OptimalWeights}}]
% Define $A\eqdef 2\,
%  ( \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \kappa I_N)$, where $I_N$ is the $N\times N$ identity matrix, and set $b\eqdef 2  \big(
% y^\top_t  \hat{\mathbf{Y}}_t\big)^{\top}$. 
% The matrix $\hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t$ is positive semi-definite.  Since $\kappa>0$ then $\det(\kappa I_N)=\kappa^N>0$ and thus, the matrix $A$ is positive definite.  

% Let $B\eqdef \mathbf{1}_N\in \mathbb{R}^{N\times 1}$, where for $i=1,\dots,N$ we have $B_i=1$.  
% Note that $B$ has rank $1\le N$.

% Observe that the loss function $\Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 + \sum_{j=1}^N \kappa\, | w^j_t|^2 $ can be written as
% \allowdisplaybreaks
% \begin{align}
%     \Big\| y_t  - \sum_{j=1}^N w^j_t \hat{Y}^j_t \Big\|^2 
%     + 
%     \sum_{j=1}^N \kappa\, | w^j_t|^2 
% = &
%     \frac1{2}\, 
%     w^\top A w 
%   - b^{\top} w 
%    + y_t^\top y_t
% \eqdef Q(w)
% .
% \end{align}
% Therefore, the server's optimization problem in Equation \eqref{eq:server} can be written as a quadratic program with linear constraint 
% \begin{equation}
% \label{eq:server__QPLC}
% \begin{aligned}
%     \min_{w\in \mathbb{R}^N}\,
%     &
%     \frac1{2} \,
%     w^{\top} A w - b^{\top} w
% \\
% \mbox{s.t.} & \,\,
% B^{\top} w = \eta .%1.
% \end{aligned}
% \end{equation}
% Since $A$ is positive definite and since $\operatorname{rank}(B)=1\le N$ then the quadratic program in Equation \eqref{eq:server__QPLC} is a non-degenerate quadratic program with a feasible linear constraint set.
% By \citep[Proposition 6.3]{gallier2020linear}, there exists a unique solution to the constrained quadratic program and it is given by the Karush-Kuhn-Tucker (KKT) system
% \begin{align}
% \label{eq:KKT_1}
% A\,w + B\lambda & = b
% \\
% \label{eq:KKT_2}
% B^{\top} w & = \eta .%1.
% \end{align}
% Since $A$ is positive definite, it is invertible.  Therefore, Equation \eqref{eq:KKT_1} allows us to isolate $w$
% \begin{align}
% \label{eq:KKT_1__manip1}
% w  = A^{-1}\,(b - B\lambda)
% .
% \end{align}
% Plugging the expression for $w$, which we just obtained in Equation \eqref{eq:KKT_1__manip1}, back into Equation \eqref{eq:KKT_2} yields
% \allowdisplaybreaks
% \begin{align}
% \nonumber
% % 1
% \eta
% = & B^{\top} \big(A^{-1}\,(b - B\lambda)\big)
% \\
% \nonumber
% \therefore \,
% % 1 
% \eta
% = & B^{\top} \big(A^{-1}\,b - A^{-1}B\lambda \big) 
% = B^{\top}A^{-1}\,b - \lambda B^{\top}A^{-1}B
% \\
% \nonumber
% \therefore \,
%     \lambda B^{\top}A^{-1}B
% = & 
%     B^{\top}A^{-1}\,b-
%     \eta%1
% \\
% \label{eq:KKT_2__manip1}
% \therefore \,
%     \lambda 
% = & 
%     \frac{
%         B^{\top}A^{-1}\,b-
%         \eta%1
%     }{
%         B^{\top}A^{-1}B
%     }
% .
% \end{align}
% Plugging the value for $\lambda$, just obtained in Equation \eqref{eq:KKT_2__manip1}, back into Equation \eqref{eq:KKT_1__manip1} yields the optimizer $w^{\star}\in \mathbb{R}^N$ to Equation \eqref{eq:server__QPLC}
% \allowdisplaybreaks
% \begin{align}
% \nonumber
% w^{\star}   & = A^{-1}\,\big(b - B\lambda\big)
% \\
% \nonumber
% & = 
%  A^{-1}\,b -  \lambda\, A^{-1}B
% \\
% \nonumber
% & = 
%  A^{-1}\,b -  
%  \biggl(
%     \frac{
%         B^{\top}A^{-1}\,b-
%         \eta%1
%     }{
%         B^{\top}A^{-1}B
%     }
%  \biggr)
%  \, A^{-1}B
% \\
% \label{eq:KKT_1__manip2}
% \therefore \,
% w^{\star} & = 
%  A^{-1}\,
%  \Biggl(
%      b -  
%      \biggl(
%         \frac{
%             B^{\top}A^{-1}\,b-
%             \eta%1
%         }{
%             B^{\top}A^{-1}B
%         }
%      \biggr)B
%  \Biggr)
% .
% \end{align}
% Plugging in our definitions for $A$, $b$, and $B$ back into Equation \eqref{eq:KKT_1__manip2} yields the conclusion.
% \end{proof}


% \subsection{{Proof of Theorem \ref{thm:NashEqmExistence}}}
% \label{s:Proofs__ss:thm:NashEqmExistence}
% \begin{proof} 
% We employ dynamic programming to establish the result via backward induction~\cite[Corollary 6.1]{BO1998}.  
% Let $V_i(t,\hat{\mathbf{y}})$, $i=1,\dots,N$ be the value functions of the $N$ agents at time $t$ associated with \eqref{eq:ENCODER}, 
% \eqref{eq:DECODER_RESIDUALS}, and \eqref{eq:Objective_nth_expert}. 
% %\begin{align}  
% % & V_i(t, \hat{\mathbf{y}}) 
% %=  \sup_{\beta^i} \mathbb{E} \Big\{  
% % \Big\| y^i_t - \sum_{i=1}^N w^i 
% % \hat{y}^i \Big\|^2 
% %  + \| \beta^i \|^2    
% %+ V_i(t+1, \hat{\mathbf{y}} + 
% % \sum_{j=1}^N  e_j Z^{j\top}_t\beta^j) 
% %  \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
% %   & V_i(T, \hat{\mathbf{y}}) 
% %   = \notag 
% %\end{align} 
% From \eqref{eq:Objective_nth_expert}, the value functions at time $t=T$ with $\hat{Y}_T=\hat{\mathbf{y}}$ satisfy 
% $V_i(T, \hat{\mathbf{y}}) = 0$ and thus take the form 
% \begin{align} 
%  V_i(T, \hat{\mathbf{y}}) = \hat{\mathbf{y}}^\top  P_i(T) \hat{\mathbf{y}}  
%   + 2 S_i(T)^\top \hat{\mathbf{y}} + r_i(T) , \quad i = 1, \dots, N , 
% \end{align} 
% with $P_i(T)=0$ and $S_i(T)=0$ determined by \eqref{eqn:Pi} and \eqref{eqn:Si}. 

% \begin{comment} 
% By the dynamic programming principle, the value functions at $T-1$ with $\hat{Y}_{T-1}= \hat{\mathbf{y}}=[\hat{y}^{1\top}, \dots, \hat{y}^{N\top}]^\top$ satisfy  
% \begin{align} 
% V_i(T-1, \hat{\mathbf{y}}) 
% = & \min_{\beta^i} \mathbb{E} \Big\{   \Big\| y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2     
%   \notag \\ 
%  & \hspace{5cm} +  V_i(T, \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_{T-1} \beta^j ) 
%    \Big| \hat{Y}_{T-1} = \mathbf{\hat{y}}  \Big\} \notag \\ 
% = & \min_{\beta^i} \mathbb{E} \Big\{  \Big\| y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2    \Big\} , 
%    \label{DPeqnVi(T-1)}
% \end{align} 
% where the condition $\hat{Y}_{T-1}=\hat{\mathbf{y}}$ is removed from the expectation because $Z^j_{T-1}$, $j=1, \dots, N$ are independent of $\hat{Y}_{T-1}$. 
% Since the objective \eqref{DPeqnVi(T-1)} to be minimized is strictly convex in $\boldsymbol{\beta}=[\beta^{1 \top}, \dots, \beta^{N \top} ]^\top$, the first-order necessary conditions for minimization are also sufficient 
% and therefore we have the unique set of equations 
% %By the first order condition for the right side of \eqref{DPeqnVi(T-1)}, the equilibrium strategy 
% %$\boldsymbol{\beta}=[\beta^{1 \top}, \dots, \beta^{N \top} ]^\top$ satisfies  
% \begin{align} 
%  & \mathbb{E} \Big\{  \gamma_i \beta^i + Z^{j\top}_{T-1} \mathbf{e}_j^\top \mathbf{w}_{T-1} 
%   \Big[ y_{T} - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}}  
%    - \mathbf{w}_{T-1}^\top \sum_{j=1}^N \mathbf{e}_j Z^j_{T-1} \beta^j    \Big] 
%   \Big\}   = 0,  
%  \quad i = 1, \dots, N ,  \notag 
% \end{align} 
% which can be written in the compact form 
% \begin{align} 
%  & \big( \Gamma + \widehat{\mathbf{A}}(T-1) +  \mathbf{A}(T-1) \big) \boldsymbol{\beta}_{T-1}  
% =    \big[  \mathbf{D}(T-1)^\top \mathbf{w}_{T-1} (y_T - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}} ) - \mathbf{B}(T-1) \hat{\mathbf{y}} - \mathbf{C}(T-1) \big]     .  
% \notag 
% \end{align} 
% Since \eqref{eqn:Pi} admits a solution by the hypothesis of the Theorem, it follows from the definitions of $\Gamma$, $\mathbf{A}(\cdot)$ and $\widehat{\mathbf{A}}(\cdot)$ in Table \ref{tab:matricesEqnPiSi} that 
% $\Gamma + \widehat{\mathbf{A}}(T-1) +  \mathbf{A}(T-1)$ is positive definite. 
% Consequently, the equilibrium $\boldsymbol{\beta}_{T-1}=[\beta_{T-1}^{1 \top}, \dots, \beta_{T-1}^{N \top} ]^\top$ at time $T-1$ is given by  
% \begin{align} 
%   \boldsymbol{\beta}_{T-1} 
%   = & - \big(  \Gamma  + \widehat{\mathbf{A}}(T-1) + \mathbf{A}(T-1) \big)^{-1} \cdot   \notag \\ 
%   & \big[  \mathbf{D}(T-1)^\top \mathbf{w}_{T-1} (y_T - \mathbf{w}_{T-1}^\top \hat{\mathbf{y}} ) - \mathbf{B}(T-1) \hat{\mathbf{y}} - \mathbf{C}(T-1) \big]   . 
% \label{eqmbetaT-1}
% \end{align} 
% By substituting \eqref{eqmbetaT-1} into \eqref{DPeqnVi(T-1)} and by requiring it to be satisfied for all possible $\hat{\mathbf{y}}$, we arrive at \eqref{eqn:Pi} and \eqref{eqn:Si} for $t=T-1$. 
% Further substitution of this solution into \eqref{DPeqnVi(T-1)} leads to
% \begin{align} 
%   V_i(T-1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(T-1) \hat{\mathbf{y}}  
%   + 2 S_i(T-1)^\top \hat{\mathbf{y}} + r_i(T-1) , \quad i = 1, \dots, N ; \notag  
%  \end{align} 
% that is, $V_i(T-1, \hat{\mathbf{y}})$ take the affine-quadratic form at $t=T-1$. 
% \end{comment} 

% Assume by induction that for some $t\in \{ 1, \dots, T-1\}$ and for all $s\in\{t +1, \dots , T\}$, 
% %the equilibrium strategy for the $N$ agents take the form $\boldsymbol{\beta}_{t+1} = \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t)$, 
% the value functions $\{V_i(s, \hat{\mathbf{y}})\}_{i=1}^N$ at time $s$ with $\hat{Y}_s = \hat{\mathbf{y}}$ take the affine-quadratic form 
% \begin{align} 
%   V_i(s, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(s) \hat{\mathbf{y}}  
%   + 2 S_i(s)^\top \hat{\mathbf{y}} + r_i(s) , \quad i = 1, \dots, N , \notag  
%  \end{align} 
% with $P_i(s)$ and $S_i(s)$ determined by \eqref{eqn:Pi} and \eqref{eqn:Si} on the time span $s\in \{t+1, \dots, T\}$. 
% We show that at time $t$ with $\hat{Y}_t=\hat{\mathbf{y}}$, the equilibrium strategy is given by $\boldsymbol{\beta}_t=[\beta^{1\top}_t, ..., \beta^{N\top}_t ]^\top=\mathbf{G}(t)\hat{\mathbf{y}} + \mathbf{H}(t)$, 
% and the value functions $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ take the affine-quadratic form 
% \begin{align} 
%   V_i(t, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) , \quad i = 1, \dots, N , 
%   \label{vi(t,y)ansatz}
%  \end{align} 
% with $P_i(t)$ and $S_i(t)$ determined by \eqref{eqn:Pi} and \eqref{eqn:Si}, respectively. 
% % \eqref{eqmvecbeta}. 

 
% By the dynamic programming principle and the induction hypothesis, 
% $\{V_i(t, \hat{\mathbf{y}})\}_{i=1}^N$ satisfy the system of dynamic programming equations:  
% \allowdisplaybreaks
% \begin{align} 
% V_i(t, \hat{\mathbf{y}}) 
% = & \min_{\beta^i} \mathbb{E} \Big\{  e^{-\alpha_i (T-1-t)} 
%  \Big[ \Big\| y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2   \Big]   \notag \\ 
%   & \hspace{5.5cm} 
%   +   V_i(t+1, \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_t \beta^j ) 
%    \Big| \hat{Y}_t = \mathbf{\hat{y}}  \Big\} \notag \\ 
%   = & \min_{\beta^i} \mathbb{E} 
%   \Big\{   e^{-\alpha_i (T-1-t)} 
%  \Big[ \Big\| y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)  \Big\|^2 
%   + \gamma_i \| \beta^i \|^2   \Big]    \notag \\ 
%  & \hspace{2cm}  +   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big]^\top P_i(t+1) 
%   \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big] \notag \\ 
%  &   \hspace{3.5cm}  + 2    S_i(t+1)^\top \Big[ \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t  \beta^j  \Big] 
%   +   r_i(t+1)      \Big\} , \quad 
%    i = 1, \dots, N , 
%   \label{DPeqnVi(t)}  
% \end{align} 
% where the condition $\hat{Y}_{t}=\hat{\mathbf{y}}$ is removed from the expectation because $\{Z^j_{t}\}_{j=1}^N$ are independent of $\hat{Y}_{t}$. 
% Since the objective \eqref{DPeqnVi(t)} to be minimized is strictly convex in $\boldsymbol{\beta}=[\beta^{1 \top}, \dots, \beta^{N \top} ]^\top$, the first-order necessary conditions for minimization are also sufficient 
% and therefore we have the unique set of equations 
% %The first order condition for the right side of \eqref{DPeqnVi(t)} is given by  
% \begin{align} 
% & \mathbb{E} \Big\{   - e^{-\alpha_i (T-1-t)} Z^{i\top}_t \mathbf{e}_i^\top \mathbf{w}_t 
%  \Big[ y_{t+1} - \mathbf{w}_t^\top \big( \hat{\mathbf{y}} + \sum_{j=1}^N \mathbf{e}_j Z^j_t \beta^j \big)   \Big] 
%  + e^{-\alpha_i (T-1-t)} \gamma_i \beta^i    \notag \\  
% &  \hspace{3cm} +  Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \Big( \hat{\mathbf{y}} + \sum_{j=1}^N  \mathbf{e}_j Z^j_t \beta^j \Big) 
%   + Z^{i\top}_t \mathbf{e}_i^\top S_i(t+1) \Big\}  =0 , 
%   \quad i = 1, \dots, N , \notag 
% % \label{betaifirstorderV(y)} 
% \end{align} 
% which can be written in the compact form  
% \begin{align} 
%  &  \big[ e^{-\boldsymbol{\alpha}(T -1 - t)}  \boldsymbol{\Gamma}  
%   + e^{-\boldsymbol{\alpha}(T -1 - t)} \widehat{\mathbf{A}}(t) 
%    + \mathbf{A}(t) \big] \boldsymbol{\beta}_t  \nonumber \\ 
%    & \hspace{10ex}+ \mathbf{B} (t) \hat{\mathbf{y}} + \mathbf{C}(t) 
%   - e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top  \hat{\mathbf{y}} ) 
%  = 0. 
% \end{align} 
% Since \eqref{eqn:Pi} admits a solution on $\{t+1, \dots, T\}$ by the hypothesis of the theorem, it follows from the definitions of $\boldsymbol{\Gamma}$, $\mathbf{A}(\cdot)$ and $\widehat{\mathbf{A}}(\cdot)$ in Table \ref{tab:matricesEqnPiSi} that 
% $ e^{-\boldsymbol{\alpha} (T-1-t) } \boldsymbol{\Gamma} 
%   + e^{-\boldsymbol{\alpha}(T -1 - t)} \widehat{\mathbf{A}}(t)  + \mathbf{A}(t)$ is positive definite. 
% Consequently, the equilibrium strategy $\boldsymbol{\beta}_t=[\beta^{1 \top}_t, \dots, \beta^{N \top}_t ]^\top$ at time $t$ is then given by 
% \begin{align} 
%  \boldsymbol{\beta}_t = &  \big[ e^{-\boldsymbol{\alpha} (T-1-t) } \Gamma 
%   + e^{-\boldsymbol{\alpha}(T -1 - t)} \widehat{\mathbf{A}}(t)  + \mathbf{A}(t) \big]^{-1} \cdot \notag \\  
% & \qquad \big[  e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t (y_{t+1} - \mathbf{w}_t^\top  \hat{\mathbf{y}} ) 
% - \mathbf{B}(t) \hat{\mathbf{y}} - \mathbf{C}(t) 
%   \big]  \notag \\ 
% = & \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t).   
% \label{eqmbetat}   
% \end{align} 
% By substituting \eqref{eqmbetat} into \eqref{DPeqnVi(t)}, we obtain that $\{ V_i(t, \hat{\mathbf{y}}) \}_{i=1}^N$ take the affine-quadratic form \eqref{vi(t,y)ansatz}; that is, for $i=1,\dots,N$:
% %Substituting \eqref{eqmbetat} into \eqref{DPeqnVi(t)}, we obtain 
% \begin{align} 
%  & \hat{\mathbf{y}}^\top  P_i(t) \hat{\mathbf{y}}  
%   + 2 S_i(t)^\top \hat{\mathbf{y}} + r_i(t) \notag \\ 
%   \qquad&= \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big]^\top  
%  \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \widehat{\mathbf{e}}_i \widehat{\mathbf{e}}_i^\top \big]  \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big]  
%  \notag \\ 
%  & \qquad+ 2 \big[  - e^{-\alpha_i(T-1-t)} (y_{t+1} - \mathbf{w}_t^\top \hat{\mathbf{y}} )^\top \mathbf{w}_t^\top  
%   + \hat{\mathbf{y}}^\top P_i(t+1)  + S_i^\top(t+1)  \big] 
%   \mathbf{D}(t) 
%    \big[ \mathbf{G}(t) \hat{\mathbf{y}} + \mathbf{H}(t) \big] 
%  \notag \\ 
%  & \qquad+ e^{-\alpha_i(T-1-t)} \big\| y_{t+1} - \mathbf{w}_t^\top \hat{\mathbf{y}} \big\|^2 + \hat{\mathbf{y}}^\top P_i(t+1) \hat{\mathbf{y}} 
%  + 2 S_i^\top(t+1) \hat{\mathbf{y}} + r_i(t+1) . 
%  \notag 
% \end{align} 
% Since the above equations hold for all possible $\hat{\mathbf{y}}$, 
% by matching the coefficients of the quadratic and linear terms of $\hat{\mathbf{y}}$, we obtain $P_i(t)$ and $S_i(t)$ as determined by \eqref{eqn:Pi} and \eqref{eqn:Si}. 
% By induction, we have shown that the equilibrium strategy takes the form \eqref{eqmvecbeta} with the matrix-valued coefficients determined by \eqref{eqn:Pi} and \eqref{eqn:Si}.  
% %By matching the coefficients of quadratic terms of $\hat{\mathbf{y}}$, we obtain \eqref{eqn:Pi} for $P_i(t)$;   
% %by matching the coefficients of the linear terms of $\hat{\mathbf{y}}$, we obtain \eqref{eqn:Si} for $S_i(t)$. 
% %\begin{align} 
% %  V_i(T-1, \hat{\mathbf{y}} ) =  \hat{\mathbf{y}}^\top  P_i(T-1) \hat{\mathbf{y}}  
% %  + 2 S_i(T-1)^\top \hat{\mathbf{y}} + r_i(T-1) , \quad i = 1, \dots, N ; \notag  
% % \end{align} 
% %that is, $V_i(T-1, \hat{\mathbf{y}})$ take the affine-quadratic form at $t=T-1$. 
% %and by requiring it to be satisfied for all possible $\hat{\mathbf{y}}$, and by requiring it to be satisfied for all possible $\hat{\mathbf{y}}$, 
% %we arrive at \eqref{eqn:Pi} and \eqref{eqn:Si} for $t=T-1$. Further substitution of this solution into \eqref{DPeqnVi(T-1)} leads to
% \end{proof} 

% \subsection{Proofs of Corollaries} 
% \label{s:ProofCorollaries}

% \textbf{Corollary \ref{cor:Random_NeuralNetwork}}

% \begin{proof}
% %Set $a^i_t\eqdef A^{(i)}x_t+b^{(i)}$.  By Theorem \ref{thm:OptimalWeights}, for $i,j=1,\dots,N$ we have
% From Theorem \ref{thm:NashEqmExistence}, the sub-matrices of $\mathbf{A}(t)=\big[ A^{(i,j)}(t) \big]_{1\leq i,j \leq N}$ 
% are 
% \begin{align} 
% A^{(i,j)}(t) 
% =
%  & \mathbb{E} \big[ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big] 
%  \notag \\ 
%  = & 
%  \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j \mathbb{E} \big[ Z^{i\top}_t  Z^j_t \big] ,
%  \quad 1 \leq i, j \leq N .  
%   \notag 
% \end{align} 
% The diagonal sub-matrices 
% $A^{(i,i)}(t) = \big[ ( A^{(i, i)}(t) )_{jk} \big]_{1\leq j, k\leq d_z}$ are given by  
% \begin{align} 
%  ( A^{(i,i)}(t) )_{jk}  
%  = &
%   \mathbf{e}_i^\top  P_i(t+1) \mathbf{e}_i
%   \mathbb{E} \big[ (Z_{t+1}^{i\top} Z_{t+1}^i)_{jk} \big]  
%     \notag \\ 
% = &
%   \mathbf{e}_i^\top  P_i(t+1) \mathbf{e}_i
%   \mathbb{E} \big[ (Z_{t+1}^i)_j (Z_{t+1}^i)_k \big]  , 
%     \notag 
% \end{align} 
% where $\mathbb{E}\big[ (Z_{t+1}^i)_j (Z_{t+1}^i)_k \big]$ are given by \eqref{E[(Zij)b(Zik)]}. 

% Since the white noises $\{W^i_t\}_{i, t}$, are independent,  
% $\{ Z^i_t \}_{i, t}$ are independent. 
% The off-diagonal sub-matrices of $\mathbf{A}(t)$ are written as   
% \begin{align} 
% A^{(i,j)}(t) 
%  =&  \mathbb{E} \big[ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big]  \notag \\ 
%  = & \mathbb{E} \big[  Z^{i\top}_t \big]  \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j  \mathbb{E} \big[ Z^j_t \big] , 
% \notag  
% % = & a(t, i)^\top \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j a(t, j) , 
% \end{align} 
% where the explicit form of $\mathbb{E} \big[ Z^{i}_t \big]$ is given by \eqref{E[Zi]}. 
% The explicit forms of the matrices $\widehat{\mathbf{A}}(t)=\big[ \widehat{A}^{(i,j)}(t) \big]_{i,j =1}^N$ 
% and $\mathbf{D}_i(t) = \big[ D_i^{(j,k)}(t) \big]_{j,k = 1}^N$,  $i = 1, ..., N$ are determined in a similar manner. 
% The explicit forms of $\mathbf{B}(t)$, $\mathbf{C}(t)$ and $\mathbf{D}(t)$ are determined by \eqref{E[Zi]} and 
% $a(t, i) = \mathbb{E}[Z^i_{t+1}]$. 
% \end{proof}

% \begin{comment} 
% \begin{proof} [{Proof of Corollary \ref{cor:Random_NN}}]
% %Set $a^i_t\eqdef A^{(i)}x_t+b^{(i)}$.  By Theorem \ref{thm:OptimalWeights}, for $i,j=1,\dots,N$ we have
% From Proposition \ref{prop:NashEqmExistence}, the sub-matrices of $\mathbf{A}(t)=\big( A^{(i,j)}(t) \big)_{1\leq i,j \leq N}$ 
% are 
% \begin{align} 
% A^{(i,j)}(t) 
% =
%  & \mathbb{E} \big[ Z^i_t e_i^\top P_i(t+1) e_j Z^{j\top}_t \big]  
%  =  \mathbb{E} \big[ Z^i_t  ( P_i(t+1) )_{ij}  Z^{j\top}_t \big] \notag 
% \end{align} 
% By Lemma \ref{lem:Mean_Cov_ResModel}, the entries in the diagonal sub-matrices $A^{(i,i)}(t)$ of $\mathbf{A}(t)$ are given by  
% \begin{align} 
% ( A^{(i,i)}(t) )_{jk} = &
%   \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii}\,
%     \begin{cases}
%             ( (a_t)_j^2 + \sigma^i_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = a(t, i)_j a(t,i)_k 
%     & \mbox{ if }   j \neq k
%     \end{cases} 
%     \notag 
% \end{align} 


% Since the white noises $\{W^i_t\}_{i, t}$, are independent, \eqref{DTRCsystemReLU} implies that 
% $Z^i_t$ and $Z^j_t$ are independent for $i\neq j$. 
% The off-diagonal sub-matrices of $\mathbf{A}(t)$ can be written as   
% \begin{align} 
% A^{(i,j)}(t) 
%  %= & \mathbb{E} [ (e_i Z^{i\top}_t)^\top P_i(t+1) e_j Z^{j\top}_t ] \notag \\ 
%  %= & \mathbb{E} [  Z^i_t ]  e_i^\top P_i(t+1) e_j  \mathbb{E} [ Z^{j\top}_t ] \notag \\ 
%  = & \mathbb{E} [  Z^i_t ]  ( P_i(t+1) )_{ij}  \mathbb{E} [ Z^{j\top}_t ] 
% \notag \\ 
%  = & a(t, i) ( P_i(t+1) )_{ij} a(t, j)^\top
% \end{align} 
% where $\mathbb{E} [  Z^i_t ]$ and $\mathbb{E} [  Z^j_t ]$ where computed explicitly using Lemma \ref{lem:Mean_Cov_ResModel}. 
% \end{proof} 
% \end{comment} 


% The following lemma gives enough information to compute the relevant matrices in Theorem \ref{thm:NashEqmExistence}.
% \begin{lemma}[Mean and Covariance of $Z_{\cdot}^i$ in Corollary \ref{cor:Random_NeuralNetwork} for $d_y=1$]
% \label{lem:Mean_Cov_ResModel} 
% %In the setting of Corollary \ref{cor:Random_NeuralNetwork}, let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that 
% Under the conditions \\specified in Corollary \ref{cor:Random_NeuralNetwork}, %for a given $b \in \mathbb{R}$, 
% and for each $t \in \mathbb{N}$, $i = 1, \dots, N$, and $j, k = 1, \dots, d_z$, the following hold:
% \begin{align} 
% % \label{eq:mean_variance_computations}
% %\nonumber
%  &       \mathbb{E}[Z_{t+1}^i] 
%     = 
%         a^i_t 
%         \odot
%         \Big(
%             \bar{1}_{d_z} 
%             - 
%             \Phi\bullet \big(
%                 \frac{-a^i_t}{\sigma_t^i}%\cdot 
%             \big)
%         \Big)
%         +
%             \frac{\sigma_t^i}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-(a^i_t \odot a^i_t )}{2\, (\sigma_t^i)^2 }
%             % \,
%         \Big) , 
%         \label{E[Zi]}
% \\ 
% &
% \begin{aligned} 
%      \mathbb{E}\big[(Z_{t+1}^i)_j  (Z_{t+1}^i)_k\big] 
%     = 
%     \begin{cases}
%              ( (a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 )
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big) 
%             \\
%             \hspace{2cm}
%             +
%             (a^i_t)_j\,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big( 
%                 \frac{ - (a^i_t \odot a^i_t )_j }{2\,(\sigma_t^i)^2 }
%             \Big) ,   
%         \quad & \mbox{ if } j=k , 
% \\
%    \mathbb{E}\big[ (Z_{t+1}^i)_j \big] 
%     \mathbb{E} \big[ (Z_{t+1}^i)_k \big]  , 
% \quad & \mbox{ if } j\neq k, 
% \end{cases}
% \end{aligned} 
% \label{E[(Zij)b(Zik)]}
% \end{align} 
% where $\odot$ denotes the Hadamard product,\footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$.}
% %$\bar{1}_{d_z} \in \mathbb{R}^{d_z}$ denotes the row vector will all entries equal to $1$, 
% and $\Phi$ is the standard normal CDF.  
% %and $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of Corollary \ref{cor:Random_NeuralNetwork}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion. 
% \end{proof}

% The multi-dimensional version of Corollary \ref{cor:Random_NeuralNetwork} is proven here.  Overall it is of a similar form with some additional technicalities.
% \begin{corollary}[Random Feature Network with $d_y>1$] 
% \label{cor:Random_NN_dy>1}
% In the setting of Corollary \ref{cor:Random_NeuralNetwork} with $d_y>1$, we have the block matrices
% \begin{align*}
% & \mathbf{A}(t)
%  = 
% \big[ A^{(i,j)}(t) \big]_{i,j=1}^N , 
% \hspace{0.5cm} 
% \widehat{\mathbf{A}}(t) = \big[ \widehat{A}^{(i,j)}(t) \big]_{i, j = 1}^N , 
% \notag \\  
%  & \mathbf{B}(t)  = 
%  \begin{bmatrix} 
%   P_1(t+1) \mathbf{e}_1 a(t, 1), \dots, P_N(t+1) \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top  ,  
%  \notag \\ 
%  & \mathbf{C}(t)  = 
%  \begin{bmatrix} 
%   S_1(t+1)^\top \mathbf{e}_1 a(t, 1), \dots, S_N(t+1)^\top  \mathbf{e}_N a(t, N) \\ 
%  \end{bmatrix}^\top , 
%   \notag \\   
% & \mathbf{D}(t) 
%   = 
%  \begin{bmatrix} 
%  \mathbf{e}_1 a(t,1), \dots  , \mathbf{e}_N a(t, N) 
%  \end{bmatrix} , 
%  \quad 
%   \mathbf{D}_i(t) = [ D_i^{(j,k)}(t) ]_{j,k = 1}^N , \quad i = 1, \dots, N . \notag 
% % \big( D_i^{(j,k)} \big)_{j,k=1}^N , \quad i = 1, ..., N. \notag 
% \end{align*}
% For $t=1,\dots,N$ and $t\in \mathbb{N}_+$, each $a(t,i)$ is defined as follows
% \begin{align} 
% & a^i_t\eqdef A^{i} [x_t,\dots, x_t ] + b^{i} = \big[ (a^i_t)_1^\top , \dots, (a^i_t)_{d_y}^\top \big]^\top \in \mathbb{R}^{d_y \times d_z} , \notag \\ 
% & a(t,i)
% \eqdef 
%    \big[ a(t, i)_1^\top , \dots, a(t, i)_{d_y}^\top \big]^\top
%    \in \mathbb{R}^{d_y \times d_z} 
%    , \notag \\ 
% & a(t, i)_k = (a^i_t)_k 
%         \odot
%         \left(
%             \bar{1}_{d_z} 
%             - 
%             \Phi\bullet \left(
%                 \frac{- (a^i_t)_k}{(\sigma_t^i)_k}%\cdot 
%             \right)
%         \right)
%     \notag \\     
%     & \hspace{4cm}+
%             \frac{(\sigma_t^i)_k}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\left(
%             \frac{-( (a^i_t)_k \odot (a^i_t)_k )}{2\, ( (\sigma_t^i)_k )^2 }
%             % \,
%         \right)  , \quad 
%         k = 1, \dots, d_y , 
%         \label{a(t,i)k}
% \end{align} 
% and $\odot$ and $\Phi$ are defined in Lemma \ref{lem:Mean_Cov_ResModel}. 
% The sub-matrices of $\mathbf{A}(t)$, $\widehat{\mathbf{A}}(t)$, 
% and $\{ \mathbf{D}_i(t) \}_{i=1}^N$,   
% are given by 
% %of $\mathbf{A}(t)$, $\widehat{\mathbf{A}}(t)$, 
% %and $\{ \mathbf{D}_i(t) \}_{i=1}^N$, are given by 
% %respectively, in the setting of Corollary \ref{cor:Random_NeuralNetwork}, 
% \begin{align} 
%  & A^{(i,j)}(t) =
% \begin{cases} 
% \sum_{k, l = 1 }^{d_y} 
% ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl}
% \mathbb{E} \big[  (Z^i_t)_k^\top  (Z^i_t)_l \big] , \quad & \mbox{if} \,\, i = j , \\
%   a(t, i)^\top \mathbf{e}_i^\top  P_i(t+1) \mathbf{e}_j a(t, j) , \quad & \mbox{if} \,\, i \neq j  , 
%  \end{cases} 
%  \notag \\ 
%  & \widehat{A}^{(i,j)}(t) = 
%  \begin{cases} 
%  \sum_{k, l = 1 }^{d_y} w^i_t w^i_t \mathbb{E} \big[  (Z^i_t)_k^\top 
%    (Z^i_t)_l \big]    , \quad & \mbox{if} \,\, 
%   i = j , \\ 
%  a(t, i)^\top  w^i_t w^j_t a(t, j) , \quad & \mbox{if} \,\, i \neq j   , 
% \end{cases} 
% \notag \\ 
% %\end{align} 
% %\begin{align} 
% & D_i^{(r,s)}(t) = 
% \begin{cases}
%  \sum_{k,l = 1}^{d_y} ( \mathbf{e}_r^\top P_i(t+1) \mathbf{e}_r )_{kl} 
%  \mathbb{E} \big[ (Z^r_t)_k^\top 
%   (Z^r_t)_l \big]  , \quad & \mbox{if} \,\, r=s , \\ 
% a(t,r)^\top \mathbf{e}_r^\top P_i(t+1) \mathbf{e}_s a(t, s) , \quad & \mbox{if} 
% \,\, r \neq s .  
% \notag 
% \end{cases}
% \end{align} 
% The matrices 
% $\mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_l \big]
% = \big( \mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_l \big]_{pq} \big)_{p,q=1}^{d_z}$ for  
% $k$, $l=1, \dots, d_y$ are given as follows: 
% if $k$ and $l$ are distinct then
% \begin{align} 
% % & k\neq l : \,
%   \mathbb{E} \big[  (Z^i_t)_k^\top  (Z^i_t)_l \big]_{pq}   
% % = &  \mathbb{E} \Big[  (Z^i_t)_{kp}  (Z^i_t)_{lq} \Big] 
% % \notag \\ 
% % = & 
% % \mathbb{E} \big[  (Z^i_t)_{kp} \big]  
% %  \mathbb{E} \big[ (Z^i_t)_{lq} \big]  
% % \notag \\ 
%  =  
%  a(t, i)_{kp}  
%   a(t, i)_{lq} ;   
% \end{align} 
% otherwise $\mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_k \big]_{pq} 
%  = \mathbb{E} \big[ (Z^i_t)_{kp} (Z^i_t)_{kq} \big]$ and 
% \begin{align} 
% % % & k = l : \, 
% %  \mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_k \big]_{pq} 
%  % = 
%  \mathbb{E} \big[ (Z^i_t)_{kp} (Z^i_t)_{kq} \big] 
% %  \notag 
% %   \\ 
% % & \hspace{1cm} 
% = 
% \begin{cases}
%             \big[ ( (a^i_t)_k \odot (a^i_t)_k )_p + (\sigma^i_t)_k^2 \big]  
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_{kp}}{ (\sigma_t^i)_k }
%                 )
%             \Big) 
%              \\
%             \hspace{2cm}
%             +
%             (a^i_t)_{kp}   \,
%                 \frac{ (\sigma_t^i)_k }{\sqrt{2\pi}}
%             \,
%             \exp\Big(
%                 \frac{ - ( (a^i_t)_k \odot (a^i_t)_k )_p}{2\, (\sigma_t^i)_k^2 }
%             \Big) , 
%             \quad 
%         & \mbox{ if } p = q , 
% \\
%     \mathbb{E}[(Z_{t+1}^i)_{kp}]
%     \mathbb{E}[(Z_{t+1}^i)_{kq}] 
%      = a(t, i)_{kp} a(t,i)_{kq} ,  
%     \quad 
%      & \mbox{ if }   p \neq q . 
%     \end{cases}   
%  \label{E[(Zi)kp(Zi)kq]} 
% \end{align} 

% \end{corollary} 



% \begin{proof}%[{Proof of Corollary \ref{cor:Random_NN_dy>1}}] 
% If $d_y>1$, we have for each $i=1, \dots, N$ that   
% \begin{align} 
%  Z^i_t = \operatorname{ReLU}  \bullet \big( A^i [x_t, \dots, x_t] + b^i + \sigma^i_t W^i_t \big)  
%  = \big[ (Z^{i}_t)_1^\top , \dots , (Z^{i}_t)_{d_y}^\top \big]^\top 
%  \in \mathbb{R}^{d_y \times d_z} 
%  \label{Zi=[Zi1T,...,ZidyT]T}
% \end{align} 
% with $(Z^{i}_t)_k = (a^i_t)_k + (\sigma^i_t)_k W^i_t$, $k=1,\dots, d_y$. 
% %\begin{align} 
% % a^i_t = A^i x_t + b^i = \big[ (a^i_t)_1^\top , \cdots, (a^i_t)_{d_y}^\top \big]^\top \in \mathbb{R}^{d_y \times d_z} , \quad 
% % \sigma^i_t = \big[ (\sigma^i_t)_1 , \cdots , (\sigma^i_t)_{d_y} \big]^\top \in \mathbb{R}^{d_y \times 1} , \notag 
% %\end{align} 

% Denote
% \begin{align}  
% & \mathbb{E} \big[ Z^{i}_{t} \big] =  a(t, i)  
%   =  \big[ a(t, i)_1^\top , \cdots, a(t, i)_{d_y}^\top \big]^\top \in \mathbb{R}^{d_y \times d_z} . 
%   \notag 
% \end{align} 
% By \eqref{E[Zi]}, we obtain \eqref{a(t,i)k} for each $\mathbb{E} \big[ (Z^i_{t})_k \big] = a(t, i)_k$. 


% For $i\neq j$, $Z^i_t$ and $Z^j_t$ are independent since the random noises $W^i_t$ and $W^j_t$ are independent, 
% then $A^{(i,j)}(t)$ can be represented as 
% \begin{align} 
%   A^{(i,j)}(t) = &
%  \mathbb{E} [ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t ] \notag \\ 
%  =& \mathbb{E} [ Z^{i\top}_t ] \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j \mathbb{E} [ Z^j_t ] \notag \\ 
%  =& a(t, i)^\top \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j a(t,j) . 
%  \notag 
% \end{align} 

% For $i=j$, by \eqref{Zi=[Zi1T,...,ZidyT]T} the diagonal sub-matrices $A^{(i,i)}(t)$ can be writen as  
% \begin{align} 
%  A^{(i,i)}(t) = &
%  \mathbb{E} \big[ Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i Z^i_t \big]    \notag  \\ 
% % = & \sum_{k, l = 1 }^{d_y} \mathbb{E} \big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \big]  
% % \notag \\ 
%   = & \sum_{k, l = 1 }^{d_y} 
%   ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} 
%   \mathbb{E} \big[  (Z^i_t)_k^\top  (Z^i_t)_l \big] . 
%  \notag 
% \end{align} 


% \begin{comment} 
% By \eqref{E[(Zi)jb(Zi)k]}, we have 
% \begin{align} 
% & ( A^{(i,i)}(t) )_{jk} \notag \\ 
% = &
%   \mathbb{E}[(Z_{t+1}^i)_j ( P_i(t+1) )_{ii} (Z_{t+1}^i)_k] \notag \\ 
%     = &
%         ( P_i(t+1) )_{ii} \cdot \,
%     \begin{cases}
%             ( ( a^i_t \odot a^i_t )_j + (\sigma^i_t)^2 ) 
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j   \,
%                 \frac{\sigma_t^i}{\sqrt{2\pi}}
%             \,
%             \exp\Big(
%                 \frac{-(a^i_t \odot a^i_t )_j}{2\, (\sigma_t^i)^2 }
%             \Big) , 
%             \notag \\ 
%     \hspace{9.5cm} 
%         \mbox{ if } j=k , 
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k] 
%      = a(t, i)_j a(t,i)_k ,  
%     \hspace{3.2cm}
%      \mbox{ if }   j \neq k . 
%     \end{cases} 
%     \notag 
% \end{align} 
% \end{comment}

% For $k=l$, since $(Z^{i}_t)_k = (a^i_t)_k + (\sigma^i_t)_k W^i_t$ is a $d_z$-dimensional row vector, 
% we can use \eqref{E[(Zij)b(Zik)]} to determine \eqref{E[(Zi)kp(Zi)kq]} for the matrix 
% $\mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_l \big]
% = \big( \mathbb{E} \big[ (Z^i_t)_k^\top (Z^i_t)_l \big]_{pq} \big)_{p,q=1}^{d_z}$.  
% \begin{comment} 
% \begin{align} 
%   \mathbb{E} \big[  (Z^i_t)_k^\top (Z^i_t)_k \big]_{pq} 
%  = & 
%  \mathbb{E} \big[  (Z^i_t)_{kp} (Z^i_t)_{kq} \big]
%  \notag \\ 
%  = & 
% % ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kk} \cdot \,
%     \begin{cases}
%             \big[ ( (a^i_t)_k \odot (a^i_t)_k )_p + (\sigma^i_t)_k^2 \big]  
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_{kp}}{ (\sigma_t^i)_k }
%                 )
%             \Big) 
%             \notag \\
%             \hspace{3.4cm}
%             +
%             (a^i_t)_{kp}   \,
%                 \frac{ (\sigma_t^i)_k }{\sqrt{2\pi}}
%             \,
%             \exp\Big(
%                 \frac{ - ( (a^i_t)_k \odot (a^i_t)_k )_p}{2\, (\sigma_t^i)_k^2 }
%             \Big) , 
%             \quad 
%         & \mbox{ if } p = q , 
% \\
%     \mathbb{E}[(Z_{t+1}^i)_{kp}]
%     \mathbb{E}[(Z_{t+1}^i)_{kq}] 
%      = a(t, i)_{kp} a(t,i)_{kq} ,  
%      \quad
%      & \mbox{ if }   p \neq q . 
%     \end{cases} 
%  \notag 
% \end{align} 
% \end{comment} 

% For $k\neq l$, we use the fact that $W^i_t$ is a vector of independent random variables to determine the matrix 
% $\mathbb{E} \big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \big]$ such that
% \begin{align} 
%   \mathbb{E} \big[  (Z^i_t)_k^\top ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_l \big]_{pq}   
%  = & 
%  \mathbb{E} \big[  (Z^i_t)_{kp} ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} (Z^i_t)_{lq} \big] 
%  \notag \\ 
%  = & 
%  \mathbb{E} \big[  (Z^i_t)_{kp} \big] ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} 
%   \mathbb{E} \big[ (Z^i_t)_{lq} \big]  
%  \notag \\ 
%  = & 
%  a(t, i)_{kp} ( \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_i )_{kl} 
%   a(t, i)_{lq}  . 
%   \notag 
% \end{align} 
% The explicit forms of the matrices $\widehat{\mathbf{A}}(t)=\big[ \widehat{A}^{(i,j)}(t) \big]_{i,j =1}^N$ 
% and $\mathbf{D}_i(t) = \big[ D_i^{(j,k)}(t) \big]_{j,k = 1}^N$,  $i = 1, \dots, N$ are determined in a similar manner. 
% The explicit forms of $\mathbf{B}(t)$, $\mathbf{C}(t)$ and $\mathbf{D}(t)$ are determined by \eqref{E[Zi]} and 
% $a(t, i) = \mathbb{E}[Z^i_{t+1}]$. 
% %For each $k=1$, ..., $d_y$, $(Z^{i}_t)_k = (a^i_t)_k + (\sigma^i_t)_k W^i_t$ is a $d_z$-dimensional row vector, and 
% %we can apply Lemma \ref{lem:Mean_Cov_ResModel}, \eqref{E[Zi]} and \eqref{E[(Zij)b(Zik)]}  to obtain $\mathbb{E}[ (Z^i_{t+1})_k ]$ 
% %and $\mathbb{E}[(Z_{t+1}^i)_{kp} (Z_{t+1}^i)_{kq}]$, respectively. 
% \end{proof} 


% \begin{comment} 
% \begin{lemma}[Mean and Covariance of $Z_{\cdot}^i$ in Corollary \ref{cor:Random_NeuralNetwork} for $d_y>1$]
% \label{lem:Mean_Cov_ResModel(dy>1)}
% Consider the setting of Corollary \ref{cor:Random_NeuralNetwork}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{align} 
% % \label{eq:mean_variance_computations}
% %\nonumber
% %\begin{aligned}
% &        \mathbb{E}[ (Z_{t+1}^i)_k ] 
%     = 
%         (a^i_t)_k 
%         \odot
%         \Big(
%             \bar{1}_{d_z} 
%             - 
%             \Phi\bullet \big(
%                 \frac{-(a^i_t)_k}{(\sigma_t^i)_k}%\cdot 
%             \big)
%         \Big)
%         +
%             \frac{(\sigma_t^i)_k}{\sqrt{2\pi}}
%         \,
%         \exp\bullet\Big(
%             \frac{-( (a^i_t)_k \odot (a^i_t)_k )}{2\, (\sigma_t^i)_k^2 }
%             % \,
%         \Big) , 
%        % \quad k = 1, ..., d_y 
% \label{E[(Zi)k]}
% \\
% &
% \begin{aligned} 
% &        \mathbb{E}[(Z_{t+1}^i)_{kp}  (Z_{t+1}^i)_{kq}] 
%     = 
%     \begin{cases}
%             \big[ ( (a^i_t)_k \odot (a^i_t)_k )_p + (\sigma^i_t)_k^2 \big]  
%             \cdot
%             \Big(
%                 1 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_{kp}}{ (\sigma_t^i)_k }
%                 )
%             \Big) 
%              \\
%             \hspace{3.4cm}
%             +
%             (a^i_t)_{kp}   \,
%                 \frac{ (\sigma_t^i)_k }{\sqrt{2\pi}}
%             \,
%             \exp\Big(
%                 \frac{ - ( (a^i_t)_k \odot (a^i_t)_k )_p}{2\, (\sigma_t^i)_k^2 }
%             \Big) , 
%             \quad 
%         & \mbox{ if } p = q , 
% \\
%     \mathbb{E}[(Z_{t+1}^i)_{kp}]
%     \mathbb{E}[(Z_{t+1}^i)_{kq}] 
%      = a(t, i)_{kp} a(t,i)_{kq} ,  
%      \quad
%      & \mbox{ if }   p \neq q . 
%     \end{cases} 
% \label{E[(Zi)kp(Zi)kq]} 
% \end{aligned}
% \end{align}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,}~%
% %$\bar{1}_{d_z} \in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, 
% and $\Phi$ is the standard normal CDF.  
% %$a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma} 

% \begin{proof} 
% For each $k=1$, ..., $d_y$, $(Z^{i}_t)_k = (a^i_t)_k + (\sigma^i_t)_k W^i_t$ is a $d_z$-dimensional row vector, and 
% we can apply Lemma \ref{lem:Mean_Cov_ResModel} to obtain $\mathbb{E}[ (Z^i_{t+1})_k ]$ 
% and $\mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k]$. 
% \end{proof} 
% \end{comment} 



% %\newpage




% \begin{comment} 
% \begin{lemma}[{Mean and Covariance of $Z_{\cdot}^i$ in the Example \ref{ex:Random_NeuralNetwork}}]
% \label{lem:Mean_Cov_ResModel}
% Consider the setting of Example \ref{ex:Random_NeuralNetwork}, and let $b\in \mathbb{R}$.  For each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j,k=1,\dots,d_z$, we have that
% \begin{equation}
% % \label{eq:mean_variance_computations}
% \nonumber
% \begin{aligned}
%         \mathbb{E}[Z_{t+1}^i] 
%     = &
%         a^i_t 
%         \odot
%         \Big(
%             \bar{1} 
%             - 
%             \Phi\bullet(
%                 \frac{-1}{\sigma_t^i}%\cdot 
%                 a^i_t
%             )
%         \Big)
%         +
%         \sqrt{
%             \frac{\sigma_t^i}{2\pi}
%         }
%         \,
%         \exp\bullet\Big(
%             \frac{-1}{2\,\sigma_t^i}
%             % \,
%             (a^i_t)^2
%         \Big)
% \\
%         \mathbb{E}[(Z_{t+1}^i)_j b (Z_{t+1}^i)_k] 
%     = &
%         b\,
%     \begin{cases}
%             ( (a^i_t)_j^2 + \sigma^i_t)
%             \odot
%             \Big(
%                 \bar{1} 
%                 - 
%                 \Phi(
%                     \frac{-(a^i_t)_j}{\sigma_t^i}
%                 )
%             \Big)
%             +
%             (a^i_t)_j\,
%             \sqrt{
%                 \frac{\sigma_t^i}{2\pi}
%             }
%             \,
%             \exp\Big(
%                 \frac{-(a^i_t)_j^2}{2\,\sigma_t^i}
%             \Big)
%     & 
%         \mbox{ if } j=k
% \\
%     \mathbb{E}[(Z_{t+1}^i)_j]
%     \mathbb{E}[(Z_{t+1}^i)_k]
% \end{cases}
% \end{aligned}
% \end{equation}
% where $\odot$ denotes the Hadamard product%
% \footnote{The Hadamard product of any pair of vectors $a,b\in \mathbb{R}^K$ and any $K\in \mathbb{N}$ is given by
% $a\odot b\eqdef (a_kb_k)_{k=1}^K$,},~%
% $\bar{1}\in \mathbb{R}^{d_z}$ denotes the vector will all entries equal to $1$, $\Phi$ is the standard normal CDF, $a_t^2\eqdef (a_{t\,j}^2)_{j=1}^{d_z}$, $b\in \mathbb{R}$, $j,k=1,\dots,d_z$.
% \end{lemma}
% \begin{proof}
% In the setting of Example \ref{ex:Random_NeuralNetwork}, for each $t\in \mathbb{N}$, every $i=1,\dots,N$, and $j=1,\dots,d_z$, we have that
% $(Z_{t+1}^i)_j$ is a normal random variable with mean $
% (a_t)_j$ and variance $(\sigma_t^i)_j$; where we have used the fact that the components of $W_t^i$ are independent whenever their indices differ. 
% Consequentially, the computation of the mean and variance of the rectified Gaussian distribution, computed in \citep[page 90 and Appendix A]{Beauchamp_Distribution_RectifiedGaussian2018}, yields the conclusion.
% \end{proof}
% \end{comment} 

% \section{The Algorithm}
% \label{s:AlgoMain}

% In this section, we summarize the FL algorithm.

% \begin{algorithm}[H]%[hpt!]%
% \SetKwInOut{Require}{Require}
% \caption{Proposed Federated Learning Algorithm}
% \label{alg:FedMain}
% \SetAlgoLined
% \LinesNumberedHidden
% \Require{Expert models $\{\varphi^{i}\}_{i=1}^N$, Synchronization Frequency $\tau \in \mathbb{N}_+$}
% \DontPrintSemicolon
% \vspace{0.2cm}
% \For(\tcp*[f]{Generate prediction for time $t$}){$t:1, 2, \dots$} 
%  {
% \For(\tcp*[f]{Update experts in parallel}){$i:1,\dots,N$ in parallel}{
% $\beta_{t-1}^i \leftarrow \big( X^{i \top}_{t-1} X^i_{t-1} + \gamma_i I_{d_z} \big)^{-1}\, X_{t-1}^{i \top} \bar{y}^i_{t} $
% \tcp*{Local weighted regression}
% Generate $\varepsilon_{t-1}^i$
% \tcp*{Generate random state}
% $Z^i_{t-1}\leftarrow \varphi^{i}(x_{[0:t-1]}, Z_{t-2}^i, \varepsilon_{t-1}^i)$
% \tcp*{Update hidden state}
% $\hat{Y}^i_t \leftarrow \hat{Y}_{t-1}^i + Z^i_{t-1} \, \beta_{t-1}^i $
% \tcp*{Update residual prediction}
% } 
% %%% Get Mixture Weights
% \tcp{Compute mixture weights} 
% % \For(\tcp*[f]{Update Experts in Parallel}){$t:1,\dots,T$ in parallel}{
% $\hat{\mathbf{Y}}_{t-1} \leftarrow  (\hat{Y}^{1\top}_{t-1}, ..., \hat{Y}^{N\top}_{t-1})^\top$ \\
% $A \leftarrow 2\,N \hat{\mathbf{Y}}^\top_{t-1} \hat{\mathbf{Y}}_{t-1} + \kappa I_N$ \\
% $b\leftarrow 2 (y^\top_{t-1}  \hat{\mathbf{Y}}_{t-1})^{\top}$ \\
% $ w_{t-1} \leftarrow  A^{-1}\, \left( b - \frac{\mathbf{1}_N^{\top}A^{-1} b \, - \, \eta}{\strut \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N} \cdot\,\mathbf{1}_N
% \right)$ \\ 
% %%%% Synchronization Step
% \If{$t \bmod \tau =  0$ and $t>0$}{
% \tcp{Synchronize local agents via Nash game}
% $\boldsymbol{\beta}^{\text{sync}}_{t-2}, \hat{\mathbf{Y}}^{\text{sync}}_{t-1} \leftarrow $ Run Synchronize Subroutine: Algorithm \ref{alg:sync_subroutine}
% \tcp*{Synchronized Weights}
% \For(\tcp*[f]{Compute new predictions}){$i:1,\dots,N$ in parallel}{
% $\beta_{t-1}^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_{t-2})^i$ \;
% Generate $\varepsilon_{t-1}^i$ 
% \tcp*{Generate random state} 
% $\hat{Y}^i_{t} \leftarrow (\hat{\mathbf{Y}}^{\text{sync}}_{t-1})^i +  \varphi^{i}(x_{[0:t-1]}, Z_{t-2}^i, \varepsilon_{t-1}^i) \beta^i_{t-1}$ \tcp*{Correct local predictions} 
% }
% }
% $\hat{Y}_t = w_{t-1}^\top \hat{\mathbf{Y}}_{t}$
% \tcp*{Ensemble final prediction for time $t$}
% }
% \end{algorithm}

% Note that in Algorithm \ref{alg:sync_subroutine}, described below, for simplicity, the indexing is presented from $0$ to $T$, representing the historical length of time over which the Nash synchronization takes place, i.e. the ''look-back'' length. In practice, the input values should correspond to those of the FL algorithm starting at $T = t-1$, proceeding backwards from there.

% % \begin{algorithm}[H]%[ht!]%
% % \caption{Proposed Federated Learning Algorithm}
% % \label{alg:FedMain}
% % \begin{algorithmic}
% % \SetAlgoLined
% % \Require Current time $t\in \mathbb{N}$, Hidden States $\{Z_t^i\}_{i=1}^N$, expert models $\{\varphi^i\}_{i=1}^N$, Synchronization Frequency $T\in \mathbb{N}_+$, Batch size $1\le b\le N$.
% % \DontPrintSemicolon
% %         \tcp*{Update Mixture Weights}
% %         % \State \eIf{$t \bmod T\neq 0$}{
% %             \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
% %                 \State \tcc{Update Experts in Parallel}
% %                 \State \ForParallel{\State $\beta_t^i \leftarrow 
% %         \big( X^{i \top}_t X^i_t + \gamma_i I_{d_z} \big)^{-1}\, X_t^{i \top} \bar{y}^i_t $
% %                     \tcp*{Local Weighted Regression}
% %                     \State Generate $\varepsilon_t^i$
% %                     \tcp*{Generate Random State}
% %                     \State $Z_{t+1}\leftarrow \varphi(x_{[0:t]},\varepsilon_t^i,Z_{t+1}^i)$
% %                     \tcp*{Update Hidden State}
% %                     \State 
% %                       $\hat{Y}^i_t
% %                       \leftarrow
% %                       \hat{Y}_{t-1}^i
% %                       + 
% %                       \beta_t^i \,
% %                       Z_t$
% %                       \tcp*{Update Residual Prediction}
% %                         }
% %                    % }{
% %         %%% Get Mixture Weights
% %         \State \tcc{Compute Mixture Weights} 
% %         \State $\hat{\mathbf{Y}}_t \leftarrow  (\hat{Y}^1_t, ..., \hat{Y}^N_t)$ 
% %         \State $A \leftarrow 2\,N \hat{\mathbf{Y}}^\top_t \hat{\mathbf{Y}}_t + \kappa I_N$ 
% %         \State $b\leftarrow 2 (y^\top_t  \hat{\mathbf{Y}}_t)^{\top}$, 
% %         \State $ w_t  
% %         \leftarrow  
% %              A^{-1}\,
% %              \big(
% %                  b -  
% %                  % \biggl(
% %                     \frac{
% %                         \mathbf{1}_N^{\top}A^{-1} b \, - \, \eta 
% %                     }{
% %                         \mathbf{1}_N^{\top}A^{-1}\mathbf{1}_N
% %                     }
% %                 \cdot
% %                  % \biggr)
% %                  \,\mathbf{1}_N
% %              \big)$
% %             %%%% Synchronization Step
% %             % \State \eIf{$t \bmod T\neq 0$}{
% %             \State \tcc{Synchronize Local Experts via Nash game}
% %             \State \eIf{$t \bmod T =  0$ and $t>0$}{
% %                 \State $\boldsymbol{\beta}^{\text{sync}}_t \leftarrow $ Run Synchronize Subroutine: Algorithm \ref{alg:sync_subroutine}
% %                 \tcp*{Synchronized Weights}
% %                 \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
% %                     \State \ForParallel{
% %                     \State $\beta_t^i \leftarrow (\boldsymbol{\beta}^{\text{sync}}_t)_i$\;
% %                     \State Generate $\varepsilon_t^i$ \tcp*{Generate Random State}
% %                     \State $
% %                     \hat{Y}^i_t
% %                     \leftarrow
% %                     \hat{Y}^i_{t-1}
% %                     + 
% %                     (\beta_t^i)^{\top}\,
% %                     \varphi(x_{[0:t]},\varepsilon_t^i,Z_t^i)
% %                     $\;
% %                 }
% %               }
% %     \State \tcc{Server Synchronizes Local Expert Predictions}
% %     %%
% %     \State \Return $\hat{\mathbf{Y}}_t w_t$.
% %     \tcp*{Ensemble Prediction}
% % \end{algorithmic}
% % %\textbf{Note:} The helper functions $\mathbf{A},\mathbf{B},\mathbf{C},\Gamma$, and $\boldsymbol{\alpha}$ are defined in %circa Proposition \ref{prop:NashEqmExistence} and the matrices $K$, $G$, and $\mathbf{c}$ are defined in \eqref{eq:Gc_Def}.
% % \end{algorithm}

% \begin{algorithm}[H]%[hbp!]%
% \SetKwInOut{Require}{Require}
% \caption{Synchronization Subroutine}
% \label{alg:sync_subroutine}
% \SetAlgoLined
% \LinesNumberedHidden
% \Require{Observed target values $\{ ( y^1_t, \ldots, y^N_t)\}_{t=0}^T$, Hidden States $\{Z_t^1, \ldots, Z_t^N\}_{t=0}^T$ \\
% Mixture weights $w_\cdot = \{ (w^1_t, \ldots, w^N_t) \}_{t=0}^T$ $\leftarrow$ From Algorithm \ref{alg:FedMain}}
% \DontPrintSemicolon
% \vspace{0.2cm}
% \DontPrintSemicolon
% \tcp{Initialize updates} 
% $\mathbf{w}_T=(w^1_T I_{d_{y}}, \dots, w^N_T I_{d_{y}})^\top$\\
% \For{$i:1,\dots,N$ in parallel}{
% $P_i(T)  = 0$ \\
% $S_i(T) = 0$ 
% }
% \tcp{Generate iterates}
% \For(){$t=T-1,\dots,0$}{
% \tcp{Update driving parameters} 
% $\mathbf{w}_t=(w^1_t I_{d_{y}}, \dots, w^N_t I_{d_{y}})^\top$ \\
% %$\mathbf{A}(t)=  \big[ \mathbb{E} \big( Z^{i\top}_t \mathbf{e}_i^\top P_i(t+1) \mathbf{e}_j Z^j_t \big) \big]_{i,j=1}^N$ \\
% $\mathbf{A}(t) = \mathbb{E} \big\{ [ P_1(t+1) \mathbf{e}_1 Z^1_t, \, \dots, \, P_N(t+1) \mathbf{e}_N Z^N_t ]^\top 
%  [ \mathbf{e}_1 Z^1_t, \dots, \mathbf{e}_N Z^N_t ] \big\}$ \\  
%  $\widehat{\mathbf{A}}(t) = \mathbb{E} \big\{ [ \mathbf{e}_1 Z^1_t, \, \dots, \, \mathbf{e}_N Z^N_t ]^\top \mathbf{w}_t \mathbf{w}_t^\top  
%  [ \mathbf{e}_1 Z^1_t, \dots, \mathbf{e}_N Z^N_t ] \big\}$ \\  
% $\mathbf{B}(t)= \mathbb{E} [ P_1(t+1) \mathbf{e}_1 Z^1_t, \, \dots, \, P_N(t+1) \mathbf{e}_N Z^N_t ]^\top $ \\
% $\mathbf{C}(t)= \mathbb{E} [ S_1^\top(t+1) \mathbf{e}_1 Z^1_t, \, \dots, \, S_N^\top(t+1) \mathbf{e}_N Z^N_t ]^\top$ \\
% $\mathbf{D}(t)  
%  = \mathbb{E}  
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \cdots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix}$ \\ 
%    $\mathbf{G}(t) = - \big[ e^{-\boldsymbol{\alpha}(T-1-t)} ( \Gamma + \widehat{\mathbf{A}}(t) ) 
%   + \mathbf{A}(t)    \big]^{-1} 
%  \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}^\top(t) \mathbf{w}_t \mathbf{w}_t^\top + \mathbf{B}(t) \big] $ 
%  \notag \\ 
%   $\mathbf{H}(t) = \big[ e^{-\boldsymbol{\alpha}(T-1-t)} (\Gamma + \widehat{\mathbf{A}}(t) ) + \mathbf{A}(t)   \big]^{-1} 
%   \big[ e^{-\boldsymbol{\alpha}(T-1-t)} \mathbf{D}(t)^\top \mathbf{w}_t y_{t+1} - \mathbf{C}(t) \big] $
%  \notag \\
% \For{$i:1,\dots,N$ in parallel}{
% \vspace{-0.4cm}
% \begin{flalign*} 
% \mathbf{D}_i(t) & =  \mathbb{E} \big\{   
%  \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \dots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix}^\top 
%   P_i(t+1) 
%   \begin{bmatrix} 
%     \mathbf{e}_1 Z^1_t    , \, 
%     \mathbf{e}_2 Z^2_t   ,  \,
%  \dots , \, 
%   \mathbf{e}_N Z^N_t    
%  \end{bmatrix} 
%  \big\} & \\ 
%   P_i(t) &=  
%   \mathbf{G}(t)^\top 
%   \big[ \widehat{\mathbf{A}}(t) + \mathbf{D}_i(t) + e^{-\alpha_i(T-1-t)} 
%   \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] 
%    \mathbf{G}(t) &\\   
%   & \qquad + \big[ e^{-\alpha_i(T-1-t)}\mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big] 
%    \mathbf{D}(t) \mathbf{G}(t)  &\\ 
%   & \qquad + \mathbf{G}(t)^\top \mathbf{D}(t)^\top \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1) \big]^\top
%   &\\ 
% & \qquad + e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  &\\
% %%%%%
%  S_i(t)  &= \mathbf{G}^\top(t) \big[ \widehat{\mathbf{A}}(t) + \qquad\mathbf{D}_i(t) 
%    + e^{-\alpha_i(T-1-t)} \gamma_i \hat{\mathbf{e}}_i \hat{\mathbf{e}}_i^\top  \big] \mathbf{H}(t) &\\ 
% & \qquad + \big[ e^{-\alpha_i(T-1-t)} \mathbf{w}_t \mathbf{w}_t^\top + P_i(t+1)  \big] \mathbf{D}(t) \mathbf{H}(t) &\\  
% & \qquad + \mathbf{G}^\top(t) \mathbf{D}^\top(t) \big[ - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1) \big]  &\\
% & \qquad - \mathbf{w}_t y_{t+1} e^{-\alpha_i(T-1-t)} + S_i(t+1)
% \end{flalign*}
% \vspace{-0.6cm}
% }
% }
% \tcp{Update game strategy} 
% $\hat{Y}_0 = (y^{1\top}_0, \dots, y^{N\top}_0)^\top$ \\
% \For{$t=0, \dots, T-1$}{
% $\boldsymbol{\beta}_t 
% %= [\beta^{1\top}_t, \dots, \beta^{N \top}_t ]^\top 
% =  \mathbf{G}(t) \hat{Y}_t + \mathbf{H}(t)$ \\
% $\hat{Y}_{t+1} = \hat{Y}_t + \diag[Z^1_t, \dots, Z^N_t ] \boldsymbol{\beta}_t$
% }

% \Return $\boldsymbol{\beta}_{T-1}$, $\hat{\mathbf{Y}}_{T}$
% \end{algorithm} 

% \section{Additional Experiment Details}
% \label{s:ExperimentDetials}

% This appendix provides additional technical details for the experiments, including experimental design, dataset descriptions, and details in Appendix \ref{s:ExperimentDetials__ss::datasets}. Appendix \ref{s:OptimalParamterChoices} outlines the hyperparameter search space and the optimal hyperparameters used in the experiments. Further ablation studies in Appendix \ref{a:Ablations}, covering validation results for the BoC Exchange Rate and ETT datasets in which the performance on validation segments are reported. This is followed by a study informing the choice of activation function for ESNs and a discussion of the importance of data normalization in both ESNs and RFNs.

% In this work, time-series performance is measured with mean-squared error (MSE) relative to the reference sequence. For a sequence of length $T$, predictions $\hat{y}_i \in \mathbb{R}^n$, and targets $y_i \in \mathbb{R}^n$, MSE is computed as 
% \begin{align*}
%     \text{MSE} = \frac{1}{T} \sum_{i=1}^T \Vert \hat{y}_i - y_i \Vert^2.
% \end{align*}

% \subsection{Datasets} 
% \label{s:ExperimentDetials__ss::datasets}

% In this appendix, the details for each of the time-series datasets considered in the numerical experiments are laid out. In all, five unique time series are considered. Each incorporates different complexities for time-series prediction, as well as varying length scales and dimensionalities. Throughout this section, time-series inputs are denoted as $\mathbf{x}$, targets as $\mathbf{y}$, and predictions as $\hat{\mathbf{y}}$

% \subsubsection{Periodic Signal}

% The Periodic Signal series is the simplest in terms of construction, but can be challenging for time-series prediction due to its highly oscillatory nature. The series has $200$ data points taking on a minimum value of -0.9 and a maximum value of 0.9. The target regularly oscillates between these two values throughout the series. At each time step, $t$, a single target lag is used to make model predictions such that $\mathbf{x}_{t-1} = \mathbf{y}_{t-1}$ in predicting $\mathbf{y}_t$. Figure \ref{fig:periodic_series} displays the target values of the series.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/periodic_series.pdf}
%     \caption{Periodic time series with 200 target values.}
%     \label{fig:periodic_series}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/logistic_map_dataset.pdf}
%     \caption{Logistic map series progressing over $200$ time steps.}
%     \label{fig:logistic_map_dataset}
% \end{figure}


% \subsubsection{Logistic Map}

% The Logistic Map dataset is a synthetic time series based on the dynamics of the logistic map. The generating function from the EchoTorch library \citep{echotorch} is used to produce a time series with $200$ total data points. The default parameters for the EchoTorch dataset are applied, namely $\alpha=5$, $\beta=11$, $\gamma=13$, $c=3.6$, and $b=0.13$. Figure \ref{fig:logistic_map_dataset} shows the resulting series. The target variable, $\mathbf{y}$, has a single dimension. As with the Periodic dataset, a single step lag is provided as input for model predictions. That is, for time step $t$ and target $\mathbf{y}_t$, the input is $\mathbf{x}_{t-1} = \mathbf{y}_{t-1}$.

% \subsubsection{Concept Shift} \label{concept_drift_description}

% The Concept Drift dataset considers a rapid, but smooth, change in the relationship of $\mathbf{x}$ and $\mathbf{y}$ halfway through the trajectory. The series consists of $200$ points drawn from the following analytical relationship. Let $p$ be evenly spaced in the interval $[0, 2\pi]$. Then
% \begin{align*}
%     x_1 = p, && x_2 = p, && x_3 = \sqrt{p}.
% \end{align*}
% For $p \in \left[0, \frac{7}{8}\pi \right]$, $\mathbf{y} \in \mathbb{R}^2$ is
% \begin{align*}
%     y_{1, 1}(x_1, x_2, x_3) &= x_1^2 + \sin x_2 + x_1  x_3 + \frac{1}{2} \cos(10 x_1), \\
%     y_{2, 1}(x_1, x_2, x_3) &= x_1  \cos x_2 + x_3 - e^{-x_2}.
% \end{align*}
% For $p \in \left[\frac{9}{8} \pi, 2\pi\right]$,
% \begin{align*}
%     y_{1, 2}(x_1, x_2, x_3) &= x_1 + x_2 - \sin x_3, \\
%     y_{2, 2}(x_1, x_2, x_3) &= \cos x_1  \sin x_2 + x_3^2 + \frac{1}{4} \cos(10 x_1).
% \end{align*}
% The phase transition, which occurs when $p \in \left[\frac{7}{8} \pi, \frac{9}{8} \pi \right]$ is facilitated by the piecewise function
% \begin{align*}
%     \alpha(x) = \begin{cases}
%       1.0 & x < \frac{7}{8} \pi, \\
%       \cos(2(x_1 - \frac{7}{8}\pi) & \frac{7}{8} \pi \geq x \leq \frac{9}{8} \pi, \\
%       0.0 & x > \frac{9}{8} \pi. \\
%     \end{cases}
% \end{align*}
% The final series is then written
% \begin{align*}
%     y_1(x_1, x_2, x_3) &= \alpha(x_1) \cdot y_{1, 1}(x_1, x_2, x_3) + (1-\alpha(x_1)) \cdot y_{1, 2}(x_1, x_2, x_3), \\
%     y_2(x_1, x_2, x_3) &= \alpha(x_1) \cdot y_{2, 1}(x_1, x_2, x_3) + (1-\alpha(x_1)) \cdot y_{2, 2}(x_1, x_2, x_3).
% \end{align*}
% Figure \ref{fig:concept_drift} provides a visualization of the series as a function of $x_1$.
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/concept_drift_plot.pdf}
%     \caption{Visualization of the Concept Drift time series as a function of $x_1$.}
%     \label{fig:concept_drift}
% \end{figure}

% \subsubsection{Bank of Canada Exchange Rate}
% \label{s:ExperimentDetials__ss::datasets__sss:::BoC}
% The Bank of Canada (BoC) Exchange Rate dataset \citep{boc_exchange_rates} records the daily exchange rates for $12$ different currencies, relative to the Canadian dollar (CAD), from May 1, 2007 to April 28, 2017. This constitutes $3,651$ observations per currency. Any one of the exchange rates may be used as a target with lagged currency values used as inputs. In the numerical experiments, the target exchange rate is USD and inputs for model predictions at a given time step $t$ are $\{\text{USD}_{t-1}$, $\text{USD}_{t-2}$, $\text{AUD}_{t-1}$, $\text{AUD}_{t-2}$, $\text{EUR}_{t-1}$, $\text{EUR}_{t-2}$, $\text{GBP}_{t-1}$, $\text{GBP}_{t-2}$, $\text{JPY}_{t-1}$, $\text{JPY}_{t-2}\}$. Here, for example, $\text{JPY}_{t-1}$ is the exchange rate for the Japanese Yen from the previous time step. The experiments in the body of the paper consider the first $2000$ dailey rates. Figure \ref{fig:boc_dataset} provides a visualization of the dataset for a subset of currencies over the entire time range.
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/boc_exchange_rates.pdf}
%     \caption{Exchange rates relative to the Canadian dollar for a subset of the $12$ currencies tracked in the BoC Exchange Rate time series.}
%     \label{fig:boc_dataset}
% \end{figure}

% \subsubsection{Electricity Transformer Temperature} 
% \label{s:ExperimentDetials__ss::datasets__sss:::ETT}
% The Electricity Transformer Temperature (ETT) datasets were first introduced in \citep{haoyietal-informer-2021} as a difficult benchmark for the Informer time-series model. The target value for prediction in each dataset is the oil temperature (OT) at a given time within one of two electricity transformers. The datasets span a time-frame from July 1, 2016 to June 26, 2018. In particular, the ETT-small-h1 time series is studied, which records temperature measurements every hour during this date-span along with measurements of six other input features.

% In the experiments in the body of this paper, the first $2000$ data points are used. All six input features (HUFL, HULL, MUFL, MULL, LUFL, LULL) are used to make predictions. When predicting $\text{OT}_t$, inputs include $\text{OT}_{t-1}$, $\text{OT}_{t-2}$, along with $\text{X}_{t-1}$, $\text{X}_{t-2}$, $\text{X}_{t-3}$, where $\text{X}$ represents an aforementioned input feature. Finally, all values in the dataset have been normalized by dividing the input and target sequences by the maximum value seen across the time series of interest. As will be discussed in Appendix \ref{normalization_study}, this is an important pre-processing step, because large input and target values tend to cause instabilities in the numerical computations and/or saturate the activation functions of the ESN and RFN models. While an exact normalization value may not be available during online prediction, an approximate normalizing scalar is likely sufficient. Figure \ref{fig:ett_dataset} exhibits a slice of the first $3,000$ steps in the time series along with the value of the input features at that time.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/ett_dataset.pdf}
%     \caption{A snapshot of the normalized ETT-Small-h1 dataset with target value OT over time, along with the corresponding features used to help make predictions.}
%     \label{fig:ett_dataset}
% \end{figure}

% \begin{table}[H]
% \centering
% \caption{Summary of hyperparameters searched for transformer models across datasets and whether Nash-game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$, $\eta=1.0$, $d_z = 2$, and synchronization frequency, $\tau = 1$, regardless of other hyperparameters. Bold numbers correspond to the optimal parameters based on mean MSE in the experiments.}
% \label{tab:transformer_hyperparams}
% \resizebox{0.65\linewidth}{!}{\begin{tabular}{llcccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & Client $T$ & Game $T$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{\mathbf{3}, 4, 5, 6, \mathbf{7}\}$ & $\{2, \mathbf{3}, 4\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $\{\mathbf{1}, 2, 3, 4\}$ \\
% & False & $\{0.001, \mathbf{0.01}, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{1, \mathbf{10}\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, 4, \mathbf{5}, 6\}$ & $\{2, \mathbf{3}, 4\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, 10, \mathbf{15}\}$ & $\{3, \mathbf{4}, 5, 6\}$ & $\{\mathbf{1}, 2, 3, 4\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1, 1, 5\}$ & $\{1, \mathbf{10}, 15\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{1, \mathbf{10}\}$ & $\{3, \mathbf{4}, 5\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, 6, 7, \mathbf{8}\}$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{\mathbf{2}, 3, 4\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.001, 0.01, 0.1, \mathbf{1}, 5\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{3}, 4, 5, 6\}$ & $\{2, 3, \mathbf{4}\}$ \\
% & False & $\{0.001, 0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{3, 4, 5, \mathbf{6}\}$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

% \subsection{Best Hyperparameter Choices By Experiment}
% \label{s:OptimalParamterChoices}

% For all simulations, unless otherwise stated, a hyperparameter search is performed to find the best set of hyperparameters minimizing the average MSE for the time series in question. The full set of hyperparameters explored for each dataset, model, and Nash game setting are recorded in Tables \ref{tab:transformer_hyperparams}-\ref{tab:esn_hyperparams}. In each experiment, the parameters $\kappa$ and $\eta$ are each fixed to $1.0$. Additionally, for the transformer experiments, $d_z$ is fixed at $2$ for simplicity and empirical observations of better performance. Note that $\sigma$ is also not used in transformer models and is therefore irrelevant in hyperparameter tuning. The hyperparameter optimization is done post-hoc. However, the results compare the best possible performance of the two approaches in this idealized setting. In addition, several experiments in Appendix \ref{validation_studies} compare performance after hyperparameter tuning on validation time series.

% \begin{table}[H]
% \centering
% \caption{Summary of hyperparameters searched for RFN models across datasets and whether Nash-game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$ and $\eta=1.0$, regardless of other hyperparameters. Bold numbers correspond to the optimal parameters based on mean MSE in the experiments.}
% \label{tab:rfn_hyperparams}
% \resizebox{0.99\linewidth}{!}{\begin{tabular}{llccccccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & $\sigma$ & $d_z$ & Client $T$ & Game $T$ & Sync Freq. \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.0001}, 0.001, 0.01, 0.1, 1\}$ & $\{0.1, 1, 10, \mathbf{15}\}$ & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{3, 4, \mathbf{5}, 6, 7\}$ & $\{2, 3, 4, \mathbf{5}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.0001}, 0.001, 0.01, 0.1, 1\}$ & $\{0.1, 1, 10, \mathbf{15}\}$ & $\{0.01, \mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 4, 5, 6, 7\}$ & $\{\mathbf{2}, 3, 4, 5, 6\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 0.1, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $\{\mathbf{2}, 3, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, \mathbf{0.01}, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{0.1}, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{0.01, 0.1, \mathbf{1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{10, \mathbf{15}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{1, \mathbf{2}\}$ & $\{2, 3, 4, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{\mathbf{0.01}, 0.1, 1, 5\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, \mathbf{1}\}$ & $\{1, \mathbf{2}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.1}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.0001}, 0.001, 0.01\}$ & $\{10, \mathbf{15}\}$ & $\{0.01, \mathbf{0.1}\}$ & $\{3, 4, \mathbf{5}\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{2, \mathbf{3}, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.0001, 0.001, \mathbf{0.01}\}$ & $\{10, \mathbf{15}\}$ & $\{\mathbf{0.01}, 0.1\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, 0.1, \mathbf{1.0}\}$ & $\{3, \mathbf{6}\}$ & $\{2, 3, \mathbf{5}\}$ & $\{\mathbf{2}, 3, 4\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{0.1}, 1.0\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 3, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.01}, 0.1, 1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{2, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.01, 0.1, \mathbf{1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, 1\}$ & $\{\mathbf{1}, 2\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{2, \mathbf{3}\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, \mathbf{0.1}, 1, 5\}$ & $\{\mathbf{10}, 15\}$ & $\{0.1, \mathbf{1}\}$ & $\{1, \mathbf{2}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

% \begin{table}[ht]
% \centering
% \caption{Summary of hyperparameters searched for ESN models across datasets and whether Nash-game synchronization was used. The top section corresponds to the two expert setting and the bottom to five experts. In all settings, $\kappa=1.0$ and $\eta=1.0$, regardless of other hyperparameters. Bold numbers correspond to the optimal parameters based on mean MSE in the experiments.}
% \label{tab:esn_hyperparams}
% \resizebox{0.99\linewidth}{!}{\begin{tabular}{llccccccc}
% \toprule
% Dataset & Nash & $\alpha$ & $\gamma$ & $\sigma$ & $d_z$ & Client $T$ & Game $T$ & Sync Freq. \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2, 3\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{0.1, \mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{2, 5, \mathbf{10}\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{3, \mathbf{6}, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{1}, 2, 3\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{1, 2, \mathbf{3}\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $-$ & $-$ \\
% \midrule
% \multirow{2}{*}{Periodic} & True & $\{\mathbf{0.001}, 0.01, 0.1, 1, 10\}$ & $\{0.01, 0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{\mathbf{3}, 6\}$ & $\{\mathbf{2}, 5, 10\}$ & $\{\mathbf{3}, 4, 5\}$ & $\{\mathbf{1}, 2, 3\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}, 1, 10\}$ & $\{0.01, 0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Logistic} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{0.01, \mathbf{1}\}$ & $\{3, \mathbf{6}, 12\}$ & $\{2, \mathbf{5}, 10\}$ & $\{\mathbf{3}, 5\}$ & $\{\mathbf{1}, 2\}$ \\
% & False & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{0.1, 1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6, 12\}$ & $\{\mathbf{2}, 5, 10\}$ & $-$ & $-$ \\
% \multirow{2}{*}{Concept} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}, 6\}$ & $\{2, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{1\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{1, \mathbf{10}\}$ & $\{\mathbf{0.01}, 1\}$ & $\{\mathbf{3}\}$ & $\{\mathbf{2}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{BoC} & True & $\{\mathbf{0.001}, 0.01, 0.1\}$ & $\{\mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{3, \mathbf{5}\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.001, 0.01, \mathbf{0.1}\}$ & $\{\mathbf{10}\}$ & $\{\mathbf{1}\}$ & $\{3, \mathbf{6}\}$ & $\{\mathbf{3}, 5\}$ & $-$ & $-$ \\
% \multirow{2}{*}{ETT} & True & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{\mathbf{1}, 2, 3\}$ & $\{\mathbf{2}, 3, 4, 5\}$ & $\{\mathbf{2}, 3\}$ & $\{\mathbf{1}\}$ \\
% & False & $\{0.01, 0.1, 1, \mathbf{5}\}$ & $\{\mathbf{1}, 10\}$ & $\{\mathbf{1}\}$ & $\{1, 2, \mathbf{3}\}$ & $\{2, \mathbf{3}, 4, 5\}$ & $-$ & $-$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

% Experiments considering ESN and RFN models demonstrate an inherent randomness due, for example, to the construction of their affine maps and perturbative noise. Thus, for these models, simulations are run with three random seeds ($2024$, $2025$, $2026$) in all settings and results are averaged over the three runs. This is done for both hyperparameter tuning and reporting of final results.

% \subsection{Pre-training Details for transformer Models}
% \label{a:TransExpHyper}

% During the pre-training phase of the transformer model, the encoder and the final linear decoder layer are trained to predict the target sequence given the input sequence. This is achieved using a causal mask, which ensures that the transformer relies only on the current and previous time step inputs to predict  $\hat{y}_{t+1}$. The output of the transformer’s encoder is then passed to a final trainable linear layer to predict the target at $t+1$. After pre-training for a few epochs, the encoder of the transformer, excluding the final linear layer, is used as the encoder model in the main experiments.

% The first layer of the transformer is an embedding layer that maps the input dimension to the transformer's hidden dimension. A positional encoding layer is then added to the input. The resulting input is then passed to the transformer encoder.  The transformer encoder consists of two transformer layers, each consisting of self-attention and feed-forward networks. The number of expected features is set to $d_z \times d_y$, the number of heads is set to $2$, and the dimension of the feed-forward network is set to $16$, which are selected based on some initial hyperparameter tuning of the model. The dropout is set to $0.1$ for all experiments. The decoder layer is the final linear layer that transforms the encoder’s output $Z_t$ from a dimension of $d_y \times d_z$ to $d_y$.  This final layer is dropped and tuned following the main algorithm.

% \subsection{Further Ablation Studies}
% \label{a:Ablations}

% This section contains additional, relevant ablation studies, the conclusions of which can be useful for the successful use of the FL algorithm.

% \subsubsection{Validation Time Series Results} \label{validation_studies}

% Studies applying ESN and RFN models with and without Nash-game synchronization on validation slices of the BoC Exchange Rate and ETT time series are reported in this section. In the experiments of Sections \ref{s:Examples__ss:RFN__sss:Results} and \ref{s:Examples__ss:ESN__sss:Results}, the first $2000$ data points from each of these series are considered. Herein, a slice of the BoC Exchange Rate series from index $1600$ to $3600$ is used, along with a slice from the ETT series from index $3500$ to $5500$. Note that there is a small amount of overlap for the BoC Exchange Rate dataset due to length limitations. 

% As in previous results, three prediction runs with random seeds of $2024$, $2025$, and $2026$ are used and the resulting MSEs averaged. The optimal hyperparameters from previous experiments for each setting are applied. A summary of the results is presented in Table \ref{tab:validation_studies}. In all but one of the settings, predictions with Nash-game synchronizations significantly outperform those without on the unseen data. For the setting where predictions without the Nash game outperform those with it, the drop in performance for Nash-game synchronization is traced back to a single prediction in one of the runs that generated an obvious and significant outlier. It is likely that this aberrant prediction is caused by a numerical instability in the Nash optimization and could easily be detected and discarded during online prediction. The remaining two runs produced MSEs on the order of $1\mathrm{e}{\text{-}5}$, which is a marked improvement over the non-Nash setting.

% \begin{table}[ht!]
%     \centering
%     \caption{Results, averaged over three runs for ESN and RFN models on validation slices of the BoC Exchange Rate and ETT time series. The optimal hyperparameters from the studies in Sections \ref{s:Examples__ss:RFN__sss:Results} and \ref{s:Examples__ss:ESN__sss:Results} are used.}
%     \label{tab:validation_studies}
%     \begin{tabular}{lllcc}
%     \toprule
%     Model & \# of Experts & Dataset & Nash game & No Nash game \\
%     \midrule
%     \multirow{4}{*}{ESN} & \multirow{2}{*}{2} & BoC Exchange Rate & $\mathbf{2.85886\mathrm{e}{\text{-}5}}$& $1.47168\mathrm{e}{\text{-}4}$ \\
%     & & ETT Series & $\mathbf{2.64996\mathrm{e}{\text{-}3}}$ & $4.15773\mathrm{e}{\text{-}3}$ \\
%     & \multirow{2}{*}{5} & BoC Exchange Rate & $\mathbf{5.87193\mathrm{e}{\text{-}5}}$ & $1.22207\mathrm{e}{\text{-}3}$ \\
%     & & ETT Series & $\mathbf{2.64991\mathrm{e}{\text{-}3}}$ & $3.82797\mathrm{e}{\text{-}3}$ \\
%     \midrule
%     \multirow{4}{*}{RFN} & \multirow{2}{*}{2} & BoC Exchange Rate & $3.17312\mathrm{e}{\text{-}2}$ & $\mathbf{7.54179\mathrm{e}{\text{-}3}}$ \\
%     & & ETT Series & $\mathbf{5.12075\mathrm{e}{\text{-}3}}$ & $1.92244\mathrm{e}{\text{-}2}$ \\
%     & \multirow{2}{*}{5} & BoC Exchange Rate & $\mathbf{4.20660\mathrm{e}{\text{-}5}}$ & $6.28034\mathrm{e}{\text{-}2}$ \\
%     & & ETT Series & $\mathbf{2.65513\mathrm{e}{\text{-}3}}$ & $1.28415\mathrm{e}{\text{-}1}$ \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \subsubsection{ReLU Activations and ESN Recursion} \label{activation_discussion}

% Recently, it has been shown that ESN models with ReLU activations have desirable properties, including Universality \citep{Gonon1}. A natural question then is why use Hard Sigmoid activations in the models explored here. Peripherally, the work in \citep{Li6} extends many of the properties proven in \citep{Gonon1} to ESNs for general activation functions. However, the primary motivation is that the unbounded nature of the ReLU activation function can result in significant growth in the Froebenius norm of the latent representations, $Z_t$. Such growth produces poorly conditioned matrices. This can be problematic for both the numerical solution of the ridge-regression problems required for predictions without the Nash game and the more complex systems required for the proposed Nash-game synchronization.

% Consider the following code to replicate the recurrence relationship for the latent space of the ESN. 

% \begin{minted}[bgcolor=white]{python}
% import torch
% from torch.nn import ReLU
% from typing import Tuple
% import statistics

% def generate_random_tensor(
%     shape: Tuple[int, ...], device: torch.device = torch.device("cpu")
% ) -> torch.Tensor:
%     return torch.randn(shape, device=device)

% def generate_linalg_components(
%     x_dim: int, y_dim: int, z_dim: int
% ) -> Tuple[torch.Tensor, torch.Tensor, torch.Tensor]:
%     A = generate_random_tensor((y_dim, x_dim))
%     B = generate_random_tensor((y_dim, y_dim))
%     b = generate_random_tensor((y_dim, z_dim))
%     return A, B, b

% def generate_random_state(
%     sigma_t: torch.Tensor, z_dim: int, y_dim: int
% ) -> torch.Tensor:
%     W_t = torch.normal(mean=torch.zeros((1, z_dim)), std=1.0)
%     random_state = torch.matmul(sigma_t, W_t)
%     return random_state

% torch.manual_seed(42)
% x_0_sequence = torch.arange(0.1, 1.1, 0.1)
% x_1_sequence = torch.arange(0.2, 2.2, 0.2)
% x_sequence = torch.stack([x_0_sequence, x_1_sequence], dim=1)
% z_dim, y_dim, x_dim = 5, 3, 2
% sigma_t = torch.Tensor([0.1, 0.2, 0.3]).reshape(-1, 1)
% largest_values = []

% for _ in range(100):
%     A, B, b = generate_linalg_components(x_dim, y_dim, z_dim)
%     Z = torch.zeros((y_dim, z_dim))
%     for x_t in x_sequence:
%         input = x_t.reshape(-1, 1)
%         input_matrix = input.repeat(1, z_dim)
%         random_state = generate_random_state(sigma_t, z_dim, y_dim)
%         AX = torch.matmul(A, input_matrix)
%         BZ = torch.matmul(B, Z)
%         Z = ReLU()(AX + BZ + b + random_state)
%     largest_values.append(torch.max(Z).item())

% print(f"Mean: {statistics.mean(largest_values)}")
% print(f"Max: {max(largest_values)}")
% \end{minted}

% \noindent In the above, the input features are quite reasonable and the length of the time series is only 10 time steps long. In spite of this, for unlucky draws, the magnitudes of elements in $Z$ grow extremely rapidly. The largest of which is $87025$ in this simulation. Over the $100$ simulation trajectories, the mean value for the largest element in $Z$ is $1937$. While the distribution is fairly skewed by outliers, this example demonstrates the potential hazard in using ReLU activations in ESNs over long time series. Using a bounded activation function, such as the Hard Sigmoid, in the experiments above, largely mitigates this issue.

% \subsubsection{ESN and RFN Models on Unnormalized Data} \label{normalization_study}

% In Appendix \ref{s:ExperimentDetials__ss::datasets__sss:::ETT}, the importance of normalizing the inputs and outputs of the ETT time series is briefly mentioned. In this section, some studies considering the impact of failing to scale data when using ESN or RFN models is discussed. Consider a toy dataset composed of three Brownian motion trajectories with drift \citep{Glasserman1}. For each trajectory, the Brownian motion has a $\mu = 1.0$ and $\sigma = 1.0$. At each time step, $t$, the target is simply the sum of $x_t = 0.1\cdot t$ and the value of trajectory $i$ at that time step, $b_{i, t}$. The inputs are simply $x_t$ and $b_{i, t}$. So the model need only learn to properly add these two values together to make an accurate prediction. In the examples below, a time series of length $200$ is used, three trajectories are sampled as targets, two experts are present for the mixture, and ESN models are used.

% As seen in Figure \ref{fig:normalization}, the values of the Brownian trajectories quickly grow fairly large, implying that the model inputs also grow steadily. Examining the server predictions without Nash synchronization, it is clear that the server is unable to mix predictions from the two clients to make predictions for target variable $y_2$. The root cause of this failure is seen in considering the predictions produced by the individual clients. Both clients fail to produce meaningful predictions for $y_2$. Furthermore, Client 1 produces extremely poor predictions for all target dimensions. Thus, the server must rely exclusively on predictions from Client 0 to produce any meaningful predictions at all. Note that these issues remain present, even after significant hyperparameter tuning.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/normalization/server_predictions_plot.pdf}
%     \includegraphics[width=0.8\linewidth]{figures/normalization/client_predictions_plot.pdf}
%     \caption{Predictions for the server (top) and individual clients (bottom) for the synthetic Brownian motion dataset. Due to the large input and target values, the clients, especially Client 1, fail to produce good predictions using ESN models.}
%     \label{fig:normalization}
% \end{figure}

% The driver of these failures is a collapse in the latent representations, $Z_t$, from which clients derive their predictions. Recall that, for ESN models, 
% \begin{align*}
%     Z_t^i &= \text{Hard Sigmoid} \bullet \left (A^i x_t + B^i Z_{t-1}^i b^i + \sigma^i W_t^i \right) \\
%     \hat{Y}_{t+1}^i &= \hat{Y}_t^i + Z_t^i \beta_t^i.
% \end{align*}
% If a row of $Z_t^i$ were to become zero, the previous prediction $\hat{Y}_t^i$ remains constant in that dimension, regardless of $\beta_t^i$. If the inputs to the Hard Sigmoid become negative enough, this can happen repeatedly. In the case of Figure \ref{fig:normalization}, after a few steps, the latent matrix $Z$ becomes zero across the board for Client 1 and the second row becomes zero for Client 0. 

% This deficiency may be addressed in several ways. For example, a $\tanh$ function might be substituted for the Hard Sigmoid activation, thereby removing the vanishing representation problem. However, the issue of saturating the extremes of the activation function remains present. Experimentally, a suitable solution for the ETT time series is normalization of the input and output variables by some computed maximum. This approach was applied for all experiments. However, it is likely that an ideal setup would be a combination of $\tanh$ activation and normalization.

% \end{document} 
